Homotopy limits in the category of dg-categories in terms of $\mathrm{A}_{\infty}$-comodules

In this paper, we apply an explicit construction of a simplicial powering in dg-categories, due to Holstein (2016) and Arkhipov and Poliakova (2018), as well as our own results on homotopy ends (Arkhipov and {\O}rsted 2018), to obtain an explicit model for the homotopy limit of a cosimplicial system of dg-categories. We apply this to obtain a model for homotopy descent in terms of $\mathrm{A}_{\infty}$-comodules, proving a conjecture by Block, Holstein, and Wei (2017) in the process.

==> _commands/_commands_1.tex <==
\makeatletter

%\input{_commands/objectmath/_objectmath_6008}

\input{_commands/automath/_automath_5022}

\input{_commands/basics/_basics_1}

\input{_commands/maps/maps_11}

\input{_commands/operators/operators_1}

\input{_commands/smalloperators/_smalloperators_1}

%Smaller versions of \otimes, \oplus, and \times, to be used in expressions concerning elements (a\sotimes b as apposed to A\otimes B)



\input{_commands/catlimits/_catlimits_3}


%\newcommand\comp{^{\scriptscriptstyle\bullet}}

%\newcommand\bicomp{^{\scriptscriptstyle\bullet\bullet}}


\input{_commands/arrows/_arrows_1}

\input{_commands/categories/_categories_2}

%\input{_commands/lie/_lie_1}

\input{_commands/abbreviations/_abbreviations_1}

\input{_commands/index/_index_1}

\input{_commands/page/_page_1}


\input{_commands/derivatives/_derivatives_1}



\input{_commands/slots/_slots_1}

\input{_commands/tuples/_tuples_2}

\input{_commands/delims/_delims_3}


\input{_commands/homology/_homology_1000}

\input{_commands/alg_geo/_alg_geo_1}


\input{_commands/intervals/_intervals_1}


\input{_commands/wraptext/_wraptext_1}
	

	
\input{_commands/widebar/_widebar_1}

%\makeatother

==> _commands/abbreviations/_abbreviations_1.tex <==
%Abbreviations:

\ExplSyntaxOn
\cs_new:Npn\newabbreviation#1#2#3{
	\cs_new:cpn { an#1 }{#2#3\xspace}
	\cs_new:cpn { An#1 }{\uppercase{#2}#3\xspace}
	\cs_new:cpn { an#1s }{#2#3s\xspace}
	\cs_new:cpn { An#1s }{\uppercase{#2}{#3}s\xspace}
}
\ExplSyntaxOff

\newabbreviation{hau}{H}{ausdorff}
\newabbreviation{rep}{r}{epresentation}
\newabbreviation{subrep}{s}{ubrepresentation}
\newabbreviation{irr}{i}{rreducible}
\newabbreviation{irrep}{i}{rreducible representation}
\newabbreviation{indec}{i}{ndecomposable}
\newabbreviation{coho}{c}{ohomology}
\newabbreviation{homal}{h}{omological}
\newabbreviation{homy}{h}{omology}
\newabbreviation{rhs}{r}{ight-hand side}
\newabbreviation{lhs}{l}{eft-hand side}
\newabbreviation{ses}{s}{hort exact sequence}
\newabbreviation{les}{l}{ong exact sequence}
\newabbreviation{cech}{\v{C}}{ech}

==> _commands/alg_geo/_alg_geo_1.tex <==
% for \reg etc, to be ed later.

%\input{_alg_geo/sheaf/sheaf_1}

\newmapclass{sheaf}[
	parent=map,
	%command=\mathscr,
	singlekeys={
		{sheafify} { upper={+} },
%		{*} { n=* },
		{dual}{upper=\vee},
	},
	keyvals={
		{stalk}{ci={\keyvalue}},
		%{res}{i=\vert\keyvalue},
		{twist}{symbolputright={(\keyvalue)}},
		{equivar}{upper={\keyvalue}},
	},
	output=alg,
]

%\newhomtype{Sheaf}[
%	singlekeys={
%		{sheafify} { upper={+} },
%		{*} { n=* },
%	},
%	keyvals={
%		{stalk}{ci={\inputvar}},
%		{res}{i=\vert\inputvar},
%	},
%]

%\newcotype

\newcommand\affineA{\mathbb{A}}
\newcommand\projectiveP{\mathbb{P}}
\newcommand\aff[2][]{
	\affineA^{\!\!#2}
	\ifblank{#1}
	{
		% do nothing
	}
	{
		_{#1}
	}
}
\newcommand\pspace[2][]{
	\projectiveP^{#2}
	\ifblank{#1}
	{
		% do nothing
	}
	{
		_{\!\!#1}
	}
}

\DeclareMathOperator\Specproto{Spec}

\newmap{\Spec}{\Specproto}
\let\spec=\Spec

\DeclareMathOperator\Projproto{Proj}

\newmap{\Proj}{\Projproto}
\let\proj=\Proj

%\let\sheaf=\mathscr

%\newcommand\shF{\sheaf{F}}
%\newcommand\shG{\sheaf{G}}
%\newcommand\shH{\sheaf{H}}
%\newcommand\shO{\sheaf{O}}
%\newcommand\shC{\sheaf{C}}
%\newcommand\shZ{\sheaf{Z}}
%\newcommand\shB{\sheaf{B}}

\newsheaf{\shF}{\mathscr{F}}
\newsheaf{\shG}{\mathscr{G}}
\newsheaf{\shH}{\mathscr{H}}
\newsheaf{\shO}{\mathscr{O}}
\newsheaf{\shC}{\mathscr{C}}
\newsheaf{\shZ}{\mathscr{Z}}
\newsheaf{\shB}{\mathscr{B}}

%\newcommand\reg[1]{ % regular functions
%	\shO
%	\ifblank{#1}
%	{
%		% do nothing
%	}
%	{
%		_{#1}
%	}
%}

%\newcommand\Reg{\shO} % regular functions without subscript

\newcommand\shhomsymbol{\mathscr{H\!\!{\scriptscriptstyle O\!\!\!M}}}


\newsheaf{\reg}{\mathscr{O}}

\newmap{\shhom}{\shhomsymbol}[parent=Hom,output=sheaf]


%\newoptcohomology\shhom{\shHom}
%\newhomologytheory{sh}{\shH}{\shC}{\shZ}{\shB}

%\newoptcohomology\sections{\Gamma}

==> _commands/arrows/_arrows_1.tex <==
\newcommand\isoto{\xrightarrow{ %isomorphism arrow
		\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}}}

\newcommand\medisoto{\xrightarrow{ %isomorphism arrow
		\,\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\,}}

\newcommand\longisoto{\xrightarrow{ %isomorphism arrow
		\;\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\;}}

\newcommand\isofrom{\xleftarrow{ %isomorphism arrow
		\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}}}

\newcommand\medisofrom{\xleftarrow{ %isomorphism arrow
		\,\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\,}}

\newcommand\longisofrom{\xleftarrow{ %isomorphism arrow
		\;\smash{\raisebox{-0.65ex}{\ensuremath{\scriptstyle\sim}}}\;}}
		


\providecommand*{\twoheadrightarrowfill@}{%
  \arrowfill@\relbar\relbar\twoheadrightarrow
}
\providecommand*{\twoheadleftarrowfill@}{%
  \arrowfill@\twoheadleftarrow\relbar\relbar
}
\providecommand*{\xtwoheadrightarrow}[2][]{%
  \ext@arrow 0579\twoheadrightarrowfill@{#1}{#2}%
}
\providecommand*{\xtwoheadleftarrow}[2][]{%
  \ext@arrow 5097\twoheadleftarrowfill@{#1}{#2}%
}


\newcommand\xto[1]{
	\xrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xinto[1]{
	\xhookrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xonto[1]{
	\xtwoheadrightarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xfrom[1]{
	\xleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xinfrom[1]{
	\xhookleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\xonfrom[1]{
	\xtwoheadleftarrow{\smash{\raisebox{-.2em}[0pt][0pt]{$\scriptscriptstyle#1$}}}
}

\newcommand\from{\leftarrow}
\newcommand\longto\longrightarrow
\newcommand\longfrom{\longleftarrow}

\newcommand{\hooklongrightarrow}{\lhook\joinrel\longrightarrow}
\newcommand{\twoheadlongrightarrow}{\relbar\joinrel\twoheadrightarrow}

\newcommand{\hooklongleftarrow}{\longleftarrow\joinrel\rhook}
\newcommand{\twoheadlongleftarrow}{\twoheadleftarrow\joinrel\relbar}

\newcommand\into{\hookrightarrow}
\newcommand\longinto{\hooklongrightarrow}

\newcommand\onto{\twoheadrightarrow}
\newcommand\longonto{\twoheadlongrightarrow}

\newcommand\infrom{\hookleftarrow}
\newcommand\longinfrom{\hooklongleftarrow}
\newcommand\onfrom{\twoheadleftarrow}
\newcommand\longonfrom{\twoheadlongleftarrow}

==> _commands/automath/_automath_5022.tex <==
\ExplSyntaxOn


\msg_new:nnnn { automath } { keyval_not_found } { Unknown~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\msg_new:nnnn { automath } { arg_keyval_not_found } { Unknown~argument~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\msg_new:nnnn { automath } { tl_not_found } { Unknown~data~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}
%IM should be changed so that this is passed to the actual object, not 
%IM the parent object, e.g., by having a third argument containing the
%IM actual object in \g_automath_tl_get:nn


\msg_new:nnnn { automath } { parent_not_found } { Unknown~class~#1~set~as~parent~of~object~#2~on~input~line~\msg_line_number: } {}

% Extra cs variants we need:

\cs_generate_variant:Nn \keyval_parse:NNn { cco }
\cs_generate_variant:Nn \tl_if_blank:nTF { vTF }

\tl_set:Nn \automath_bullet_tl {\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}
\tl_set:Nn \automath_double_bullet_tl {\automath_bullet_tl\automath_bullet_tl}

%IM make a command \automathrender that is a frontend to _render:nn,
%IM accessible from non-expl3 settings
%IM Similarly, \newobject and \newclass
%IM Similarly, \automathifdotTF (tests if equal to .) and
%IM \automathifblankTF (??).

%IM allow things like | |_\infty and -^2, e.g. \var{slot}[g=2]
%IM this could for instance be accomplished by allowing passing
%IM options to the output class. In order for this to work,
%IM we need a new interface for output classes, e.g. \var[opt1]{sym}[opt2]
%IM
%IM Better: make two commands, \var and \varwithoptions{opt1}{sym}[opt2]

%IMplement notation \var[\big]

%IM output=self requires functions taking only one argument.

%IM new class type: flextuple or simply tuple

%IM allow setup of slots

%IM Currently, \Set has unwanted behaviour; running \Set without arguments produces { } rather than
%IM nothing. Probably, this is a bad implementation of \arg

%IM need \mathopen and \mathclose for non-scaled pars, and also a new implementation
%IM with ifpars=true|false and partype=(), for instance. Also allow dot, like, partype=.) or /.

% This package is supposed to allow a kind of object-oriented
% mathematics. All objects are created as instances of some
% specific CLASS, and hence classes must be created before objects.
%
% The fundamental form of all output made with this system is of the
% form
%		symbol ^ { upper index } _ { lower index } ( argument )
% (though in one of the types of classes, the argument is meant to be
% empty).
%
% There are (currently) three types of classes with slightly different
% input interfaces
%	* VARIABLES, simple commands that do not take argument, like
%	  x, y_0, X^*, etc.
%	  The standard syntax is
%	  \command[options]
%	* MAPS, function-like commands that do take arguments, like
%	  f(x), g_1'(x), Hom_A(x,y), End(Z), etc.
%	  The standard syntax is
%	  \command[options]{optional argument in braces}
%	* COHOMOLOGIES, function-like commands that take two arguments,
%	  an index and an argument in parentheses, like H^0(X),
%	  Z_0(X), etc.
%	  The standard syntax is
%	  \command[options]{mandatory index argument}{optional argument in braces}

%IMPLEMENT COMPLEXES
%IMPLEMENT changes to allow notation { ! } { ... } instead of {!} { ... }

%IM Maybe the difference between \map{f} and \var[arg=f,output=map] should be removed

% Consequently, there are three different "new class" commands.
% All three of them make heavy use of the command
% \g_automath_new_object:nn, to be defined below, which is the
% low-level command for creating new objects of any class.

% Whenever you create a new class, named ⟨myclass⟩, you will get
% two commands with names based on ⟨myclass⟩ (so make sure
% that these are free):
% 		* \new⟨myclass⟩, which creates a new instance of the
%		  class ⟨myclass⟩.
%		* \⟨myclass⟩, a command to create a quick instance of
%		  ⟨myclass⟩ on the go; it will take an extra initial argument
%		  corresponding to the symbol. So if it has, say, map type,
%		  you can write \⟨myclass⟩{f}[options]{x} to get a ⟨myclass⟩
%		  object with symbol f and argument x.

% The two first of these classes go through great lengths to implement
% a way to write primes the classical way, like \varx' for x',
% since I assume that this is a feature most classical TeX users will
% appreciate. The last class, cohomology, goes to equal lengths to allow notations like \co*{X} for the *'th cohomology of X




\DeclareDocumentCommand\newvariableclass{mO{}} % new variable-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}t{'}t{'}}{
		% the actual \#1 command
		\IfBooleanTF{ ##3 }
		{
			\IfBooleanTF { ##4 }
			{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, prime, prime } }
			{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, prime } }
		}
		{	\automathrenderclass { #1 } { symbol = { ##1 }, ##2 }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}t{'}t{'}}{
		\IfBooleanTF{ ##4 }
		{
			\IfBooleanTF { ##5 }
			{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, prime, prime } }
			{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, prime } }
		}
		{	\automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3 }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } ##1 { parent = #1, symbol = { ##2 }, ##3 }
		% create the object with name ##1
		\DeclareDocumentCommand{##1}{O{}t{'}t{'}}{
		% the actual \##1 command
			\IfBooleanTF{ ####2 }
			{
				\IfBooleanTF { ####3 }
				{ \automathrenderobject { ##1 } { ####1, prime, prime } }
				{ \automathrenderobject { ##1 } { ####1, prime } }
			}
			{	\automathrenderobject { ##1 } { ####1 }	}
		}
	}
}

%IM Consider using \automathIfNoValueOrDotTF on the argument

\DeclareDocumentCommand\newmapclass{mO{}} % new map-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}t{'}t{'}G{}}{
		% the actual \#1 command
			\IfBooleanTF{ ##3 }
			{
				\IfBooleanTF { ##4 }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, prime, prime, arg={##5} } }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, prime,arg={##5} } }
			}
			{	\automathrenderclass { #1 } { symbol={##1}, ##2,arg={##5} }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}t{'}t{'}G{}}{
			\IfBooleanTF{ ##4 }
			{
				\IfBooleanTF { ##5 }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, prime, prime, arg={##6} } }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, prime,arg={##6} } }
			}
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3,arg={##6} }	}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } ##1 { parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}t{'}t{'}G{}}{
		% the actual \##1 command
			\IfBooleanTF{ ####2 }
			{
				\IfBooleanTF { ####3 }
				{ \automathrenderobject { ##1 } { ####1, prime,prime, arg={####4} } }
				{ \automathrenderobject { ##1 } { ####1, prime, arg={####4} }
				}
			}
			{	\automathrenderobject { ##1 } { ####1, arg={####4} }	}
		}
	}
}

\DeclareDocumentCommand\newcohomologyclass{mO{}} % new cohomology-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}mG{}}{
		% the actual \#1 command
		\automathifeqTF { ##3 }{ * }
		{	\automathrenderclass { #1 } { symbol={##1}, ##2, *, arg={##4} }	}
		{
			\automathifeqTF { ##3 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##1}, ##2, **, arg={##4} }	}
			{
				\automathifblankordotTF { ##3 }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, arg={##4} } }
				{ \automathrenderclass { #1 } { symbol={##1}, ##2, degreedefault={##3}, arg={##4} } }
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}mG{}}{
		\automathifeqTF { ##4 }{ * }
		{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, *, arg={##5} }	}
		{
			\automathifeqTF { ##4 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, **, arg={##5} }	}
			{
				\automathifblankordotTF { ##4 }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, arg={##5} } }
				{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, degreedefault={##4}, arg={##5} } }
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}mG{}}{
			% the actual \##1 command
			\automathifeqTF { ####2 } { * }
			{	\automathrenderobject { ##1 } {  ####1, *, arg={ ####3 } }	}
			{
				\automathifeqTF { ####2 } { ** }
				{	\automathrenderobject { ##1 } {  ####1, **, arg={ ####3 } }	}
				{
					\automathifblankordotTF { ####2 }
					{ \automathrenderobject { ##1 } {  ####1, arg={ ####3 } } }
					{ \automathrenderobject { ##1 } {  ####1, degreedefault={ ####2 }, arg={ ####3 } } }
				}
			}
		}
	}
}

\DeclareDocumentCommand\newcomplexclass{mO{}} % new cohomology-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}g}{
		% the actual \#1 command
		\automathifeqTF { ##3 }{ * }
		{	\automathrenderclass { #1 } { symbol={##1}, ##2, * }	}
		{
			\automathifeqTF { ##3 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##1}, ##2, ** }	}
			{
				\IfValueTF { ##3 }
				{
					\automathifblankordotTF { ##3 }
					{ \automathrenderclass { #1 } { symbol={##1}, ##2 } }
					{ \automathrenderclass { #1 } { symbol={##1}, ##2, degreedefault={##3} } }
				}
				{
					\automathrenderclass { #1 } { symbol={##1}, ##2 }
				}
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}g}{
		\automathifeqTF { ##4 }{ * }
		{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, * }	}
		{
			\automathifeqTF { ##4 }{ ** }
			{	\automathrenderclass { #1 } { symbol={##2}, ##1, ##3, ** }	}
			{
				\IfValueTF { ##4 }
				{
					\automathifblankordotTF { ##4 }
					{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3 } }
					{ \automathrenderclass { #1 } { symbol={##2}, ##1, ##3, degreedefault={##4} } }
				}
				{
					\automathrenderclass { #1 } { symbol={##2}, ##1, ##3 }
				}
			}
		}
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, symbol = { ##2 }, ##3 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}g}{%
			% the actual \##1 command
			\automathifeqTF { ####2 } { * }
			{	\automathrenderobject { ##1 } {  ####1, * }	}
			{
				\automathifeqTF { ####2 } { ** }
				{	\automathrenderobject { ##1 } {  ####1, ** }	}
				{
					\IfValueTF { ####2 }
					{
						\automathifblankordotTF { ####2 }
						{ \automathrenderobject { ##1 } {  ####1 } }
						{ \automathrenderobject { ##1 } {  ####1, degreedefault={ ####2 } } }
					}
					{
						\automathrenderobject { ##1 } {  ####1 }
					}
				}
			}
		}
	}
}

%
\DeclareDocumentCommand\newtupleclass{mO{}} % new tuple-type class
{
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } { #2 }
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}m}{
		% the actual \#1 command
		\automathrenderclass { #1 }{ symbol = { ##1 }, ##2, arg = { ##3 } }
	}
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmmO{}}{
		\automathrenderclass { #1 }{ symbol = { ##2 }, ##1, ##3, arg = { ##4 } }
	}
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmmmmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 } % creates the object with name ##1
		{ parent = #1, leftpar = { ##2 }, argsep = { ##3 }, rightpar = { ##4 }, argdots = { ##5 }, ##6 }
		\DeclareDocumentCommand{##1}{O{}G{}}{
		% the actual \##1 command
			\IfNoValueTF { ####2 }
			{	\automathrenderobject { ##1 } { ####1 } }
			{	\automathrenderobject { ##1 } { ####1, arg = { ####2 } } }
		}
	}
}

\DeclareDocumentCommand\newdelimiterclass{mO{}} % new delimiter-type class
{
	%IM this needs updating: We need an option not to use the arg keyvals,
	%IM for right now, autopars do not work for \Set
	% #1 = class name
	% #2 = options
	\automathnewclass { #1 } {
		keyvals={
			{arg}{argwithoutkeyval=\keyvalue},
			%Currently, no braces around \keyvalue is necessary for \automathdelimsize to work
			% with par=auto
		},
		#2
	}
	\exp_args:Nc\DeclareDocumentCommand{#1}{mO{}m}
	{ \automathrenderclass { #1 } { symbol = { ##1 }, ##2, arg = { ##3 } } }
	% the actual \#1 command
	\exp_args:Nc\DeclareDocumentCommand{#1withoptions}{mmO{}m}
	{ \automathrenderclass { #1 } { symbol = { ##2 }, ##1, ##3, arg = { ##4 } } }
	\exp_args:Nc\DeclareDocumentCommand{new#1}{mmmO{}}
	{
		% the command for creating a new object of class #1
		% ##1 = command name, with backslash
		% ##2 = symbol
		% ##3 = options
		\automathnewobject { #1 } { ##1 }{ parent = #1, leftpar = { ##2 }, rightpar = { ##3 }, ##4 }
		% creates the object with name ##1
		\DeclareDocumentCommand{##1}{O{}G{}}{
		% the actual \##1 command
			\IfNoValueTF { ####2 }
			{	\automathrenderobject { ##1 } { ####1 }	}
			{	\automathrenderobject { ##1 } { ####1, arg = { { ####2 } } } }
		}
	}
}

\cs_generate_variant:Nn \tl_if_eq:nnTF { xnTF }

\cs_generate_variant:Nn \tl_if_eq:nnF { xnF }

\cs_generate_variant:Nn \tl_if_eq:nnT { xnT }

\DeclareDocumentCommand{\automathifblankordotTF}{mmm}
{
	\tl_if_blank:nTF { #1 }
	{	#2	}
	{
		\tl_if_eq:xnTF { \tl_trim_spaces:n { #1 } } { . } { #2 } { #3 }
	} 
}

\DeclareDocumentCommand{\automathifblankordotT}{mm}
{
	\tl_if_blank:nTF { #1 }
	{	#2	}
	{
		\tl_if_eq:xnT { \tl_trim_spaces:n { #1 } } { . } { #2 }
	} 
}

\DeclareDocumentCommand{\automathifblankordotF}{mm}
{
	\tl_if_blank:nF { #1 }
	{
		\tl_if_eq:xnF { \tl_trim_spaces:n { #1 } } { . } { #2 }
	} 
}

\cs_set_eq:NN\automathifeqTF\tl_if_eq:nnTF

\cs_set_eq:NN\automathifeqT\tl_if_eq:nnT

\cs_set_eq:NN\automathifeqF\tl_if_eq:nnF



\cs_new:Npn \g_automath_new_class:nn#1#2{
	% create a new class
	% #1 = name of class
	% #2 = standard keyval setup; the parent class by default is automathvariable
	\g_automath_new_object:nnn { automathvariable } { #1 } { #2 }
}


\cs_set_eq:NN\automathnewclass\g_automath_new_class:nn

\seq_new:N \automath_all_objects_seq


\seq_put_right:Nn \automath_all_objects_seq { automathvariable }



\cs_new:Npn \g_automath_new_object:nnn#1#2#3{ % create new object
	% #1 = class of command
	% #2 = name of command, without backslash
	% #3 = standard keyval setup

	\g_automath_tl_provide:nn { #2 } { parent }

	\tl_set:cn { g_automath_#2_parent } { automathvariable }


	\cs_set:cpn { g_automath_#2_keyval:nn } ##1##2 % command controlling keyvals
	{ \g_automath_keyval:nnnn { ##2 } { ##1 } { #1 } { #2 } }

	\cs_set:cpn { g_automath_#2_singlekey:n } ##1 % command controlling singlekeys
	{ \g_automath_singlekey:nnn { ##1 } { #1 } { #2 } }
	

	% Now a similar collection of keyval commands for the *argument*
	
	\cs_set:cpn { g_automath_#2_arg_keyval:nn } ##1##2
	{ \g_automath_arg_keyval:nnnn { ##2 } { ##1 } { #1 } { #2 } }
	
	\cs_set:cpn { g_automath_#2_arg_singlekey:n } ##1
	{ \g_automath_arg_singlekey:nnn { ##1 } { #1 } { #2 } }

	
	% initially sets up the keyval interface of the object
	\g_automath_keys_set:nn { #2 } { parent=#1, #3 }
	
	\seq_put_right:Nx \automath_all_objects_seq { #2 }
}




% Get-type commands:
%IM All of this data should have g_ removed and get _tl

\cs_new:Npn \g_automath_tl_get:nn#1#2% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	%\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\bool_if:cTF { g_automath_#1_#2_if_provided }
		%{ \use:c { g_automath_#1_#2 } }
		%{ \g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2} }
		\use:c { g_automath_#1_#2 }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
			%\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			%\g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2}%
			\g_automath_tl_get:cn { g_automath_#1_parent } { #2 }
		%}
	}%
}

\cs_new:Npn \g_automath_tl_get_exp_not:nn#1#2% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	%\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\bool_if:cTF { g_automath_#1_#2_if_provided }
		%{ \use:c { g_automath_#1_#2 } }
		%{ \g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2} }
		%\use:c { g_automath_#1_#2 }
		\exp_not:v { g_automath_#1_#2 }
		%\exp_not:n { \use:c { g_automath_#1_#2 } }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
			%\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			%\g_automath_tl_get:nn{\g_automath_tl_get:nn{#1}{parent}}{#2}%
			\g_automath_tl_get:cn { g_automath_#1_parent } { #2 }
		%}
	}%
}

\cs_generate_variant:Nn \g_automath_tl_get:nn { cn }



\cs_new:Npn \g_automath_tl_get_store:nnN#1#2#3% maybe should be PROTECTED??
{
	% #1 = name of object
	% #2 = the data to get
	% #3 = where to store it
	%\exp_args:Nnno
	\tl_if_exist:cTF { g_automath_#1_#2 }%IM replace by check for if_provided
	{%
		%\use:c { g_automath_#1_#2 }%
		\tl_set_eq:Nc #3 { g_automath_#1_#2 }
		%\tl_set:Nn#3 { automathvariable }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
%		\tl_if_eq:nnTF { #1 } { automathvariable }
%		{
%			\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
%		}
%		{
			%\g_automath_tl_get_store:nnN{\g_automath_tl_get:nn{#1}{parent}}{#2}#3%
			\g_automath_tl_get_store:cnN { g_automath_#1_parent } { #2 } #3
%		}
	}%
}

\cs_generate_variant:Nn \g_automath_tl_get_store:nnN { cnN, nnc, cnc }

\cs_new:Npn\g_automath_tl_provide:nn#1#2
{
	%\tl_if_exist:cF { g_automath_#1_#2 } { \tl_new:c { g_automath_#1_#2 } }
	%\bool_if_exist:cF { g_automath_#1_#2_if_provided } { \bool_new:c { g_automath_#1_#2_if_provided } }
	%\bool_set_true:c { g_automath_#1_#2_if_provided }
	\tl_if_exist:cF { g_automath_#1_#2 } { \tl_set:cn { g_automath_#1_#2 } {} }
}

%\cs_new:Npn\g_automath_tl_unprovide:nn#1#2
%{
	%\tl_if_exist:cF { g_automath_#1_#2 } { \tl_new:c { g_automath_#1_#2 } }
	%\bool_if_exist:cF { g_automath_#1_#2_if_provided } { \bool_new:c { g_automath_#1_#2_if_provided } }
	%\bool_set_true:c { g_automath_#1_#2_if_provided }
%}

\cs_new:Npn\g_automath_tl_inherit:nn#1#2
{
	\tl_if_exist:cF { g_automath_#1_#2 }
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
		%IM could be replaced by simply { #1 } { #2 } once the check is made
		%IM based on "if_provided"
	}
}

\cs_new:Npn\g_automath_tl_inherit_x:nn#1#2
{
	\tl_if_exist:cF { g_automath_#1_#2 }
	{
			\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
	{
		\g_automath_tl_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
		%IM could be replaced by simply { #1 } { #2 } once the check is made
		%IM based on "if_provided"
	}
}




\cs_new:Npn \g_automath_seq_get_store:nnN#1#2#3{% maybe should be PROTECTED??
	% #1 = name of object
	% #2 = the sequence to get
	% #3 = the command to store it in
	%\seq_if_exist:cTF { g_automath_#1_#2 }%
	\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{%
		%\seq_set_eq:Nc#3 { g_automath_#1_#2 }
		\bool_if:cTF { g_automath_#1_#2_if_provided }
		{ \seq_set_eq:Nc#3 { g_automath_#1_#2 } }
		{ \g_automath_seq_get_store:cnN{ g_automath_#1_parent }{#2}#3 }
	}%
	{%
		%\exp_args:No
		%\exp_args:No
		%\tl_if_eq:nnTF { #1 } { automathvariable }
		%{
		%	\msg_error:nnnn { automath } { data_not_found } { #2 } { #1 }
		%}
		%{
			\g_automath_seq_get_store:cnN{ g_automath_#1_parent }{#2}#3%
		%}
	}%
}

\cs_generate_variant:Nn \g_automath_seq_get_store:nnN { cnN, nnc, cnc }

\cs_new:Npn\g_automath_seq_inherit:nn#1#2
{
	\bool_if_exist:cTF { g_automath_#1_#2_if_provided }
	{
		\bool_if:cF { g_automath_#1_#2_if_provided }
		{
			\g_automath_seq_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
			\bool_set_true:c { g_automath_#1_#2_if_provided }
		}
	}
	{
		\bool_new:c { g_automath_#1_#2_if_provided }
		\bool_set_true:c { g_automath_#1_#2_if_provided }
		\seq_if_exist:cF { g_automath_#1_#2 } { \seq_new:c { g_automath_#1_#2 } }
		\g_automath_seq_get_store:cnc { g_automath_#1_parent } { #2 } { g_automath_#1_#2 }
	}
}





\cs_new:Npn \g_automath_prop_provide:nn#1#2
{
	% #1 = name of the object
	% #2 = name of the prop
	\prop_if_exist:cF { g_automath_#1_#2 } { \prop_new:c { g_automath_#1_#2 } }
}


\cs_new:Npn \g_automath_keyval_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = keyval data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_keyvals } { #2 }#3%\l_automath_keyval_get_temp
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_keyval_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_keyval_get:nnNTF { vnNTF }

\cs_new:Npn \g_automath_singlekey_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = singlekey data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_singlekeys } { #2 } #3
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_singlekey_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_singlekey_get:nnNTF { vnNTF }

%\cs_new:N\l_automath_arg_keyval_get_parent_temp

\cs_new:Npn \g_automath_arg_keyval_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = keyval data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_arg_keyvals } { #2 }#3%\l_automath_keyval_get_temp
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 }
		{ \g_automath_arg_keyval_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_arg_keyval_get:nnNTF { vnNTF }

\prop_new:N\l_automath_arg_keyval_get_temp

\cs_new:Npn \g_automath_arg_singlekey_get:nnNTF#1#2#3#4#5{%
	% #1 = name of the object
	% #2 = singlekey data to get
	% #3 = command to store possible data in
	% #4 = if true (not to be used)
	% #5 = if false
	\prop_get:cnNTF { g_automath_#1_custom_arg_singlekeys } { #2 } #3
	{	#4	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #5 } { \g_automath_arg_singlekey_get:vnNTF { g_automath_#1_parent } { #2 } #3 { #4 } { #5 } }
	}
}

\cs_generate_variant:Nn \g_automath_arg_singlekey_get:nnNTF { vnNTF }

\cs_new:Npn\g_automath_bool_get:nnTF#1#2#3#4
{
	% #1 = name of the object
	% #2 = boolean to get
	% #3 = if true
	% #4 = if false
	\bool_if_exist:cTF { g_automath_#1_if_#2_if_provided }
	{
		\bool_if:cTF { g_automath_#1_if_#2_if_provided }
		{
			\bool_if:cTF { g_automath_#1_if_#2 } { #3 } { #4 }
		}
		{
			\tl_if_eq:nnTF { #1 } { automathvariable }
			{ #4 } { \g_automath_bool_get:vnTF { g_automath_#1_parent } { #2 } { #3 } { #4 } }
		}
	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{ #4 } { \g_automath_bool_get:vnTF { g_automath_#1_parent } { #2 } { #3 } { #4 } }
	}
}

\cs_generate_variant:Nn \g_automath_bool_get:nnTF { xnTF, cnTF, vnTF }

\cs_new:Npn\g_automath_bool_provide:nn#1#2
{
	% #1 = name of the object
	% #2 = boolean to provide
	\bool_if_exist:cTF { g_automath_#1_if_#2_if_provided }
	{
		\bool_if:cF { g_automath_#1_if_#2_if_provided }
		{	\bool_set_true:c { g_automath_#1_if_#2_if_provided }	}
	}
	{
		\bool_new:c { g_automath_#1_if_#2 }
		\bool_new:c { g_automath_#1_if_#2_if_provided }
		\bool_set_true:c { g_automath_#1_if_#2_if_provided }
	}
}

\cs_new:Npn\g_automath_cs_get:nnn#1#2#3
{
	% #1 = name of the object
	% #2 = command sequence to get
	% #3 = what to apply said sequence to
	\cs_if_exist:cTF { g_automath_#1_#2:n }
	{	\use:c { g_automath_#1_#2:n } { #3 }	}
	{
		\tl_if_eq:nnTF { #1 } { automathvariable }
		{
			% should probably throw an error by now, but later!
		}
		{
			\g_automath_cs_get:xnn { \g_automath_tl_get:nn{#1}{parent} } { #2 } { #3 }
		}
	}
}

\cs_generate_variant:Nn \g_automath_cs_get:nnn { xnn }


%\cs_set_eq:NN \automathnewobject \g_automath_new_object:nnn

\cs_generate_variant:Nn \g_automath_new_object:nnn { nxn }

\cs_set:Npn \automathnewobject#1#2#3
{	\g_automath_new_object:nxn { #1 }{ \cs_to_str:N #2 } { #3 }	}


%Now everything that has to do with creation of new objects


\cs_new:Npn \g_automath_keys_set:nn#1#2
{
	% #1 = object
	% #2 = keys
	\keyval_parse:cco %IM think about wthether o-type is really necessary.
	{ g_automath_#1_singlekey:n }
	{ g_automath_#1_keyval:nn }
	{ #2 }
}

\cs_new:Npn \g_automath_arg_keys_set:nn#1#2
{
	% #1 = object
	% #2 = keys
	\keyval_parse:cco %IM -||-
	{ g_automath_#1_arg_singlekey:n }
	{ g_automath_#1_arg_keyval:nn }
	{ #2 }
}

\DeclareDocumentCommand\setupclass{mm}{ % a user-level command for setting up the object
	% #1 = class
	% #2 = setup
	%\exp_args:Nx
	%\use:c { g_automath_#1_keys_set:n }
	\g_automath_keys_set:nn { #1 }{ #2 }
}

\DeclareDocumentCommand\setupobject{mm}{%
	% #1 = object
	% #2 = setup
	%\use:c { g_automath_\cs_to_str:N#1_keys_set:n }
	\g_automath_keys_set:nn { \cs_to_str:N #1 } { #2 }
}




\cs_new_protected:Npn \g_automath_render:nn#1#2
{
	%IM Render and return should be merged; return could be equivalent to the keys {render, clearstuff}
	%IM No reason to have the same code twice
	% the main command for rendering the command corresponding to the object #2 of class #1 with options #3
	\group_begin:
		%\use:c{ g_automath_#1_keys_set:n } { #2 } % set up the keyval interface
		\g_automath_keys_set:nn { #1 } { #2 }
		\tl_set:Nx\l__automath_symbol_temp { \g_automath_tl_get:nn { #1 } { symbol } } %IM chang to "store" solution
		%\g_automath_tl_get_store:nnN { #1 } { symbol } \l__automath_symbol_temp
		\g_automath_seq_get_store:nnN { #1 } { commands_sequence } \l__automath_commands_sequence_temp_seq
		%\seq_map_inline:cn { g_automath_#1_commands_sequence }
		\seq_map_inline:Nn\l__automath_commands_sequence_temp_seq
		{
			\tl_set:Nx \l__automath_symbol_temp
			{
				\exp_not:n { ##1 } { \exp_not:V \l__automath_symbol_temp }
			}
		}
		\tl_set:Nx\l__automath_render_temp
		{ % set a temporary command that contains the entire output
				%IM should test if symbol, index etc. are non-empty,
				%IM hen assign one by one. The same at return.
				\exp_not:V \l__automath_symbol_temp
%				% Setup indices:
				\exp_not:N\g_automath_upper_index:n
				{
					\g_automath_tl_get:nn { #1 } { upper_index }
				}
				\exp_not:N\g_automath_lower_index:n {
					\g_automath_tl_get:nn { #1 } { lower_index }
				}
		}%
		\g_automath_bool_get:nnTF { #1 } { par }
		{
			\tl_put_right:Nx \l__automath_render_temp
			{
				\exp_not:N
				\g_automath_parentheses:nnnn
				{ \g_automath_tl_get:nn { #1 } { par_size } }
				{ \g_automath_tl_get:nn { #1 } { par_open } }
				{ \g_automath_tl_get:nn { #1 } { par_close } }
				{ \g_automath_tl_get:nn { #1 }{ arg } } % apply argument command to argument
			}
		}
		{
			\tl_put_right:Nx \l__automath_render_temp
			{	\g_automath_tl_get:nn { #1 }{ arg }	}
		}
		\g_automath_bool_get:nnTF { #1 } { output } %IM p-q tests show that this does not work
		{
			\tl_set:Nx \l__automath_render_temp
			{
				\exp_not:c { \g_automath_tl_get:nn { #1 } { output }withoptions } { \g_automath_tl_get:nn { #1 } { output_options } } { \exp_not:V 
				\l__automath_render_temp }
			}
		}
		{
			% if false; do nothing
		}
	\exp_last_unbraced:NV
	\group_end:
	\l__automath_render_temp
}

\cs_set_eq:NN\automathrenderclass\g_automath_render:nn % a front-end command

\cs_set:Npn\automathrenderobject#1#2
{
	\g_automath_render:nn { \cs_to_str:N #1 } { #2 }
}




\cs_generate_variant:Nn \tl_put_right:cn { cf }

\cs_new:Npn\g_automath_primitive_singlekey_return:n#1
{
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_seq_inherit:nn { #1 } { commands_sequence }
	\seq_map_inline:cn { g_automath_#1_commands_sequence }
	%IM must do the same as for the symbol, also to upper index etc.
		{
			\tl_set:cx { g_automath_#1_symbol }
			{
				\exp_not:n {\exp_not:N ##1}  { \exp_not:v { g_automath_#1_symbol } }
				%IM no idea why we needed and extra \exp_not:n
			}
		}
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%IMPLEMENT THIS!!!
	\tl_set:cx { g_automath_#1_symbol }
	{
		%\g_automath_tl_get:nn { #1 }{ symbol }
		\exp_not:v { g_automath_#1_symbol }
		% Setup indices:
		\exp_not:N\g_automath_upper_index:n
		{
			%\exp_not:f { \g_automath_tl_get:nn { #1 } { upper_index } }
			%IM for unknown reasons, :f did the trick here
			\exp_not:v { g_automath_#1_upper_index }
		}
		\exp_not:N\g_automath_lower_index:n {
			%\exp_not:v { g_automath_#1_lower_index }
			%\exp_not:f { \g_automath_tl_get:nn { #1 } { lower_index } }
			%\exp_not:x { \exp_not:n { \g_automath_tl_get:nn { #1 } { lower_index } }}
			%IM for unknown reasons, :f did the trick here
			\exp_not:v { g_automath_#1_lower_index }
		}
	}
	\g_automath_bool_get:nnTF { #1 } { par }
	{
		%\g_automath_tl_inherit:nn { #1 } { par_size }
		\g_automath_tl_get_store:nnN { #1 } { par_size } \l__automath_render_par_size_temp
		\tl_put_right:cn { g_automath_#1_symbol }
		{
			\exp_not:N
			\g_automath_parentheses:nnnn
		}
		\tl_put_right:cx { g_automath_#1_symbol }
		{
			%{ \exp_not:v { g_automath_#1_par_size } }
			{ \exp_not:V \l__automath_render_par_size_temp }
			{ \g_automath_tl_get:nn { #1 } { par_open } }
			{ \g_automath_tl_get:nn { #1 } { par_close } }
			{ \exp_not:v { g_automath_#1_arg } }
		}
	}
	{
		\tl_put_right:cx { g_automath_#1_symbol }
		{	\exp_not:v { g_automath_#1_arg }	}
	}
	\tl_clear:c { g_automath_#1_upper_index }
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_true:c { g_automath_#1_if_first_upper }
	\tl_clear:c { g_automath_#1_lower_index }
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_true:c { g_automath_#1_if_first_lower }
	\tl_clear:c { g_automath_#1_arg }
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_true:c { g_automath_#1_if_first_arg }
	\seq_clear:c { g_automath_#1_commands_sequence }
	%IM maybe one should enclose the new symbol in another group
	%IM should also reset stuff like par size
	%IM reset leftpar, rightpar, parsize etc. also
}


%Commands for rendering the argument:



\cs_new:Npn \g_automath_lower_index:n #1{
	% controls rendering of lower indices
	\tl_if_blank:nF { #1 } { \sb{#1} }
}




\cs_new:Npn \g_automath_upper_index:n #1{
	% controls rendering of upper indices
	\tl_if_blank:nF { #1 } { \sp{#1} }
}





\tl_new:N\automathdelimsize


%\cs_generate_variant:Nn \g_automath_parentheses:nnnn { vnnn, vvvn }

\cs_new:Npn \g_automath_parentheses:nnnn#1#2#3#4
{
	\tl_if_blank:nF { #4 }
	{
		\str_case:nnF { #1 }
		{
			{ normal } {
				\group_begin:
				\mathopen#2 #4 \mathclose#3
				\group_end:
			}
			{ auto } {
				\group_begin:
				\tl_set:Nn\automathdelimsize{\middle}
				\left#2 #4 \right#3
				\group_end:
			}
			{ * } {
				\group_begin:
				\tl_set:Nn\automathdelimsize{\middle}
				\left#2 #4 \right#3
				\group_end:
			}
%			{ \big } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\big
%				\mathopen\big#2 #4 \mathclose\big#3
%				\group_end:
%			}
%			{ \Big } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\Big
%				\mathopen\Big#2 #4 \mathclose\Big#3
%				\group_end:
%			}
%			{ \bigg } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\bigg
%				\mathopen\bigg#2 #4 \mathclose\bigg#3
%				\group_end:
%			}
%			{ \Bigg } {
%				\group_begin:
%				\tl_set_eq:NN\automathdelimsize\Bigg
%				\mathopen\Bigg#2 #4 \mathclose\Bigg#3
%				\group_end:
%			}
		}
		{
			\group_begin:
			\tl_set_eq:NN\automathdelimsize#1
			\mathopen#1#2 #4 \mathclose#1#3
			\group_end:
		}
	}
}

\cs_new:Npn \g_automath_symbol_parentheses:nnnn#1#2#3#4
{
	\tl_if_blank:nF { #4 }
	{
		\str_case:nnF { #1 }
		{
			{ normal } { \mathopen#2 #4 \mathclose#3 }
			{ auto } { \left#2 #4 \right#3 }
			{ * } { \left#2 #4 \right#3 }
		}
		{ \mathopen#1#2 #4 \mathclose#1#3 }
	}
}


% Now for the commands that implement the keyval interface.
% These commands are used by the command \g_automath_#1_keys_set, see
% above.
% There is a fixed collection of primitive commands.
% Furthermore, the user has the option to create a collection
% of new commands, which are all stored in the token list
% called \g_automath_#1_custom_keyvals
% These keyvals contain code that must be executable by other keys
% (e.g., primitive ones)
% The key value is accessible to the user via the temporary command
% \keyvalue



\cs_new:Npn\g_automath_primitive_keyval_parent:nn#1#2{
	% Must inherit everything from the parent class
	%\tl_clear_new:c { g_automath_#1_parent }
	%\g_automath_tl_provide:nn { #1 } { parent }
	%IM This should always be declared, so no need for if_provided checks
	%IM This does not work, for unknown reasons:
%	\seq_if_in:NxTF \automath_all_objects_seq { #2 }
%	{	\tl_set:cn { g_automath_#1_parent } { #2 }	}
%	{ \msg_error:nnnn { automath } { parent_not_found } { #2 } { #1 } }
	%IM control if exists!
	\tl_set:cn { g_automath_#1_parent } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_keyvals:nn#1#2{
	% Add new keyvals via the interface
	% keyvals={
	%	{key1}{do something with \keyvalue},
	%	{key2}{g=\keyvalue,i=\keyvalue},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_keyvals }
	\clist_map_inline:nn { #2 }{
		\g_automath_keyval_equality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_keyval_equality_format:nnn#1#2#3{
	%\prop_put:cnn { g_automath_#1_custom_keyvals }{#2}{#3}
	\prop_put:cnn { g_automath_#1_custom_keyvals }{#2}{#3}
	%IM Remove spaces in #2
}

\cs_new:Npn\g_automath_primitive_keyval_singlekeys:nn#1#2{
	% Add sinple keys, taking no values, via the
	% interface
	% singlekeys={
	%	{key1}{print something},
	%	{key2}{g=42,i=42},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_singlekeys }
	\clist_map_inline:nn { #2 }{
		\g_automath_keyval_noequality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_keyval_noequality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_singlekeys }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_argkeyvals:nn#1#2{
	% Add new keyvals via the interface
	% keyvals={
	%	{key1}{do something with \keyvalue},
	%	{key2}{g=\keyvalue,i=\keyvalue},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_arg_keyvals }
	\clist_map_inline:nn { #2 }{
		\g_automath_arg_keyval_equality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_arg_keyval_equality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_arg_keyvals }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_argsinglekeys:nn#1#2{
	% Add sinple keys, taking no values, via the
	% interface
	% singlekeys={
	%	{key1}{print something},
	%	{key2}{g=42,i=42},
	% }
	\g_automath_prop_provide:nn { #1 } { custom_arg_singlekeys }
	\clist_map_inline:nn { #2 }{
		\g_automath_arg_keyval_noequality_format:nnn{#1}##1
	}
}

\cs_new:Npn \g_automath_arg_keyval_noequality_format:nnn#1#2#3{
	\prop_put:cnn { g_automath_#1_custom_arg_singlekeys }{#2}{#3}
}

\cs_new:Npn\g_automath_primitive_keyval_symbol:nn#1#2{
	% Sets the value of the symbol
	%\tl_clear_new:c { g_automath_#1_symbol }
	%\g_automath_tl_provide:nn { #1 } { symbol }
	\g_automath_tl_provide:nn { #1 } { symbol }
	\tl_set:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_symbol } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_slot:nn#1#2{
	% Sets the value of the symbol
	%\tl_clear_new:c { g_automath_#1_symbol }
	%\g_automath_tl_provide:nn { #1 } { symbol }
	\g_automath_tl_provide:nn { #1 } { slot }
	\tl_set:cn { g_automath_#1_slot } { \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_symbol } { #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_symbolputright:nn#1#2{
	% Sets the value of the symbol
%	\tl_if_exist:cTF { g_automath_#1_symbol }
%	{
%		% do nothing
%	}
%	{
%		\tl_set:cn { g_automath_#1_symbol } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { symbol } }
%	}
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\tl_put_right:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_symbolputleft:nn#1#2{
	% Sets the value of the symbol
%	\tl_if_exist:cTF { g_automath_#1_symbol }
%	{
%		% do nothing
%	}
%	{
%		\tl_set:cn { g_automath_#1_symbol } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { symbol } }
%	}
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\tl_put_left:cn { g_automath_#1_symbol } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_command:nn#1#2{
	% Adds one entry on the left of the command
	% sequence to be applied to the symbol
%	\seq_if_exist:cTF { g_automath_#1_commands_sequence }
%	{
%		% do nothing
%	}
%	{
%		\seq_new:c { g_automath_#1_commands_sequence }
%%		%\seq_set_eq:c
%%		%IMplement this
%		\g_automath_seq_get_store:nnc { \g_automath_tl_get:nn { #1 } { parent } } { commands_sequence } { g_automath_#1_commands_sequence }
%	}
	\g_automath_seq_inherit:nn { #1 } { commands_sequence }
	%\seq_put_right:co { g_automath_#1_commands_sequence } { \exp_not:N #2 } %IM maybe \exp_not:n { #2 }?
	\seq_put_right:cn { g_automath_#1_commands_sequence } { #2 } %IM maybe \exp_not:n { #2 }?
	%\seq_put_right:co { g_automath_#1_commands_sequence } { \exp_not:n{\exp_not:N#2} } %IM maybe \exp_not:n { #2 }?
	%\seq_put_right:cn { g_automath_#1_commands_sequence } { \exp_not:N #2 } %IM maybe \exp_not:n { #2 }?
}

\cs_new:Npn\g_automath_primitive_keyval_argwithkeyval:nn#1#2{
	% Sets the argument (printed in parentheses
	% after the symbol)
	\g_automath_arg_keys_set:nn { #1 } {{{ #2 }}}
	%IM for unknown reasons, one needs these extra braces.
}

\cs_new:Npn\g_automath_primitive_keyval_argwithoutkeyval:nn#1#2{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg }
%		{ \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }
%		%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_provide:nn { #1 } { arg } %IM maybe replace by _x, as above
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	\str_case:nnTF { #2 } { { * } { } { - } { } { slot } { } }
	{ \tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { \g_automath_tl_get:nn { #1 } { slot } } } }
	{	\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \exp_not:n{#2} } }	}
	%\tl_put_right:cx { g_automath_#1_arg } { #2 }
	%\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { #2 } }
	%\tl_put_right:cx { g_automath_#1_arg } { #2 }
	%IM :cx should probably be considered, too, at the place
	%IM where arguments are added via keyval.
	%IM THIS IS VERY WEIRD!!!
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
}


%				{ postcommand } {
%					% to be implemented; a command applied to the
%					% entire  
%				}


\cs_new:Npn\g_automath_primitive_keyval_argsep:nn#1#2
{
	%\tl_clear_new:c { g_automath_#1_argsep }
	\g_automath_tl_provide:nn { #1 } { argsep }
	\tl_set:cn { g_automath_#1_argsep } { \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_argdots:nn#1#2
{
	%\tl_clear_new:c { g_automath_#1_argdots }
	\g_automath_tl_provide:nn { #1 } { argdots }
	\tl_set:cn { g_automath_#1_argdots } { \exp_not:n { #2 } }
}


\cs_new:Npn\g_automath_primitive_keyval_output:nn#1#2
{
	% the class that the output of the command has
	%\g_automath_tl_provide:nn { #1 } { output }
	%IM Add this again!!!
	\tl_set:cn { g_automath_#1_output } { #2 }
	%IM check if defined, and also allow output=self for e.g.
	%IM derived functors. RHom should be same class as Hom
	%IM but R(sheaf hom) should be a sheaf.
}

\cs_new:Npn\g_automath_primitive_keyval_nowoutput:nn#1#2
{
	\g_automath_primitive_keyval_parent:nn { #1 } { #2 }
	\g_automath_primitive_keyval_output:nn { #1 } { #2 }
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
}

\cs_new:Npn\g_automath_primitive_keyval_outputoptions:nn#1#2{
	\g_automath_tl_provide:nn { #1 } { output_options }
	%\tl_put_right:cf { g_automath_#1_output_options } { \exp_not:n { #2 } }
	%\tl_put_right:cf { g_automath_#1_output_options } { #2 }
	\tl_put_right:cn { g_automath_#1_output_options } { #2 }
}
				
\cs_new:Npn\g_automath_primitive_keyval_ifoutput:nn#1#2{ %IMPLEMENT THIS
	% tells whether to use the output class or not
	\g_automath_bool_provide:nn { #1 } { output }
	\str_if_eq:nnTF { #2 } { true }
	{
		\bool_set_true:c { g_automath_#1_if_output }
	}
	{
		\str_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_output }	}
		{
			%IM do nothing right now, but should
			%IM probably throw an error
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_gradingpos:nn#1#2{
		% tells whether to use upper or lower indices
		\g_automath_bool_provide:nn { #1 } { upper_grading }
		\str_case:nnTF { #2 }
		{
			{ upper }
			{
				\bool_set_true:c { g_automath_#1_if_upper_grading }
			}
			{ lower }
			{
				\bool_set_false:c { g_automath_#1_if_upper_grading }
			}
		}
		{
			% do nohting
		}
		{
			% do nothing at the moment, but should probably throw an error
		}
}

\cs_set_eq:NN \g_automath_primitive_keyval_gradingposition:nn \g_automath_primitive_keyval_gradingpos:nn

\cs_new:Npn\g_automath_primitive_keyval_upper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}



\cs_new:Npn\g_automath_primitive_keyval_supper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cx { g_automath_#1_upper_index }
		{ \exp_not:n { \g_automath_tl_get:nn { #1 } { uppersep } } }
		\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}

\cs_new:Npn\g_automath_primitive_keyval_lower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_slower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cx { g_automath_#1_lower_index }
		{ \exp_not:n { \g_automath_tl_get:nn { #1 } { lowersep } } }
		\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_generate_variant:Nn \tl_if_blank:nTF { cTF, vTF }

\cs_new:Npn \g_automath_primitive_upper_lower_auxiliary_first_arg:nn#1#2 { #1 }

\cs_new:Npn \g_automath_primitive_upper_lower_auxiliary_second_arg:nn#1#2 { #2 }

\cs_new:Npn\g_automath_primitive_keyval_uppersep:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_first_arg:nn #2 \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}


\cs_new:Npn\g_automath_primitive_keyval_lowersep:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { \g_automath_primitive_upper_lower_auxiliary_first_arg:nn #2 \g_automath_primitive_upper_lower_auxiliary_second_arg:nn #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_cupper:nn#1#2{
	% adds to the upper index
	\g_automath_tl_inherit_x:nn { #1 } { upper_index }
%	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_upper }
	{	\tl_put_right:cn { g_automath_#1_upper_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_upper_index } { , \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\bool_set_false:c { g_automath_#1_if_first_upper }
}


\cs_new:Npn\g_automath_primitive_keyval_clower:nn#1#2{
	% adds to the lower index
	\g_automath_tl_inherit_x:nn { #1 } { lower_index }
%	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { #2 } }
	%\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:N \exp_not:n { \exp_not:n{#2} } }
	\g_automath_bool_get:nnTF { #1 } { first_lower }
	{	\tl_put_right:cn { g_automath_#1_lower_index } { \exp_not:n { #2 } }	}
	{
		\tl_put_right:cn { g_automath_#1_lower_index } { , \exp_not:n { #2 } }
	}
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\bool_set_false:c { g_automath_#1_if_first_lower }
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstarg:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_arg }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_arg }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstupper:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_upper }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_upper }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_upper }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstlower:nn#1#2
{
	\g_automath_bool_provide:nn { #1 } { first_lower }
	\tl_if_eq:nnTF { #2 } { true }
	{	\bool_set_true:c { g_automath_#1_if_first_lower }	}
	{
		\tl_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_first_lower }	}
		{
			%IM Throw error later
		}
	}
}

\cs_new:Npn\g_automath_primitive_keyval_iffirstd:nn#1#2
{
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
	{ \g_automath_primitive_keyval_iffirstupper:nn { #1 } { #2 } }
	{ \g_automath_primitive_keyval_iffirstlower:nn { #1 } { #2 } }
}

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstdeg:nn\g_automath_primitive_keyval_iffirstd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstdegree:nn\g_automath_primitive_keyval_iffirstd:nn

\cs_new:Npn\g_automath_primitive_keyval_iffirsti:nn#1#2
{
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
	{ \g_automath_primitive_keyval_iffirstlower:nn { #1 } { #2 } }
	{ \g_automath_primitive_keyval_iffirstupper:nn { #1 } { #2 } }
}

\cs_set_eq:NN\g_automath_primitive_keyval_iffirstindex:nn\g_automath_primitive_keyval_iffirsti:nn

\cs_new:Npn\g_automath_primitive_keyval_setuppersep:nn#1#2
{
	\g_automath_tl_provide:nn { #1 } { uppersep }
	\tl_set:cn { g_automath_#1_uppersep } { \exp_not:n { #2 }}
}

\cs_new:Npn\g_automath_primitive_keyval_setlowersep:nn#1#2
{
	\g_automath_tl_provide:nn { #1 } { lowersep }
	\tl_set:cn { g_automath_#1_lowersep } { \exp_not:n { #2 }}
}

\cs_new:Npn\g_automath_primitive_keyval_d:nn#1#2
{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_upper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_lower:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_deg:nn\g_automath_primitive_keyval_d:nn

\cs_set_eq:NN\g_automath_primitive_keyval_degree:nn\g_automath_primitive_keyval_d:nn

\cs_new:Npn\g_automath_primitive_keyval_sd:nn#1#2
{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_supper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_slower:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_sdeg:nn\g_automath_primitive_keyval_sd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_sdegree:nn\g_automath_primitive_keyval_sd:nn

\cs_new:Npn\g_automath_primitive_keyval_cd:nn#1#2{ %IM Maybe remove this.
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_cupper:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_clower:nn { #1 } { #2 }
	}
}




\cs_set_eq:NN\g_automath_primitive_keyval_cdeg:nn\g_automath_primitive_keyval_cd:nn

\cs_set_eq:NN\g_automath_primitive_keyval_cdegree:nn\g_automath_primitive_keyval_cd:nn


\cs_new:Npn\g_automath_primitive_keyval_i:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_lower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_upper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_index:nn\g_automath_primitive_keyval_i:nn

\cs_new:Npn\g_automath_primitive_keyval_si:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_slower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_supper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_sindex:nn\g_automath_primitive_keyval_si:nn

\cs_new:Npn\g_automath_primitive_keyval_ci:nn#1#2{
	% adds to the n-index (upper by default)
	%\bool_if:cTF { g_automath_#1_if_upper_grading }
	\g_automath_bool_get:nnTF { #1 } { upper_grading }
		{
		%\tl_put_right:co { g_automath_#1_upper_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_clower:nn { #1 } { #2 }
	}
	{
		%\tl_put_right:co { g_automath_#1_lower_index } { \exp_not:n { #2 } }
		\g_automath_primitive_keyval_cupper:nn { #1 } { #2 }
	}
}

\cs_set_eq:NN\g_automath_primitive_keyval_cindex:nn\g_automath_primitive_keyval_ci:nn


\cs_new:Npn\g_automath_primitive_keyval_par:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_par_size }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_size } { \exp_not:N #2 }
	\g_automath_primitive_keyval_ifpar:nn { #1 } { true }
}

\cs_new:Npn\g_automath_primitive_keyval_parsize:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_par_size }{ \exp_not:n { #2 } }
}

\cs_new:Npn\g_automath_primitive_keyval_leftpar:nn#1#2{
	\tl_set:cn { g_automath_#1_par_open }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_open }{ #2 }
	%\tl_set:cx { g_automath_#1_par_open }{ \exp_not:n { \exp_not:n { #2 } } }
	%\tl_set:cx { g_automath_#1_par_open }{ \exp_not:N #2 }
	%\tl_set:cn { g_automath_#1_par_open }{ \exp_not:n{\noexpand#2} }
}

\cs_new:Npn\g_automath_primitive_keyval_rightpar:nn#1#2{
	\tl_set:cn { g_automath_#1_par_close }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_par_close}{ #2 }
	%\tl_set:cn { g_automath_#1_par_close }{ \exp_not:N #2 }
	%\tl_set:cn { g_automath_#1_par_close }{ \exp_not:n{\noexpand#2} }
}

\cs_new:Npn\g_automath_primitive_keyval_ifpar:nn#1#2{ %IMPLEMENT THIS
	% tells whether to use the output class or not
	\g_automath_bool_provide:nn { #1 } { par }
	\str_if_eq:nnTF { #2 } { true }
	{
		\bool_set_true:c { g_automath_#1_if_par }
	}
	{
		\str_if_eq:nnTF { #2 } { false }
		{	\bool_set_false:c { g_automath_#1_if_par }	}
		{
			%IM do nothing right now, but should
			%IM probably throw an error
		}
	}
}



\cs_new:Npn\g_automath_primitive_keyval_spar:nn#1#2
{
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
	\tl_set:cx { g_automath_#1_symbol }
	{
		{ \exp_not:n { \exp_not:n { #2 } } }
		{ \g_automath_tl_get:nn { #1 } { spar_open } }
		{ \g_automath_tl_get:nn { #1 } { spar_close } }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	\tl_put_left:cn { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
	}
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:n { \exp_not:N #2 } }
%		{ \g_automath_tl_get:nn { #1 } { spar_open } }
%		{ \g_automath_tl_get:nn { #1 } { spar_close } }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set_eq:cN { g_automath_#1_symbol } \l__automath_spar_temp
}

\cs_new:Npn\g_automath_primitive_singlekey_spar:n#1{
	\g_automath_tl_inherit:nn { #1 } { spar_size }
%	\g_automath_tl_inherit:nn { #1 } { spar_open }
%	\g_automath_tl_inherit:nn { #1 } { spar_close }
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:v { g_automath_#1_spar_size } }
%		{ \g_automath_tl_get:nn { #1 } { spar_open } }
%		{ \g_automath_tl_get:nn { #1 } { spar_close } }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set_eq:cN { g_automath_#1_symbol } \l__automath_spar_temp
	%\tl_set:cx { g_automath_#1_symbol } {\exp_not:V\l__automath_spar_temp}
	\tl_set:cx { g_automath_#1_symbol }
	{
		{ \exp_not:v { g_automath_#1_spar_size } }
		%IM Could replace this by \exp_not:V and a temporary command,
		%IM like in _return
		{ \g_automath_tl_get:nn { #1 } { spar_open } }
		{ \g_automath_tl_get:nn { #1 } { spar_close } }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	\tl_put_left:cn { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
	}
}

\cs_new:Npn\g_automath_auxiliary_first_arg:nn#1#2 { #1 }
\cs_new:Npn\g_automath_auxiliary_second_arg:nn#1#2 { #2 }

%\cs_new:Npn\g_automath_primitive_keyval_otherspar:nn#1#2
%{
%	\g_automath_tl_inherit:nn { #1 } { spar_size }
%	\g_automath_tl_inherit:nn { #1 } { symbol }
%	\g_automath_primitive_singlekey_return:n { #1 }
%%	\tl_set:Nn\l__automath_spar_temp
%%	{
%%		\exp_not:N
%%		\g_automath_symbol_parentheses:nnnn
%%	}
%%	\tl_put_right:Nx\l__automath_spar_temp
%%	{
%%		{ \exp_not:v { g_automath_#1_spar_size } }
%%		{ \g_automath_auxiliary_first_arg:nn#2 }
%%		{ \g_automath_auxiliary_second_arg:nn#2 }
%%		{ \exp_not:v { g_automath_#1_symbol } }
%%	}
%%	\tl_set:cx { g_automath_#1_symbol } { \exp_not:V\l__automath_spar_temp }
%	\tl_set:cx { g_automath_#1_symbol }
%	{
%		%{ \exp_not:c { g_automath_#1_spar_size } }
%		{ \exp_not:n { \use:c { g_automath_#1_spar_size } } }
%		{ \g_automath_auxiliary_first_arg:nn #2 }
%		{ \g_automath_auxiliary_second_arg:nn #2 }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_put_left:cn { g_automath_#1_symbol }
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%}

\cs_new:Npn\g_automath_primitive_keyval_otherspar:nn#1#2
{
	\g_automath_primitive_keyval_otherspar_auxiliary:nnn { #1 } #2
}

\cs_new:Npn\g_automath_primitive_keyval_otherspar_auxiliary:nnn#1#2#3
{
	\g_automath_tl_inherit:nn { #1 } { spar_size }
	\g_automath_tl_inherit:nn { #1 } { symbol }
	\g_automath_primitive_singlekey_return:n { #1 }
%	\tl_set:Nn\l__automath_spar_temp
%	{
%		\exp_not:N
%		\g_automath_symbol_parentheses:nnnn
%	}
%	\tl_put_right:Nx\l__automath_spar_temp
%	{
%		{ \exp_not:v { g_automath_#1_spar_size } }
%		{ \g_automath_auxiliary_first_arg:nn#2 }
%		{ \g_automath_auxiliary_second_arg:nn#2 }
%		{ \exp_not:v { g_automath_#1_symbol } }
%	}
%	\tl_set:cx { g_automath_#1_symbol } { \exp_not:V\l__automath_spar_temp }
	\tl_set:cx { g_automath_#1_symbol }
	{
		\exp_not:N
		\g_automath_symbol_parentheses:nnnn
		%{ \exp_not:c { g_automath_#1_spar_size } }
		%{ \exp_not:n { \use:c { g_automath_#1_spar_size } } }
		%{ normal }
		{ \exp_not:n { \exp_not:v { g_automath_#1_spar_size } } }
		{ #2 }
		{ #3 }
		{ \exp_not:v { g_automath_#1_symbol } }
	}
	%\tl_put_left:cn { g_automath_#1_symbol }
	%{
	%	\exp_not:N
	%	\g_automath_symbol_parentheses:nnnn
	%}
}

\cs_new:Npn\g_automath_primitive_keyval_sparsize:nn#1#2{
	% sets the size of the parentheses
	\tl_set:cn { g_automath_#1_spar_size }{ \exp_not:n { #2 } }
	%\tl_set:cn { g_automath_#1_spar_size } { #2 }
	%\tl_set:cx { g_automath_#1_spar_size } { \exp_args:N #2 }
}

\cs_new:Npn\g_automath_primitive_keyval_leftspar:nn#1#2{
	\tl_set:cn { g_automath_#1_spar_open }{ \exp_not:n { \exp_not:n { #2 } } }
	%IM Two \exp_not necessary for unknown reasons
	%IM Doing the same at leftpar yields an error.
}

\cs_new:Npn\g_automath_primitive_keyval_rightspar:nn#1#2{
	\tl_set:cn { g_automath_#1_spar_close }{ \exp_not:n { \exp_not:n { #2 } } }
	%IM Two \exp_not necessary for unknown reasons
	%IM Doing the same at leftpar yields an error.
}


%\def\keyvalue{} % create the command \keyvalue





%\msg_new:nnnn { automath } { singlekey_not_found } { Unknown~key~#1~passed~to~object~#2~on~input~line~\msg_line_number: } {}

\cs_new:Npn \g_automath_keyval:nnnn#1#2#3#4{
	% Takes care of keyvals, keys with a value
	% For the sake of implementation, the arguments
	% come in a strange order
	% #1 = value of key
	% #2 = name of the key
	% #3 = class
	% #4 = object
	\tl_set:Nn\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	%\tl_set:Nn\keyvalue{#1}
	%\tl_set:No\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	%IM think about using extra {...} to avoid interference with keyval str
	\g_automath_keyval_get:nnNTF { #4 } { #2 } \l_automath_custom_keyval_temp
	{
		\exp_args:Nnx
		%\use:c { g_automath_#4_keys_set:n }
		\g_automath_keys_set:nn { #4 }
		{ \l_automath_custom_keyval_temp }
	}
	{
		\cs_if_exist:cTF { g_automath_primitive_keyval_#2:nn }
		{
			\use:c { g_automath_primitive_keyval_#2:nn }{ #4 }{ #1 }%
		}
		{
			\msg_error:nnnn { automath } { keyval_not_found } { #2 } { #4 }
		}
	}
}

\cs_new:Npn \g_automath_singlekey:nnn#1#2#3
{
	% #1 = name of the key
	% #2 = class
	% #3 = object
%	% takes care of single keys, keys without a value
	\g_automath_singlekey_get:nnNTF { #3 } { #1 } \l_automath_custom_singlekey_temp
	{
		%\exp_args:NNno
		%\exp_args:Nno
		\exp_args:Nnx
		%\use:c { g_automath_#3_keys_set:n }
		\g_automath_keys_set:nn { #3 }
		{
			{ \l_automath_custom_singlekey_temp }
		}
	}
	{
		%\use:c { g_automath_primitive_singlekey_#1:n }{ #3 }%
		%\cs_if_exist:cTF { g_automath_primitive_singlekey_#1:n }
		%{
		%	\use:c { g_automath_primitive_singlekey_#1:n }{ #3 }%
		%}
		\str_case:nnTF { #1 }
		{
			{ return }
			{
				\g_automath_primitive_singlekey_return:n { #3 }
			}
			{ widetilde }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widetilde }
				\g_automath_primitive_keyval_command:nn { #3 } { \widetilde }
			}
			{ tilde }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widetilde }
				\g_automath_primitive_keyval_command:nn { #3 } { \tilde }
			}
			{ widebar } %IM remove in package
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \exp_not:N\widebar }
			}
			{ overline }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \overline }
			}
			{ smallbar }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \widebar }
				\g_automath_primitive_keyval_command:nn { #3 } { \bar }
			}
			{ bold }
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \mathbf }
				\g_automath_primitive_keyval_command:nn { #3 } { \mathbf }
			}
			{ upright } %IM remove in package
			{
				%\g_automath_keyval:nnn { #1 }{ addcommand } { \mathup }
				\g_automath_primitive_keyval_command:nn { #3 } { \mathup }
			}
			{ par }
			{
				%\g_automath_primitive_keyval_par:nn { #3 }{ normal }
				\g_automath_primitive_keyval_ifpar:nn { #3 } { true }
			}
			{ nopar }
			{
				%\g_automath_primitive_keyval_par:nn { #3 }{ none }
				\g_automath_primitive_keyval_ifpar:nn { #3 } { false }
			}
			{ spar }
			{
				\g_automath_primitive_singlekey_spar:n { #3 }
			}
			%			{ * } { \g_automath_keyval:nnn { #1 } { n } { \automath_bullet_tl }}
			%			{ ** }{ \g_automath_keyval:nnn { #1 } { n } { \automath_double_bullet_tl }}
			%IM add these again, together with \big, etc., maybe with [auto]
			{ bullet }
			{
				%\g_automath_keyval:nnn { #1 } { n } { \automath_bullet_tl } % bullet in the n-index
				%\g_automath_primitive_keyval_d:nn { #3 } { \automath_bullet_tl }
				\g_automath_keys_set:nn { #3 } { degreedefault = \automath_bullet_tl }
			}
			{ doublebullet }
			{
				%\g_automath_keyval:nnn { #1 } { n } { \automath_double_bullet_tl } % double bullet in the n-index
				%\g_automath_primitive_keyval_d:nn { #3 } { \automath_double_bullet_tl }
				\g_automath_keys_set:nn { #3 } { degreedefault = \automath_double_bullet_tl }
			}
			{ prime }
			{
				%\g_automath_keys_set:nnn { #3 } { upper } { \prime }
				\g_automath_primitive_keyval_upper:nn { #3 } { \prime }
			}
			{ ibullet }
			{
				%\g_automath_keyval:nnn { #3 } { i } { \automath_bullet_tl } % bullet in the i-index
				\g_automath_primitive_keyval_i:nn { #3 } { \automath_bullet_tl }
			}
			{ idoublebullet }
			{
				%\g_automath_keyval:nnn { #3 } { i } { \automath_double_bullet_tl } % double bullet in the i-index
				\g_automath_primitive_keyval_i:nn { #3 } { \automath_double_bullet_tl }
			}
			%			% Some commands to clear some registers:
			{ clearcommand }
			{
				\seq_clear:c { g_automath_#3_commands_sequence }
				%IMplement again
			}
			{ clearkeyvals } %IM also allow removing one keyval etc.
			{
				\tl_clear:c { g_automath_#3_custom_keyvals }
			}
			{ clearsinglekeys }
			{
				\tl_clear:c { g_automath_#3_custom_singlekeys }
			}
			{ clearargkeyvals }
			{
				\tl_clear:c { g_automath_#3_arg_custom_keyvals }
			}
			{ clearargsinglekeys }
			{
				\tl_clear:c { g_automath_#3_arg_custom_singlekeys }
			}
			{ clearupper }
			{
				\tl_clear:c { g_automath_#3_upper_index }
			}
			{ clearlower }
			{
				\tl_clear:c { g_automath_#3_lower_index }
			}
			{ cleararg }
			{
				\tl_clear:c { g_automath_#3_arg }
			}
			{ cleard } %IM clean up
			{
				\bool_if:cTF { g_automath_#3_if_upper_grading }
				{
					\tl_clear:c { g_automath_#3_upper_index }
				}
				{
					\tl_clear:c { g_automath_#3_lower_index }
				}
			}
			{ cleari } %IM clean up
			{
				\bool_if:cTF { g_automath_#3_if_upper_grading }
				{
					\tl_set:cn { g_automath_#3_lower_index } { } %empty
				}
				{
					\tl_set:cn { g_automath_#3_upper_index } { } %empty
				}
			}
			{ clearoutputoptions }
			{
				\tl_clear:c { g_automath_#3_output_options }
			}
		}
		{
			% if true; do nothing
		}
		{
			%\msg_error:nnnn { automath } { singlekey_not_found } { #1 } { #3 }
			%\g_automath_primitive_keyval_i:nn { #3 } { #1 }%
			%\use:c { g_automath_#3_keys_set:n } { default = {#1} }
			\g_automath_keys_set:nn { #3 } { default = { #1 } }
		}
	}
}

%IMplement the same thing for upper, lower

\cs_new:Npn \g_automath_arg_primitive_keyval_sep_auxiliary_function_withsep:nn#1#2
{
	#1#2
}

\cs_new:Npn \g_automath_arg_primitive_keyval_sep_auxiliary_function_withoutsep:nn#1#2
{
	#2
}

\cs_new:Npn \g_automath_primitive_arg_keyval_sep:nn#1#2
{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	%\tl_if_empty:cTF { g_automath_#1_arg }
	\g_automath_bool_get:nnTF { #1 } { first_arg }
	{
		\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \g_automath_arg_primitive_keyval_sep_auxiliary_function_withoutsep:nn #2 } }
		%IM These do not use :x, unlike the ones below
	}
	{
		\tl_put_right:cn { g_automath_#1_arg } { \exp_not:n { \g_automath_arg_primitive_keyval_sep_auxiliary_function_withsep:nn #2 } }
	}
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
	%IM this is not the right place to set this as true; probably it should
	%IM be in the user's setup of the arg key.
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_false:c { g_automath_#1_if_first_arg }
}

\cs_new:Npn \g_automath_primitive_arg_keyval_standardsep:nn#1#2
{
%	\tl_if_exist:cTF { g_automath_#1_arg }
%	{
%		% do nothing
%	}
%	{
%		\tl_new:c { g_automath_#1_arg }
%		\tl_set:cx { g_automath_#1_arg } { \g_automath_tl_get:nn { \g_automath_tl_get:nn { #1 } { parent } } { arg } }%IM change to :cn if we get a better if_first_arg system
%	}
	\g_automath_tl_inherit_x:nn { #1 } { arg }
	%\bool_if:cTF { g_automath_if_first_arg }
	%\g_automath_bool_get:nnTF { #3 } { first_arg }
	\g_automath_bool_get:nnTF { #1 } { first_arg }
	{
		%\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n{\exp_not:n { #2 } }}
		\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { #2 } }
		%IM Recently corrected
	}
	{
		\tl_put_right:cx { g_automath_#1_arg } { \exp_not:n { \g_automath_tl_get:nn { #1 } { argsep } } \exp_not:n { #2 } }
	}
	\g_automath_primitive_keyval_ifoutput:nn { #1 } { true }
	\g_automath_bool_provide:nn { #1 } { first_arg }
	\bool_set_false:c { g_automath_#1_if_first_arg }
}

\cs_new:Npn \g_automath_arg_keyval:nnnn#1#2#3#4
{
	% Takes care of keyvals, keys with a value
	% For the sake of implementation, the arguments
	% come in a strange order
	% #1 = value of key
	% #2 = name of the key
	% #3 = class
	% #4 = object
	\tl_set:Nn\keyvalue{\exp_not:n{#1}} % stores the content of the key in the temporary command \keyvalue
	\g_automath_arg_keyval_get:nnNTF { #4 } { #2 } \l_automath_custom_arg_keyval_temp
	{
		\exp_args:Nnx
		\g_automath_arg_keys_set:nn { #4 } { \l_automath_custom_arg_keyval_temp }
	}
	{
		\cs_if_exist:cTF { g_automath_primitive_arg_keyval_#2:nn }
		{
			\use:c { g_automath_primitive_arg_keyval_#2:nn }{ #4 }{ #1 }%
		}
		{
			\msg_error:nnnn { automath } { arg_keyval_not_found } { #2 } { #4 }
		}
	}
}


\cs_new:Npn \g_automath_arg_singlekey:nnn#1#2#3
{
	% #1 = name of the key
	% #2 = class
	% #3 = object
%	% takes care of single keys, keys without a value
	\g_automath_arg_singlekey_get:nnNTF { #3 } { #1 } \l_automath_custom_arg_singlekey_temp
	{
		%\exp_args:NNno
		%\exp_args:Nno
		\exp_args:Nnx
		%\use:c { g_automath_#3_arg:n }
		\g_automath_arg_keys_set:nn { #3 }
		{
			\l_automath_custom_arg_singlekey_temp
		}
	}
	{
		\str_case:nnTF { #1 }
		{
			{...}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { argdots } }
				%IMplement the same for symbols
			}
			{-}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
				%IMplement the same for symbols
				%IM Also, allow editing slots
			}
			{*}{
							\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
							%IMplement the same for symbols
							%IM Also, allow editing slots
			}
			{slot}{
				\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \g_automath_tl_get:nn { #3 } { slot } }
				%IMplement the same for symbols
			}
		}
		{
			% if true; do nothing
		}
		{
			\g_automath_tl_inherit_x:nn { #3 } { arg }
			%\bool_if:cTF { g_automath_if_first_arg }
			%\g_automath_bool_get:nnTF { #3 } { first_arg }
%			\tl_if_empty:cTF { g_automath_#3_arg }
%			{
%				\tl_put_right:cn { g_automath_#3_arg } { \exp_not:n { #1 } }
%			}
%			{
%				\tl_put_right:cn { g_automath_#3_arg } { \g_automath_tl_get:nn { #3 } { argsep } \exp_not:n { #1 } }
%				%IMplement "arg", similarly to "default"
%				%IMPORTANT: Think about using x-type expansion here,
%				%IM which is done in the other place where arguments are
%				%IM added. This should maybe be the standard.
%			}
%			\g_automath_primitive_keyval_ifoutput:nn { #3 } { true }
			%\exp_args:Nnx\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { \exp_not:n { #1 } } }
			%\exp_args:Nnx\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { #1 } }
			%\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { #1 }
			%
			%
			%
			%
			%
			%\g_automath_primitive_arg_keyval_standardsep:nn { #3 } { \exp_not:n { #1 } }
			\g_automath_arg_keys_set:nn { #3 } { default={\exp_not:n { #1 } }}
			%\g_automath_arg_keys_set:nn { #3 } { default={#1}}
			%IM THis \exp_not:n was added late, might be needed elsewhere, too.
		}
	}
}

%\tl_new:N\g_automath_automathvariable_parent
%\tl_set:Nn\g_automath_automathvariable_parent { automathvariable }

\g_automath_tl_provide:nn { automathvariable } { output }
\tl_set:Nn\g_automath_automathvariable_output{ automathvariable }


\g_automath_tl_provide:nn { automathvariable } { upper_index }

\g_automath_tl_provide:nn { automathvariable } { uppersep }

\tl_set:Nn \g_automath_automathvariable_uppersep { , }

%IM do the same with all the others, INCLUDING if_upper_grading and symbol
%IM Also, need commands like forgetupperindex, reverting to the class standard

\g_automath_tl_provide:nn { automathvariable } { lower_index }

\g_automath_tl_provide:nn { automathvariable } { lowersep }

\tl_set:Nn \g_automath_automathvariable_lowersep { , }


\g_automath_tl_provide:nn { automathvariable } { preupper }

\g_automath_tl_provide:nn { automathvariable } { postupper }

\g_automath_tl_provide:nn { automathvariable } { prelower }

\g_automath_tl_provide:nn { automathvariable } { postlower }

\g_automath_tl_provide:nn { automathvariable } { prearg }

\g_automath_tl_provide:nn { automathvariable } { postarg }
%IMplement these later

\g_automath_tl_provide:nn { automathvariable } { arg }

\g_automath_tl_provide:nn { automathvariable } { argsep }
\tl_set:Nn \g_automath_automathvariable_argsep {,}

\g_automath_tl_provide:nn { automathvariable } { slot }
\tl_set:Nn \g_automath_automathvariable_slot { \slot }

\g_automath_tl_provide:nn { automathvariable } { argdots }
\tl_set:Nn \g_automath_automathvariable_argdots {\ldots}

\g_automath_tl_provide:nn { automathvariable } { symbol }

\bool_new:N\g_automath_automathvariable_commands_sequence_if_provided
\bool_set_true:N\g_automath_automathvariable_commands_sequence_if_provided
\seq_new:N\g_automath_automathvariable_commands_sequence

%\tl_new:N\g_automath_automathvariable_output_options

\g_automath_bool_provide:nn { automathvariable } { upper_grading }
\bool_set_true:N \g_automath_automathvariable_if_upper_grading

\g_automath_bool_provide:nn { automathvariable } { output }

\g_automath_tl_provide:nn { automathvariable } { output_options }

\g_automath_bool_provide:nn { automathvariable } { first_arg }
\bool_set_true:N\g_automath_automathvariable_if_first_arg

\g_automath_bool_provide:nn { automathvariable } { first_upper }
\bool_set_true:N\g_automath_automathvariable_if_first_upper

\g_automath_bool_provide:nn { automathvariable } { first_lower }
\bool_set_true:N\g_automath_automathvariable_if_first_lower

\g_automath_bool_provide:nn { automathvariable } { par }
\bool_set_true:N\g_automath_automathvariable_if_par




%\tl_set:Nn\g_objectmath_automathvariable_upper_index { hej }
%\tl_set:Nn \g_automathvariable_output { automathvariable }
%\bool_new:N \g_automathvariable_output_if_provided
%\bool_set_true:N \g_automathvariable_output_if_provided


\newvariableclass{automathvariable}[
	%parent=automathvariable,
	symbol=,
	gradingpos=upper,
	%upper=,
	%lower=,
	leftpar=(,
	rightpar=),
	par=normal,
	leftspar=(,
	rightspar=),
	sparsize=normal,
	%arg=,
	ifoutput=false,
	output=automathvariable,
	singlekeys={
		{*}{bullet},
		{**}{doublebullet},
		{smash}{command=\noexpand\smash},
	},
	keyvals={
		{default}{si={\keyvalue}},
		{arg}{argwithkeyval={\keyvalue}},
		{degreedefault}{sd={\keyvalue}},
	},
	argkeyvals={
		{default}{standardsep={\keyvalue}},
	}
	%command=,
]

\ExplSyntaxOff

==> _commands/basics/_basics_1.tex <==
%Basic number sets
%\newcommand\N{\mathbb{N}}
%\newcommand\Z{\mathbb{Z}}
%\newcommand\Q{\mathbb{Q}}
%\newcommand\R{\mathbb{R}}
%\newcommand\C{\mathbb{C}}
%\newcommand\F{\mathbb{F}}
%\newcommand\Zmod[1]{\Z/#1}
%\newcommand\differentialD{d\!}

\newvariableclass{var}[
	parent=automathvariable,
	output=var,
	singlekeys={
		{inv}{upper=-1},
		{conj}{command=\noexpand\overline},
		{varconj}{command=\noexpand\bar},
		{Varconj}{command=\noexpand\widebar},
		{closure}{command=\noexpand\overline},
		{varclosure}{command=\noexpand\bar},
		{Varclosure}{command=\noexpand\widebar},
		{interior}{upper=\circ},
		{pol}{
			nowoutput=algop,
			outputoptions={par,leftpar=\lbrack,rightpar=\rbrack,},
		},
		{field}{
			nowoutput=algop,
			outputoptions={par,leftpar=(,rightpar=),},
		},
		{powerseries}{
			%nowoutput=algop,
			%outputoptions={par,leftpar=\noexpand\llbracket,rightpar=\noexpand\rrbracket,},
			nowoutput=algoppowerseries,
		},
		{freealg}{
			nowoutput=algopfreealg,
			%nowoutput=algop,
			%outputoptions={par,leftpar=\langle,rightpar=\rangle},
		},
		{laurent}{
			nowoutput=algoplaurent,
		},
		%These are for categories:
		{fg}{upper=\mathup{fg}},
		{interiorgroupoid}{upper=\circ},
		{localize}{
			return,
			nowoutput=localizedcategory,
		},
		{fin}{upper=\mathup{fin}},
		{varfin}{upper=\mathup{f}},
		{findim}{upper=\mathup{f}},
		{op}{upper=\mathup{op}},
		{invim} { upper = -1, nopar, output=sheaf },
		{dirim} { lower={\ast}, nopar, output=sheaf },
		{pull} { upper={\ast} },
		{push}{ lower = {\ast} },
		{shpull}{ upper={\ast}, nopar, output=sheaf },
		{shpush}{ lower={\ast}, nopar, output=sheaf },
		{shriekpush} { lower=!, nopar, output=sheaf },
		{shriekpull} { upper=!, nopar, output=sheaf },
		{!push} { lower=!, nopar, output=sheaf },
		{!pull} { upper=!, nopar, output=sheaf },
		{sharp} { upper=\# },
		{inv} { upper=-1 },
		{pre} { upper=-1 },
%		{shpull} { g=-1 },
		{squared} { upper=2 },
	},
	keyvals={
		{power}{upper={\keyvalue}},
		{invar}{upper={\keyvalue}},
		{coinvar}{lower={\keyvalue}},
		{oplus}{upper={\oplus\keyvalue}},
		{coprod}{upper={\smallcoprod\keyvalue}},
		{prod}{upper={\smallprod\keyvalue}},
		{mod}{symbolputright={/\keyvalue}},
		{modn}{symbolputright={/\keyvalue}},
		{shift}{symbolputright={[\keyvalue]}},
		{power}{upper={\keyvalue}},
		{diag}{upper={\keyvalue}},
		{functors}{upper={\keyvalue}},
		{der} { upper = {(\keyvalue)} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{bigres} { return, symbolputright=\big\vert, lower={\keyvalue} },
		{Bigres} { return, symbolputright=\Big\vert, lower={\keyvalue} },
		{biggres} { return, symbolputright=\bigg\vert, lower={\keyvalue} },
		{Biggres} { return, symbolputright=\Bigg\vert, lower={\keyvalue} },
		% Derived functors:
		{Lder} { symbolputleft=L^{\keyvalue}},
		{Rder} { symbolputleft=R^{\keyvalue}},
	},
]

\newvar\vx{x}
\newvar\vy{y}
\newvar\vz{z}

\newvariableclass{classset}[
	parent=var,
%	keyvals={
%		{power}{upper={\keyvalue}},
%		{invar}{upper={\keyvalue}},
%		{coinvar}{lower={\keyvalue}},
%	},
%	singlekeys={
%		{closure}{command=\noexpand\overline},
%		{varclosure}{command=\noexpand\bar},
%		{Varclosure}{command=\noexpand\widebar},
%		{interior}{upper=\circ},
%	},
]

\newcommand\newdelimsize{\noexpand\automathdelimsize}

\newvariableclass{alg}[
	parent=classset,
	output=alg,
%	keyvals={
%		{oplus}{upper={\oplus\keyvalue}},
%		{coprod}{upper={\smallcoprod\keyvalue}},
%		{prod}{upper={\smallprod\keyvalue}},
%		{mod}{symbolputright={/\keyvalue}},
%		{modn}{symbolputright={/\keyvalue}},
%		{shift}{symbolputright={[\keyvalue]}},
%		{power}{upper={\keyvalue}},
%		{diag}{upper={\keyvalue}},
%		{functors}{upper={\keyvalue}},
%	},
%	singlekeys={
%		{pol}{
%			nowoutput=algop,
%			outputoptions={par,leftpar=\lbrack,rightpar=\rbrack,},
%		},
%		{field}{
%			nowoutput=algop,
%			outputoptions={par,leftpar=(,rightpar=),},
%		},
%		{powerseries}{
%			%nowoutput=algop,
%			%outputoptions={par,leftpar=\noexpand\llbracket,rightpar=\noexpand\rrbracket,},
%			nowoutput=algoppowerseries,
%		},
%		{freealg}{
%			nowoutput=algopfreealg,
%			%nowoutput=algop,
%			%outputoptions={par,leftpar=\langle,rightpar=\rangle},
%		},
%		{laurent}{
%			nowoutput=algoplaurent,
%		},
%		%These are for categories:
%		{fg}{upper=\mathup{fg}},
%		{interiorgroupoid}{upper=\circ},
%		{localize}{
%			return,
%			nowoutput=localizedcategory,
%		},
%		{fin}{upper=\mathup{fin}},
%		{varfin}{upper=\mathup{f}},
%		{findim}{upper=\mathup{f}},
%		{op}{upper=\mathup{op}},
%	},
]


\newalg\N{\mathbb{N}}
\newalg\Z{\mathbb{Z}}
\newalg\Q{\mathbb{Q}}
\newalg\R{\mathbb{R}}
\newalg\C{\mathbb{C}}
\newalg\F{\mathbb{F}}
%\newmap\Zmod{\mathbb{Z}}[
%	%parent=alg,
%	leftpar=/,
%	rightpar=,
%	output=alg,
%]





%\DeclareDocumentCommand\D{sd()mo}{
%	%The first star is pure mark-up; it marks that
%	%the #2 argument is a measure rather than a
%	%variable. It is better to use it, even though
%	%it (with the current settings) has not consequence
%	%for the output.
%	\differentialD
%	\IfNoValueTF{#2}{
%		%do nothing
%	}{
%		^{#2}
%	}
%	#3
%	\IfNoValueTF{#4}{
%		%do nothing
%	}{
%		(#4)
%	}
%}

\begin{comment}
\newcommand\DD{\,\D}
\newcommand\E{e}
\newcommand\I{i}
\newcommand\conj\widebar
\newcommand\subs\subset
\newcommand\sups\superset
\newcommand\propersubs\subsetneq
\newcommand\propersups\supsetneq
\newcommand\inv{^{-1}}
\newcommand\pre{^{-1}}
\newcommand\trans{^{\textup{T}}}
\newcommand\adj{^{*}}
\newcommand\dual{^{*}}
\newcommand\push{_{*}}
\newcommand\pull{^{*}}
\newcommand\units{^{\times}}
\newcommand\op{^{\mathup{op}}}
\newcommand\ort{^{\perp}}

\end{comment}

%\newcommand\sym[1]{\mathfrak{S}_{#1}} % the symmetric group



%\newcommand\iso{\cong}




%\DeclarePairedDelimiter\tup{(}{)} % tuples

\begin{comment}
\newcommand\matlogo{\mathup{M}}
\DeclareDocumentCommand\tempmat{mmm}{
	\matlogo_{#1\times #2}(#3)
}
\DeclareDocumentCommand\tempsqmat{mm}{
	\matlogo_{#1}(#2)
}
\DeclareDocumentCommand\mat{ms}{
	\IfBooleanTF{#2}{Exercise
		\tempmat{#1}
	}{
	\tempsqmat{#1}
}
}
\end{comment}


%\DeclareDocumentCommand\mat{msm}{\mathup{M}_{
%		\IfBooleanTF{#2}{
%			(#1)
%		}{
%			#1
%		}
%		}(#3)}
%
%\DeclareDocumentCommand\matmn{msmsm}{
%	\mat{
%		\IfBooleanTF{#2}{(#1)}{#1}
%		\times
%		\IfBooleanTF{#4}{(#3)}{#3}
%	}{#5}
%}


%\newcommand\der[1]{^{(#1)}} % derivative

%\newcommand\exterior[1]{{\textstyle\bigwedge^{\!\!#1}}} %for exterior powers


\newcommand\smallprod{\mathbin{\text{\rotatebox[origin=c]{180}{$\amalg$}}}}
\newcommand\smallcoprod{\amalg}

\newcommand\smallbullet{\raisebox{-0.25ex}{\scalebox{1.2}{$\cdot$}}}

%\newcommand\comp{^{\smallbullet}} %cocomplexes
%\newcommand\hocomp{_{\smallbullet}} %complexes
%\newcommand\simp{_{\smallbullet}} % complexes
%\let\hocomp=\simp

%\newcommand\bicomp{^{\smallbullet\smallbullet}}
%\newcommand\bihocomp{_{\smallbullet\smallbullet}}
%\newcommand\bisimp{_{\smallbullet\smallbullet}}
%\let\bihocomp=\bisimp

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareMathSymbol{\intprod}{\mathbin}{MnSyC}{'270} %internal product of forms, "into"

==> _commands/categories/_categories_1.tex <==
\newcommand\category[1]{\textup{\textbf{#1}}}%For categories


%Specific categories

\newcommand\catxmod[1]{\category{$#1$-mod}}
	\newcommand\catRmod{\catxmod{R}}
	\newcommand\catSmod{\catxmod{S}}
	\newcommand\catAmod{\catxmod{A}}
	\newcommand\catBmod{\catxmod{B}}
\newcommand\catxmodf[1]{\category{$#1$-mod\textsuperscript{f}}}
	\newcommand\catRmodf{\catxmodf{R}}
	\newcommand\catSmodf{\catxmodf{S}}
	\newcommand\catAmodf{\catxmodf{A}}
	\newcommand\catBmodf{\catxmodf{B}}
\newcommand\catmodx[1]{\category{mod-$#1$}}
	\newcommand\catmodR{\catmodx{R}}
	\newcommand\catmodS{\catmodx{S}}
	\newcommand\catmodA{\catmodx{A}}
	\newcommand\catmodB{\catmodx{B}}
\newcommand\catxmodx[2]{\category{$#1$-mod-$#2$}}
	\newcommand\catRmodR{\catxmodx{R}{R}}
	\newcommand\catRmodS{\catxmodx{R}{S}}
	\newcommand\catAmodA{\catxmodx{A}{A}}
	\newcommand\catAmodB{\catxmodx{A}{B}}
\newcommand\catxbimod[1]{\catxmodx{#1}{#1}}
	\newcommand\catRbimod{\catxbimod{R}}
	\newcommand\catAbimod{\catxbimod{A}}
\newcommand\catxdgmod[1]{\category{$#1$-DGmod}}
	\newcommand\catRdgmod{\catxdgmod{R}}
	\newcommand\catSdgmod{\catxdgmod{S}}
	\newcommand\catAdgmod{\catxdgmod{A}}
	\newcommand\catBdgmod{\catxdgmod{B}}
\newcommand\catdgmodx[1]{\category{DGmod-$#1$}}
	\newcommand\catdgmodR{\catdgmodx{R}}
	\newcommand\catdgmodS{\catdgmodx{S}}
	\newcommand\catdgmodA{\catdgmodx{A}}
	\newcommand\catdgmodB{\catdgmodx{B}}
\newcommand\catxdgcomod[1]{\category{$#1$-DGcomod}}
	\newcommand\catCdgcomod{\catxcomod{C}}
\newcommand\catdgcomodx[1]{\category{DGcomod-$#1$}}
	\newcommand\catdgcomodC{\catcomodx{C}}
\newcommand\catxdgcontra[1]{\category{$#1$-DGcontra}}
	\newcommand\catCdgcontra{\catxdgcontra{C}}
\newcommand\catdgcontrax[1]{\category{dgcontra-$#1$}}
	\newcommand\catdgcontraC{\catdgcontrax{C}}
\newcommand\catvect{\category{Vect}}
\newcommand\catvectf{\category{Vect\textsuperscript{f}}}
\newcommand\catvectx[1]{\catvect\pars{#1}}
	\newcommand\catvectk{{\catvectx{k}}}
\newcommand\catvectfx[1]{\catvectf\pars{#1}}
	\newcommand\catvectfk{{\catvectfx{k}}}
\newcommand\catset{\category{Set}}
\newcommand\catcat{\category{Cat}}
\newcommand\catab{\category{Ab}}
\newcommand\catgrp{\category{Grp}}
\newcommand\catcom{\category{Com}}
\newcommand\catcomx{\catcom\pars}
\newcommand\catalg{\category{Alg}}
\newcommand\catalgx[1]{\category{Alg}\pars{#1}}
	\newcommand\catalgk{{\catalg{k}}}
\newcommand\catrng{\category{Rng}}
\newcommand\cattop{\category{Top}}
\newcommand\cathot[1]{\category{Hot}\pars{#1}}
\newcommand\catproj{\category{Proj}}
\newcommand\catprojx[1]{\catproj\pars{#1}}
	\newcommand\catprojA{{\catprojx{A}}}
\newcommand\catinj{\category{Inj}}
\newcommand\catinjx[1]{\catinj{#1}}
	\newcommand\catinjA{\catinjx{A}}
\newcommand\catacycl{\category{Acycl}}
	\newcommand\catacyclx[1]{\catacycl\pars{#1}}
	\newcommand\catacyclA[1]{{\catacyclx{A}}}
\newcommand\catacyclabs{\category{Acycl\textsubscript{abs}}}
	\newcommand\catacyclabsx[1]{\catacyclabs\pars{#1}}
	\newcommand\catacyclabsA[1]{{\catacyclabsx{A}}}
\newcommand\catacyclco{\category{Acycl\textsubscript{co}}}
	\newcommand\catacyclcox[1]{\catacyclco\pars{#1}}
	\newcommand\catacyclcoA[1]{{\catacyclcox{A}}}
\newcommand\catacyclctr{\category{Acycl\textsubscript{ctr}}}
	\newcommand\catacyclctrx[1]{\catacyclctr\pars{#1}}
	\newcommand\catacyclctrA[1]{{\catacyclctrx{A}}}


\newcommand\Lperp[1]{{}^{\perp}#1}
\newcommand\lperp[1]{\lperp{(#1)}}
\newcommand\Rperp[1]{#1^{\perp}}
\newcommand\rperp[1]{\Rperp{(#1)}}

\newcommand\catderivedD{\mathscr{D}}
\newcommand\catder[2][]%
{
	\catderivedD
	\ifblank{#1}
	{
		% do nothing
	}
	{
		^{#1}
	}
	\pars{#2}
}
\newcommand\catderp[1]{\catderivedD^{+}\pars{#1}}
\newcommand\catderm[1]{\catderivedD^{-}\pars{#1}}
\newcommand\catderpm[1]{\catderivedD^{\pm}\pars{#1}}
\newcommand\catderb[1]{\catderivedD^{b}\pars{#1}}
\newcommand\catderabs[1]{\catderivedD^{\mathup{abs}}\pars{#1}}
	\newcommand\catderabsp[1]{\catderivedD^{\mathup{abs},+}\pars{#1}}
	\newcommand\catderabsm[1]{\catderivedD^{\mathup{abs},-}\pars{#1}}
	\newcommand\catderabspm[1]{\catderivedD^{\mathup{abs},\pm}\pars{#1}}
	\newcommand\catderabsb[1]{\catderivedD^{\mathup{abs},b}\pars{#1}}
\newcommand\catderco[1]{\catderivedD^{\mathup{co}}\pars{#1}}
	\newcommand\catdercop[1]{\catderivedD^{\mathup{co,+}}\pars{#1}}
	\newcommand\catdercom[1]{\catderivedD^{\mathup{co,-}}\pars{#1}}
	\newcommand\catdercopm[1]{\catderivedD^{\mathup{co,\pm}}\pars{#1}}
	\newcommand\catdercob[1]{\catderivedD^{\mathup{co,b}}\pars{#1}}
\newcommand\catderctr[1]{\catderivedD^{\mathup{ctr}}\pars{#1}}
	\newcommand\catderctrp[1]{\catderivedD^{\mathup{ctr,+}}\pars{#1}}
	\newcommand\catderctrm[1]{\catderivedD^{\mathup{ctr,-}}\pars{#1}}
	\newcommand\catderctrpm[1]{\catderivedD^{\mathup{ctr,\pm}}\pars{#1}}
	\newcommand\catderctrb[1]{\catderivedD^{\mathup{ctr,b}}\pars{#1}}

==> _commands/categories/_categories_2.tex <==
%\newcommand\categoryformat[1]{\textup{\textbf{#1}}} % no current format

%\newvariableclass{category}[parent=alg,command=\categoryformat]
%\newmapclass{categoryof}[parent=category]

%\newmapclass{category}[parent=alg,command=\categoryformat,output=alg]

%\newmapclass{category}[
%	parent=alg,output=category,
%	]

\newmapclass{localizedcategory}[
	parent=alg,
	leftpar=\lbrack,rightpar=\rbrack,
	argkeyvals={
		{default}{{standardsep={\keyvalue^{-1}}}},
	},
]

\newcommand\categoryformat[1]{\textup{#1}}

\newmapclass{category}[parent=alg,command=\categoryformat]

\newcommand\catxmod[1]{\category{$#1$-mod}}
\newcategory\catRmod{$R$-mod}
\newcategory\catAmod{$A$-mod}

\newcommand\catmodx[1]{\category{mod-$#1$}}
\newcategory\catmodR{mod-$R$}
\newcategory\catmodA{mod-$A$}

\newcommand\catxmodx[2]{\category{$#1$-mod-$#2$}}
\newcategory\catRmodR{$R$-mod-$R$}
\newcategory\catAmodA{$A$-mod-$A$}


\newcommand\catxdgmod[1]{\category{$#1$-dgmod}}
\newcategory\catRdgmod{$R$-dgmod}
\newcategory\catAdgmod{$A$-dgmod}

\newcommand\catdgmodx[1]{\category{dgmod-$#1$}}
\newcategory\catdgmodR{dgmod-$R$}
\newcategory\catdgmodA{dgmod-$A$}

\newcommand\catxdgmodx[2]{\category{$#1$-dgmod-$#2$}}
\newcategory\catRdgmodR{$R$-dgmod-$R$}
\newcategory\catAdgmodA{$A$-dgmod-$A$}


\newcommand\catxcomod[1]{\category{$#1$-comod}}
\newcategory\catRcomod{$R$-comod}
\newcategory\catAcomod{$A$-comod}

\newcommand\catcomodx[1]{\category{comod-$#1$}}
\newcategory\catcomodR{comod-$R$}
\newcategory\catcomodA{comod-$A$}

\newcommand\catxcomodx[2]{\category{$#1$-comod-$#2$}}
\newcategory\catRcomodR{$R$-comod-$R$}
\newcategory\catAcomodA{$A$-comod-$A$}


%\newcategoryof\catvect{Vect}

\newcategory\catset{Set}
\newcategory\cattop{Top}


\newcategory\catvect{Vect}
\newcategory\catcat{Cat}
\newcategory\catab{Ab}
\newcategory\catgrp{Grp}
\newcategory\catcom{Com}
\newcategory\catalg{Alg}

\newcategory\catdgalg{dgAlg}
\newcategory\catainftyalg{\(\categoryformatmath{A_{\infty}}\)Alg}
\newcategory\catdgcat{dgCat}
\newcategory\catainftycat{\(\categoryformatmath{A_{\infty}}\)Cat}


\newcategory\catfun{Fun}
\newcategory\catdgfun{dgFun}
\newcategory\catainftyfun{\(\categoryformatmath{A_{\infty}}\)Fun}


\newmapclass{derivedcategory}[
	parent=alg,
	output=alg,
	singlekeys={
		{b}{upper=b},
		{+}{upper=+},
		{-}{upper=-},
		{+-}{upper=\pm},
		{pm}{upper=\pm},
		{ge0}{upper=\ge0},
		{le0}{upper=\le0},
		{fil}{upper=\mathup{fil}},
	},
]

\newderivedcategory\der{\mathscr{D}}



%\newcommand\category[1]{\textup{\textbf{#1}}}%For categories




%Specific categories


%
%
%\newcommand\catxmod[1]{\category{$#1$-mod}}
%	\newcommand\catRmod{\catxmod{R}}
%	\newcommand\catSmod{\catxmod{S}}
%	\newcommand\catAmod{\catxmod{A}}
%	\newcommand\catBmod{\catxmod{B}}
%\newcommand\catxmodf[1]{\category{$#1$-mod\textsuperscript{f}}}
%	\newcommand\catRmodf{\catxmodf{R}}
%	\newcommand\catSmodf{\catxmodf{S}}
%	\newcommand\catAmodf{\catxmodf{A}}
%	\newcommand\catBmodf{\catxmodf{B}}
%\newcommand\catmodx[1]{\category{mod-$#1$}}
%	\newcommand\catmodR{\catmodx{R}}
%	\newcommand\catmodS{\catmodx{S}}
%	\newcommand\catmodA{\catmodx{A}}
%	\newcommand\catmodB{\catmodx{B}}
%\newcommand\catxmodx[2]{\category{$#1$-mod-$#2$}}
%	\newcommand\catRmodR{\catxmodx{R}{R}}
%	\newcommand\catRmodS{\catxmodx{R}{S}}
%	\newcommand\catAmodA{\catxmodx{A}{A}}
%	\newcommand\catAmodB{\catxmodx{A}{B}}
%\newcommand\catxbimod[1]{\catxmodx{#1}{#1}}
%	\newcommand\catRbimod{\catxbimod{R}}
%	\newcommand\catAbimod{\catxbimod{A}}
%\newcommand\catxdgmod[1]{\category{$#1$-DGmod}}
%	\newcommand\catRdgmod{\catxdgmod{R}}
%	\newcommand\catSdgmod{\catxdgmod{S}}
%	\newcommand\catAdgmod{\catxdgmod{A}}
%	\newcommand\catBdgmod{\catxdgmod{B}}
%\newcommand\catdgmodx[1]{\category{DGmod-$#1$}}
%	\newcommand\catdgmodR{\catdgmodx{R}}
%	\newcommand\catdgmodS{\catdgmodx{S}}
%	\newcommand\catdgmodA{\catdgmodx{A}}
%	\newcommand\catdgmodB{\catdgmodx{B}}
%\newcommand\catxdgcomod[1]{\category{$#1$-DGcomod}}
%	\newcommand\catCdgcomod{\catxcomod{C}}
%\newcommand\catdgcomodx[1]{\category{DGcomod-$#1$}}
%	\newcommand\catdgcomodC{\catcomodx{C}}
%\newcommand\catxdgcontra[1]{\category{$#1$-DGcontra}}
%	\newcommand\catCdgcontra{\catxdgcontra{C}}
%\newcommand\catdgcontrax[1]{\category{dgcontra-$#1$}}
%	\newcommand\catdgcontraC{\catdgcontrax{C}}
%\newcommand\catvect{\category{Vect}}
%\newcommand\catvectf{\category{Vect\textsuperscript{f}}}
%\newcommand\catvectx[1]{\catvect\pars{#1}}
%	\newcommand\catvectk{{\catvectx{k}}}
%\newcommand\catvectfx[1]{\catvectf\pars{#1}}
%	\newcommand\catvectfk{{\catvectfx{k}}}
%\newcommand\catset{\category{Set}}
%\newcommand\catcat{\category{Cat}}
%\newcommand\catab{\category{Ab}}
%\newcommand\catgrp{\category{Grp}}
%\newcommand\catcom{\category{Com}}
%\newcommand\catcomx{\catcom\pars}
%\newcommand\catalg{\category{Alg}}
%\newcommand\catalgx[1]{\category{Alg}\pars{#1}}
%	\newcommand\catalgk{{\catalg{k}}}
%\newcommand\catrng{\category{Rng}}
%\newcommand\cattop{\category{Top}}
%\newcommand\cathot[1]{\category{Hot}\pars{#1}}
%\newcommand\catproj{\category{Proj}}
%\newcommand\catprojx[1]{\catproj\pars{#1}}
%	\newcommand\catprojA{{\catprojx{A}}}
%\newcommand\catinj{\category{Inj}}
%\newcommand\catinjx[1]{\catinj{#1}}
%	\newcommand\catinjA{\catinjx{A}}
%\newcommand\catacycl{\category{Acycl}}
%	\newcommand\catacyclx[1]{\catacycl\pars{#1}}
%	\newcommand\catacyclA[1]{{\catacyclx{A}}}
%\newcommand\catacyclabs{\category{Acycl\textsubscript{abs}}}
%	\newcommand\catacyclabsx[1]{\catacyclabs\pars{#1}}
%	\newcommand\catacyclabsA[1]{{\catacyclabsx{A}}}
%\newcommand\catacyclco{\category{Acycl\textsubscript{co}}}
%	\newcommand\catacyclcox[1]{\catacyclco\pars{#1}}
%	\newcommand\catacyclcoA[1]{{\catacyclcox{A}}}
%\newcommand\catacyclctr{\category{Acycl\textsubscript{ctr}}}
%	\newcommand\catacyclctrx[1]{\catacyclctr\pars{#1}}
%	\newcommand\catacyclctrA[1]{{\catacyclctrx{A}}}
%
%
%\newcommand\Lperp[1]{{}^{\perp}#1}
%\newcommand\lperp[1]{\lperp{(#1)}}
%\newcommand\Rperp[1]{#1^{\perp}}
%\newcommand\rperp[1]{\Rperp{(#1)}}
%
%\newcommand\catderivedD{\mathscr{D}}
%\newcommand\catder[2][]%
%{
%	\catderivedD
%	\ifblank{#1}
%	{
%		% do nothing
%	}
%	{
%		^{#1}
%	}
%	\pars{#2}
%}
%\newcommand\catderp[1]{\catderivedD^{+}\pars{#1}}
%\newcommand\catderm[1]{\catderivedD^{-}\pars{#1}}
%\newcommand\catderpm[1]{\catderivedD^{\pm}\pars{#1}}
%\newcommand\catderb[1]{\catderivedD^{b}\pars{#1}}
%\newcommand\catderabs[1]{\catderivedD^{\mathup{abs}}\pars{#1}}
%	\newcommand\catderabsp[1]{\catderivedD^{\mathup{abs},+}\pars{#1}}
%	\newcommand\catderabsm[1]{\catderivedD^{\mathup{abs},-}\pars{#1}}
%	\newcommand\catderabspm[1]{\catderivedD^{\mathup{abs},\pm}\pars{#1}}
%	\newcommand\catderabsb[1]{\catderivedD^{\mathup{abs},b}\pars{#1}}
%\newcommand\catderco[1]{\catderivedD^{\mathup{co}}\pars{#1}}
%	\newcommand\catdercop[1]{\catderivedD^{\mathup{co,+}}\pars{#1}}
%	\newcommand\catdercom[1]{\catderivedD^{\mathup{co,-}}\pars{#1}}
%	\newcommand\catdercopm[1]{\catderivedD^{\mathup{co,\pm}}\pars{#1}}
%	\newcommand\catdercob[1]{\catderivedD^{\mathup{co,b}}\pars{#1}}
%\newcommand\catderctr[1]{\catderivedD^{\mathup{ctr}}\pars{#1}}
%	\newcommand\catderctrp[1]{\catderivedD^{\mathup{ctr,+}}\pars{#1}}
%	\newcommand\catderctrm[1]{\catderivedD^{\mathup{ctr,-}}\pars{#1}}
%	\newcommand\catderctrpm[1]{\catderivedD^{\mathup{ctr,\pm}}\pars{#1}}
%	\newcommand\catderctrb[1]{\catderivedD^{\mathup{ctr,b}}\pars{#1}}

==> _commands/catlimits/_catlimits_1.tex <==
%Inverse and direct limits that look nicer:

\newcommand\newdirlim[2]{
	%#1 = command name
	%#2 = text name
	\newcommand#1{
		\mathop{
			\smash{
				\operatorname*{#2}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#2}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
	}
}

\newcommand\newinvlim[2]{
	%#1 = command name
	%#2 = text name
	\newcommand#1{
		\mathop{
			\smash{
				\operatorname*{#2}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#2}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
	}
}



\newdirlim\dirlim{lim}
\newinvlim\invlim{lim}

\newdirlim\holim{holim}
%newinvlim\invholim{holim}


\begin{comment}
\newcommand\dirlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xrightarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}

\newcommand\invlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xleftarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}
\end{comment}

\begin{comment}
\newcommand\dirlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xrightarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}

\newcommand\invlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xleftarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}
\end{comment}

==> _commands/catlimits/_catlimits_2.tex <==
%Inverse and direct limits that look nicer:

\newcommand\dirlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

\newcommand\invlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}



%\newdirlim\dirlim{lim}
%\newinvlim\invlim{lim}

%\newdirlim\holim{holim}
%newinvlim\invholim{holim}

\newmapclass{catlim}[
	parent=algop,
	keyvals={
		{diag}{lower={\keyvalue}},
		{default}{diag={\keyvalue}},
		%{weight}{symbolputright={{}^{\keyvalue}},return,command=\mathop,symbolputright=\limits},
		{weight}{return,upper={\keyvalue}},
	},
]


\newcatlim\dirlim{\dirlimformat{lim}}
\newcatlim\invlim{\invlimformat{lim}}
\newcatlim\dirholim{\dirlimformat{holim}}
\newcatlim\invholim{\invlimformat{holim}}



\begin{comment}
\newcommand\dirlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xrightarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}

\newcommand\invlim{
	\mathop{
		\smash{
			\lim\limits_{
				{}
				\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$\xleftarrow{\hspace*{1.15em}}$}}
			}
		}
		\vphantom{\textstyle\lim_n}
	}
}
\end{comment}

\begin{comment}
\newcommand\dirlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xrightarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}

\newcommand\invlim{
	\mathop{
		\vphantom{g}
		\smash{
			\lim\limits
			_{
				\raisebox{.1em}[0pt][0pt]{$
					\xleftarrow{\hphantom{\hspace*{.95em}}}
					$}
			}
		}
	}
}
\end{comment}

==> _commands/catlimits/_catlimits_3.tex <==
%Inverse and direct limits that look nicer:

\newcommand\dirlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xrightarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

\newcommand\invlimformat[1]{
	%#1 = text name
		\mathop{
			\smash{
				\operatorname*{#1}\limits_{
					{}
					\raisebox{.21em}[0pt][0pt]{\scalebox{.85}{$
						\xleftarrow{%
							%\hspace*{
							%	\widthof{space}
							%}%
							\hphantom
							{%
								\!\!\!\!
								\scalebox{1.17}{$
									{\operatorname{#1}}
								$}
								\!\!\!
							}
						}
					$}}
				}
			}
			\vphantom{\textstyle\lim_n}
		}
}

%\NewDocumentCommand\dirlimcommand{me{_^}}{%
%	\mathchoice
%		{ \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { {} ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \dirlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%}

%\NewDocumentCommand\invlimcommand{me{_^}}{%
%	\mathchoice
%		{ \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { {} ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%	    { \invlimformat { #1 } \IfValueT{#2} { _{#2} } \IfValueT {#3} { ^ { #3 } } }
%}





%\newdirlim\dirlim{lim}
%\newinvlim\invlim{lim}

%\newdirlim\holim{holim}
%newinvlim\invholim{holim}

\newmapclass{catlim}[
	parent=algop,
	keyvals={
		{diag}{lower={\keyvalue}},
		{default}{diag={\keyvalue},return},
		%{weight}{symbolputright={{}^{\keyvalue}},return,command=\mathop,symbolputright=\limits},
		{weight}{upper={\keyvalue},return},
	},
]


\newcatlim\dirlim{\dirlimformat{lim}}
\newcatlim\invlim{\invlimformat{lim}}
\newcatlim\dirholim{\dirlimformat{holim}}
\newcatlim\invholim{\invlimformat{holim}}


==> _commands/delims/_delims_1.tex <==

% \abs{x} for absolute values:
\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
	\slotifempty{#1}
}

\DeclarePairedDelimiterX\size[1]\lvert\rvert{
	\slotifempty{#1}
}

\newcommand\varsize[1]{\#}

% \norm{x} for norms:
\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
	\slotifempty{#1}
}
% \inner{u}{v} for inner products:
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
	\slotifempty{#1},\slotifempty{#2}
}

\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
	\slotifempty{#1},\slotifempty{#2}
}


%For set notation \Set{ x \in X \given x > 0 }
\newcommand\SetSymbol[1][]{
	\nonscript\:
	#1\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}
%\providecommand\given{}

\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\set{\lbrace}{\rbrace}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

==> _commands/delims/_delims_2.tex <==

% \abs{x} for absolute values:
\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
	\slotifempty{#1}
}

\DeclarePairedDelimiterX\size[1]\lvert\rvert{
	\slotifempty{#1}
}

\newcommand\varsize[1]{\#}

% \norm{x} for norms:
\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
	\slotifempty{#1}
}
% \inner{u}{v} for inner products:
\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
	\slotifempty{#1},\slotifempty{#2}
}

\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
	\slotifempty{#1},\slotifempty{#2}
}


%For set notation \Set{ x \in X \given x > 0 }
\newcommand\SetSymbol[1][]{
	\nonscript\:
	#1\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}
%\providecommand\given{}

\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\set{\lbrace}{\rbrace}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

==> _commands/delims/_delims_3.tex <==

%% \abs{x} for absolute values:
%\DeclarePairedDelimiterX\abs[1]\lvert\rvert{
%	\slotifempty{#1}
%}
%
%\DeclarePairedDelimiterX\size[1]\lvert\rvert{
%	\slotifempty{#1}
%}
%
%\newcommand\varsize[1]{\#}
%
%% \norm{x} for norms:
%\DeclarePairedDelimiterX\norm[1]\lVert\rVert{ %normer
%	\slotifempty{#1}
%}
%% \inner{u}{v} for inner products:
%\DeclarePairedDelimiterX{\inner}[2]{\langle}{\rangle}{ %indre produkter
%	\slotifempty{#1},\slotifempty{#2}
%}
%
%\DeclarePairedDelimiterX\com[2]{[}{]}{ %commutator
%	\slotifempty{#1},\slotifempty{#2}
%}


%%For set notation \Set{ x \in X \given x > 0 }
%\newcommand\SetSymbol[1][]{
%	\nonscript\:
%	#1\vert
%	\allowbreak
%	\nonscript\:
%	\mathopen{}
%}
%\providecommand\given{}

%\newcommand\where{\errmessage{The command \noexpand\where was used outside an allowed environment on input line \the\inputlineno.}}

\newcommand\where{
	\nonscript\:
	\automathdelimsize\vert
	\allowbreak
	\nonscript\:
	\mathopen{}
}

%\DeclarePairedDelimiterX\Set[1]{\lbrace}{\rbrace}{
%	\renewcommand\where{\SetSymbol[\delimsize]}
%	\,#1\, %Note that I added the spaces around the inner part
%}

\newdelimiterclass{delim}[
	parent=var,
	output=var,
	keyvals={
		{ord}{outputoptions={lower={\keyvalue}}}, % for e.g. the n-norm
	},
]

\newdelim\Set{\lbrace}{\rbrace}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=classset,
	]


\newtuple\set{\lbrace}{,}{\rbrace}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\newdelim\Gen{\langle}{\rangle}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=alg,
	]


\newtuple\gen{\langle}{,}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}


\newdelim\Vargen{(}{)}[
	keyvals={
		{argdefault}{argnokeyval=\,,argnokeyval=\keyvalue,argnokeyval=\,},
	},
	output=alg,
	]


\newtuple\vargen{(}{,}{)}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\newdelim\cl{[}{]} % equivalence classes

\newdelim\abs{\lvert}{\rvert}

\newdelim\norm{\lVert}{\rVert}

% Using the same principles, we define \Gen and \gen for algebraic generation,
% using ⟨⟩ and \Altgen and \altgen using ()


\begin{comment}

\DeclarePairedDelimiterX\Gen[1]{\langle}{\rangle}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\gen{\langle}{\rangle}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

\DeclarePairedDelimiterX\Vargen[1]{(}{)}{
	\renewcommand\where{\SetSymbol[\delimsize]}
	\,#1\, %Note that I added the spaces around the inner part
}

\newflextuple\vargen{(}{)}{,}{\ldots} %For non-contruction sets like \set{0,1,2,\ldots}

%Two commands \Prob{...} og \Mean{...} for probabilities and means. They support the same command \given as before

\DeclarePairedDelimiterXPP\lgen[2]{}{\langle}{\rangle}{_{#1}}{
	#2
}

\DeclarePairedDelimiterXPP\Lgen[2]{}{\langle}{\rangle}{_{#1}}{
	\renewcommand\given{\SetSymbol[\delimsize]}
	\,#2\, %Note that I added the spaces around the inner part
}

\DeclarePairedDelimiterXPP\Prob[1]{P}(){}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}
\DeclarePairedDelimiterXPP\Mean[1]{\mathbb{E}}[]{}{
	\renewcommand\where{\nonscript\:\delimsize\vert\nonscript\:
		\mathopen{}}
	#1}


\DeclarePairedDelimiterXPP\pol[2]{#1}{[}{]}{}{ % polynomials
	#2
}

\DeclarePairedDelimiterXPP\rat[2]{#1}{(}{)}{}{ % rational functions
	#2
}

\DeclarePairedDelimiterXPP\fal[2]{#1}{\langle}{\rangle}{}{ % free algebra
	#2
}

\DeclarePairedDelimiter\cl{[}{]} % equivalence classes

\newcommand\varcl{\widebar}

% the commands \pars, for the backwards notation \pars{...}[\big] and \pars{...}*

\DeclarePairedDelimiter{\@parentheses}{(}{)}

\DeclareDocumentCommand\parentheses{mso}
{
	\IfBooleanTF{#2}
	{
		\@parentheses*
	}
	{
		\IfNoValueTF{#3}
		{
			\@parentheses
		}
		{
			\@parentheses[#3]
		}
	}
	{
		#1
	}
}

\newcommand\identity[1]{#1}
\newcommand\pars{}

\ExplSyntaxOn



\cs_set:Npn \pars#1{%
	\tl_if_blank:nTF{ #1 }
	{
		% do nothing
	}
	{
		\str_case:nnTF { #1 }
		{
			{.} {}
			{:} {\identity}
			{*} {\parentheses{\slot}}
			{-} {\parentheses{\slot}}
		}
		{
			% do nothing
		}
		{
			\parentheses{#1}%
		}%
	}
}

\ExplSyntaxOff

\end{comment}

==> _commands/derivatives/_derivatives_1.tex <==
\begin{comment}
\NewDocumentCommand\dif{D(){}O{}m}{
	\frac{
		\D(#1){#2}
	}{
		\D{#3}
		\IfNoValueTF{#1}{
			%do nothing
		}{
			^{#1}
		}
	}
}

\NewDocumentCommand\tdif{D(){}O{}m}{
	\tfrac{
		\D(#1){#2}
	}{
		\D{#3}
		\IfNoValueTF{#1}{
			%do nothing
		}{
			^{#1}
		}
	}
}

\newcommand*\cont[2][]{
		\ifblank{#1}{
			C(#2)
		}{
			C^{#1}(#2)
		}
	}
\newcommand*\continto[3][]{
	\ifblank{#1}{
		C(#2,#3)
	}{
	C^{#1}(#2,#3)
}
}
\end{comment}

==> _commands/homology/_homology_1.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
					%\use:c { _homology_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
					%\use:c{ _homology_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cx { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	%\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			\use:c { _homology_#1_keys_set:n } { main={#3} }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
	%\group_end:

	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\group_begin:
			\exp_args:Nv
			\_homology_upper_index:n
			{
				_homology_#1_main_index
			}
			%\exp_args:NNNo\exp_args:NNo
			\exp_args:Nv
			\_homology_lower_index:n
			{
				_homology_#1_second_index
			}
		\group_end:
	}
	{
		\group_begin:
			\exp_args:Nv\_homology_upper_index:n
			{
				\group
				_homology_#1_second_index
			}
			\exp_args:Nv\_homology_lower_index:n
			{
				_homology_#1_main_index
			}
		\group_end:
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}




\newcomplex\dif{d}
\newcomplex\pdif{\partial}
\newcomplex\ddif{\delta}

\newsimplex\face{d}
\newsimplex\pface{\partial}
\newsimplex\dface{\delta}


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\ExplSyntaxOff


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_1000.tex <==
\newcohomologyclass{cohomology}[
	parent=var,
	gradingpos=upper,
	keyvals={
		{shift}{ symbolputright={[\keyvalue]} },
	},
	singlekeys={
		{cech}{ command=\noexpand\check },
		%{cech} { command=\check },
		{hyper}{ command=\mathbb },
	},
	argkeyvals={
		{cover}{ {\keyvalue} },
		{coef}{sep={;}{\keyvalue}},
		{c}{sep={;}{\keyvalue}},
	},
]


\newmapclass{homset}[
	parent=cohomology,
]

\newcomplexclass{complex}[
	parent=cohomology,
]

\newcohomologyclass{homology}[
	parent=cohomology,
	gradingpos=lower,
]


\newcomplexclass{simplex}[
	parent=cohomology,
	gradingpos=lower,
]


\newhomset{\Hom}{\operatorname{Hom}}
\newhomset{\Ext}{\operatorname{Ext}}
\newhomset{\Map}{\operatorname{Map}}

%\newcohomology{homp}{\operatorname{Hom}}
%\let\Hom=\Hompre

%\let\hom=\homp
%\let\Hom=\homp

%\DeclareMathOperator\Extproto{Ext}

%\newcohomology{\ext}{\Extproto}

%\let\Ext=\ext

%\newhomset{\extone}{\Extproto}

\newcomplex\comX{X}
\newcomplex{\comY}{Y}
\newcomplex{\comZ}{Z}
\newcomplex{\comM}{M}
\newcomplex{\comN}{N}
\newcomplex{\comP}{P}
\newcomplex{\comQ}{Q}
\newcomplex{\comI}{I}
\newcomplex{\comJ}{J}
\newcomplex{\comA}{A}
\newcomplex{\comB}{B}
\newcomplex{\comC}{C}
\newcomplex{\comD}{D}
\newcomplex{\comE}{E}
\newcomplex{\comF}{F}
%\end{comment}

%\newcohomology\co{H}
%\newhomology\ho{H}
%
%\newcohomology\coch{C}
%\newhomology\hoch{C}
%
%\newcohomology\cocy{Z}
%\newhomology\hocy{Z}
%
%\newcohomology\coby{B}
%\newhomology\hoby{B}

\begin{comment}

\end{comment}

\ExplSyntaxOn
\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\exp_args:Nc\newcohomology{#1co}{#2}
	\exp_args:Nc\newhomology{#1ho}{#2}[parent=#1co]
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\exp_args:Nc\newhomology{#1hoch}{#3}[parent=#1co]
	\exp_args:Nc\newcohomology{#1coch}{#3}[parent=#1co]
	\exp_args:Nc\newhomology{#1hocy}{#4}[parent=#1co]
	\exp_args:Nc\newcohomology{#1cocy}{#4}[parent=#1co]
	\exp_args:Nc\newhomology{#1hobo}{#5}[parent=#1co]
	\exp_args:Nc\newcohomology{#1cobo}{#5}[parent=#1co]
}
\ExplSyntaxOff


\newhomologytheory{}{H}{C}{Z}{B}

\newhomologytheory{sh}{\mathscr{H}}{\mathscr{C}}{\mathscr{Z}}{\mathscr{B}}

\setupobject\shco{output=sheaf}


\newcohomologyclass{derivedfunctor}[parent=cohomology,nopar,output=map]
\newderivedfunctor\Lder{L}
\newderivedfunctor\Rder{R}




\newcohomology\exterior{\Lambdaup}[upper=\!\!]



\newcohomology\Bar{\operatorname{Bar}}

\newcohomology\Cob{\operatorname{Cob}}

==> _commands/homology/_homology_2.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
					%\use:c { _homology_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
					%\use:c{ _homology_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			%\use:c { _homology_#1_index_go_auto: }
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			\use:c { _homology_#1_keys_set:n } { main={#3} }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
	%\group_end:
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo

			\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
			\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
			\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
			\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnnn{#1}{ \cs_to_str:N#1 }{ sheaf, indextype=upper} { #2 } { #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_homology_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\ExplSyntaxOff


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_3.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn { #1 }
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1  {\_homology_parentheses:w{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_big:n #1  {\_homology_parentheses:w[\big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Big:n #1  {\_homology_parentheses:w[\Big]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_bigg:n #1  {\_homology_parentheses:w[\bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_Bigg:n #1  {\_homology_parentheses:w[\Bigg]{\_homology_interpret:n{#1}}}

\cs_new:Npn \_homology_parentheses_auto:n #1  {\_homology_parentheses:w*{\_homology_interpret:n{#1}}}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
				\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx \_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		\exp_args:Nnx\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_4.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }		
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_5.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:cn { _homology_#1_main_index } { #3 }
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ \big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { * }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { ** }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/homology/_homology_6.tex <==
% Constructions like Hom, cohomology etc.

\begin{comment}
\newcommand*{\Cdot}[1][1.25]{%
  \mathpalette{\CdotAux{#1}}\cdot%
}
\newdimen\CdotAxis
\newcommand*{\CdotAux}[3]{%
  {%
    \settoheight\CdotAxis{$#2\vcenter{}$}%
    \sbox0{%
      \raisebox\CdotAxis{%
        \scalebox{#1}{%
          \raisebox{-\CdotAxis}{%
            $\mathsurround=0pt #2#3$%
          }%
        }%
      }%
    }%
    % Remove depth that arises from scaling.
    \dp0=0pt %
    % Decrease scaled height.
    \sbox2{$#2\bullet$}%
    \ifdim\ht2<\ht0 %
      \ht0=\ht2 %
    \fi
    % Use the same width as the original \cdot.
    \sbox2{$\mathsurround=0pt #2#3$}%
    \hbox to \wd2{\hss\usebox{0}\hss}%
  }%
}

\def\smallbullet{\Cdot[1.5]}
\end{comment}


\ExplSyntaxOn

%\input{_commands/homology/ktype/_ktype_1}



%\DeclarePairedDelimiter{\@parentheses}{(}{)}




\bool_new:N\_if_first_homology:
\bool_set_true:N\_if_first_homology:

\tl_new:N\_homology_seperator:
\tl_new:N\_homology_coefficient_seperator:

\tl_set:Nn \_homology_seperator: {,}
\tl_set:Nn \_homology_coefficient_seperator: {;}
\tl_set:Nn \_homology_dots: {\ldots}
\tl_set:Nn \_homology_slot: {\slot}
\tl_set:Nn \_homology_bullet: {\smallbullet}
\tl_set:Nn \_homology_double_bullet: {\smallbullet\smallbullet}
\tl_set:Nn \_homology_sheaf_restrict { \vert }
\tl_set:Nn \_homology_sheaf_stalk_sep { , }
\tl_set:Nn \_homology_sheafify_symbol {+}



\cs_new:Npn \_homology_slot_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_slot:}
		{*} {\_homology_slot:}
		{-} {\_homology_slot:}
		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_bullet_if_bar:n #1
{
	\str_case:nnTF { #1 }
	{
%		{.} {\_homology_bullet:}
		{*} {\_homology_bullet:}
		{**} {\_homology_double_bullet:}
%		{-} {\_homology_bullet:}
%		{...} {\_homology_dots:}
	}
	{
		% do nothing
	}
	{
		#1
	}
}

\cs_new:Npn \_homology_parse_ordinaries:n #1
{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
	}
	{
		\_homology_seperator:
	}
	\_homology_slot_if_bar:n{#1}
}

\cs_new:Npn \_homology_parse_specials:nn#1#2{
	\bool_if:NTF\_if_first_homology:
	{
		\bool_set_false:N \_if_first_homology:
		\str_case:nnTF{ #1 }
		{
			{c} {}
			{coef} {}
			{b} {}
			{base} {}
			{s} {}
			{sh} {}
			{sheaf} {}
			{cov} {}
			{cover} {}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
	{
		\str_case:nnTF{ #1 }
		{
			{c} {\_homology_coefficient_seperator:}
			{coef} {\_homology_coefficient_seperator:}
			{b} {\_homology_seperator:}
			{base} {\_homology_seperator:}
			{s} {\_homology_seperator:}
			{sh} {\_homology_seperator:}
			{sheaf} {\_homology_seperator:}
			{cov} {\_homology_seperator:}
			{cover} {\_homology_seperator:}
		}
		{
			\_homology_slot_if_bar:n{#2}
		}
		{
			#1=#2
		}
	}
}


\cs_new:Npn \_homology_interpret:n #1
{
	\group_begin:
		\bool_set_true:N \_if_first_homology:
		\keyval_parse:NNn \_homology_parse_ordinaries:n \_homology_parse_specials:nn {{{ #1 }}}%
			% the two extra braces are necessary because \keyval_parse:NNn seems to expand its input twice
	\group_end:
}


\cs_new:Npn \_homology_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


%\DeclarePairedDelimiter{\_homology_parentheses:w}{(}{)}

\cs_new:Npn \_homology_parentheses_normal:n #1
{
	(
		\_homology_interpret:n{#1}
	)
}

\cs_new:Npn \_homology_parentheses_big:n #1
{
	\big(
		\_homology_interpret:n{#1}
	\big)
}

\cs_new:Npn \_homology_parentheses_Big:n #1
{
	\Big(
		\_homology_interpret:n{#1}
	\Big)
}

\cs_new:Npn \_homology_parentheses_bigg:n #1
{
	\bigg(
		\_homology_interpret:n{#1}
	\bigg)
}

\cs_new:Npn \_homology_parentheses_Bigg:n #1
{
	\Bigg(
		\_homology_interpret:n{#1}
	\Bigg)
}

\cs_new:Npn \_homology_parentheses_auto:n #1
{
	\left(
		\_homology_interpret:n{#1}
	\right)
}


\cs_new:Npn \_homology_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_homology_parentheses_normal:n { #2 }}
		{ big } { \_homology_parentheses_big:n { #2 }}
		{ \big } { \_homology_parentheses_big:n { #2 }}
		{ Big } { \_homology_parentheses_Big:n { #2 }}
		{ \Big } { \_homology_parentheses_Big:n { #2 }}
		{ bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ \bigg } { \_homology_parentheses_bigg:n { #2 }}
		{ Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_homology_parentheses_Bigg:n { #2 }}
		{ auto } { \_homology_parentheses_auto:n { #2 }}
		{ * } { \_homology_parentheses_auto:n { #2 }}
		{ none } { \_homology_no_parentheses:n { #2 }}
		{ } { \_homology_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_homology_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_homology_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
				%#1
			}
		}
	}
}

\cs_new:Npn \_homology_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_homology_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_homology_bullet_if_bar:n { ##1 } }
				\exp_args:No\_homology_bullet_if_bar:n { #1 }
				%#1
			}
		}
	}
}



\tl_new:N \_homology_commands_tl_temp


\cs_new:Npn \_homology_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _homology_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _homology_#1_commands_sequence }
			}
			{
				\_homology_keyval:nnn { #1 } { command } { none }
				\_homology_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _homology_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _homology_#1_if_upper_index }
				}
				{ lower }
				{
					\bool_set_false:c { _homology_#1_if_upper_index }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ main } {
			%\use:c { _homology_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_main_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { main } { none }
				\_homology_keyval:nnn { #1 } { addmain } { #3 }
			}
		}
		{ addmain } {
			\tl_put_right:co { _homology_#1_main_index } { #3 } 
		}
		{ index } {
			\_homology_keyval:nnn { #1 } { main } { #3 }
		}
		{ addindex } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }			
		}
		{ second } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _homology_#1_second_index } { } %empty
			}
			{
				\_homology_keyval:nnn { #1 } { second } { none }
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
		}
		{ addsecond } {
			\tl_put_right:cn { _homology_#1_second_index } { #3 }
		}
		{ par } {
			\str_set:cn { _homology_#1_par_size }{ #3 }
		}
		{ n } {
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
		}
		{ rest } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_restrict #3 } }
		{ stalk } {
			\tl_if_empty:cTF { _homology_#1_second_index }
			{
				\_homology_keyval:nnn { #1 } { addsecond } { #3 }
			}
			{
				\_homology_keyval:nnn { #1 } { addsecond } { \_homology_sheaf_stalk_sep #3 }
			}
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_homology_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_homology_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_homology_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_homology_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_homology_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_homology_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sheaf } { \_homology_keyval:nnn { #1 }{ addcommand } { \sheaf } }
		{ sheafify } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_sheafify_symbol } }
		{ big }{ \_homology_keyval:nnn { #1 }{ par } { big } }
		{ Big }{ \_homology_keyval:nnn { #1 }{ par } { Big } }
		{ bigg }{ \_homology_keyval:nnn { #1 }{ par } { bigg } }
		{ Bigg }{ \_homology_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_homology_keyval:nnn { #1 } { addmain } { \_homology_bullet: }}
		{ ** }{ \_homology_keyval:nnn { #1 } { addmain } { \_homology_double_bullet: }}
		{ indexbullet } { \_homology_keyval:nnn { #1 } { addsecond } { \_homology_bullet: }}
		{ indexdoublebullet }{ \_homology_keyval:nnn { #1 } { addsecond } { \_homology_double_bullet: }}
	}
	{
		% do nothing
	}
	{
		\_homology_keyval:nnn { #1 }{ addsecond } { #2 }
	}
}





\cs_new:Npn \_homology_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _homology_#1_commands_sequence }
	
	\bool_new:c { _homology_#1_if_upper_index }
	\tl_new:c { _homology_#1_main_index }
	\tl_new:c { _homology_#1_second_index }
	
	\cs_new:cpn { _homology_#1_keyval:nn } ##1##2
	{
		\_homology_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _homology_#1_indexkey:n } ##1
	{
		\_homology_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _homology_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _homology_#1_indexkey:n }
			{ _homology_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _homology_#1_par_size }
	
	
	\cs_new_protected:cpn { _homology_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_homology_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _homology_#1_commands_sequence }
			{
				\tl_set:Nx \_homology_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_homology_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_homology_commands_tl_temp
	}
	
	\use:c { _homology_#1_keys_set:n } {
		#2
	}
}

\newcommand\homologysetup[2]{
	%\exp_args:Nx
	\use:c { _homology_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N \_homology_par_size_temp

\cs_new:Npn \_homology_parse_symbol:nnn #1#2#3
{
	\group_begin:
		\use:c { _homology_#1_keys_set:n } { #2 }
		\tl_if_blank:nTF { #3 }
		{
			% do nothing
		}
		{
			%\use:c { _homology_#1_keys_set:n } { main={#3} }
			\_homology_keyval:nnn { #1 } { addmain } { #3 }
			%\exp_args:Nnno\_homology_keyval:nnn { #1 } { addmain } { \_homology_bullet_if_bar:n { #3 } }
		}
		
		\use:c { _homology_#1_command:n }%
		{
			\use:c { _homology_#1_symbol: }
		}
		\tl_gset:Nv\_homology_main_index_temp { _homology_#1_main_index }
		\tl_gset:Nv\_homology_second_index_temp { _homology_#1_second_index }
		\str_gset_eq:Nc\_homology_par_size_temp { _homology_#1_par_size }
	\group_end:
	\bool_if:cTF { _homology_#1_if_upper_index }
	{
		%\exp_args:NNNo\exp_args:NNo
		\exp_args:NV \_homology_upper_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_lower_index:n \_homology_second_index_temp
	}
	{
		\exp_args:NV \_homology_lower_index:n \_homology_main_index_temp
		\exp_args:NV \_homology_upper_index:n \_homology_second_index_temp
	}
}

\str_new:N \_homology_cs_str_temp

\cs_new:Npn\_homology_newcohomology:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{omg}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_homology_parse_symbol:nnn { #2 } { } { ##2 }
			}
			{
				\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
			}
			\IfNoValueTF { ##3 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:No
				\_homology_parentheses:nn { \_homology_par_size_temp } { ##3 }
			}%
		\group_end:		
	}
}

%\DeclareDocumentCommand{\homologysetup}{argspec}{code}

\DeclareDocumentCommand\newcohomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newhomology{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcohomology:nnnn{#1}{ \cs_to_str:N#1 }{ #2 } { indextype=lower, #3 }%
	}
}



\cs_new:Npn\_homology_newhom:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \hom
	% #2 = name without backshash, e.g. hom
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{ossg}{
		\group_begin:
			\IfBooleanTF{ ##2 }
			{
				\IfBooleanTF { ##3 }
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=** } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=**,##1 } { }
					}
				}
				{
					\IfNoValueTF { ##1 }
					{
						\_homology_parse_symbol:nnn { #2 } { main=* } { }
					}
					{
						\_homology_parse_symbol:nnn { #2 } { main=*, ##1 } { }
					}
				}
			}
			{
				\IfNoValueTF { ##1 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
			}
			\IfNoValueTF { ##4 }%
			{%
				%do nothing
			}%
			{%
				\exp_args:Nx\_homology_parentheses:nn { \str_use:c { _homology_#2_par_size }} { ##4 }
			}%
		\group_end:		
	}
}

\DeclareDocumentCommand\newhom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcohom{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower, #3 }%
	}
}

\DeclareDocumentCommand\newsheaf{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newhom:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { sheaf, indextype=upper, #3 }%
	}
}



\cs_new:Npn\_homology_newcomplex:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \comX
	% #2 = name without backshash, e.g. comX
	% #3 = cohomology symbol
	% #4 = other options
%	\IfNoValueTF{ #4 }
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_homology_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
	\_homology_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\IfNoValueTF { ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { } { ##2 }
				}
			}
			{
				\IfNoValueTF{ ##2 }
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { }
				}
				{
					\_homology_parse_symbol:nnn { #2 } { ##1 } { ##2 }
				}
			}
		\group_end:		
	}
}

\DeclareDocumentCommand\newcomplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=upper , #3 }%
	}
}

\DeclareDocumentCommand\newsimplex{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn { #1 } { \cs_to_str:N#1 } { #2 } { indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_homology_newcomplex:nnnn{#1}{ \cs_to_str:N#1 } { #2 } { indextype=lower , #3 }%
	}
}




%\newcomplex\dif{d}
%\newcomplex\pdif{\partial}
%\newcomplex\ddif{\delta}

%\newsimplex\face{d}
%\newsimplex\pface{\partial}
%\newsimplex\dface{\delta}

\ExplSyntaxOff


\newhom\homp{\Hom}

\let\hom=\homp

\DeclareMathOperator\Extproto{Ext}

\newcohomology\ext{\Extproto}

\let\Ext=\ext

\newhom\extone{\Extproto}

\newcomplex\comX{X}
\newcomplex\comY{Y}
\newcomplex\comZ{Z}
\newcomplex\comM{M}
\newcomplex\comN{N}
\newcomplex\comP{P}
\newcomplex\comQ{Q}
\newcomplex\comI{I}
\newcomplex\comJ{J}
\newcomplex\comA{A}
\newcomplex\comB{B}
\newcomplex\comC{C}
\newcomplex\comD{D}
\newcomplex\comE{E}
\newcomplex\comF{F}


\newcommand\newhomologytheory[5]{
	% #1 = name
	% #2 = H symbol
	% #3 = C symbol
	% #4 = Z symbol
	% #5 = B symbol
	\expandafter\newhomology\csname#1ho\endcsname{#2}
	\expandafter\newcohomology\csname#1co\endcsname{#2}
	%\expandafter\newoptcohomology\csname#1coring\endcsname{#2}
	\expandafter\newhomology\csname#1hoch\endcsname{#3}
	\expandafter\newcohomology\csname#1coch\endcsname{#3}
	\expandafter\newhomology\csname#1hocy\endcsname{#4}
	\expandafter\newcohomology\csname#1cocy\endcsname{#4}
	\expandafter\newhomology\csname#1hobo\endcsname{#5}
	\expandafter\newcohomology\csname#1cobo\endcsname{#5}
}




\newhomologytheory{}{H}{C}{Z}{B}

==> _commands/index/_index_1.tex <==
\DeclareDocumentCommand\textdef{som}{% for inline text definitions
	\IfBooleanTF{#1}{%
		\textbf{#3}%
	}{%
	\IfNoValueTF{#2}%
	{%
		\index{#3}%
	}%
	{%
		\index{#2}%
	}%
	\textbf{#3}%
}%
}

==> _commands/intervals/_intervals_1.tex <==
% Commands for intervals


	\newcommand\open\tradopen
	\newcommand\openpm\tradopenpm
	\newcommand\ropen\tradropen
	\newcommand\ropenpm\tradropenpm
	\newcommand\lopen\tradlopen
	\newcommand\lopenpm\tradlopenpm
	\newcommand\closed\tradclosed
	\newcommand\closedpm\tradclosedpm

%Traditional notation:

\DeclarePairedDelimiterX\tradopen[2]
	()
	{#1,#2}
\DeclarePairedDelimiterX\tradopenpm[1]
	()
	{-#1,#1}
\DeclarePairedDelimiterX\tradlopen[2]
	(]
	{#1,#2}
\DeclarePairedDelimiterX\tradlopenpm[1]
	(]
	{-#1,#1}
\DeclarePairedDelimiterX\tradropen[2]
	[)
	{#1,#2}
\DeclarePairedDelimiterX\tradropenpm[1]
	[)
	{-#1,#1}
\DeclarePairedDelimiterX\tradclosed[2]
	[]
	{#1,#2}
\DeclarePairedDelimiterX\tradclosedpm[1]
	[]
	{-#1,#1}

% Bourbaki notation:
\DeclarePairedDelimiterX\bouropen[2]
	][ 
	{#1,#2}
\DeclarePairedDelimiterX\bouropenpm[1]
	][
	{-#1,#1}
\DeclarePairedDelimiterX\bourlopen[2]
	]]
	{#1,#2}
\DeclarePairedDelimiterX\bourlopenpm[1]
	]]
	{-#1,#1}
\DeclarePairedDelimiterX\bourropen[2]
	[[
	{#1,#2}
\DeclarePairedDelimiterX\bourropenpm[1]
	[[
	{-#1,#1}
\DeclarePairedDelimiterX\bourclosed[2]
	[]
	{#1,#2}
\DeclarePairedDelimiterX\bourclosedpm[1]
	[]
	{-#1,#1}

==> _commands/lie/_lie_1.tex <==
%Lie stuff:

\newcommand\lieg{\mathfrak{g}}
\newcommand\lieh{\mathfrak{h}}
\newcommand\liegl{\mathfrak{gl}}
\newcommand\liesl{\mathfrak{sl}}
\newcommand\liesu{\mathfrak{su}}
\newcommand\lieso{\mathfrak{so}}

\let\g=\lieg
\let\h=\lieh

==> _commands/maps/_maps_1.tex <==

%\DeclarePairedDelimiter{\@parentheses}{(}{)}

\ExplSyntaxOn



\bool_new:N\_if_first_map:
\bool_set_true:N\_if_first_map:

\tl_new:N\_map_seperator:
\tl_new:N\_map_coefficient_seperator:

\tl_set:Nn \_map_seperator: {,}
\tl_set:Nn \_map_coefficient_seperator: {;}
\tl_set:Nn \_map_dots: {\ldots}






\cs_new:Npn \_map_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_map_parentheses:w}{(}{)}

\cs_new:Npn \_map_parentheses_normal:n #1  {\_map_parentheses:w{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_big:n #1  {\_map_parentheses:w[\big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Big:n #1  {\_map_parentheses:w[\Big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_bigg:n #1  {\_map_parentheses:w[\bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Bigg:n #1  {\_map_parentheses:w[\Bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_auto:n #1  {\_map_parentheses:w*{\tup_process{#1}}}


\cs_new:Npn \_map_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_map_parentheses_normal:n { #2 }}
		{ big } { \_map_parentheses_big:n { #2 }}
		{ \big } { \_map_parentheses_big:n { #2 }}
		{ Big } { \_map_parentheses_Big:n { #2 }}
		{ \Big } { \_map_parentheses_Big:n { #2 }}
		{ bigg } { \_map_parentheses_bigg:n { #2 }}
		{ \bigg } { \_map_parentheses_bigg:n { #2 }}
		{ Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ auto } { \_map_parentheses_auto:n { #2 }}
		{ * } { \_map_parentheses_auto:n { #2 }}
		{ none } { \_map_no_parentheses:n { #2 }}
		{ } { \_map_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_map_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_map_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}

\cs_new:Npn \_map_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_map_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}



\tl_new:N \_map_commands_tl_temp


\cs_new:Npn \_map_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _map_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _map_#1_commands_sequence }
			}
			{
				\_map_keyval:nnn { #1 } { command } { none }
				\_map_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _map_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _map_#1_if_upper_index }
					%\use:c { _map_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _map_#1_if_upper_index }
					%\use:c{ _map_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ upper } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_upper_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { upper } { none }
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
		}
		{ addupper } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_upper_index } { #3 }
		}
		{ index } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { lower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { upper } { #3 }
			}
		}
		{ addindex } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}		
		}
		{ lower } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_lower_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { lower } { none }
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ addlower } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_lower_index } { #3 }
		}
		{ par } {
			\str_set:cn { _map_#1_par_size }{ #3 }
		}
		{ n } {
			\bool_if:cTF {_map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ rest } { \_map_keyval:nnn { #1 } { addlower } { | #3 } }
		{ der } {
			\_map_keyval:nnn { #1 } { addupper } { ( #3 ) }
		}
		{ to } {
			\_map_keyval:nnn { #1 } { addupper } { #3 }
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_map_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_map_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_map_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_map_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_map_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_map_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_map_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sharp } { \_map_keyval:nnn { #1 } { addupper } { \# } }
		{ pull } { \_map_keyval:nnn { #1 } { addupper } { * } }
		{ push }{ \_map_keyval:nnn { #1 } { addlower } { * } }
		{ inv } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ pre } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ shpull } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ squared } { \_map_keyval:nnn { #1 } { addupper } { 2 } }
		{ \big }{ \_map_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_map_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_map_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_map_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_map_keyval:nnn { #1 } { addupper } { * }}
		{ ** }{ \_map_keyval:nnn { #1 } { addupper } { ** }}
	}
	{
		% do nothing
	}
	{
		\_map_keyval:nnn { #1 }{ addindex } { #2 }
	}
}





\cs_new:Npn \_map_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _map_#1_commands_sequence }
	
	\bool_new:c { _map_#1_if_upper_index }
	\tl_new:c { _map_#1_upper_index }
	\tl_new:c { _map_#1_lower_index }
	
	\cs_new:cpn { _map_#1_keyval:nn } ##1##2
	{
		\_map_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _map_#1_indexkey:n } ##1
	{
		\_map_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _map_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _map_#1_indexkey:n }
			{ _map_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _map_#1_par_size }
	
	
	\cs_new_protected:cpn { _map_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_map_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _map_#1_commands_sequence }
			{
				\tl_set:Nx \_map_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_map_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_map_commands_tl_temp
	}
	
	\use:c { _map_#1_keys_set:n } {
		#2
	}
}

\str_new:N\_map_par_size_temp

\cs_new:Npn \_map_parse_symbol:nnn #1#2
{
	\group_begin:
		\use:c { _map_#1_keys_set:n } { #2 }		
		
		\use:c { _map_#1_command:n }%
		{
			\use:c { _map_#1_symbol: }
		}
	%\group_end:
		\tl_gset:Nv\_map_upper_index_temp { _map_#1_upper_index }
		\tl_gset:Nv\_map_lower_index_temp { _map_#1_lower_index }
		\str_gset_eq:Nc\_map_par_size_temp { _map_#1_par_size }
	\group_end:
	\exp_args:NV \_map_upper_index:n \_map_upper_index_temp
	\exp_args:NV \_map_lower_index:n \_map_lower_index_temp
}

\str_new:N \_map_cs_str_temp

%\cs_new:Npn\_map_newcomap:nnnnn#1#2#3#4#5
%{
%	\IfNoValueTF{ #4 }
%	{
%		\_map_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%		}
%	}
%	{
%		\_map_new_command:nn { #2 }{
%			#3,
%			symbol={ #4 },
%			#5
%		}
%	}
%	\DeclareDocumentCommand{#1}{omg}{
%		\group_begin:
%			\IfNoValueTF { ##1 }
%			{
%				\_map_parse_symbol:nnn { #2 } { } { ##2 }
%			}
%			{
%				\_map_parse_symbol:nnn { #2 } { ##1 } { ##2 }
%			}
%			\IfNoValueTF { ##3 }%
%			{%
%				%do nothing
%			}%
%			{%
%				\exp_args:Nx\_map_parentheses:nn { \str_use:c { _map_#2_par_size }} { ##3 }
%			}%
%		\group_end:		
%	}
%}
%
%\DeclareDocumentCommand\newcomap{mmo}{%
%	\IfNoValueTF{ #3 }
%	{
%		\exp_args:Nnx
%		\_map_newcomap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
%	}
%	{
%		\exp_args:Nnx\_map_newcomap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
%	}
%}
%
%\DeclareDocumentCommand\newmap{mmo}{%
%	\IfNoValueTF{ #3 }
%	{
%		\exp_args:Nnx\_map_newcomap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
%	}
%	{
%		\exp_args:Nnx\_map_newcomap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
%	}
%}



\cs_new:Npn\_map_newmap:nnnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_map_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_map_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_map_parse_symbol:nnn { #2 } { }
			}
			{
				\_map_parse_symbol:nnn { #2 } { ##1 }
			}
			\IfNoValueTF { ##2 }%
			{%
				%do nothing
			}%
			{%
				%\exp_args:Nv
				\exp_args:No\_map_parentheses:nn { \_map_par_size_temp } { ##2 }
			}%
		\group_end:		
	}
}



\DeclareDocumentCommand\newmap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcomap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}

\ExplSyntaxOff

\newmap\mf{f}
\newmap\mg{g}
\newmap\mh{h}
\newmap\mphi{\phi}
\newmap\mvarphi{\varphi}
\newmap\mpsi{\psi}
\newmap\mF{F}
\newmap\mG{G}
\newmap\mH{H}
\newmap\mPhi{\Phi}
\newmap\mPsi{\Psi}

\newmap\dif{d}[par=none]
\newmap\pdif{\partial}[par=none]
\newmap\ddif{\delta}[par=none]

\newcomap\face{d}[par=none]
\newcomap\pface{\partial}[par=none]
\newcomap\dface{\delta}[par=none]

==> _commands/maps/_maps_2.tex <==

%\DeclarePairedDelimiter{\@parentheses}{(}{)}

\ExplSyntaxOn



\bool_new:N\_if_first_map:
\bool_set_true:N\_if_first_map:

\tl_new:N\_map_seperator:
\tl_new:N\_map_coefficient_seperator:

\tl_set:Nn \_map_seperator: {,}
\tl_set:Nn \_map_coefficient_seperator: {;}
\tl_set:Nn \_map_dots: {\ldots}






\cs_new:Npn \_map_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_map_parentheses:w}{(}{)}

\cs_new:Npn \_map_parentheses_normal:n #1  {\_map_parentheses:w{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_big:n #1  {\_map_parentheses:w[\big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Big:n #1  {\_map_parentheses:w[\Big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_bigg:n #1  {\_map_parentheses:w[\bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Bigg:n #1  {\_map_parentheses:w[\Bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_auto:n #1  {\_map_parentheses:w*{\tup_process{#1}}}


\cs_new:Npn \_map_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_map_parentheses_normal:n { #2 }}
		{ big } { \_map_parentheses_big:n { #2 }}
		{ \big } { \_map_parentheses_big:n { #2 }}
		{ Big } { \_map_parentheses_Big:n { #2 }}
		{ \Big } { \_map_parentheses_Big:n { #2 }}
		{ bigg } { \_map_parentheses_bigg:n { #2 }}
		{ \bigg } { \_map_parentheses_bigg:n { #2 }}
		{ Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ auto } { \_map_parentheses_auto:n { #2 }}
		{ * } { \_map_parentheses_auto:n { #2 }}
		{ none } { \_map_no_parentheses:n { #2 }}
		{ } { \_map_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_map_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_map_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}

\cs_new:Npn \_map_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_map_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}



\tl_new:N \_map_commands_tl_temp


\cs_new:Npn \_map_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _map_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _map_#1_commands_sequence }
			}
			{
				\_map_keyval:nnn { #1 } { command } { none }
				\_map_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _map_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _map_#1_if_upper_index }
					%\use:c { _map_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _map_#1_if_upper_index }
					%\use:c{ _map_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ upper } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_upper_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { upper } { none }
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
		}
		{ addupper } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_upper_index } { #3 }
		}
		{ index } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { lower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { upper } { #3 }
			}
		}
		{ addindex } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}		
		}
		{ lower } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_lower_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { lower } { none }
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ addlower } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_lower_index } { #3 }
		}
		{ par } {
			\str_set:cn { _map_#1_par_size }{ #3 }
		}
		{ n } {
			\bool_if:cTF {_map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ rest } { \_map_keyval:nnn { #1 } { addlower } { | #3 } }
		{ der } {
			\_map_keyval:nnn { #1 } { addupper } { ( #3 ) }
		}
		{ to } {
			\_map_keyval:nnn { #1 } { addupper } { #3 }
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_map_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_map_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_map_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_map_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_map_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_map_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_map_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sharp } { \_map_keyval:nnn { #1 } { addupper } { \# } }
		{ pull } { \_map_keyval:nnn { #1 } { addupper } { * } }
		{ push }{ \_map_keyval:nnn { #1 } { addlower } { * } }
		{ shriek } { \_map_keyval:nnn { #1 } { addlower } { ! } }
		{ ! } { \_map_keyval:nnn { #1 } { addlower } { ! } }
		{ inv } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ pre } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ shpull } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ squared } { \_map_keyval:nnn { #1 } { addupper } { 2 } }
		{ \big }{ \_map_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_map_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_map_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_map_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_map_keyval:nnn { #1 } { addupper } { * }}
		{ ** }{ \_map_keyval:nnn { #1 } { addupper } { ** }}
	}
	{
		% do nothing
	}
	{
		\_map_keyval:nnn { #1 }{ addindex } { #2 }
	}
}





\cs_new:Npn \_map_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _map_#1_commands_sequence }
	
	\bool_new:c { _map_#1_if_upper_index }
	\tl_new:c { _map_#1_upper_index }
	\tl_new:c { _map_#1_lower_index }
	
	\cs_new:cpn { _map_#1_keyval:nn } ##1##2
	{
		\_map_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _map_#1_indexkey:n } ##1
	{
		\_map_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _map_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _map_#1_indexkey:n }
			{ _map_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _map_#1_par_size }
	
	
	\cs_new_protected:cpn { _map_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_map_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _map_#1_commands_sequence }
			{
				\tl_set:Nx \_map_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_map_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_map_commands_tl_temp
	}
	
	\use:c { _map_#1_keys_set:n } {
		#2
	}
}

\str_new:N\_map_par_size_temp

\cs_new:Npn \_map_parse_symbol:nnn #1#2
{
	\group_begin:
		\use:c { _map_#1_keys_set:n } { #2 }		
		
		\use:c { _map_#1_command:n }%
		{
			\use:c { _map_#1_symbol: }
		}
	%\group_end:
	\tl_gset:Nv\_map_upper_index_temp { _map_#1_upper_index }
	\tl_gset:Nv\_map_lower_index_temp { _map_#1_lower_index }
	\str_gset_eq:Nc\_map_par_size_temp { _map_#1_par_size }
	\group_end:
	\exp_args:NV \_map_upper_index:n \_map_upper_index_temp
	\exp_args:NV \_map_lower_index:n \_map_lower_index_temp
}

\str_new:N \_map_cs_str_temp




\cs_new:Npn\_map_newmap:nnnn#1#2#3#4#5
{
	\IfNoValueTF{ #4 }
	{
		\_map_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
		}
	}
	{
		\_map_new_command:nn { #2 }{
			#3,
			symbol={ #4 },
			#5
		}
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_map_parse_symbol:nnn { #2 } { }
			}
			{
				\_map_parse_symbol:nnn { #2 } { ##1 }
			}
			\IfNoValueTF { ##2 }%
			{%
				%do nothing
			}%
			{%
				%\exp_args:Nv
				\exp_args:No\_map_parentheses:nn { \_map_par_size_temp } { ##2 }
			}%
		\group_end:		
	}
}



\DeclareDocumentCommand\newmap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx
		\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper } { #2 } { }%
	}
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=upper} { #2 } { #3 }%
	}
}

\DeclareDocumentCommand\newcomap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower } { #2 } { }%
	}
	{
		\exp_args:Nnx\_map_newmap:nnnnn{#1}{ \cs_to_str:N#1 }{ indextype=lower} { #2 } { #3 }%
	}
}



\newmap\mf{f}
\newmap\mg{g}
\newmap\mh{h}
\newmap\mphi{\phi}
\newmap\mvarphi{\varphi}
\newmap\mpsi{\psi}
\newmap\mF{F}
\newmap\mG{G}
\newmap\mH{H}
\newmap\mPhi{\Phi}
\newmap\mPsi{\Psi}

\newmap\dif{d}[par=none]
\newmap\pdif{\partial}[par=none]
\newmap\ddif{\delta}[par=none]

\newcomap\face{d}[par=none]
\newcomap\pface{\partial}[par=none]
\newcomap\dface{\delta}[par=none]

\newmap\mapproto{}

\DeclareDocumentCommand\map{mog}
{
	\group_begin:
		\IfNoValueTF { #2 }
		{
			\_map_parse_symbol:nnn { mapproto } { symbol={#1} }
		}
		{
			\_map_parse_symbol:nnn { mapproto } { symbol={#1}, #2 }
		}
		\IfNoValueTF { #3 }%
		{%
			%do nothing
		}%
		{%
			%\exp_args:Nv
			\exp_args:No\_map_parentheses:nn { \_map_par_size_temp } { #3 }
		}%
	\group_end:		
}

\ExplSyntaxOff

==> _commands/maps/_maps_3.tex <==

%\DeclarePairedDelimiter{\@parentheses}{(}{)}

\ExplSyntaxOn



\bool_new:N\_if_first_map:
\bool_set_true:N\_if_first_map:

\tl_new:N\_map_seperator:
\tl_new:N\_map_coefficient_seperator:

\tl_set:Nn \_map_seperator: {,}
\tl_set:Nn \_map_coefficient_seperator: {;}
\tl_set:Nn \_map_dots: {\ldots}






\cs_new:Npn \_map_no_parentheses:n #1
{%
	% command for the X part of notations like H^n X
	% without parentheses; at the moment, simply outputs
	% X withut further ado, but could contain spaces in the future
	#1%
}


\DeclarePairedDelimiter{\_map_parentheses:w}{(}{)}

\cs_new:Npn \_map_parentheses_normal:n #1  {\_map_parentheses:w{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_big:n #1  {\_map_parentheses:w[\big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Big:n #1  {\_map_parentheses:w[\Big]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_bigg:n #1  {\_map_parentheses:w[\bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_Bigg:n #1  {\_map_parentheses:w[\Bigg]{\tup_process{#1}}}

\cs_new:Npn \_map_parentheses_auto:n #1  {\_map_parentheses:w*{\tup_process{#1}}}


\cs_new:Npn \_map_parentheses:nn #1#2
{
	\str_case:nnTF { #1 }
	{
		{ normal } { \_map_parentheses_normal:n { #2 }}
		{ big } { \_map_parentheses_big:n { #2 }}
		{ \big } { \_map_parentheses_big:n { #2 }}
		{ Big } { \_map_parentheses_Big:n { #2 }}
		{ \Big } { \_map_parentheses_Big:n { #2 }}
		{ bigg } { \_map_parentheses_bigg:n { #2 }}
		{ \bigg } { \_map_parentheses_bigg:n { #2 }}
		{ Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ \Bigg } { \_map_parentheses_Bigg:n { #2 }}
		{ auto } { \_map_parentheses_auto:n { #2 }}
		{ * } { \_map_parentheses_auto:n { #2 }}
		{ none } { \_map_no_parentheses:n { #2 }}
		{ } { \_map_parentheses_normal:n { #2 } }
	}
	{
		%do nothing
	}
	{
		%do nothing
	}
}



\cs_new:Npn \_map_lower_index:n #1{
	%\tl_if_blank:nTF { #1 }
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
			% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sb{
				%\_map_bullet_if_bar:n { #1 }
				%\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}

\cs_new:Npn \_map_upper_index:n #1{
	\bool_if:nTF
	{
		\tl_if_blank_p:n { #1 }
		||
		\str_if_eq_p:nn { #1 } { . }
	}
	{
		% do nothing
	}
	{
		\IfNoValueTF { #1 }
		{
			% do nothing
		}
		{
			\sp{
				%\_map_bullet_if_bar:n { #1 }
				%\exp_args:Nnf\tl_map_inline:nn{ #1 }{ \_map_bullet_if_bar:n { ##1 } }
				#1
			}
		}
	}
}



\tl_new:N \_map_commands_tl_temp


\cs_new:Npn \_map_keyval:nnn#1#2#3{
	\str_case:nnTF { #2 }
	{
		{ symbol } { \tl_set:cn { _map_#1_symbol: } { #3 } }
		{ command } {
			\str_if_eq:nnTF { #3 }{ none }
			{
				\seq_clear:c { _map_#1_commands_sequence }
			}
			{
				\_map_keyval:nnn { #1 } { command } { none }
				\_map_keyval:nnn { #1 } { addcommand } { #3 }
			}
		}
		{ addcommand } {
			\seq_put_right:cn { _map_#1_commands_sequence } { #3 }
		}
		{ indextype } {
			\str_case:nnTF { #3 }
			{
				{ upper }
				{
					\bool_set_true:c { _map_#1_if_upper_index }
					%\use:c { _map_#1_index_go_auto: }
				}
				{ lower }
				{
					\bool_set_false:c { _map_#1_if_upper_index }
					%\use:c{ _map_#1_index_go_auto: }
				}
			}
			{
				% do nohting
			}
			{
				% do nothing
			}
		}
		{ upper } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_upper_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { upper } { none }
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
		}
		{ addupper } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_upper_index } { #3 }
		}
		{ index } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { lower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { upper } { #3 }
			}
		}
		{ addindex } {
			\bool_if:cTF { _map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}		
		}
		{ lower } {
			%\use:c { _map_#1_index_go_auto: }
			\str_if_eq:nnTF { #3 }{ none }
			{
				\tl_set:cn { _map_#1_lower_index } { } %empty
			}
			{
				\_map_keyval:nnn { #1 } { lower } { none }
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ addlower } {
			%\use:c { _map_#1_index_go_auto: }
			\tl_put_right:cn { _map_#1_lower_index } { #3 }
		}
		{ par } {
			\str_set:cn { _map_#1_par_size }{ #3 }
		}
		{ n } {
			\bool_if:cTF {_map_#1_if_upper_index } {
				\_map_keyval:nnn { #1 } { addupper } { #3 }
			}
			{
				\_map_keyval:nnn { #1 } { addlower } { #3 }
			}
		}
		{ rest } { \_map_keyval:nnn { #1 } { addlower } { | #3 } }
		{ der } {
			\_map_keyval:nnn { #1 } { addupper } { ( #3 ) }
		}
		{ to } {
			\_map_keyval:nnn { #1 } { addupper } { #3 }
		}
	}
	{
		% if true
	}
	{
		% if false
	}
}

\cs_new:Npn \_map_indexkey:nn#1#2
{
	\str_case:nnTF { #2 }
	{
		{ cech }{ \_map_keyval:nnn { #1 }{ addcommand } { \check } }
		{ hyper }{ \_map_keyval:nnn { #1 }{ addcommand } { \mathbb } }
		{ tilde }{ \_map_keyval:nnn { #1 }{ addcommand } { \widetilde } }
		{ bar } { \_map_keyval:nnn { #1 }{ addcommand } { \widebar } }
		{ bold } { \_map_keyval:nnn { #1 }{ addcommand } { \mathbf } }
		{ upright } { \_map_keyval:nnn { #1 }{ addcommand } { \mathup } }
		{ sharp } { \_map_keyval:nnn { #1 } { addupper } { \# } }
		{ pull } { \_map_keyval:nnn { #1 } { addupper } { * } }
		{ push }{ \_map_keyval:nnn { #1 } { addlower } { * } }
		{ shriek } { \_map_keyval:nnn { #1 } { addlower } { ! } }
		{ ! } { \_map_keyval:nnn { #1 } { addlower } { ! } }
		{ inv } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ pre } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ shpull } { \_map_keyval:nnn { #1 } { addupper } { -1 } }
		{ squared } { \_map_keyval:nnn { #1 } { addupper } { 2 } }
		{ \big }{ \_map_keyval:nnn { #1 }{ par } { big } }
		{ \Big }{ \_map_keyval:nnn { #1 }{ par } { Big } }
		{ \bigg }{ \_map_keyval:nnn { #1 }{ par } { bigg } }
		{ \Bigg }{ \_map_keyval:nnn { #1 }{ par } { Bigg } }
		{ * } { \_map_keyval:nnn { #1 } { addupper } { * }}
		{ ** }{ \_map_keyval:nnn { #1 } { addupper } { ** }}
	}
	{
		% do nothing
	}
	{
		\_map_keyval:nnn { #1 }{ addindex } { #2 }
	}
}





\cs_new:Npn \_map_new_command:nn#1#2{
	% #1 = name of command, without backslash
	% #2 = keyval setup
	\seq_new:c { _map_#1_commands_sequence }
	
	\bool_new:c { _map_#1_if_upper_index }
	\tl_new:c { _map_#1_upper_index }
	\tl_new:c { _map_#1_lower_index }
	
	\cs_new:cpn { _map_#1_keyval:nn } ##1##2
	{
		\_map_keyval:nnn { #1 } { ##1 } { ##2 }
	}
	\cs_new:cpn { _map_#1_indexkey:n } ##1
	{
		\_map_indexkey:nn { #1 } { ##1 }
	}
	\cs_new:cpn { _map_#1_keys_set:n } ##1
	{
		\exp_args:Ncco
			\keyval_parse:NNn
			{ _map_#1_indexkey:n }
			{ _map_#1_keyval:nn }
			{  ##1 }
	}
	\str_new:c { _map_#1_par_size }
	
	
	\cs_new_protected:cpn { _map_#1_command:n } ##1
	{
		\group_begin:
			\tl_set:Nn \_map_commands_tl_temp { ##1 }
			\seq_map_inline:cn { _map_#1_commands_sequence }
			{
				\tl_set:Nx \_map_commands_tl_temp
				{
					\exp_not:n { ####1 } { \exp_not:V \_map_commands_tl_temp }
				}
			}
		\exp_args:NV \group_end: \_map_commands_tl_temp
	}
	
	\use:c { _map_#1_keys_set:n } {
		#2
	}
}

\newcommand\mapsetup[2]{
	%\exp_args:Nx
	\use:c { _map_\cs_to_str:N#1_keys_set:n } {
		#2
	}
}

\str_new:N\_map_par_size_temp

\cs_new:Npn \_map_parse_symbol:nnn #1#2
{
	\group_begin:
		\use:c { _map_#1_keys_set:n } { #2 }		
		
		\use:c { _map_#1_command:n }%
		{
			\use:c { _map_#1_symbol: }
		}
	%\group_end:
	\tl_gset:Nv\_map_upper_index_temp { _map_#1_upper_index }
	\tl_gset:Nv\_map_lower_index_temp { _map_#1_lower_index }
	\str_gset_eq:Nc\_map_par_size_temp { _map_#1_par_size }
	\group_end:
	\exp_args:NV \_map_upper_index:n \_map_upper_index_temp
	\exp_args:NV \_map_lower_index:n \_map_lower_index_temp
}

\str_new:N \_map_cs_str_temp




\cs_new:Npn\_map_newmap:nnnn#1#2#3#4
{
	% #1 = command name, e.ge \co
	% #2 = name without backshash, e.g. co
	% #3 = cohomology symbol
	% #4 = other options
	\_map_new_command:nn { #2 }{
		symbol = { #3 },
		#4
	}
	\DeclareDocumentCommand{#1}{og}{
		\group_begin:
			\IfNoValueTF { ##1 }
			{
				\_map_parse_symbol:nnn { #2 } { }
			}
			{
				\_map_parse_symbol:nnn { #2 } { ##1 }
			}
			\IfNoValueTF { ##2 }%
			{%
				%do nothing
			}%
			{%
				%\exp_args:Nv
				\exp_args:No\_map_parentheses:nn { \_map_par_size_temp } { ##2 }
			}%
		\group_end:		
	}
}



\DeclareDocumentCommand\newmap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_map_newmap:nnnn { #1 } { \cs_to_str:N#1 }{ #2 }{ indextype=upper }%
	}
	{
		%\exp_args:Nnx
		\_map_newmap:nnnn { #1 } { \cs_to_str:N#1 }{ #2 }{ indextype=upper, #3 }%
	}
}

\DeclareDocumentCommand\newcomap{mmo}{%
	\IfNoValueTF{ #3 }
	{
		%\exp_args:Nnx
		\_map_newmap:nnnn { #1 } { \cs_to_str:N#1 }{ #2 }{ indextype=lower }%
	}
	{
		%\exp_args:Nnx
		\_map_newmap:nnnn { #1 } { \cs_to_str:N#1 }{ #2 }{ indextype=lower, #3 }%
	}
}



\newmap\mf{f}
\newmap\mg{g}
\newmap\mh{h}
\newmap\mphi{\phi}
\newmap\mvarphi{\varphi}
\newmap\mpsi{\psi}
\newmap\mF{F}
\newmap\mG{G}
\newmap\mH{H}
\newmap\mPhi{\Phi}
\newmap\mPsi{\Psi}

\newmap\dif{d}[par=none]
\newmap\pdif{\partial}[par=none]
\newmap\ddif{\delta}[par=none]

\newcomap\face{d}[par=none]
\newcomap\pface{\partial}[par=none]
\newcomap\dface{\delta}[par=none]

\newmap\mapproto{}

\DeclareDocumentCommand\map{mog}
{
	\group_begin:
		\IfNoValueTF { #2 }
		{
			\_map_parse_symbol:nnn { mapproto } { symbol={#1} }
		}
		{
			\_map_parse_symbol:nnn { mapproto } { symbol={#1}, #2 }
		}
		\IfNoValueTF { #3 }%
		{%
			%do nothing
		}%
		{%
			%\exp_args:Nv
			\exp_args:No\_map_parentheses:nn { \_map_par_size_temp } { #3 }
		}%
	\group_end:		
}

\ExplSyntaxOff

==> _commands/maps/maps_10.tex <==
\newmapclass{map}[
	parent=var,
	output=var,
	singlekeys={
		{invim} { upper = -1, nopar, output=sheaf },
		{dirim} { lower={\ast}, nopar, output=sheaf },
		{pull} { upper={\ast} },
		{push}{ lower = {\ast} },
		{shpull}{ upper={\ast}, nopar, output=sheaf },
		{shpush}{ lower={\ast}, nopar, output=sheaf },
		{shriekpush} { lower=!, nopar, output=sheaf },
		{shriekpull} { upper=!, nopar, output=sheaf },
		{!push} { lower=!, nopar, output=sheaf },
		{!pull} { upper=!, nopar, output=sheaf },
		{sharp} { upper=\# },
		{inv} { upper=-1 },
		{pre} { upper=-1 },
%		{shpull} { g=-1 },
		{squared} { upper=2 },
	},
	keyvals={
		{der} { upper = {(\keyvalue)} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{res} { return, symbolputright=\vert, lower={\keyvalue} },
		{bigres} { return, symbolputright=\big\vert, lower={\keyvalue} },
		{Bigres} { return, symbolputright=\Big\vert, lower={\keyvalue} },
		{biggres} { return, symbolputright=\bigg\vert, lower={\keyvalue} },
		{Biggres} { return, symbolputright=\Bigg\vert, lower={\keyvalue} },
		% Derived functors:
		{Lder} { symbolputleft=L^{\keyvalue}},
		{Rder} { symbolputleft=R^{\keyvalue}},
	},
]

\newmap{\mf}{f}
\newmap{\mg}{g}{}
\newmap{\mh}{h}{}
\newmap{\mphi}{\phi}
\newmap{\mvarphi}{\varphi}
\newmap{\mpsi}{\psi}
\newmap{\mF}{F}
\newmap{\mG}{G}
\newmap{\mH}{H}
\newmap{\mPhi}{\Phi}
\newmap{\mPsi}{\Psi}

\newmap{\dif}{d}[nopar]
\newmap{\pdif}{\partial}[nopar]
\newmap{\ddif}{\delta}[nopar]

\newmap{\face}{d}[gradingpos=lower,nopar]
\newmap{\pface}{\partial}[gradingpos=lower,nopar]
\newmap{\dface}{\delta}[gradingpos=lower,par=nopar]


%\newcommand\idproto{\mathupright{id}}

\newmap{\id}{\mathup{id}}
\newmap{\bigid}{\mathup{Id}}



\newmap{\Span}{\operatorname{span}}
\newmap{\Ker}{\operatorname{Ker}}
\newmap{\Image}{\operatorname{Im}}
\newmap{\Coker}{\operatorname{Coker}}
\newmap{\Realpart}{\operatorname{Re}}

%\renewcommand*\Im{\operatorname{Im}}
%\renewcommand*\Re{\operatorname{Re}}
\let\Im=\Image
\let\Re=\Realpart

\let\ker=\Ker
\let\coker=\Coker
\let\im=\Im
\let\Id=\id

%\newmap{\End}{\operatorname{End}} % moved to homology
%\newmap{\Hom}{\operatorname{Hom}}
\newmap{\GL}{\operatorname{GL}}
\newmap{\SL}{\operatorname{SL}}
\newmap{\SU}{\operatorname{SU}}
\newmap{\SO}{\operatorname{SO}}
\newmap{\Sym}{\operatorname{Sym}}
\newmap{\Aut}{\operatorname{Aut}}
%\newmap{\Mor}{\operatorname{Mor}
%\newmap{\Fun{Fun}
%\newmap{\Ext{Ext}
%\newmap{\Tor{Tor}

\newmapclass{algop}[
	parent=map,
	output=alg,
	nopar,
]

\newalgop{\catend}{\int}

\newalgop{\catcoend}{\int}[gradingpos=lower]

\newalgop\Sum{\sum}[
	keyvals={
		{from}{lower={\keyvalue}},
		{to}{upper={\keyvalue}},
	},
]

\newalgop\Int{\int}[parent=Sum]

==> _commands/maps/maps_11.tex <==
\newmapclass{map}[
	parent=var,
	output=var,
%	singlekeys={
%		{invim} { upper = -1, nopar, output=sheaf },
%		{dirim} { lower={\ast}, nopar, output=sheaf },
%		{pull} { upper={\ast} },
%		{push}{ lower = {\ast} },
%		{shpull}{ upper={\ast}, nopar, output=sheaf },
%		{shpush}{ lower={\ast}, nopar, output=sheaf },
%		{shriekpush} { lower=!, nopar, output=sheaf },
%		{shriekpull} { upper=!, nopar, output=sheaf },
%		{!push} { lower=!, nopar, output=sheaf },
%		{!pull} { upper=!, nopar, output=sheaf },
%		{sharp} { upper=\# },
%		{inv} { upper=-1 },
%		{pre} { upper=-1 },
%%		{shpull} { g=-1 },
%		{squared} { upper=2 },
%	},
%	keyvals={
%		{der} { upper = {(\keyvalue)} },
%		{res} { return, symbolputright=\vert, lower={\keyvalue} },
%		{res} { return, symbolputright=\vert, lower={\keyvalue} },
%		{bigres} { return, symbolputright=\big\vert, lower={\keyvalue} },
%		{Bigres} { return, symbolputright=\Big\vert, lower={\keyvalue} },
%		{biggres} { return, symbolputright=\bigg\vert, lower={\keyvalue} },
%		{Biggres} { return, symbolputright=\Bigg\vert, lower={\keyvalue} },
%		% Derived functors:
%		{Lder} { symbolputleft=L^{\keyvalue}},
%		{Rder} { symbolputleft=R^{\keyvalue}},
%	},
]

\newmap{\mf}{f}
\newmap{\mg}{g}{}
\newmap{\mh}{h}{}
\newmap{\mphi}{\phi}
\newmap{\mvarphi}{\varphi}
\newmap{\mpsi}{\psi}
\newmap{\mF}{F}
\newmap{\mG}{G}
\newmap{\mH}{H}
\newmap{\mPhi}{\Phi}
\newmap{\mPsi}{\Psi}

\newmap{\dif}{d}[nopar]
\newmap{\pdif}{\partial}[nopar]
\newmap{\ddif}{\delta}[nopar]

%\newmap{\face}{d}[gradingpos=lower,nopar]
%\newmap{\pface}{\partial}[gradingpos=lower,nopar]
%\newmap{\dface}{\delta}[gradingpos=lower,nopar]


%\newcommand\idproto{\mathupright{id}}

\newmap{\id}{\mathup{id}}
\newmap{\bigid}{\mathup{Id}}



\newmap{\Span}{\operatorname{span}}
\newmap{\Ker}{\operatorname{Ker}}
\newmap{\Image}{\operatorname{Im}}
\newmap{\Coker}{\operatorname{Coker}}
\newmap{\Realpart}{\operatorname{Re}}

%\renewcommand*\Im{\operatorname{Im}}
%\renewcommand*\Re{\operatorname{Re}}
\let\Im=\Image
\let\Re=\Realpart

\let\ker=\Ker
\let\coker=\Coker
\let\im=\Im
\let\Id=\id

%\newmap{\End}{\operatorname{End}} % moved to homology
%\newmap{\Hom}{\operatorname{Hom}}
\newmap{\GL}{\operatorname{GL}}
\newmap{\SL}{\operatorname{SL}}
\newmap{\SU}{\operatorname{SU}}
\newmap{\SO}{\operatorname{SO}}
\newmap{\Sym}{\operatorname{Sym}}
\newmap{\Aut}{\operatorname{Aut}}
%\newmap{\Mor}{\operatorname{Mor}
%\newmap{\Fun{Fun}
%\newmap{\Ext{Ext}
%\newmap{\Tor{Tor}

\newmapclass{algop}[
	parent=map,
	output=alg,
	nopar,
]

\newmapclass{algoplaurent}[
	parent=algop,
	par,
	leftpar=(,rightpar=),
	keyvals={
		{arg}{
			argwithoutkeyval={\!\noexpand\automathdelimsize(},
			argwithkeyval={\keyvalue},
			argwithoutkeyval={\noexpand\automathdelimsize)\!},
		},
	},
]

\newmapclass{algopfreealg}[
	parent=algop,
	par,
	leftpar=\langle,rightpar=\rangle,
]

\newmapclass{algoppowerseries}[
	parent=algop,
	par,
	leftpar=\llbracket,rightpar=\rrbracket,
]

\newalgop{\catend}{\int}

\newalgop{\catcoend}{\int}[gradingpos=lower]

\newalgop\Sum{\sum}[
	keyvals={
		{from}{lower={\keyvalue}},
		{to}{upper={\keyvalue}},
	},
]

\newalgop\Int{\int}[parent=Sum]

\newmapclass{calculusdifferential}[
	parent=map,
	argkeyvals={
		{default}{standardsep={d\!\keyvalue}},
	},
	argsep={\,},
	argdots={\cdots},
	ifpar=false,
]

\newcalculusdifferential\intD{}[iffirstarg=false]

\newcalculusdifferential\wedgeD{}[argsep={\wedge}]

==> _commands/operators/operators_1.tex <==
\newvariableclass{automathoperator}[
	parent=var,
	singlekeys={
		{der}{upper=L},
		{bbder}{upper={\noexpand\mathbb{L}}},
		{bder}{upper={\noexpand\mathbf{L}}},
	},
]

\newautomathoperator\tens{\otimes}

\newautomathoperator\fibre{\times}
\newautomathoperator\bigfibre{\amalg}

==> _commands/page/_page_1.tex <==
\newcommand*\mybreak{%for nice breaks in the middle of the text
	\fancybreak{\mbox{}\\*$*\quad *\quad *$\\*\mbox{}}%
}

\NewDocumentCommand\exc{sm}{ % for answers of exercises with the exercise number in the margin
	\IfBooleanTF{#1}{%
		%do nothing
	}{%
	\fancybreak{}%
}\noindent\mbox{}\llap{(#2)\quad}\ignorespaces}

==> _commands/slots/_slots_1.tex <==
\newcommand\slot{\mathord{-}} % for expresseions like \Hom(A,\slot);
								% can be changed to \:\cdot\:

\newcommand\slotifempty[1]{
	\ifblank{#1}{\slot}{#1}
}
\newcommand\bulletifempty[1]{
	\ifblank{#1}{\smallbullet}{#1}
}

==> _commands/smalloperators/_smalloperators_1.tex <==
\newcommand\@sotimes[1]{\vcenter{\hbox{$#1\otimes$}}}

\newcommand{\sotimes}{\mathbin{\mathchoice
  {\@sotimes\scriptstyle}
  {\@sotimes\scriptstyle}
  {\@sotimes\scriptscriptstyle}
  {\@sotimes\scriptscriptstyle}
}}

\newcommand\@soplus[1]{\vcenter{\hbox{$#1\oplus$}}}

\newcommand{\soplus}{\mathbin{\mathchoice
  {\@soplus\scriptstyle}
  {\@soplus\scriptstyle}
  {\@soplus\scriptscriptstyle}
  {\@soplus\scriptscriptstyle}
}}

\newcommand\@stimes[1]{\vcenter{\hbox{$#1\times$}}}

\newcommand{\stimes}{\mathbin{\mathchoice
  {\@stimes\scriptstyle}
  {\@stimes\scriptstyle}
  {\@stimes\scriptscriptstyle}
  {\@stimes\scriptscriptstyle}
}}

\newcommand\@scirc[1]{\vcenter{\hbox{$#1\circ$}}}

\newcommand{\scirc}{\mathbin{\mathchoice
  {\@scirc\scriptstyle}
  {\@scirc\scriptstyle}
  {\@scirc\scriptscriptstyle}
  {\@scirc\scriptscriptstyle}
}}

\begin{comment}

\newcommand\sotimes{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\otimes$}}}}
\newcommand\soplus{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\oplus$}}}}
\newcommand\stimes{\mathbin{\raisebox{0.14ex}{\scalebox{.7}{$\times$}}}}

\end{comment}

==> _commands/tuples/_tuples_1.tex <==
% The below code defines the macro \newflextuple for defining
% what I call "flextuples", tuple commands that automate
% the typesetting of tuple-like environments. They
% have customizable left and right delimiters, separators
% (i.e. comma for a standard tuple), and dot commands
% (a command that is inserted at all occurrences of "...")
% The flextuples are comma-separated on the syntax level

\ExplSyntaxOn

\clist_new:N \flexsequence_input:
\bool_new:N\flexsequence_if_first:
\cs_new:Npn \flexsequence #1#2#3
{
	% #1 = seperator
	% #2 = "..." replacement
	% #3 = contents
    \group_begin:
	\clist_set:Nn \flexsequence_input: {#3}
	\bool_set_true:N \flexsequence_if_first:
	\clist_map_variable:NNn \flexsequence_input: \flexsequence_var:
	{
		\bool_if:NTF \flexsequence_if_first:
		{
			% do nothing
			\bool_set_false:N\flexsequence_if_first:
		}
		{
			#1
		}
		\str_if_eq:onTF {\flexsequence_var:} {...}
		{
			#2
		}
		{
			\flexsequence_var:
		}
	}
	\group_end:
}

\cs_new:Npn \newflexsequence #1#2#3#4
{
	\newcommand#1[1]{\flexsequence{#2}{#3}{##1}}
}

\cs_new:Npn \newflextuple #1#2#3#4#5
{
	% #1 = name
	% #2 = left delimiter
	% #3 = right delimiter
	% #4 = seperator
	% #5 = "..." replacement
	\cs_new:cpn {\cs_to_str:N #1_process } ##1
	{
		\flexsequence{#4}{#5}{##1}
	}
	\DeclarePairedDelimiterX#1[1]{#2}{#3}{
		\use:c {\cs_to_str:N #1_process } {##1}
	}
}

\ExplSyntaxOff


\newcommand\midsequence[2]{\flexsequence{#1}{\cdots}{#2}}


\newflextuple\tup{(}{)}{,}{\ldots}

==> _commands/tuples/_tuples_2.tex <==
\newtupleclass{tuple}[parent=var,output=var]


\newtuple\tup{(}{,}{)}{\ldots}
\newtuple\pcoor{[}{\mathpunct{:}}{]}{\cdots}

==> _commands/widebar/_widebar_1.tex <==
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}

%\makeatletter
%\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%\newcommand*\widebar[1]{%
%  \begingroup
%  \def\mathaccent##1##2{%
%    \rel@kern{0.8}%
%    \overline{\rel@kern{-0.8}\macc@nucleus\rel@kern{0.2}}%
%    \rel@kern{-0.2}%
%  }%
%  \macc@depth\@ne
%  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
%  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
%  \macc@set@skewchar\relax
%  \let\mathaccentV\macc@nested@a
%  \macc@nested@a\relax111{#1}%
%  \endgroup
%}

==> _commands/wraptext/_wraptext_1.tex <==
\def\putright#1#2{\vskip\parskip
   \hbox to\hsize{\hss
      \vbox to0pt{\kern#1\baselineskip\kern-.8\baselineskip \hbox{#2}\vss}}
   \nobreak\vskip-\parskip\vskip-\baselineskip
} % for wrapping text around figures

==> _preamble/beamertheorems/_beamertheorems_11.tex <==
%\newtheorem{theorem}{Theorem}

\newtheorem{proposition}{Proposition}

==> _preamble/boldmath/_boldmath_1.tex <==
\g@addto@macro\bfseries{\boldmath} %make math in bold text automatically bold

%\g@addto@macro\bfseries{\boldmath} %make math in bold text automatically bold

==> _preamble/cleveref/da/_cleveref_da_1.tex <==
\crefname{para}{}{}
\crefname{theorem}{Sætning}{Sætningerne}
\crefname{definition}{Definition}{Definitionerne}
\crefname{example}{Eksempel}{Eksempler}
\crefname{corollary}{Korollar}{Korollarerne}
\crefname{proposition}{Proposition}{Propositionerne}
\crefname{lemma}{Lemma}{Lemmaerne}
\crefname{remark}{Bemærkning}{Bemærkningerne}
\crefname{claim}{Påstand}{Påstandene}
\crefname{exercise}{Opgave}{Opgaverne}
\crefname{textexercise}{Opgave}{Opgaverne}

\crefname{section}{afsnit}{afsnittene}
\crefname{equation}{ligning}{ligningerne}
\crefname{figure}{figur}{figurerne}
\crefname{table}{tabel}{tabellerne}
\crefname{page}{side}{siderne}
\crefname{part}{del}{delene}
\crefname{chapter}{kapitel}{kapitlerne}
\crefname{section}{afsnit}{afsnittene}
\crefname{appendix}{appendiks}{appendicer}
\crefname{enumi}{punkt}{punkterne}
\crefname{footnote}{fodnote}{fodnoterne}
\crefname{line}{linje}{linjerne}

==> _preamble/index/_index_1.tex <==
\makeindex


==> _preamble/memoir/_memoir_1.tex <==
%Setup of memoir:
\pagestyle{plain} %change to heading for running headings
\nouppercaseheads %running heads should not be capitalized
\captionnamefont{\small} %captions with small font
\captiontitlefont{\small}
\makeevenhead{headings}{\thepage}{}{\itshape\leftmark} %make headings italic instead of slanted
\makeoddhead{headings}{\itshape\rightmark}{}{\thepage}

\raggedbottomsectiontrue%less harse than \raggedbottom
%\allowdisplaybreaks %long equations may break

==> _preamble/ntheorem/_ntheorem_1.tex <==
%Theorem environments:
\usepackage[thmmarks,amsmath]{ntheorem}

% ntheorem configuration:

\input{_preamble/ntheorem/ntheorem_config/_ntheorem_config_1}



\ifdanish
	\input{_preamble/ntheorem/da/_ntheorem_da_1.tex}
\else
	\input{_preamble/ntheorem/en/_ntheorem_en_1.tex}
\fi

==> _preamble/siunitx/_siunitx_1.tex <==
\usepackage{siunitx}

%Setup of siunitx
\sisetup{
	exponent-product=\cdot,	% uses \cdot (·) as multiplication sign
							% instead \times (×)
	group-separator={\,}, 	% adds spaces after each three digits
	output-decimal-marker={.},
							% decimal marker set to point
	per-mode=symbol, 		% for e.g. m/s instead of \frac{m}{s}
}

==> descent/descent_112.tex <==
\begingroup

\chapter{Classical descent theory}


Suppose that \( \mf \colon \setX \to \setY \)~is an fpqc morphism of schemes. Then descent theory tells us that we
recover quasi-coherent sheaves on~\( \setY \) by gluing quasi-coherent sheaves on~\( \setX \). Concretely, consider the
\textdef{descent groupoid}~\( \ssetX{1} \rightrightarrows \ssetX{0} \)
given by~\( \ssetX{0} = \setX \) and~\(
	\ssetX{1} = \setX \fibre[\setY] \setX
\)
(both maps in the fibre product being~\( \mf \)),
and consider its classifying space, the internal Kan complex
in schemes given by
\[
	\ssetX{n}
	=
	\underbrace{
		\ssetX{1}
		\fibre[\ssetX{0}]
		\ssetX{1}
		\fibre[\ssetX{0}]
		\cdots
		\fibre[\ssetX{0}]
		\ssetX{1}
	}_{\text{\( n \)~factors}}
	=
	\underbrace{
		\setX
		\fibre[\setY]
		\setX
		\fibre[\setY]
		\cdots
		\fibre[\setY]
		\setX
	}_{\text{\( n + 1 \)~factors}}
\]
with the usual simplicial structure, the face maps~\(
	\face[d=i]\colon\ssetX{n}\to\ssetX{n-1}
\)
applying~\( \mf \) at the \( i \)th~step,
and the degeneracy maps~\( \degen[d=i]\colon\ssetX{n}\to\ssetX{n+1} \)
inserting the diagonal map at the \( i \)th~step.
Then the category~\( \catqcoh{\setY} \)~is equivalent
to the category of “descent data” on the
groupoid~\( \ssetX{*} \), defined in the following manner:

Let~\( \ssetX{1} \rightrightarrows \ssetX{0} \)
be any internal groupoid in the category of schemes,
and denote by~\( \ssetX{*} \)
its classifying space, the internal Kan complex
in schemes given by~\(
	\ssetX{n}
	=
	\ssetX{1}
	\fibre[\ssetX{0}]
	\cdots
	\fibre[\ssetX{0}]
	\ssetX{1}
\).
The category~\( \catdesc{\ssetX{*}} \) of \textdef{descent data} on~\( \ssetX{*} \)
has objects the pairs~\( \tup{\algM,\mtheta} \),
where \( \algM \in \catqcoh{\ssetX{0}} \),
and \(
	\mtheta \colon \face[d=1,shpull]{\algM}\to\face[d=0,shpull]{\algM}
\)
a map satisfying
the cocycle and unit conditions
\[
	\face[d=0,shpull]{\mtheta}
	\circ
	\face[d=2,shpull]{\mtheta}
	=
	\face[d=1,shpull]{\mtheta}
	\qquad\text{and}\qquad
	\degen[d=0,shpull]{\mtheta} = \id
.\]
A morphism~\( \malpha\colon\tup{\algM,\mtheta}\to\tup{\algN,\meta} \)
is a morphism~\( \malpha \colon \algM \to \algN \)
in~\( \catqcoh{\ssetX{0}} \) such that~\(
	\meta\circ\face[d=1,shpull]{\malpha} = \face[d=0,shpull]{\malpha}\circ\mtheta
\).

%the category~\( \catqcoh{\setY} \)
%is equivalent to the category consisting of
%pairs~\( \tup{\algM,\mtheta} \) where
%\( \algM \in \catqcoh{\setX} \) 

\begin{proposition}\label{res:cocycle_iff_degen=0}
	Assuming the cocycle condition,
	the assumption~\( \degen[d=0,shpull]{\mtheta}=\id \)
	is equivalent to~\( \mtheta \) being an isomorphism.
\end{proposition}

\begin{proof}
	If \( \mtheta \)~is an isomorphism,
	we may apply \(
		\degen[d=0,shpull] \degen[d=0,shpull]
		=
		\degen[d=0,shpull] \degen[d=1,shpull]
	\)
	to both sides of the cocycle condition
	and get~\(
		\degen[d=0,shpull]{ \mtheta }
		\circ
		\degen[d=0,shpull]{ \mtheta }
		=
		\degen[d=0,shpull]{ \mtheta }
	\).
	Now \( \degen[d=0,shpull]{ \mtheta } \)~is the image of an isomorphism and hence an isomorphism, so we obtain~\(
		\degen[d=0,shpull]{ \mtheta } = \id
	\).
	Conversely, if~\( \degen[d=0,shpull]{\mtheta} = \id \),
	then we use the groupoid conditions
	\[
		\face[d=1]
		( \miota\times\id )
		\diagonalmap
		=
		\degen[d=0]
		\face[d=1]
		\qquad\text{and}\qquad
		\face[d=1]
		( \id\times\miota )
		\diagonalmap
		=
		\degen[d=0]
		\face[d=0]	
	\]
	where \( \diagonalmap \)~denotes the diagonal map;
	in the first case, it is the diagonal
	map
	\[
		\diagonalmap
		\colon
		\ssetX{1}
		\to
		\ssetX{1}
		\;
		{}_{\face[d=1]}
		\!
		\fibre[limits,\ssetX{0},return,bin]
		{}_{\face[d=1]}
		\;
		\ssetX{1},
	\]
%	\[\begin{tikzcd}
%		\ssetX{1}
%		\ar[r,"\diagonalmap"]
%			& 
%	\end{tikzcd}\]
	the fibre product being taken on both sides with
	respect to the source map~\( \face[d=1] \).
	In the second equation, \( \face[d=0] \)~is used instead.
	We have~\(
		\map{\degen[d=0]\face[d=1]}[spar,shpull]{\mtheta}
		=
		\face[d=1,shpull]{{ \degen[d=0,shpull]{ \mtheta } }}
		= \id,
	\)
	and hence
	\begin{align*}
		\id
		&=
		\map{ ( \miota\times\id ) \diagonalmap }[spar,shpull]{{
			\face[d=1,shpull]{\mtheta}
		}}
		=
		\map{ ( \miota\times\id ) \diagonalmap }[spar,shpull,par]{{
			\face[d=0,shpull]{\mtheta}
			\circ
			\face[d=2,shpull]{\mtheta}
		}}
	\\
		&=
		\map{ \face[d=0] ( \miota \times \id ) \diagonalmap }[spar,qpull]{
			\mtheta
		}
		\circ
		\map{ \face[d=1] ( \miota \times \id ) \diagonalmap }[spar,qpull]{
			\mtheta
		}
		=
		\miota[qpull]{\mtheta}\circ\mtheta
	.
	\end{align*}
	Similarly, the other equation yields \(
		\id = \mtheta\circ\miota[qpull]{\mtheta}
	\).
\end{proof}

\begin{example}
	%Suppose now that \( \ringk \)~is a field
	%and denote by~\( \catsch[over=\ringk] \) the category of schemes
	%over~\( \Spec{\ringk} \),
	%equipped with any of the usual Groethendieck
	%topologies for which \( \catqcoh \)~satisfies descent.
	Suppose that \( \setY \)~is a scheme
	and \( \bigcup \setU[i] \to \setY \)~an fpqc covering,
	and define~\( \setX = \Coprod{\setU[i]} \),
	so that the morphism~\( \mf\colon\setX\to\setY \) is~fpqc.
	Then the descent groupoid is exactly
	the \textdef{\ancech groupoid}
	given by~\( \ssetX{0} = \Coprod{\setU[i]} \)
	and~\( \ssetX{1} = \Coprod{\setU[ij]} \)
	(here, we use the usual convention
	of letting~\(
		\setU[i_0\cdots i_n]
		=
		\setU[i_0]\cap\cdots\cap\setU[i_n]
	\)).
	The source map~\( \face[d=1]\colon\ssetX{1}\to\ssetX{0} \)
	is given by the embeddings~\( \setU[ij]\into\setU[i] \),
	the target map~\( \face[d=0]\colon\ssetX{1}\to\ssetX{0} \)
	is given by the embeddings~\( \setU[ij]\into\setU[j] \),
	unit~\( \ssetX{0}\to\ssetX{1} \) is given by~\( \setU[i] \xto{=} \setU[ii] \),
	composition~\(
		\face[d=1]
		\colon
		\ssetX{1}
		\fibre[\ssetX{0}]
		\ssetX{1}
		\to
		\ssetX{1}
	\)
	is given by~\( \setU[ijk]\into\setU[ik] \),
	and inversion~\( \groupoidinv\colon\ssetX{1}\to\ssetX{1} \)
	is given by~\( \setU[ij] \xto{=} \setU[ji] \).
	More generally
	\[\textstyle
		\ssetX{n}
		=
		\ssetX{1}
		\fibre[\ssetX{0}]
		\ssetX{1}
		\fibre[\ssetX{0}]
		\cdots
		\fibre[\ssetX{0}]
		\ssetX{1}
		=
		\Coprod{ \setU[i_0 \cdots i_n] }
	.\]
	If \( \mvarphi\colon\ordset{m}\to\ordset{n} \),
	the map~\( \mvarphi[pull]\colon\ssetX{n}\to\ssetX{m} \)
	is given by the embedding~\(
		\setU[i_0\cdots i_n]
		\into
		\setU[i_{\mvarphi{0}} \cdots i_{\mvarphi{m}}]
	\).
	Then a pair \( \tup{\algM,\mtheta}\in\catdesc{\ssetX{*}} \)~consists
	of collections~\( \algM = \tup{\algM[i]} \)
	of quasi-coherent sheaves~\( \algM[i]\in\catqcoh{\setU[i]} \)
	on each element in the coevering,
	and collections~\( \mtheta = \tup{\mtheta[ij]} \)
	of gluing morphisms~\(
		\mtheta[ij]
		\colon
		\algM[i,res=\setU[ij]]
		\to
		\algM[j,res=\setU[ij]]
	\),
	subject to the cocycle and unit conditions
	\[
		\mtheta[jk]\circ\mtheta[ij]=\mtheta[ik]
		\qquad\text{and}\qquad
		\mtheta[ii] = \id[\algM[i]]
		.
	\]
	As in the general case, this implies
	that all~\( \mtheta[ij] \) are automatically isomorphisms.
	A morphism~\( \malpha\colon\tup{\algM,\mtheta}\to\alg{\algN,\meta} \)
	is a tuple~\( \malpha = \tup{\malpha[i]} \)
	of morphisms~\( \malpha[i]\colon\algM[i]\to\algN[i] \)
	such that~\(\smash{
		\meta[ij]\circ\malpha[i,res=\setU[ij]]
		=
		\malpha[j,res=\setU[ij]]\circ\mtheta[ij]
	}\)
	for all~\( i,j \).
	Then the descent statement from before simply
	translates to the fact that we recover quasi-coherent sheaves on~\( \setY \)
	from these data.
\end{example}


\section{Barr--Beck theorem and comodules}

One classical way of rewriting the descent condition
is via the Barr--Beck theorem.
We state it in the generality we shall need it.
Following \textcite{maclane},
a \textdef{comonad}
on a category~\( \catC \) is an endofunctor~\(
	\mT\colon\catC\to\catC
\)
together with natural transformations~\(
	\comult\colon\mT\to\mT[squared]
\), called \textdef{comultiplication},
and~\(
	\counit\colon\mT\to\id[\catC]
\),
called \textdef{counit},
such that the following diagrams commute:
\[\begin{tikzcd}
	\mT
	\ar[r,"\comult"]
	\ar[d,"\comult"']
		& \mT[squared]
		\ar[d,"\comult\mT"]
			&	& \mT \ar[d,"\comult"] \ar[ld,equal] \ar[rd,equal]
\\
	\mT[squared]
	\ar[r,"\mT\comult"']
		& \mT[to=3]
			&[3em] \mT
				& \mT[squared] \ar[l,"\counit\mT"] \ar[r,"\mT\counit"']
					& \mT
					\invdot
\end{tikzcd}\]
A \textdef{coalgebra} for a comonad~\( \mT \)
consists of an object~\( \vx \in \catC \)
together with a morphism~\( \ca \colon \vx \to \mT[nopar]{\vx} \),
called \textdef{coaction},
such that the following diagrams commute:
\[\begin{tikzcd}
	\vx \ar[r,"\ca"] \ar[d,"\ca"']
		& \mT[nopar]{\vx} \ar[d,"\comult"]
			&[3em]
			\vx \ar[r,"\ca"] \ar[rd,equal]
				& \mT[nopar]{\vx} \ar[d,"\counit"]
\\
	\mT[nopar]{\vx} \ar[r,"\mT\ca"']
		& \mT[squared,nopar]{\vx}
			&	& \vx \invcomma,
\end{tikzcd}\]
and a map~\( \mf \colon \tup{\vx,\ca}\to\tup{\vy,\ca} \) is a map of \( \mT \)-coalgebras commuting with coaction.
We thus obtain a category~\( \catcoalg{\mT} \)
of coalgebras over~\( \mT \).

\begin{example}
	Any pair of adjoint functors~\(
		\mF \colon \catD\adjunctionarrow\catC\noloc\mG
	\)
	defines an comonad in~\( \catC \)
	by letting~\( \mT = \mF \mG \)
	and defining the comultiplicatoin
	by~\(
		\comult
		\colon
		\mT
		\to
		\mT[squared]
	\)
	by the unit of adjunction~\( \mF\mG\to \mF(\mG\mF)\mG \),
	and the counit by the counit of adjunction.
	We see that any object of the form~\( \mF{\vx} \in\catC \)
	for~\( \vx \in \catD \)
	is a coalgebra over~\( \mT \)
	via~\( \mF{x} \to \map{\mF (\mG \mF)}{\vx} \).
\end{example}


\begin{theorem}[Barr--Beck theorem]
	Suppose that \( \catC \) and \( \catD \)~are
	Abelian categories and
	\(
		\mF \colon \catD\adjunctionarrow\catC\noloc\mG
	\)~an adjunction with~\( \mF \)~faithfully flat.
	If~\( \mT = \mF \mG \)~is the associated comonad,
	\( \mF \)~descends to an equivalence
	of Abelian categories~\( \mF \colon \dgcatC \isoto \catcoalg{\mT} \).
\end{theorem}

Suppose now that \( \mf \colon \setX \to \setY \)~is a faithfully
flat morphism of affine schemes \( \setX = \Spec{\algA} \)
and~\( \setY = \Spec{\algB} \), and consider the pullback square
\[\begin{tikzcd}
	\setX \fibre[\setY] \setX
	\ar[r,"{\face[d=1]}"] \ar[d,"{\face[d=0]}"']
		& \setX \ar[d,"\mf"]
\\
	\setX \ar[r,"\mf"']
		& \setY \invdot
\end{tikzcd}\]
Then base change shows that the comonad
\[
	\mT = \mf[shpull] \mf[shpush]
	\colon
	\catqcoh{\setX}
	\longto
	\catqcoh{\setX},
	\qquad
	\algM
	\longmapsto
	\algA
	\tens[\algB]
	\algM,
\]
is equal\fxfatal{Strictly speaking, they are only isomorphic. How to deal with this?} to
\[
	\face[d=1,shpush] \face[d=0,shpull]
	\colon
	\catqcoh{\setX}
	\longto
	\catqcoh{\setX},
	\qquad
	\algM
	\longmapsto
	( \algA \tens[\algB] \algA ) \tens[\algA] \algM
.\]
Now \(
	\algC
	:=
	\algA\tens[\algB]\algA
	=
	\reg{\setX\fibre[\setY]\setX}
	=
	\reg{\ssetX{1}}
\)
is naturally a coalgebra in the monoidal category~\( \tup{ \catxmodx{\algA}{\algA} , \tens[\algA] } \)
of \( \algA \)-bimodules
via the comorphism~\(
	\face[d=1,comor]
	\colon
	\algC
	\to
	\algC \tens[\algA] \algC
\)
associated to~\(
	\face[d=1]
	\colon
	\ssetX{1} \fibre[\ssetX{0}] \ssetX{1}
	\to
	\ssetX{1}
\).
The category of \( \mT \)-coalgebras is
the same as the category~\( \catxcomod{\algC}{\catxmod{\algA}} \)
of \( \algC \)-comodules
in the category~\( \catxmod{\algA} \),
so Barr--Beck becomes the statement that
	
\begin{proposition}
	If \( \mf \colon \setX = \Spec{\algA} \to \setY = \Spec{\algB} \)~is
	faithfully flat, consider the coalgebra~\(
		\algC = \reg{\setX\fibre[\setY]\setX} = \algA \tens[\algB] \algA
	\).
	Then
	\[
		\mf[shpull]
		\colon
		\catqcoh{\setY} = \catxmod{\algB}
		\longisoto
		\catxcomod{\algC}{\catxmod{\algA}}
	\]
	is an equivalence of Abelian categories.
\end{proposition}

Even if the descent groupoid~\( \ssetX{*} \)
does not come from the covering of a scheme~\( \setY \),
the category of descend data still becomes equivalent to
comodules over the coalgebra~\( \algC = \reg{\ssetX{1}} \).
Suppose that \( \ssetX{1} \rightrightarrows \ssetX{0} \)~is
an internal groupoid in the category of
\emph{affine} schemes.
%, then \( \algC = \reg{\ssetX{1}} \)
%naturally becomes a coalgebra in the monoidal
%category~\( \tup{\catxmodx{\algA}{\algA},\tens[\algA]} \)
%of \( \algA \)-bimodules
%via the comultiplication map~\(
%	\face[d=1,comor]
%	\colon
%	\algC
%	\to
%	\algC \tens[\algA] \algC
%\).
%Furthermore, by
By
adjunction, the gluing map~\(
	\mtheta
	\colon
	\face[d=1,shpull]{\algM}
	\to
	\face[d=0,shpull]{\algM}
\)
is equivalent to a map~\(
	\ca
	\colon
	\algM
	\to
	\face[d=1,shpush]{{ \face[d=0,shpull]{ \algM } }}
	=
	\algC \tens[\algA] \algM
\).
We claim that this operation makes \( \algM \)~into a
comodule over~\( \algC \) in the category~\( \catxmod{\algA} \).


\begin{proposition}\label{res:descent=comodules}
	If \( \ssetX{1} \rightrightarrows \ssetX{0} \)
	is an internal groupoid in \emph{affine} schemes,
	then we have an equivalence of categories~\( \catdesc{\ssetX{*}} \cong \catxcomod{\algC}{\catxmod{\algA}} \),
	where the \anrhs denotes the category of \( \algC \)-comodules
	in~\( \catxmod{\algA} \).
\end{proposition}

For this, we need some technical lemmas that will come in handy later.
For a simplicial object~\( \ssetX{*} \) and any~\( n \), we shall use the notation~\( \face[max] \)
for the morphism~\( \face[d=n]\colon\ssetX{n}\to\ssetX{n-1} \).
This allows us to consider powers of these, e.g.
\( \face[max,upper=l] = \face[d=1] \cdots \face[d=n-1] \face[d=n] \).
Similarly, we write \( \face[min=l] = \face[min] \face[min] \cdots \face[min]\).
We use a similar convention in the cosimplicial
case and hence write
e.g.~\( \coface[max=l] = \coface[d=n] \coface[d=n-1]\cdots\coface[d=1] \)
and~\( \coface[min=l] = \coface[d=0] \coface[d=0] \cdots \coface[d=0] \).
%As in the proof of \cref{res:equivariance=comodules},
%base change will be crucial.
Applying
%flat
base change to the pullback diagram
\[\begin{tikzcd}
	\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
		& \ssetX{i} \ar[d,"{\face[min=i]}"]
\\
	\ssetX{j} \ar[r,"{\face[max=j]}"']
		& \ssetX{0}
\end{tikzcd}\]
we obtain
\(
	\face[max=j,shpush] \face[min=i,shpull]
	\cong
	\face[min=i,shpull] \face[max=j,shpush]
\)
and~\(
	\face[max=j,shpull] \face[min=i,shpush]
	\cong
	\face[min=i,shpush] \face[max=j,shpull]
\).\fxfatal{Probably, we only need one of them. Check which one!}
This implies

\begin{lemma}\label{res:base_change_face_maps}
	Let~\( \ssetX{1} \rightrightarrows \ssetX{0} \)
	be a monoid in the category of affine schemes,
	and write~\( \ssetX{*} \) for its classifying space.
	%with classifying space~\( \ssetX{*} \).
	Suppose we are given objects~\( \algM , \algN , \algP \in \catqcoh{\ssetX{0}} \),
	along with two maps~\(
		\mtheta
		\colon
		\face[max=i,shpull] { \algM }
		\to
		\face[min=i,shpull] { \algN }
	\)
	in~\( \catqcoh{\ssetX{i}} \)
	and~\(\smash{
		\meta
		\colon
		\face[max=j,shpull] { \algN }
		\to
		\face[min=j,shpull] { \algP }
	}\)
	in~\( \catqcoh{\ssetX{j}} \), where~\( i , j \ge 0 \).
	Then the composition
	\begin{align*}
	\MoveEqLeft
	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
		\algM \ar[r]
			\& \face[max=i,shpush] {{ \face[max=i,shpull] { \algM } }}
			\ar[r,"{\mtheta}"]
				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algN } }}
				\ar[r]
					\& \face[max=i,shpush] {{
						\face[min=i,shpull] {{
							\face[max=j,shpush] {{
								\face[max=j,shpull] {{
									\algN
								}}
							}}
						}}
					}}
	\end{tikzcd}
	\\[-.7em]
	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
		{} \ar[r,"{\meta}"']
			\& \face[max=i,shpush] {{
				\face[min=i,shpull] {{
					\face[max=j,shpush] {{
						\face[min=j,shpull] {{
							\algP
						}}
					}}
				}}
			}}
			\ar[r,symbol={\cong}]
				\&[-1.5em] \face[max=i,shpush] {{
				 \face[max=j,shpush] {{
						\face[min=i,shpull] {{
							\face[min=j,shpull] {{
								\algP
							}}
						}}
					}}
				}}
				\ar[r,symbol={=}]
					\&[-1.5em] \face[max=i+j,shpush] {{	
						\face[min=(i+j),shpull] {{ \algP }}
					}}
	\invdot
	\end{tikzcd}\end{align*}
	is the same as the composition
	\begin{align*}
	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
		\algM \ar[r]
			\& \face[max=i+j,shpush] {{
				\face[max=(i+j),shpull] {{ \algM }}
			}}
			\ar[r,"{\face[max=j,shpull]{ \mtheta }}"]
				\&\face[max=i+j,shpush] {{
					\face[max=j,shpull] {{
						\face[ min=i, shpull ] { \algN }
					}}
				}}
	\end{tikzcd}
	\\[-.7em]
	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
		\&{}= \face[max=i+j,shpush] {{
			\face[min=i,shpull] {{
				\face[ max=j, shpull ] { \algN }
			}}
		}}
		\ar[r,"{\face[min=i,shpull] { \meta }}"']
			\&\face[max=i+j,shpush] {{
				\face[min=i,shpull] {{
					\face[ min=j, shpull ] { \algP }
				}}
			}}
			\ar[r,symbol={=}]
				\&[-1.5em] \face[max=i+j,shpush] {{
					\face[min=\smash{(i+j)},shpull] {{ \algP }}
				}}
				.
	\end{tikzcd}\end{align*}
	In other words, the map is
	the unit of adjunction~\(
		\algM
		\to
		\face[max=i+j,shpush] {{
			\face[max=(i+j),shpull] { \algM }
		}}
	\)
	composed with the
	map~\(\smash{
		\face[min=i,shpull] { \meta }
		\circ
		\face[max=j,shpull] { \mtheta }
	}\).
\end{lemma}

\begin{proof}
	The statement is local, so assume
	that \( \ssetX{0} = \Spec{\algA} \)
	and~\( \ssetX{1} = \Spec{\algC} \)
	are affine.
	The two maps~\(
		\face[d=0],\face[d=1]
		\colon
		\ssetX{1}
		\rightrightarrows
		\ssetX{0}
	\) correspond to maps~\(
		\face[d=0,comor],\face[d=1,comor]
		\colon
		\algA
		\rightrightarrows
		\algC
	\),
	which turn~\( \algC \) into an \( \algA \)-bimodule, say, with~\( \face[d=1,comor] \) providing the left action and~\( \face[d=0,comor] \) the right one.
	Then \( \mtheta \) and~\( \meta \)
	become maps
	\begin{flalign*}
	&&
		\mtheta
		\colon
		\algM
		\tens[\algA]
		\algC[tens=i]
		&\longto
		\algC[tens=i]
		\tens[\algA]
		\algN
		&&\text{in~\( \catxmod{\algC[tens=i]} \)}
			&&
	\\
	&\text{and}&
		\meta
		\colon
		\algN
		\tens[\algA]
		\algC[tens=j]
		&\longto
		\algC[tens=j]
		\tens[\algA]
		\algP
		&&\text{in~\(
			\catxmod{\algC[tens=j]}
		\).}
	\end{flalign*}
	The unit of adjunction~\(
		\algM
		\to
		\face[max=i,shpush]
		\face[max=i,shpull]
		\algM
		=
		\algM
		\tens[\algA]
		\algC[tens=i]
	\)
	is then given by~\( m\mapsto m\tens1\tens\cdots\tens1 \), and
	similarly for the other units of adjunction.
	Then the statement we want simply
	says that
	\[\begin{tikzcd}[sep=small]
		\algM
		\ar[r]
		&
		\algM
		\tens[limits,\algA,return,bin]
		\algC[tens=i]
		\ar[r,"\mtheta"]
		&
		\algC[tens=i]
		\tens[limits,\algA,return,bin]
		\algN
		\ar[r]
		&
		\algC[tens=i]
		\tens[limits,\algA,return,bin]
		(
			\algN
			\tens[limits,\algA,return,bin]
			\algC[tens=j]
		)
		\ar[r,"\meta"]
		&
		\algC[tens=i]
		\tens[limits,\algA,return,bin]
		(
			\algC[tens=j]
			\tens[limits,\algA,return,bin]
			\algP
		)		
	\end{tikzcd}\]
	is equal to
	\[\begin{tikzcd}[sep=small]
		\algM
		\ar[r]
		&
		\algM
		\tens[limits,\algA,return,bin]
		\algC[tens=(i+j)]
		\ar[r,"\mtheta"]
		&
		\algC[tens=i]
		\tens[limits,\algA,return,bin]
		\algN
		\tens[limits,\algA,return,bin]
		\algC[tens=j]
		\ar[r,"\meta"]
		&
		\algC[tens=(i+j)]
		\tens[limits,\algA,return,bin]
		\algP,
	\end{tikzcd}\]
	which boils down to associativity of the tensor product.
\end{proof}

\begin{lemma}\label{res:add_comultiplication_map}
	Let the assumptions be as in~\cref{res:base_change_face_maps}.
	Suppose that we are given
	objects~\( \algM , \algN \in \catqcoh{\ssetX{0}} \)
	along with a
	map~\(
		\mtheta
		\colon
		\face[max=n,shpull] { \algM }
		\to
		\face[min=n,shpull] { \algM }
	\).
%	Then the composition
%	\[\begin{tikzcd}[sep=scriptsize]
%		\algM \ar[r]
%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%				\ar[r]
%					& \face[max=n,shpush] {{
%						\face[d=i,shpush] {{
%							\face[d=i,shpull] {{
%								\face[min=n,shpull] { \algN }
%							}}
%						}}
%					}}
%					\ar[r,symbol={=}]
%						&[-1.5em]
%						\face[min=n+1,shpush] {{
%							\face[max=\smash{(n+1)},shpull] {{ \algN }}
%						}} .
%	\end{tikzcd}\]
%	is the same as the composition
%	\[\begin{tikzcd}[sep=scriptsize]
%		\algM \ar[r]
%			& \face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%			\ar[r,"{ \face[d=i,shpull] { \mtheta } }"]
%				& \face[max=n+1,shpush] {{
%					\face[min=(n+1),shpull] { \algN }
%				}}
%					&[-1.5em]
%					\face[max=n+1,shpush] {{
%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%					}}
%					\invdot
%	\end{tikzcd}\]
	Let~\( 0 < i < n \).
	Then we have a commutative diagram
	\[\begin{tikzcd}[sep=scriptsize]
		\algM \ar[r] \ar[d,dashed]
			&[-1.5em] \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
			\ar[r,"{\mtheta}"]
			\ar[d,dashed]
				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
				\ar[d]
	\\
		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
		%\ar[r,dashed]
		\ar[r,symbol={=}]
			& \face[max=n,shpush] {{
				\face[d=i,shpush] {{
					\face[d=i,shpull] {{
						\face[max=n,shpull] { \algM }
					}}
				}}
			}}
			\ar[r,dashed,"{\face[d=i,shpull]{\mtheta}}"]
				& \face[max=n,shpush] {{
					\face[d=i,shpush] {{
						\face[d=i,shpull] {{
							\face[min=n,shpull] { \algN }
						}}
					}}
				}}
				\ar[r,symbol={=}]
					&[-1.5em]
					\face[max=n+1,shpush] {{
						\face[min=\smash{(n+1)},shpull] {{ \algN }}
					}} .
	\end{tikzcd}\]
\end{lemma}

\begin{proof}
	Clear from naturality of the unit of adjunction.
\end{proof}

\begin{proof}[Proof of \cref{res:descent=comodules}]
	%To verify coassociativity of~$\ca$, we must verify commutativity of the diagram
%	Applying base change to the pullback diagram
%	\[\begin{tikzcd}[sep=small]
%		\ssetX{2} \ar[r,"{\face[d=2]}"] \ar[d,"{\face[d=0]}"']
%			& \ssetX{1} \ar[d,"{\face[d=0]}"]
%	\\
%		\ssetX{1} \ar[r,"{\face[d=1]}"']
%			& \ssetX{0}\invcomma
%	\end{tikzcd}\]
%	we obtain $\face[d=2,shpush] { { \face[d=0,shpull] }} = \face[d=0,shpull] {{ \face[d=1,shpush] }}$, which %we shall use repeatedly.\fxfatal{Or just once?}
%	will be crucial.
%	Coassociativity of~$\ca$ is commutativity of the diagram
%	\[\begin{tikzcd}[sep=small]
%		M
%		\ar[r]
%			& \face[d=1,shpush] \face[d=1,shpull] M
%			\ar[r,"\theta"]
%			\ar[d]
%				& \face[d=1,shpush] \face[d=0,shpull] M
%				\ar[d]
%	\\
%			& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=1,shpull] M
%			\ar[r,"\theta"']
%				& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] M
%	\end{tikzcd}\]
	The coassociativity diagram
	\[\begin{tikzcd}
		M
		\ar[r,"\ca"]
			& \algC \tens[\algA] \algM
			\ar[r,yshift=1.5pt,"\id\sotimes\ca"]
			\ar[r,yshift=-1.5pt,"\comult\sotimes\id"']
				& \algC \tens[\algA] \algC \tens[\algA] \algM.
	\end{tikzcd}\]
	is the same as the diagram
	\[\begin{tikzcd}[column sep=scriptsize,row sep=scriptsize]
			&	&
				%\face[d=1,shpush] \face[d=2,shpush]
				%\face[d=2,shpull] \face[d=0,shpull] M
				\face[d=1,shpush] \face[d=0,shpull]
				\face[d=1,shpush] \face[d=1,shpull] \algM
				%\ar[r,symbol={=}]
				\ar[r,"\mtheta"]
					%&[-1.4em]
					&
					%\face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=1,shpull] \algM
%					\face[d=1,shpush] \face[d=0,shpull]
%					\face[d=1,shpull] \face[d=1,shpush] \algM
%					\ar[d,"{\face[d=0,shpull]{\mtheta}}"]
					\face[d=1,shpush] \face[d=0,shpull]
					\face[d=1,shpush] \face[d=0,shpull] \algM
					\ar[d,equal]
	\\
		M \ar[r]
			& \face[d=1,shpush] \face[d=1,shpull] \algM
			\ar[r,"\mtheta"]
			%& \face[d=1,shpush] \face[d=1,shpull] \ar[r,"\theta"] M
				& \face[d=1,shpush] \face[d=0,shpull] \algM
				\ar[u] %\ar[ru,bend left]
				\ar[d]
				%\ar[rr,bend right]
					& \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=0,shpull] \algM
%					\ar[r,symbol={=}]
%						&[-1.5em] \face[d=1,shpush] \face[d=0,shpull] \face[d=1,shpush] \face[d=0,shpull] \algM
	\\%[-.9em]
				&	& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] \algM
						\ar[ur,equal]
	\end{tikzcd}\]
	The two lemmas show that this diagram is the same as the diagram
	\[\begin{tikzcd}[column sep=scriptsize,row sep=scriptsize]
%			& \face[d=1,shpush] \face[d=2,shpush]
%			\face[d=2,shpull] \face[d=0,shpull] \algM
%			\ar[r,symbol={=}]
%				&[-1em]				
%	\\
		\algM \ar[r]
			& \face[d=1,shpush] \face[d=2,shpush]
			\face[d=2,shpull] \face[d=1,shpull] \algM
%			\ar[u,"{\face[d=2,shpull]{\mtheta}}"]
			\ar[r,"{\face[d=0,shpull]{\mtheta}\circ\face[d=2,shpull]{\mtheta}}",yshift=1.5pt]
			\ar[r,"{\face[d=1,shpull]{\mtheta}}"',yshift=-1.5pt]
				&[2em] \face[d=1,shpush] \face[d=2,shpush]
				\face[d=0,shpull] \face[d=0,shpull] \algM
	\invcomma
	\end{tikzcd}\]
	%This together with the relation~$\face[d=1,shpull]\theta = \face[d=0,shpull]\theta\circ \face[d=0,shpull]\theta$ yields the desired commutativity.
	so commutativity boils down to the relation~\(
		\face[d=1,shpull]\theta = \face[d=0,shpull]\theta\circ \face[d=0,shpull]\theta
	\).
	
	To verify the unit condition, notice that
	condition~\(
		\map{\counit\tens\id[\algA]}[spar]\circ\ca=\id[\algM]
	\),
	note that the left-hand side is the composition
	\[\begin{tikzcd}%[sep=small]
		\algM \ar[r]
			& \face[d=1,shpush] { { \face[d=1,shpull] { \algM } } }
			\ar[r, "\mtheta"]
				& \face[d=1,shpush] { { \face[d=0,shpull] { \algM } } }
				\ar[r]
					& \face[d=1,shpush] {{
						\degen[d=0,shpush] {{
							\degen[d=0,shpull] {{
								\face[d=0,shpull] { \algM }
							}}
						}}
					}}
					\invdot
	\end{tikzcd}\]
	The fact that this is the identity on~\( \algM \) follows from the commutative diagram
	\[\begin{tikzcd}
		\algM \ar[r] \ar[rd,equal]
			& \face[d=1,shpush] {{ \face[d=1,shpull] { \algM } }}
			\ar[r,"\mtheta"]
			\ar[d,dashed]
				& \face[d=1,shpush] {{ \face[d=0,shpull] { \algM } }}
				\ar[d]
	\\
			& \face[d=1,shpush] {{
				\degen[d=0,shpush] {{
					\degen[d=0,shpull] {{
						\face[d=1,shpull] { \algM }
					}}
				}}
			}}
			\ar[r,dashed,"{\degen[d=0,shpull]{\mtheta}}"]
				& \face[d=1,shpush] {{
					\degen[d=0,shpush] {{
						\degen[d=0,shpull] {{
							\face[d=0,shpull] { \algM }
						}}
					}}
				}}
				\ar[r,symbol={=}]
					&[-2em] \algM
	\end{tikzcd}\]
	and the assumption that~\( \degen[d=0,shpull] { \mtheta} = \id[\algM] \).
\end{proof}

\endgroup

==> equivariance/equivariance_400.tex <==
\begingroup

\newcommand\pull{^*}
\newcommand\sharppull{^\#}
\newcommand\push{_*}

\setupobject\face{upper={\vphantom{*}}}
\setupobject\degen{upper={\vphantom{*}}}

%\chapter{Flat descent}


%Recall the notion of an \textdef{equivariant sheaf} over an affine scheme~$X = \spec(A)$ 
%In the following, we shall deal with derived equivalences of comodule-like structures over commutative rings. More precisely, we shall deal with commutative algebras~$\algA$ over a field~$\ringk$ along with coalgebras~$\algC$ in the monoidal category~$\algC$ of $\algA$-bimodules.
%For most purposes, we shall assume that $\algC$~is \emph{flat} both as a left and as a right module.

%The motivation for the following comes from the theory of equivariant sheaves, which we now recall.

%\vspace*{-1.5em}

\noindent
Suppose that \( \ssetX{0} \) and \( \ssetX{1} \)~are
a monoid in the category of \emph{affine} schemes.
In other words, we are given a source map~\( \face[d=1]\colon\ssetX{1}\to\ssetX{0} \),
a target map~\( \face[d=0]\colon\ssetX{1}\to\ssetX{0} \),
a unit map~\( \degen[d=0]\colon\ssetX{0}\to\ssetX{1} \),
and a composition
map~\(
	\face[d=1]
	\colon
	\ssetX{1} \fibre[\ssetX{0}] \ssetX{1}
	\to
	\ssetX{1}
\),
satisfying the usual conditions.
Because of affineness, we may treat all pullbacks as composing strictly, and we shall do so.
Denote by~\( \ssetX{*} \) its classifying space,
i.e. the simplicial affine scheme given by~\(
	\ssetX{n}
	=
	\ssetX{1}
	\fibre[\ssetX{0}]
	\ssetX{1}
	\fibre[\ssetX{0}]
	\cdots
	\fibre[\ssetX{0}]
	\ssetX{1}
	%\qquad\text{(\( n \)~factors).}
\)
(\( n \)~factors).
%Suppose \( \ssetX{*} \)~is a simplicial \emph{affine} scheme over a base commutative ring~\( \ringk \).
If \( \ssetX{*} \)~were augmented by a scheme (or another kind of space)~\( \setY \), behaving like the
coequalizer~\(
	\setY
	=
	\Coeq { \ssetX{1} \rightrightarrows \ssetX{0} }
	=
	\dirlim[\catdelta[op]] { \ssetX{*} }
\),
then it is natural to try and glue quasi-coherent sheaves on~\( \ssetX{0} \) satisfying a cocycle condition into a quasi-coherent sheaf on~\( \setY \).
Even if \( \setY \)~does not exist in schemes, we can still make sense of this gluing data:\fxfatal{Switch to right comodules!}

\newdimen\mydimen
\mydimen=13.6em

\putright{8.8}{\(\begin{tikzcd}[ampersand replacement=\&]
	\face[d=2,shpull]{{\face[d=1,shpull]{M}}}
	\ar[r,symbol={=}]
	\ar[d,"{\face[d=2,shpull]{\mtheta}}"']
		\&[-2.3em] \face[d=1,shpull]{{\face[d=1,shpull]{\algM}}}
		\ar[r,"{\face[d=1,shpull]{\mtheta}}"]
			\& \face[d=1,shpull] { {\face[d=0,shpull] { \algM }} }
			\ar[r,symbol={=}]
				\&[-2.2em] \face[d=0,shpull]{ {\face[d=0,shpull] {\algM}} }
\\
	\face[d=2,shpull] { { \face[d=0,shpull] { \algM } } }
	\ar[r,symbol={=}]
		\& \face[d=0,shpull] { { \face[d=1,shpull] { \algM } } }\invdot
		\ar[rru,"{\face[d=0,shpull] { \mtheta } }"']
\end{tikzcd}\)}

\parshape=16
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \textwidth
0pt \mydimen
0pt \mydimen
0pt \mydimen
0pt \mydimen
0pt \mydimen
0pt \mydimen
%0pt \mydimen
0pt \textwidth
Thus given a quasi-coherent
sheaf~\( \algM \in \catqcoh{ \ssetX{0} } \),
we define an \textdef{equivariant structure} on~\( \algM \) to consist of an isomorphism
\[
	\mtheta
	\colon
	\face[d=1,shpull] { \algM }
	\longisoto
	\face[d=0,shpull] { \algM }
\]
satisfying the cocycle conditions
\begin{equation}\label{eq:1_new_equivariance}
	\face[d=0,shpull]{\mtheta}
	\circ
	\face[d=2,shpull]{\mtheta}
	=
	\face[d=1,shpull]{\mtheta}
	\qquad\text{and}\qquad
	\degen[d=0,shpull]{\mtheta} = \id[\algM]
	.
\end{equation}
When \( \algM \)~is equipped with an equivariant structure, we call it an
\textdef{equivariant sheaf}.
The first condition is commutativity of the diagram to the right.
Notice that if we use the isomorphisms~\( \mtheta \) as gluing data and treated~\( \mtheta \) as just the identity,
the cocycle condition on~\( \algM \) would become \( \face[d=0,shpull] { \algM } = \face[d=1,shpull] { \algM } \), and \( \algM \)~would therefore lie in the
equalizer~\(
	\Eq { {
		\face[d=0,shpull] ,
		\face[d=1,shpull]
		\colon
		\catqcoh { \ssetX { 0 } }
		\rightrightarrows
		\catqcoh { \ssetX{1} } 
		} }
	=
	\invlim[\catdelta] { \catqcoh { \ssetX {*} } }
\).
(Without this gluing, the equivariant sheaves would form a pseudolimit, with squares only commuting up to isomorphism.).
%Comparing with the direct limit expression of the (possibly non-existent) quotient~\( \setX[lmod=\algG] \) mentioned above, this shows why \( \algG \)-equivariant sheaves on~\( \setX \) behave like quasi-coherent sheaves on~\( \setX[lmod=\algG] \).
This shows why equivariant sheaves behave a bit like sheaves
on~\( \dirlim[\catdelta[op]] { \ssetX{*} } \), and indeed, descent theory provides us with sufficient conditions under which this is true on the nose.
The purpose of this project is to develop a derived notion of equivariance.

\parshape=0

%Consider the action groupoid~\( \tup { \ssetX{1} , \ssetX{2} } \) corresponding to this action, with \( \ssetX{0} = \setX \)
%and~\( \ssetX{1} = \algG\times\setX \). The source and target maps~\(
%\ssetX{1}\rightrightarrows \ssetX{0}\) are exactly~\(\map{s} = \face[d=0]\) and~\(\map{t}=\face[d=1]\) from above.
%More generally, we obtain a simplicial scheme~$\ssetX{*}$ given by
%\[
%	\ssetX{n} =
%	\ssetX{1} \fibre[\ssetX{0}]
%	\ssetX{1} \fibre[\ssetX{0}]
%	\cdots
%	\fibre[\ssetX{0}]
%	\ssetX{1}
%	=
%	\algG\times \algG\times\cdots\times \algG\times \setX
%	\qquad\text{($n$~factors)}
%	.
%\]
%Then \eqref{eq:1_equivariant_sheaf}~simply corresponds to the cocycle conditions
%\begin{equation}\label{eq:1_new_equivariance}
%	\face[d=0,pull]{\mtheta}
%	\circ
%	\face[d=2,pull]{\mtheta}
%	=
%	\face[d=1,pull]{\mtheta}, 
%\end{equation}
%%This makes sen
%which is commutativity of
%%\[\begin{tikzcd}
%%	\face[d=1,shpull] \face[d=1,shpull] M
%%	\ar[r,"\face[d=1,shpull]\theta"]
%%	\ar[d,symbol={=}]
%%		& \face[d=1,shpull] \face[d=0,shpull] M
%%		\ar[d,symbol={=}]
%%\\[-1.5em]
%%	\face[d=0,shpull] \face[d=1,shpull] M
%%		& \face[d=0,shpull] \face[d=0,shpull] M
%%\end{tikzcd}\]
%\[\begin{tikzcd}
%	\face[d=2,shpull]{{\face[d=1,shpull]{M}}}
%	\ar[r,symbol={=}]
%	\ar[d,"{\face[d=2,shpull]{\mtheta}}"']
%		&[-2.3em] \face[d=1,shpull]{{\face[d=1,shpull]{\algM}}}
%		\ar[r,"{\face[d=1,shpull]{\mtheta}}"]
%			& \face[d=1,shpull] { {\face[d=0,shpull] { \algM }} }
%			\ar[r,symbol={=}]
%				&[-2.2em] \face[d=0,shpull]{ {\face[d=0,shpull] {\algM}} }
%\\
%	\face[d=2,shpull] { { \face[d=0,shpull] { \algM } } }
%	\ar[r,symbol={=}]
%		& \face[d=0,shpull] { { \face[d=1,shpull] { \algM } } }
%		\ar[rru,"{\face[d=0,shpull] { \mtheta } }"']
%\end{tikzcd}\]
%Applying~\( \reg \), we obtain a cosimplicial system of
%rings~\( \algA[n] = \reg { \ssetX{n} } \).
%For brevity, we write \( \algA = \algA[0] \) and~\( \algC = \algA[1] \).

\begin{examplebreak}[Example: \ancech nerve]
	Suppose that \( \setY \)~is an affine scheme with an affine open cover
	\( \setY = \Union { \setU[i] } \)
	such that all intersections
	\(
		\setU [ i_0 \cdots i_n ]
		=
		\setU [ i_0 ] \cap \cdots \cap \setU [ i_n ]
	\)
	are also affine.
	Consider the \ancech nerve
	\( \ssetX{*} \)
	given by
	\(
		\ssetX{n}
		=
		\ssetX{1} \fibre[\ssetX{0}] \cdots \fibre[\ssetX{0}] \ssetX{1}
		=
		\Coprod[ i_0 \cdots i_n ] { \setU [ i_0 \cdots i_n ] }
	\).
	%,
	%where as usual, multiindices mean intersection.
	We have no ordering on the index set and allow arbitrary indices, including indices with repetitions.
	Notice
%	that we have in general
%	\[
%		\ssetX{n} =
%		\ssetX{1}
%		\fibre[\ssetX{0}]
%		\ssetX{1}
%		\fibre[\ssetX{0}]
%		\cdots
%		\fibre[\ssetX{0}]
%		\ssetX{1}
%		\qquad\text{(\( n \)~factors)}
%	\]
%	%as in the example above. And similarly to that example,
%	and
	that
	the original space~\( \setY \) behaves like the
	coequalizer
	\[\textstyle
		\setY = \Coeq {{
			\face[d=0,shpull],\face[d=1,shpull]
			\colon
			\ssetX{1}
			\rightrightarrows
			\ssetX{0}
		}}
		=
		\dirlim[\catdelta[op]] { \ssetX{*} }
		.
	\]
	By flat descent, we indeed recover a version quasi-coherent sheaves on~\( \setY \) as a version of the limit~\( \invlim[\catdelta] { \catqcoh { \ssetX{n} } } \).
\end{examplebreak}


\begin{examplebreak}[Example: Equivariant sheaves with respect to group actions]
	Suppose $\setX = \Spec{\algA}$ is an affine algebraic variety and~$\algG$ an affine algebraic group acting on~$\setX$.
	%In this case, we can treat all pullbacks as composing strictly, and we shall do so.
	%The multiplication and action maps pull back to maps~$\reg{\algG}\to\reg{\algG}\tens\reg{\algG}$
	%and $\algA\to\reg{\algG}\tens\algA$ equipping~$\reg{\algG}$ with the structure of a commutative Hopf algebra with~$\algA$ being a $\reg{\algG}$-comodule.
	%A \textdef[equivariant sheaf]{$K$-equivariant sheaf} is a quasi-coherent sheaf
	%
	%Denote by $\face[d=0],\face[d=1]\colon \algG\times \setX\to \setX$ the pair of maps given by $\face[d=0]{\vg,\vx} = \vx$ and~$\face[d=1]{\vg,\vx} = \vg{\vx}$
	%and by \( \degen[d=0] \colon \setX\to\algG\times\setX \) the
	%map~\( \degen[d=0] { \vx } = \tup{ 1 , \vx } \).
	%Given an $\algA$-module~$\algM\in\catAmod = \catqcoh{\setX}$, an \textdef{equivariant structure} is an isomorphism
	%\[
	%	\mtheta\colon \face[d=1,pull]{\algM}\longisoto \face[d=0,pull]{\algM}
	%\]
	%satisfying the condition
	%\begin{equation}\label{eq:1_equivariant_sheaf}
	%	\map{p}[23,pull]{\mtheta}
	%	\circ
	%	\map{\id[\algG]\times \face[d=1]}[spar,pull]{\mtheta}
	%	=
	%	\map{\map{m}\times\id[\setX]}[spar,pull]{\mtheta},
	%\end{equation}
	%where $\map{m}\colon \algG\times \algG\to \algG$~is the group operation and $\map{p}[23]\colon \algG\times \algG\times \setX\to \algG\times \setX$ is the projection along the first factor~$\algG$
	%\parencite[see][section~5.1]{ginzburg}.
	%By adjunction, such map~$\theta$ is the same as a map~$M\to \face[d=0,shpush] \face[d=1,shpull](M)$.
	%We reformulate this by putting~$\Gamma = \Gamma_1 = G\times X$ and, more generally,
	%\[
	%	\Gamma_n = 
	%\]
	%We reformulate this using the language of groupoids: Letting~$\Gamma_0 = X$ and $\Gamma_1 = G\times X$, we regard
	
	%Putting~$\ssetX{0} = \setX$ and $\ssetX = \ssetX{1} = \algG\times \setX$, we obtain a groupoid scheme with source and target maps~$\ssetX{1}\rightrightarrows \ssetX{0}$ given by~$\map{s} = \face[d=0]$ and~$\map{t}=\face[d=1]$, unit
	%map~\( \ssetX{0}\to\ssetX{1} \), \( \vx\mapsto \tup{1,\vx} \), and inversion map~\(  \).
	%The notion of an equivariant sheaf on~\( \setX \) with respect to this action is, morally, a sheaf on the quotient
	We want to develop a notion of quasi-coherent sheaf on~\( \setX \) that, at least morally, behaves like quasi-coherent sheaves on the quotient~\( \setX[lmod=\algG] \). Using this as the definition directly clearly fails for all but the nicest actions where one can be sure to have a scheme structure on this quotient.
	%Instead, we proceed a bit indirectly.
	%If \( \algG \) and~\( \setX \) were discrete, we could consider instead the action groupoid~\( \setX[llmod=\algG] \), which is equivalent to~\( \setX[lmod=\algG] \) considered as a discrete category.
	Instead, we
	consider
	the action groupoid~\( \ssetX{*} \)
	given by
	\(
		\ssetX{n} =
		\ssetX{1} \fibre[\ssetX{0}]
		%\ssetX{1} \fibre[\ssetX{0}]
		\cdots
		\fibre[\ssetX{0}]
		\ssetX{1}
		=
		\algG\times \algG\times\cdots\times \algG\times \setX
	%	\qquad\text{($n$~factors~\( G \))}
	\).
	%with face and degeneracy maps defined as for the nerve of a category.
	%Indeed, if the group~\( \algG \) were discrete, this would just be the nerve of the action groupoid~\( \setX[llmod=\algG] \).
	The first two elements \( \ssetX{0} , \ssetX{1} \) recover the action groupoid of this group action, with source and target
	maps~\(\ssetX{1}\rightrightarrows \ssetX{0}\)
	given by \(\map{s} = \face[d=0]\) and~\(\map{t}=\face[d=1]\).
	If the quotient~\( \setX[lmod=\algG] \) existed in schemes, then
	it would at least behave like the
	coequalizer~\(
		\Coeq { \ssetX{1} \rightrightarrows\ssetX{0} }
		= \dirlim[\catdelta[op]] { \ssetX{*} }
	\).
	Now the definition of an equivariant sheaf with respect to this simplicial scheme recovers exactly the definition of an equivariant sheaf on~\( \setX \) with respect to this group action, as defined in
	the literature.
\end{examplebreak}

\begin{comment}
and $C = \reg(\Gamma) = \reg(G)\otimes A$. The maps $d_0,d_1\colon \Gamma\to X$ pull back to maps~$A\to C$, providing~$C$ with the structure of an $A$-bimodule. Then we have that $\face[d=0,shpush] \face[d=1,shpull](M)$~is~$C \otimes_{A} M$ considered as a left $A$-module.

The motivation for the following comes from the theory of equivariant sheaves and an attempt to make this theory algebraic. However, we shall stick to the algebraic formulation. Suppose that $X = \spec(A)$ and $Y = \spec(B)$ are affine schemes, and let~$X\to Y$ be a map with corresponding ring map~$B\to A$. Form the simplicial affine scheme by~$X_0 = X = \spec(A)$, $X_1 = X\times_{Y} X = \spec(A\otimes_{B} A)$, and more generally,
\[
	X_n = X\times_{Y}\cdots\times_{Y} X = \spec(A\otimes_{B}\cdots\otimes_{B} A)
	\qquad\text{($n+1$~factors)}.
\]
%The face map~$\face1\colon X_2\to X_1$ pulls back to a map~$
%This allows us to define a 
We obtain a groupoid by letting~$s = \face0\colon X_1\to X_0$ and $t = \face1\colon X_1\to X_0$
be the source resp.\ target maps, $m=\face1\colon X_2\to X_1$ the composition map and $i = d_0\colon X_0\into X_1$ the unit.
%, thees maps equip~$X\simp$ with the structure of a groupoid with 
%The projection maps~$\face0,\face1\colon X_1\to X_0$ pull back to flat maps~$A\to A\otimes_{B} A$. Putting~$C = A\otimes_{B} A$, 
Pulling back, %we obtain a (non-counital) coassociative coalgebra structure on~$C = A\otimes_{B} A$ in the form of a map~$C\to C\otimes_{A} C$
we obtain maps~$C\to C\otimes_{A} C$ and $C\to A$, where~$C = A\otimes_{B} A$, equipping~$C$ with the structure of a coalgebra in~$\catAmodA$.

%For the constructions we will perform, we do
The constructions we will do will work for general coalgebras~$C$ in~$\catAmodA$ for rings~$A$. In this case, we may replace~$Y$ by a stack~$\stackY$ with a map~$X_0\to\stackY$ and~$X_1 = X_0\times_{\stackY} X_0$.


Let~$k$ be a field and~$A$ a commutative, Noetherian $k$-algebra of finite projective dimension. Let~$C$ be an $A$-bimodule which is flat as a right $A$-module, and let
\[
	C\longto C\otimes_{A} C, \qquad C\longto A,
\]
be a coalgebra structure on~$C$.
\end{comment}

Based on the above, one clear candidate for a higher notion of equivariance
on the simplicial scheme~\( \ssetX{*} \) is to
replace the limit by the homotopy limit,~\( \invholim[\catdelta] { \catqcoh{\ssetX{*}} } \).
We shall show that there is a different approach, obtained by
rewriting the definition of equivariance a bit using algebraic data.

%Before attempting to develop a higher notion of equivariance, we shall reformulate the definition of an equivariant sheaf a bit via more algebraic data.
%For this purpose, we assume from now on that everything is affine.
Putting~\(
	\algC
	= \reg{\ssetX{1}}
%	= \reg{\algG}\tens \algA 
\),
the maps~$\face[d=0,sharp],\face[d=1,sharp]\colon \algA\rightrightarrows \algC$ equip~$C$ with the structure of an~$A$-bimodule, with %, say, 
$\face[d=1,sharp]$~corresponding to the left action and~$\face[d=0,sharp]$ to the right one,
and~$\theta$ is an isomorphism of~$A$-modules~$M\otimes_{A} C\isoto C\otimes_{A} M$.
%Thus~$C$ becomes a coalgebra in the category~$\catAmodA$,
Furthermore, the maps
\( \comult = \face[d=1,sharp]\colon \algC \to \algC\tens[\algA]\algC \)
and \( \counit = \degen[d=0,sharp]\colon \algC \to \algA \)
equip~\( \algC \) with the structure of a coalgebra in the
category~\( \catAmodA \).
%More generally, $
%Similarly, $d_0\sharppull, d_1\sharppull,d_2\sharppull\colon C\into C\otimes_{A} C$ correspond to the right, diagonal, and left action, respectively.
%More generally, $\face[d=0,sharp],\face[d=n,sharp]\colon \reg(\Gamma_{n-1})\to\reg(\Gamma_{n})$ correspond to the left and right actions. In the case~$n=2$, $\face[d=1,sharp]\colon \algC\into \algC\tens[\algA] \algC$ is the coproduct which provides a central, diagonal action.
%\fxnote{Writing out what the maps do makes it clear that the top face map should be the left action and the bottom face map should be the right action. For instance, in the case of~$C\into C\otimes_{A} C$, the maps are given by~$c\mapsto 1\sotimes c$, $c\mapsto\comult(C)$, and~$c\mapsto c\sotimes1$. If we think of~$C$ as~$A\otimes_{\reg[\mathscr{Y}]}A$, then we get similar formulas.}
Now the isomorphism~$\mtheta$ is equivalent, by adjunction, to a map~$\ca\colon \algM\to \face[d=1,shpush] { { \face[d=0,shpull] {M} } }$, the \anrhs being~$\algC\tens[\algA] \algM$ considered as a left~$\algA$-module. We have

\begin{proposition}\label{res:equivariance=comodules}
	%If $C$~is flat as a right $A$-module, then
	%Assume that~\( \algC \) is flat as a right \( \algA \)-module.
	Assume that the maps~\( \face[d=0], \face[d=1] \)~are flat, i.e. \( \algC \)~is flat as both a left and a right \( \algA \)-module.
	Then the equivariance property~\eqref{eq:1_new_equivariance}
	%is equivalent to the map~$M\to C\otimes_{A} M$ being a $C$-comodule structure
	is equivalent %to~$\algM$ being a (counital) $\algC$-comodule via the map~$\ca\colon \algM\to \algC\tens[\algA] \algM$.\fxfatal{Add details in the proposition regarding the counit map.}
	to a structure on~\( \algM \) of a counital \( \algC \)-comodule
	in the category~\( \catxmodx{\algA}{\algA} \) via the
	map~\(\ca\colon \algM \to \algC \tens[\algA] \algM\).
\end{proposition}

\begin{proof}
	%To verify coassociativity of~$\ca$, we must verify commutativity of the diagram
	Applying flat base change to the pullback diagram
	\[\begin{tikzcd}[sep=small]
		\ssetX{2} \ar[r,"{\face[d=2]}"] \ar[d,"{\face[d=0]}"']
			& \ssetX{1} \ar[d,"{\face[d=0]}"]
	\\
		\ssetX{1} \ar[r,"{\face[d=1]}"']
			& \ssetX{0}\invcomma
	\end{tikzcd}\]
	we obtain $\face[d=2,shpush] { { \face[d=0,shpull] }} = \face[d=0,shpull] {{ \face[d=1,shpush] }}$, which %we shall use repeatedly.\fxfatal{Or just once?}
	will be crucial.
%	Coassociativity of~$\ca$ is commutativity of the diagram
%	\[\begin{tikzcd}[sep=small]
%		M
%		\ar[r]
%			& \face[d=1,shpush] \face[d=1,shpull] M
%			\ar[r,"\theta"]
%			\ar[d]
%				& \face[d=1,shpush] \face[d=0,shpull] M
%				\ar[d]
%	\\
%			& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=1,shpull] M
%			\ar[r,"\theta"']
%				& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] M
%	\end{tikzcd}\]
	The coassociativity diagram
	\[\begin{tikzcd}
		M
		\ar[r,"\ca"]
			& \algC \tens[\algA] \algM
			\ar[r,bend left,"\id\sotimes\ca"]
			\ar[r,bend right,"\comult\sotimes\id"']
				& \algC \tens[\algA] \algC \tens[\algA] \algM.
	\end{tikzcd}\]
	is the same as the diagram
	\[\begin{tikzcd}[column sep=scriptsize,row sep=scriptsize]
			&	& \face[d=1,shpush] \face[d=2,shpush] \face[d=2,shpull] \face[d=0,shpull] M
				\ar[r,symbol={=}]
					&[-1.4em] \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=1,shpull] \algM
					\ar[d,"{\face[d=0,shpull]{\mtheta}}"]
	\\
		M \ar[r]
			& \face[d=1,shpush] \face[d=1,shpull] \algM
			\ar[r,"\mtheta"]
			%& \face[d=1,shpush] \face[d=1,shpull] \ar[r,"\theta"] M
				& \face[d=1,shpush] \face[d=0,shpull] \algM
				\ar[u] %\ar[ru,bend left]
				\ar[d]
				%\ar[rr,bend right]
					& \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=0,shpull] \algM
					\ar[r,symbol={=}]
						&[-1.5em] \face[d=1,shpush] \face[d=0,shpull] \face[d=1,shpush] \face[d=0,shpull] \algM
	\\%[-.9em]
				&	& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] \algM
						\ar[ur,equal]
	\end{tikzcd}\]
	To verify that both paths around this diagram are equal,
	%note first that the two units of adjunctions $M\to \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=1,shpull] M$ and $M\to \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=1,shpull] M$ are equal because the functors $d_1
	notice first that the simplicial relation~$\face[d=1] \face[d=1] = \face[d=1] \face[d=2]$ means that the two units of adjunction $\algM\to \map{\face[d=1] \face[d=1]}[spar,shpush] {{ \map{\face[d=1] \face[d=1]}[spar,shpull] {\algM}}}$ and~$M\to \map{\face[d=1] \face[d=2]}[spar,shpush] {{ \map{ \face[d=1] \face[d=2] }[spar,shpull] { \algM } }}$ are equal.
	Denoting both by~$\eta$, the diagram
	%The diagram
%	the diagram
%	\[\begin{tikzcd}
%		M \ar[r]
%			& \face[d=1,shpush] \face[d=1,shpull] M
%			\ar[r,"\theta"]
%			\ar[d,dashed]
%				& \face[d=1,shpush] \face[d=0,shpull] M
%				\ar[rd]
%				\ar[d]
%	\\
%			& \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=1,shpull] M
%			\ar[d,symbol={=}]
%			\ar[r,"\face[d=0,shpull]\theta",dashed]
%				& \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=0,shpull] M
%				\ar[r,"\face[d=0,shpull]\theta"]
%					& \face[d=1,shpush] \face[d=0,shpull] \face[d=1,shpush] \face[d=0,shpull] M
%	\\[-1.5em]
%			& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=1,shpull] M
%			\ar[rru,bend right=7]
%	\end{tikzcd}\]
	\[\begin{tikzcd}[column sep=scriptsize,row sep=scriptsize]
			& \face[d=1,shpush] \face[d=2,shpush] \face[d=2,shpull] \face[d=1,shpull] M
			\ar[r,"{\face[d=2,shpull]{\mtheta}}",dashed]
				& \face[d=1,shpush] \face[d=2,shpush] \face[d=2,shpull] \face[d=0,shpull] \algM
				\ar[r,symbol={=}]
					&[-1.4em] \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=1,shpull] \algM
					\ar[d,"{\face[d=0,shpull]\theta}"]
	\\
		M \ar[r]
			& \face[d=1,shpush] \face[d=1,shpull] M
			\ar[u,dashed,"\eta"]
			\ar[d,dashed,"\eta"']
			\ar[r,"\theta"]
			%& \face[d=1,shpush] \face[d=1,shpull] \ar[r,"\theta"] M
				& \face[d=1,shpush] \face[d=0,shpull] M
				\ar[u] %\ar[ru,bend left]
				\ar[d]
				%\ar[rr,bend right]
					& \face[d=1,shpush] \face[d=2,shpush] \face[d=0,shpull] \face[d=0,shpull] M
					\ar[r,symbol={=}]
						&[-1.5em] \face[d=1,shpush] \face[d=0,shpull] \face[d=1,shpush] \face[d=0,shpull] M
%	\\[-.9em]
%				&	&	& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] M
%						\ar[u,symbol={=}]
	\\%[-2em]
					& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=1,shpull] M
							\ar[r,"{\face[d=1,shpull]\theta}"',dashed]
						& \face[d=1,shpush] \face[d=1,shpush] \face[d=1,shpull] \face[d=0,shpull] M
						\ar[ru,equal]
	\end{tikzcd}\]
	shows that both paths in the above diagram factor through~$\eta$.
	This together with the relation~$\face[d=1,shpull]\theta = \face[d=0,shpull]\theta\circ \face[d=0,shpull]\theta$ yields the desired commutativity.
	
	To verify the unit condition, notice that
	condition~\(
		\map{\counit\tens\id[\algA]}[spar]\circ\ca=\id[\algM]
	\),
	note that the left-hand side is the composition
	\[\begin{tikzcd}%[sep=small]
		\algM \ar[r]
			& \face[d=1,shpush] { { \face[d=1,shpull] { \algM } } }
			\ar[r, "\mtheta"]
				& \face[d=1,shpush] { { \face[d=0,shpull] { \algM } } }
				\ar[r]
					& \face[d=1,shpush] {{
						\degen[d=0,shpush] {{
							\degen[d=0,shpull] {{
								\face[d=0,shpull] { \algM }
							}}
						}}
					}}
					\invdot
	\end{tikzcd}\]
	The fact that this is the identity on~\( \algM \) follows from the commutative diagram
	\[\begin{tikzcd}
		\algM \ar[r] \ar[rd,equal]
			& \face[d=1,shpush] {{ \face[d=1,shpull] { \algM } }}
			\ar[r,"\mtheta"]
			\ar[d,dashed]
				& \face[d=1,shpush] {{ \face[d=0,shpull] { \algM } }}
				\ar[d]
	\\
			& \face[d=1,shpush] {{
				\degen[d=0,shpush] {{
					\degen[d=0,shpull] {{
						\face[d=1,shpull] { \algM }
					}}
				}}
			}}
			\ar[r,dashed,"{\degen[d=0,shpull]{\mtheta}}"]
				& \face[d=1,shpush] {{
					\degen[d=0,shpush] {{
						\degen[d=0,shpull] {{
							\face[d=0,shpull] { \algM }
						}}
					}}
				}}
				\ar[r,symbol={=}]
					&[-2em] \algM
	\end{tikzcd}\]
	and the assumption that~\( \degen[d=0,shpull] { \mtheta} = \id[\algM] \).
\end{proof}

%\begin{para}[Homotopy descent]
%	Because of this, we propose the following algebraic candidate for a higher notion of equivariance with respect to a simplicial affine scheme, when both maps~\( \ssetX{1}\rightrightarrows\ssetX{0} \) are flat:
%	\(
%		\invholim[\catdelta] { \catxcomod{\algC}{\catxmodx{\algA}{\algA}} }
%	\),
%	the homotopy limit of the category of \( \algC \)-comodules in the monoidal category~\( \catxmodx{\algA}{\algA} \).\fxfatal{MAKES NO SENSE!!! No \( n \)-variance on the \anrhs.}
%\end{para}

\begin{para}[Homotopy descent]
	Based on the above there are (at least) two algebraic candidates for a higher notion of equivariance in affine schemes, when both maps~\( \ssetX{1}\rightrightarrows\ssetX{0} \) are flat:
	\begin{itemize}
		\item One may replace~\( \catxcomod{\algC} \) by an
		\ainfty-analogue of this.
		\item %One may replace the limit above by the \emph{homotopy}
		%limit, the derived functor of the limit.
		One may replace~\( \invlim[\catdelta] {\catqcoh { \ssetX{*} }} \)
		by~\( \invholim[\catdelta] { \catcom{ \catqcoh { \ssetX{*} }} } \),
		the \emph{homotopy} limit of the categories of complexes
		of quasi-coherent sheaves on~\( \ssetX{*} \).
	\end{itemize}
	The purpose of this project is to compare these two approaches
	and show that, up to technicalities, they yield the same result.
\end{para}

\endgroup

==> holim_dgcat/holim_dgcat_5002.tex <==
\begingroup

\chapter{Homotopy limits in dg-categories}

%\section{Framings in dg-categories}
%
%A framing on the category~\( \catdgcat \) is due to
%\textcite{holstein}: If \( \dgcatA \in \catdgcat \) and \( \ssetK\in\catsset \), then let
%\(
%	\dgcatA[powering=\ssetK]
%	=
%	\catloc { \ssetK, \dgcatA }
%	=
%	\catdgfun[infty,o] { \lurie{\ssetK} , \dgcatA }
%\).

%\begin{parabreak}[Tabuada's model structure on~\( \catdgcat \)]
	Given a dg-category~\( \dgcatA \), we denote by~\( \dgcatA[z0] \) the dg-category with the same objects as~\( \dgcatA \), but with hom complexes given by
	\(
		%\Hom[ \dgcatA[z0] ] { \vx, \vy } =
		%\cocy[nopar]{0} { \Hom[\dgcatA, * ] { \vx, \vy } }
		\dgcatA[z0,spar] { \vx , \vy } = \cocy{0} { \dgcatA { \vx , \vy } }
	\),
	the set of closed maps~\( \vx \to \vy \) in~\( \dgcatA \). We define~\( \dgcatA[h0] \) analogously.
	A map~\( \mf \in \dgcatA[d=0]{ \vx , \vy } \) in~\( \dgcatA \) is called a \textdef{homotopy equivalence} if its image in~\( \dgcatA[h0] \) is an isomorphism. As in homological algebra, this amounts the existence of a map \( \mg \in \dgcatA[d=0] { \vy , \vx } \) in the other direction along with correcting morphisms \( \mr[\vx] \in \dgcatA[d=-1] { \vx , \vx } \) and \( \mr[\vy] \in \dgcatA[d=-1] { \vy , \vy } \) such that
	\[
		\dif{ \mr[\vx] } = \mg \mf - \id[\vx]
		\qquad\text{and}\qquad
		\dif{ \mr[\vy] } = \mf \mg - \id[\vy].
	\]

	We recall from
	\textcite{tabuada,tabuada_dgcats_vs_simplicial_cats}
	the existence of a model structure on the \( 1 \)-category~\( \catdgcat \) with
	\begin{itemize}
		\item weak equivalences given by \textdef{quasi-equivalences}, i.e.
		functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
		\item the induced functor~\( \mF[parent=alg,h0] \colon \dgcatA[h0] \to \dgcatB[h0] \) is an equivalence of categories in the classical, non-enriched sense;
		\item for all~\( \vx, \vy \in \dgcatA \),
		\( \mF[\vx, \vy] \colon
		\dgcatA { \vx , \vy } \to \dgcatB { \mF { \vx } , \mF { \vy } } \)
		is a quasi-isomorphism of chain complexes;
		\end{enumerate}
		\item fibrations given by dg-functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
			\item the induced map
			\(
				\mF \colon
				\dgcatA[*] { \vx, \vy }
				\to
				\dgcatB[*] { \mF { \vx } , \mF { \vy } }
			\)
			is surjective for all objects~\( \vx, \vy \in \dgcatA \), and
			\item any map \( \mf \colon \mF { \vx } \to \vy \) in~\( \dgcatB \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatB } \) lifts as \( \mf = \mF { \mg } \) for some morphism \( \mg\colon \vx \to \vx[prime] \) in~\( \dgcatA \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatA } \).
		\end{enumerate}
	\end{itemize}
%	It is cofibrantly generated,
%	with
%	\begin{itemize}
%		\item the class~\( \setgencof \) consisting of the morphism \( \varnothing \into \ringk \)
%		\item the class~\( \setgentrivcof \)
%	\end{itemize}
	This model structure is combinatorial according to
	\textcite[Proposition~1.3.1.19]{ha}.
%\end{parabreak}

We shall use the tools developed in the preceding chapters to develop a notion of homotopy descent of quasi-coherent sheaves on affine schemes.
%We write \( \face[min=n] \) and~\( \face[max=n] \) for the two unique morphisms~\( \ordset{0} \into \ordset{n} \) in~\( \catdelta \) given by
%\( \face[min=n] { 0 } = 0 \) and~\( \face[max=n] { 0 } = n \).
%In other words, \( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
%and~\( \face[max=n] = \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
Much of the inspiration is from \textcite{explicit};
however, using the tools developed earlier
(specifically~\cref{ex:A_infty_fun_k_n_to_B}),
we are able to solve their Conjecture~1 and prove their
results in complete generality.



%\begin{theorem}
%	Suppose that \( \ssetX{*} \)~is a simplicial affine scheme with each~\( \ssetX{n} \) being regular and each \( \ssetX{n}\to \ssetX{m} \) flat surjective\fxfatal{This is supposed to be the same as faithfully flat, check this.}.
%	Then we have an equivalence of categories
%	\(
%		\invholim[\catdelta] { \catqcoh{\ssetX{n}} }
%		\cong
%		\catainftycomod { \catqcoh { \ssetX{0} } }
%	\).
%\end{theorem}

Recall from \cref{res:fat_tot} that
the homotopy limit of a \( \catdelta \)-diagram in~\( \catdgcat \) is given by
\[\textstyle
	\invholim[\catdelta] { \cosimpdgcatA{n} }
	=
	\invholim[\catdelta[plus]] { \cosimpdgcatA{n} }
	=
	\End[\ordset{n}\in\catdelta[plus]] { \fibrep[deltaplus] { \cosimpdgcatA{n} }{n} }
\]
where \( \fibrep[deltaplus] \colon \catdgcat\to\catdgcat[diag={\catdelta[plus,op]},inj,smash] \) is a fibrant replacement functor, taking a dg-category~\( \dgcatB \) to an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \).
We obtain such a functor from Holstein:

\begin{theorembreak}[{Theorem \parencite[section~3]{holstein}}]\label{res:holstein_resolution}
	If \( \dgcatB \)~is a dg-category, then
	\( \simpdgcatB{*} \in \catdgcat[diag={\catdelta[plus,op]}] \)
	given by
	\[
		\simpdgcatB{n}
%		= \catloc[infty] { \simp{n} , \dgcatA }
%		= \catdgfun[infty,o] { \simp[dg]{n} , \dgcatA }
		= \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \dgcatB }
	\]
	is an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \). Here,
	the~“\( \mathbf{\circ} \)”
%	means an object is an
%	\ainfty-functor~\( \mf \) such that
%	\(
%		\mf[1]
%		\colon
%		\ordset{n}[linearize=\ringk,arg={i,j}]
%		\to
%		\dgcatB { \mf { i } , \mf { j } }
%	\)
%	sends non-zero maps to isomorp
	means that the objects are \ainfty-functors~\( \mf \) such
	that~\( \co[nopar]{0} { \mf } \colon \ordset{n}[lin=\ringk]\to\dgcatB[h0] \)
	sends non-zero maps to isomorphisms.
	Equivalently, in the notation of~\cref{ex:A_infty_fun_k_n_to_B},
	\( \co[nopar]{0}{\mf[ij]} \)~is an isomorphism for all~\( i<j \).
\end{theorembreak}

%As a consequence, we deduce that

%\begin{corollary}
	In other words,
	if \( \cosimpdgcatA{*} \)~is a cosimplicial system of dg-categories,
	then its homotopy limit is given by
	\[\textstyle
		\invholim[\catdelta] { \cosimpdgcatA{n} }
		=
		\End[\ordset{n}\in\catdelta[plus]] {{
			\catainftyfun[o] { {\ordset{n}[linearize=\ringk]}  , \cosimpdgcatA{n} }
		}}
		.
	\]
%\end{corollary}
We wish to evaluate this expression more explicitly:

\begin{proposition}\label{res:homotopy_limit_dgcat}
	Suppose~\( \cosimpdgcatA{*} \) is a cosimplicial system of dg-categories. Then the homotopy limit
	\(
		\invholim[\catdelta] { \cosimpdgcatA{*} }
	\)
	is the dg-category with objects~\( \tup { \algM , \mtheta } \)
	where~\(
		\mtheta = \tup { {\mtheta[n]} }[n\ge 1]
	\)
	is a collection of morphisms~%
	\(
		\mtheta[n]
		\in
		\Hom[\cosimpdgcatA{n} , d=1-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algM } }
		}
	\),
	satisfying
	\begin{equation}\label{eq:theta_n_equation}
		\dif[par] { {\mtheta[n]} }
		=
		-
		\map{\mtheta\circ\mtheta}[spar,n]
		+
		\Sum[from={i=1},to={n-1}] {{
			(-1)^{n-i}
%			\bigl(
				\coface[d=i] {{ \mtheta[n-1] }}
%				-
%				\coface[min=i] {{ \mtheta[n-i] }}
%				\circ
%				\coface[max=n-i] {{ \mtheta[i] }}
%			\bigr)
		}}
	\end{equation}
	and with \( \mtheta[1] \)~invertible in~\( \co{0} { \cosimpdgcatA{1} } \).\fxfatal{Think about possible issues in the case~\( n = 1 \)}
	The composition~\( \mtheta\circ\mtheta \)
	is evaluated via~\eqref{res:morphisms_in_tot_composition}
	below with the conventions~\( \dgcatdeg{\mtheta} = 1 \)
	and~\( \mtheta[0] = 0 \).
	A morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	of degree~\( \dgcatdeg{\malpha} \)
	is a collection~\(
		\malpha = \tup { \malpha[n] }[n\ge0]
	\)
	of morphisms~\(
		\malpha[n]
		\in
		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algN } }
		}[smash]
	\).
	The composition of two morphisms is
	\begin{equation}\label{res:morphisms_in_tot_composition}
		\map{\mbeta\circ\malpha}[spar,n]
		=
		\Sum[from={i=0},to={n}] {
			(-1)^{\dgcatdeg{\malpha}(n-i)}
			\coface[min=i,nopar] { \mbeta[n-i] }
			\circ
			\coface[max=n-i,nopar] { \malpha[i] }
		}
	.\end{equation}
	The differential on a morphism is
	\begin{equation}\label{res:morphisms_in_tot_differential}
%	\begin{split}
			\dif[par]{\malpha}[n]
%			&
			=
			\dif[par]{\malpha[n]}
			+
			\map{\meta\circ\malpha}[spar,n]
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[spar,n]
			+
			(-1)^{\dgcatdeg{\malpha}}
			\Sum[from={j=1},to={n-1}]
%				\bigl(
					(-1)^{n-j}
					\coface[d=j,nopar] { \malpha[n-1] }
					.
%		\\
%					&{}
%					\qquad
%					+			
%					(-1)^{\dgcatdeg{\malpha}(n-j)}
%					\coface[min=j,nopar] { \meta[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \malpha[j] }
%		\\
%					&{}
%					\qquad
%					-
%					(-1)^{\dgcatdeg{\malpha}}(-1)^{n-j}
%					\coface[min=j,nopar] { \malpha[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \mtheta[j] }
%					
%				\bigr)	
%		.\end{split}
	\end{equation}
%	where the compositions are evaluated
%	via~\eqref{res:morphisms_in_tot_composition}
%	with the convention~\(
%		\dgcatdeg{\mtheta}
%		=
%		\dgcatdeg{\meta}
%		=
%		1
%	\).
\end{proposition}

This proves Conjecture~1 in \textcite{explicit}.

%To prove this, recall from \cdots\fxfatal{Insert reference} that this homotopy limit is given by
%For brevity, write \( \cosimpdgcatA{n} = \catqcoh { \ssetX { n } } \).


\begin{comment}
	Following \textcite{holstein}, let us spell out
	the resolution found in \cref{res:holstein_resolution}.
	The dg-category~\( \simpdgcatB{n} \) has objects
	dg-functors~\( \mF\colon \simp[dg]{n} \to \dgcatA \)
	such that \( \mF {{ \mf[i,i+1] }} \)~is invertible
	in~\( \dgcatA[h0] \)
	for all~\( i \).
%	A morphism~\( \malpha \) of degree~\( l \) between~\( \mF \colon\simp[dg]{n}\to\dgcatA \)
%	and~\( \mG \colon \simp[dg]{n} \to \dgcatA \)
%	consists of a
%	Hochschield cochain
	The morphism space
	between \( \mF \) and~\( \mG \)
	is
	\[
		\simpdgcatB{n}[*]{ \mF , \mG }
		=
%		\coch[hoch]{*} {
%			{\ordset{n}[linearize=\ringk]} ,
%			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
%		}
%		=
		\Hom[*,par=\big] {
			{\tensorcoalg[par=\big]{{\ordset{n}[linearize=\ringk,spar,shift=-1]}}},
			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
		}
		=
		\Prod[l\ge0] {{
			\Hom[*,par=\big] {
				{ \ordset{n}[ linearize=\ringk,
					reduce,return,
					tens=l,return,shift=-l
					]
				},
				{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
			}
		}}
		.
	\]
	The composition operation is\fxfatal{Add details about this.}.
	
	
	The differential on a
	map~\( \malpha \in \simpdgcatB{n}[d=m]{ \mF , \mG } \)
	is given by
	\begin{align*}
%		\dif[output=map] { \malpha } {{
%			\mf[i_{l-1},i_l]
%			\sotimes
%			\mf[i_{l-2},i_{l-1}]
%			\sotimes\cdots\sotimes
%			\mf[i_0,i_1]
%		}}
		\MoveEqLeft
		\dif[output=map] { \malpha } { i_0 , ... , i_l }
		=
		\dif[\dgcatA,output=map] { \malpha } { i_0 ,..., i_l }
		+ \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\mG { i_j , ... , i_l }
			\circ
			\malpha { i_0 , ... , i_j }
		}}
	\\
		& {} + (-1)^{m} \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\malpha { i_j , ... , i_l }
			\circ
			\mF { i_0 , ... , i_j }
		}}
	\end{align*}
\end{comment}

\begin{proof}[Proof of \cref{res:homotopy_limit_dgcat}]
	Using \citeauthor{holstein}'s theorem, we obtain the formula
	\begin{align*}
		\MoveEqLeft
		{\textstyle \invholim[\catdelta] { \cosimpdgcatA{n} } }
		=
		\End[\ordset{n}\in\catdelta[plus]] {
			\catainftyfun[o] {
				{\ordset{n}[linearize=\ringk]} ,
				\cosimpdgcatA{n}
			}
		}
	\\
			& = \Eq[par=\Big] {{
				\Prod[\ordset{n}\in\catdelta[plus]] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{n}
					}
				}
				\rightrightarrows
				\Prod[\ordset{n}\into\ordset{m}] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{m}
					}
				}
			}}.
	\end{align*}
	%A
	%functor~\( \mF \in \catdgfun[infty,o] { \simp[dg]{n} , \cosimpdgcatA{n} } \)
	%is determined by the
	%objects~\( \mF { 0 } , \mF { 1 } , \ldots , \mF { n } \in \cosimpdgcatA{n} \)
	%and a collection of morphisms~\(
	%	\mF { \mf[i_0 i_1 \cdots i_n] }
	%\)
	We note initially that the set of objects
	of~\( \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n} } \)
	is the subset of~\( \Hom[\catdgcat] { \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} , \cosimpdgcatA{n} } \)
	of functors satisfying this unital condition.
	Thus an object of this equalizer is a
	collection~\( \mF = \tup { {\mF[d=n]} }[\ordset{n}\in\catdelta[plus]] \)
	of dg-functors~\(
		\mF[d=n]
		\colon
		\Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}}
		\to
		\cosimpdgcatA{n}
	\)
	satisfying~\(
		\mvarphi[push] \circ \mF[d=n] = \mF[d=m] \circ \mvarphi[push]
	\)
	for all~\( \mvarphi\colon\ordset{n}\into\ordset{m} \)
	in~\( \catdelta[plus] \) (in an enriched sense, it consists of natural transformations between the \( \catdelta[plus] \)-diagrams~\( \Cob[plus]{}{\Bar[plus]{}{{\ordset{\smallbullet}[linearize=\ringk]}}}\to\cosimpdgcatA{*} \)).
	Now if~\( 0 \le i \le n \), we may consider
	the map \( \mvarphi \colon \ordset{0}\into\ordset{n} \) taking \( 0 \) to~\( i \). Then
	\(
		\mF[d=n] { i }
		= \mF[d=n] { \mvarphi[push] { 0 } }
		= \mvarphi[push] { {\mF[d=0] { 0 }} }.
	\)
	Thus all the functors~\( \mF[d=n] \) are determined on the object level by the one object~\( \algM := \mF[d=0] { 0 } \in \cosimpdgcatA{0} \).
	Similarly, on the morphism level, \( \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} \)~is freely generated by the morphisms~\( \mf[i_0 i_1 \cdots i_k] \colon i_0 \to i_k \)
	with~\( 0 \le i_0 < i_1 < \cdots < i_k \le n \). But if we
	consider the map~\( \mvarphi \colon \ordset{k} \into \ordset{n} \) given
	by~\( \mvarphi{j} = i_j \), we have
	\( \mf[i_0 i_1 \cdots i_k,smash] = \mvarphi[push] { \mf[01\cdots k] } \).
	In other words, \( \mF \)~is determined on the object level by what it does to the non-degenerate morphism~\( \mf[01\cdots k] \in \Cob[plus]{}{\Bar[plus]{}{{\ordset{k}[linearize=\ringk]}}} \).
	Furthermore, these non-degenerate morphisms may be chosen freely.
	%; this follows, for instance, from the projective cofibrancy of~\( \simp[dg]{n} \) over~\( \catdelta[plus] \).
	Summarizing, the objects of this equalizer consist of the data of an element~\( \algM \in \cosimpdgcatA{0} \) and for each~\( n \) a morphism%\fxfatal{To see that these generate freely, one sees that \( \Delta^n \) is a pushout of stuff each of which has these free generators, so these generators lift freely (after applying~\( \lurie \)).}
	\[
		\mtheta[n]
		:=
		\mF[d=n] { \mf[01\cdots n] }
		\colon
		\face[max=n,shpush]{ \algM }
		\longto
		\face[min=n,shpush]{ \algM }
		.
	\]
	The differential is as stated since this is the image of the differential on~\( \mf[01\cdots n] \).
	
	%where \( \face[min=n] \) and \( \face[max=n] \) are the unique
	%morphisms~\( \ordset{0} \into \ordset{n} \)
	%given by \( \face[min=n] { 0 } = 0 \) and \( \face[max=n] { 0 } = n \).
	%In other words,
	%\( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
	%and \( \face[max=n] =  \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
	%We shall denote such pairs by~\( \tup { \algM , {\mtheta[ibullet]} } \).
	
	%On the morphism level, we claim the equalizer in question is in fact the full subcategory
	%of~\(
	%\Prod{\catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n}}}
	%\)
	%consisting of these objects
	
	On the morphism level, suppose
	%\( \tup { \algM , {\mtheta[ibullet]} } \)
	%and~\( \tup { \algN , {\meta[ibullet]} } \)
	\( \mF[d=n] \) and~\( \mG[d=n] \)
	are objects of the equalizer.
	%A morphism
	%\(
	%	\tup { \algM , {\mtheta[ibullet]} }
	%	\to
	%	\tup { \algN , {\meta[ibullet]} }
	%\)
	%consists of the
	%morphisms~
	A morphism~\( \mF[*] \to \mG[*] \)
	of degree~\( d \)
	consists of a
	collection~\(
		\malpha[*] = \tup { {\malpha[d=n]} }[\ordset{n}\in\catdelta[plus]]
	\)
	of morphisms \( \malpha[d=n] \colon \mF[d=n] \to \mG[d=n] \)
	in~\( \catainftyfun[o]{ {\ordset{n}[linearize=\ringk]},\cosimpdgcatA{n} } \) that simultaneously lie in the equalizer.
	%The space of morphisms~\( \mF[d=n] \to \mG[d=n] \) is\fxfatal{Yes, if \( \catainftyfun[o] \)~is a full subcategory of~\( \catainftyfun \).}
%	\[
%		\catainftyfun[o]{
%			{\ordset{n}[linearize=\ringk]},
%			\cosimpdgcatA{n}
%		} { {\mF[d=n]} , {\mG[d=n]} }
%		=
%		\coch[hoch]{*} {
%			{ \ordset{n}[linearize=\ringk,reduce] } ,
%			{ \cosimpdgcatA{n}[ symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%		}
%	\]
%	and thus the morphism space of transformations~\( \mF[*]\to\mG[*] \) is
	From \cref{ex:A_infty_fun_k_n_to_B}, we therefore
	get that the space of non-identity transformations~\( \mF[*]\to\mG[*] \) is
	\begin{align*}
		\MoveEqLeft
		\End {
%			\coch[hoch,par=\big]{*} {
%				{ \ordset{n}[linearize=\ringk,reduce] } ,
%				{ \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%			}
			\Hom[*,par=\big] {
				\tensorcoalg{{
					\ordset{n}[linearize=\ringk,reduce,return,shift=-1],
					\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
						\cosimpdgcatA{n}
					}
				}}
			}
		}
%	\\
		=
		\End {
			\Hom[*,par=\big,
			%{\catcom{k}[diag=\ordset{n}\times\ordset{n}]}
			] {
				%\tensorcoalg{ {\ordset{n}[linearize=\ringk,reduce]} }
				\textstyle\dirsum[limits,l\ge0,return,operator] { {\ordset{n}[linearize=\ringk,reduce,return,tens=l]} }
				,
				{
%					\cosimpdgcatA{n}[
%						symbolputleft=\!\!,
%						leftrestrict=\mF[n],
%						rightrestrict=\mG[n]
%					]
					\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
						\cosimpdgcatA{n}
					}
				}
			}
		}
	%\\
	%	&=
	%	\End[ \ordset{n}\in\catdelta[plus] ] {
	%		\Hom[\catdgcat] { \simp[dg]{n} ,  }
	%	}
	\\
		&=
		\End {
			\Prod[l\ge0] {
				\Prod[0\le i_0<\cdots<i_l\le n] {
					\Hom[*,\ringk,par=\big%,\catcom{k}
					] {
						\ringk
						\mf[i_{n-1} i_n]
						%\sotimes
						%\mf[i_{n-2} i_{n-1} ]
						\sotimes
						\cdots
						\sotimes
						\mf[ i_0 i_1 ]
						,
						{\cosimpdgcatA{n}[arg={
							{\mF[d=n] { i_0 } } ,
							{\mG[d=n] { i_n } }
						}]}
					 }
				}
			}
		}
	\end{align*}
	(note that
	%\( \ordset{n}\to \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] \)
	\(
		\ordset{n}\mapsto
		\map{ \mF[d=n]\times\mG[d=n] }[spar,qpull] {
			\cosimpdgcatA{n}
		}
	\)~defines a semicosimplicial dg-quiver).
	%This means that \( \malpha \)~is determined freely\fxfatal{Add in details}
	%by what it does to 
	%As a cosimplicial quiver, \( \ordset{n}\mapsto \tensorcoalg { \ordset{n}[linearize=\ringk,reduce] } \) is freely generated
	Thus the transformation~\( \malpha[*] \) is freely determined
	by what it does to the
	non-degenerate elements~\( \mf[n-1,n] \sotimes \cdots \sotimes \mf[0,1] \),
	i.e.\ by the
	elements
	\[
		\malpha[d=n] {{ \mf[n-1,n] \sotimes \cdots \sotimes\mf[0,1] }}
		\in
		\cosimpdgcatA{n}[arg={
			{\mF[d=n] { i_0 } } ,
			{\mG[d=n] { i_n } }
		}]
		.
	\]
	Calling this element~\( \malpha[n] \),
	we obtain the desired description.
\end{proof}

\section{Homotopy descent of dg-schemes}

\newclassset\dgschemeX{\mathbf{X}}
\newclassset\dgschemeY{\mathbf{Y}}
\newclassset\dgschemeZ{\mathbf{Z}}
\newclassset\dgschemeU{\mathbf{U}}
\newsheaf\shM{\mathscr{M}}

By a \textdef{dg-scheme}\fxfatal{Riche and friends have all kinds of extra assumptions, including Noetherian and blah blah blah, but I do not see right now what we need it for.},
we shall mean a pair~\( \dgschemeX = \tup{\setX,\dgcatA[\dgschemeX]} \),
where \( \dgcatA[\dgschemeX] \)~is a sheaf of non-positively graded,
super-commutative \( \reg[\setX] \)-dg-algebras.
A \textdef{quasi-coherent dg-sheaf} over~\( \dgschemeX \)
is a sheaf of \( \dgcatA[\dgschemeX] \)-dg-modules~\( \shM[*] \)
on~\( \setX \)
such that each graded piece~\( \shM[d=i] \)
is a quasi-coherent sheaf of \( \reg[\setX] \)-modules.
The dg-category of such is denoted~\( \catdgqcoh{\dgschemeX} \).
It is called a \textdef{coherent dg-sheaf}
if its cohomology~\( \co{*}{ \shM } \)
is a locally finitely generated as a sheaf of
graded \( \co{*}{ \dgcatA[\dgschemeX] } \)-modules.
%The dg-category of such is denoted~\( \catqcoh{\dgschemeX} \),
%and its dg-derived category is denoted~\( \der[dg]{\catqcoh{\dgschemeX}} \).
%Its homotopy category~\( \co[nopar]{0}{\der[dg]{\catqcoh{\dgschemeX}}} \)
%recovers the classical derived category~\( \der{\catqcoh{\dgschemeX}} \).
The dg-derived categories of these
are denoted~\( \der[dg,smash,nopar]{ \catdgqcoh{\dgschemeX} } \)
and~\( \der[dg,smash,nopar]{ \catdgcoh{\dgschemeX} } \).
Their homotopy categories recover the classical derived categories,
\[
	\co{0}{{ \der[dg,nopar]{ \catdgqcoh{\dgschemeX} } }}
	=
	\der[nopar]{ \catqcoh{\setX} }
\qquad\text{and}\qquad
	\co{0}{{ \der[dg,nopar]{ \catdgcoh{\dgschemeX} } }}
	=
	\der[b,nopar]{ \catcoh{\setX} }
\]

Suppose now that \( \set{ \dgschemeU[i] \to \dgschemeY } \)~is an
affine fpqc covering of a dg-scheme~\( \dgschemeY \),
and write \( \dgschemeU[i_0\cdots i_n] = \dgschemeU[i_0]\cap\cdots\cap\dgschemeU[i_n] \).
Consider the \ancech groupoid~\(
	\dgschemeX[1]
	\rightrightarrows
	\dgschemeX[0]
\)
associated to this covering
%Consider the \textdef{\ancech nerve} with respect to this covering.
%This is the internal Kan complex in affine dg-schemes
%given by~\( \dgschemeX[0] = \Coprod{ \dgschemeU[i] } \),
%\( \dgschemeX[1] = \Coprod{ \dgschemeU[ij] } \), and more generally,
and the associated classifying space, the \ancech nerve, given by
\[\textstyle
	\dgschemeX[n]
	=
	\dgschemeX[1]
	\fibre[\dgschemeX[0]]
	\dgschemeX[1]
	\fibre[\dgschemeX[0]]
	\cdots
	\fibre[\dgschemeX[0]]
	\dgschemeX[1]
	=
	\Coprod{
		\dgschemeU[i_0 i_1 \cdots i_n]
	}
\]
(we note that we do not have to take derived intersections
as the maps involved are flat).
The simplicial structure on~\( \dgschemeX[ibullet] \)
is given by the usual formula.
Then \( \catdgqcoh{\dgschemeX[ibullet]} \)~becomes
a cosimplicial system of dg-categories
via pullbacks (which are already derived because of~fpqc).
Then descent theory in derived algebraic geometry tells
us that the natural map
\[\textstyle
%	\der[dg,nopar]{
		\catdgqcoh{\dgschemeY}
%	}
	\to
	\invholim[\catdelta]{
		%\der[dg,nopar]{
			\catdgqcoh{\dgschemeX[ibullet]}
		%}
	}
\]
is a quasi-equivalence of dg-categories, the homotopy limit being taken in dg-categories.


%\begin{theorem}\label{res:A_infty_comodules}
%	%Suppose that \( \ssetX{*} \)~is a simplicial affine scheme
%	%for which all face maps~\( \face[d=i]\colon\ssetX{n}\to\ssetX{n-1} \) are flat.
%	As in the introduction, suppose that \( \ssetX{1} \rightrightarrows \ssetX{0} \)~are a monoid in affine schemes
%	such that \( \face[d=0] \) and~\( \face[d=1] \) are flat,
%	and let~\( \ssetX{*} \) be its classifying space.
%	Let~\( \algC \) be the coalgebra~\( \algC = \reg { \ssetX{1} } \)
%	over the commutative ring~\( \algA = \reg { \ssetX { 0 } } \).
%	Then we have an equivalence of categories
%	\[\textstyle
%		\invholim[\catdelta] { \catcom { \catqcoh{\ssetX{n}} } }
%		\cong
%%		\catcomod[infty,hcu,formal] { \algC }
%		\catxcomod{ \algC }[infty,hcu,formal]
%	.\]
%	%where \( \algC \)~is the coalgebra \( \algC = \reg { \ssetX{1} } \), the underlying commutative ring
%	%is~\( \algA = \reg { \ssetX { 0 } } \).
%	%\fxfatal{For unity condition, we should add flatness somewhere.}\fxfatal{{\color{red}NEED HOMOTOPY COUNITAL CONDITION!}}
%	The \anrhs denotes the dg-category of \textdef{homotopy-counital}
%	%right
%	left
%	\ainfty-comodules over~\( \algC \) in the category~\( \catxmodx{\algA}{\algA} \), which, for us, means that the second coaction map~\( \ca[2]\colon\algM\to\algC\tens[\algA]\algM \)~is
%	homotopy-invertible. The “\categoryformat{formal}”
%	part means that we omit the condition that
%	the product~\(
%		\Prod[i\ge1]{ \ca[i] }
%		\colon
%		\algM
%		\to
%		\Prod[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\)
%	factors through the direct sum~\(
%		\dirsum[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\).
%	(We hope later to find sufficient conditions under which  we can remove
%	this “\categoryformat{formal}”.)
%\end{theorem}

\begin{theorem}\label{res:A_infty_comodules}
	Suppose that
	\( \dgschemeX[1] \rightrightarrows \dgschemeX[0] \)
	is a groupoid in dg-schemes with
	source and target maps~\( \face[d=0],\face[d=1] \)
	both~fpqc, and consider the associated classifying space~\( \dgschemeX[ibullet] \).
	Write~\( \cosimpdgcatA{n} = \dgcatA[\dgschemeX[n],smash] \)
	for the associated cosimplicial system of dg-algebras.
	Let~\( \dgcatA = \cosimpdgcatA{0} \)
	and~\( \dgcatC = \cosimpdgcatA{1} \),
	and note that \( \dgcatC \)~is a
	counital
	coalgebra\fxfatal{Is it cocomplete? Also, remember to assume it is \emph{affine}, or the \( \dgcatA \)'s will only be \emph{sheaves}.} in~\( \catxdgmodx{\dgcatA}{\dgcatA} \)
	via the map~\(
		\comult
		=
		\face[d=1,comor]
		\colon
		\dgcatC
		\to
		\dgcatC\tens[\dgcatA]\dgcatC
	\).
	Then we have an equivalence of dg-categories
	\[\textstyle
		\invholim[\catdelta]{
			%\der[dg,nopar]{
				\catdgqcoh{ \dgschemeX[ibullet] }
			%}
		}
		\cong
		\catxcomod{\dgcatC}[infty,hcu,formal]{\dgcatA}
		,
	\]
	where the \anrhs denotes the dg-category
	of formal, homotopy-counital \ainfty-comodules
	over~\( \dgcatC \)
	in~\( \catxdgmod{\dgcatA} \).
\end{theorem}

%\newmap\adjunit{u}[nopar]
%
%\begin{lemma}
%	Let the assumptions be as in the theorem.
%	For any~\( n\ge 0 \),
%	we shall write~\(
%		\adjunit[d=n]
%		\colon
%		\id[\cosimpdgcatA{0}]
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] }}
%	\)
%	for the unit of adjunction.
%	If~\( \algM \in \cosimpdgcatA{0} \),
%	we wirte~\( \adjunit[d=n,\algM] \) for the
%	map~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \).
%	
%	Let \( \algM , \algN , \algP \)~be objects of~\( \cosimpdgcatA{0} \),
%	and suppose we are given maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	\)
%	in~\( \cosimpdgcatA{j} \).
%	Then
%	\[
%%		\face[max=j,shpush] {{
%%			\face[min=j,shpull] {{ \adjunit[j] { \meta } }}
%%		}}[spar]
%		\adjunit
%		\circ
%		%\adjunit[i] { \mtheta }
%		\face[max=i,shpull] { \mtheta }
%		\circ
%		\adjunit[d=i,\algM]
%		=
%		\map {
%			\face[min=i,shpull] { \meta }
%			\circ
%			\face[max=j,shpull] { \mtheta }
%		}[spar]
%		\circ
%		\adjunit[i+j]
%	\]
%\end{lemma}

%We initially consider terms of the
%form~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \).
%As in the proof of \cref{res:equivariance=comodules},
%base change will be crucial.
%Applying flat base change to the pullback diagram
%\[\begin{tikzcd}
%	\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%		& \ssetX{i} \ar[d,"{\face[min=i]}"]
%\\
%	\ssetX{j} \ar[r,"{\face[max=j]}"']
%		& \ssetX{0}
%\end{tikzcd}\]
%we obtain
%\(
%	\face[max=j,shpush] \face[min=i,shpull]
%	\cong
%	\face[min=i,shpull] \face[max=j,shpush]
%\)
%and~\(
%	\face[max=j,shpull] \face[min=i,shpush]
%	\cong
%	\face[min=i,shpush] \face[max=j,shpull]
%\).
%This implies
%
%\begin{lemma}\label{res:base_change_face_maps}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given objects~\( \algM , \algN , \algP \in \cosimpdgcatA{0} \),
%	along with two maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(\smash{
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	}\)
%	in~\( \cosimpdgcatA{j} \), where~\( i , j \ge 0 \).
%	Then the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i,shpush] {{ \face[max=i,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algN } }}
%				\ar[r]
%					\& \face[max=i,shpush] {{
%						\face[min=i,shpull] {{
%							\face[max=j,shpush] {{
%								\face[max=j,shpull] {{
%									\algN
%								}}
%							}}
%						}}
%					}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{} \ar[r,"{\meta}"']
%			\& \face[max=i,shpush] {{
%				\face[min=i,shpull] {{
%					\face[max=j,shpush] {{
%						\face[min=j,shpull] {{
%							\algP
%						}}
%					}}
%				}}
%			}}
%			\ar[r,symbol={\cong}]
%				\&[-1.5em] \face[max=i,shpush] {{
%				 \face[max=j,shpush] {{
%						\face[min=i,shpull] {{
%							\face[min=j,shpull] {{
%								\algP
%							}}
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					\&[-1.5em] \face[max=i+j,shpush] {{	
%						\face[min=(i+j),shpull] {{ \algP }}
%					}}
%	\invdot
%	\end{tikzcd}\end{align*}
%	is the same as the composition
%	\begin{align*}
%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i+j,shpush] {{
%				\face[max=(i+j),shpull] {{ \algM }}
%			}}
%			\ar[r,"{\face[max=j,shpull]{ \mtheta }}"]
%				\&\face[max=i+j,shpush] {{
%					\face[max=j,shpull] {{
%						\face[ min=i, shpull ] { \algN }
%					}}
%				}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\&{}= \face[max=i+j,shpush] {{
%			\face[min=i,shpull] {{
%				\face[ max=j, shpull ] { \algN }
%			}}
%		}}
%		\ar[r,"{\face[min=i,shpull] { \meta }}"']
%			\&\face[max=i+j,shpush] {{
%				\face[min=i,shpull] {{
%					\face[ min=j, shpull ] { \algP }
%				}}
%			}}
%			\ar[r,symbol={=}]
%				\&[-1.5em] \face[max=i+j,shpush] {{
%					\face[min=\smash{(i+j)},shpull] {{ \algP }}
%				}}
%				.
%	\end{tikzcd}\end{align*}
%	In other words, the map is
%	the unit of adjunction~\(
%		\algM
%		\to
%		\face[max=i+j,shpush] {{
%			\face[max=(i+j),shpull] { \algM }
%		}}
%	\)
%	composed with the
%	map~\(\smash{
%		\face[min=i,shpull] { \meta }
%		\circ
%		\face[max=j,shpull] { \mtheta }
%	}\).
%\end{lemma}
%
%\begin{lemma}\label{res:add_comultiplication_map}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given
%	objects~\( \algM , \algN \in \cosimpdgcatA{0} \)
%	along with a
%	map~\(
%		\mtheta
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\).
%%	Then the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta}"]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%%				\ar[r]
%%					& \face[max=n,shpush] {{
%%						\face[d=i,shpush] {{
%%							\face[d=i,shpull] {{
%%								\face[min=n,shpull] { \algN }
%%							}}
%%						}}
%%					}}
%%					\ar[r,symbol={=}]
%%						&[-1.5em]
%%						\face[min=n+1,shpush] {{
%%							\face[max=\smash{(n+1)},shpull] {{ \algN }}
%%						}} .
%%	\end{tikzcd}\]
%%	is the same as the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%			\ar[r,"{ \face[d=i,shpull] { \mtheta } }"]
%%				& \face[max=n+1,shpush] {{
%%					\face[min=(n+1),shpull] { \algN }
%%				}}
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}}
%%					\invdot
%%	\end{tikzcd}\]
%	Let~\( 1 \le i < n \).
%	Then we have a commutative diagram
%	\[\begin{tikzcd}[sep=scriptsize]
%		\algM \ar[r] \ar[d,dashed]
%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%			\ar[d,dashed]
%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%				\ar[d]
%	\\
%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%		\ar[r,dashed]
%			& \face[max=n,shpush] {{
%				\face[d=i,shpush] {{
%					\face[d=i,shpull] {{
%						\face[max=n,shpull] { \algM }
%					}}
%				}}
%			}}
%			\ar[r,"{\face[d=i,shpull]{\mtheta}}"]
%				& \face[max=n,shpush] {{
%					\face[d=i,shpush] {{
%						\face[d=i,shpull] {{
%							\face[min=n,shpull] { \algN }
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					&[-1.5em]
%					\face[max=n+1,shpush] {{
%						\face[min=\smash{(n+1)},shpull] {{ \algN }}
%					}} .
%	\end{tikzcd}\]
%\end{lemma}

\begin{proof}[Proof of \cref{res:A_infty_comodules}]
	\Cref{res:homotopy_limit_dgcat} gives us the general form
	of the homotopy limits of~\( \cosimpdgcatA{*} \),
	so we use the same notation.
%	By adjunction, the resulting
%	morphism~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\),
%	where \( n\ge 1 \),
%	is equivalent to a
%	map
%	\(
%		\algM
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%		\xto{\mtheta[n]}
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%	\).
%	We add to this collection~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
%	Putting~\( \ca[n] = \mtheta[n-1] \) for all~\( n\ge 1 \),
	Thus an object of the homotopy limit
	is a pair~\( \tup{\algM,\mtheta} \),
	where
	\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)~is
	a collection of maps~\(
		\mtheta[n]
		\colon
		\face[max=n,shpull] { \algM }
		\to
		\face[min=n,shpull] { \algM }
	\) of degree~\( 1-n \),
	and a morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	is a collection~\(
		\malpha = \tup{\malpha[n]}[n\ge0]
	\)
	of maps~\(
		\malpha[n]
		\colon
		\face[max=n,shpull]{\algM}
		\to
		\face[min=n,shpull]{\algN}
	\)
	of degree~\( \dgcatdeg{\malpha} - n \).
%	For a morphism~\(
%		\malpha
%		\colon
%		\tup{\algM,\mtheta}
%		\to
%		\tup{\algN,\meta}
%	\)
%	in the homotopy limit,
	For such a morphism,
	we scale it to define a new morphism~\( \malpha[tilde] \) by
	\(
		\malpha[tilde,n]
		=
		(-1)^{\dgcatdeg{\malpha}(n+1)}
		\malpha[n]
	\).
%	For an object~\( \tup{\algM,\mtheta} \),
%	we extend the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	by \( \mtheta[0] = \dif[\algM] \), the differential on~\( \algM \).
	Regarding this~\( \mtheta \) as a degree~\( 1 \)
	morphism~\( \tup{\algM,\mtheta}\to\tup{\algM,\mtheta} \),
	we use the same notation as for morphisms and
	write~\(
		\mtheta[tilde,n]
		=
		(-1)^{n+1}
		\mtheta[n]
	\) for~\( n\ge 1 \).
%	We also write~\( \dif[tilde,\algM] = - \dif[\algM] \).
	We notice that \eqref{res:morphisms_in_tot_composition} becomes
	\[
		\map{\mbeta\circ\malpha}[spar,widetilde,n]
		=
		\Sum[from={i=0},to={n}]{
			(-1)^{\dgcatdeg{\mbeta}i}
			\face[min=i,shpull]{{ \mbeta[tilde,n-i] }}
			\circ
			\face[max=(n-i),shpull]{{ \malpha[tilde,i] }}
		}.
	\]
	Thus
	\eqref{eq:theta_n_equation}~becomes
	%\[%\begin{equation}\label{eq:infinity_comod_theta_equation}
	\begin{align*}
		%\dif[par]{{\mtheta[tilde,n]}}
%		\MoveEqLeft
%		(-1)^{n}
%		(
%			\face[min=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		(-1)^{n+1}
		\dif[ {\face[min=n,shpull]{\algM}} ]
		\circ
		\mtheta[tilde,n]
%		-
%		(-1)^{1-n}
%	\\
%		&
%		{}
		-
		\mtheta[tilde,n]
		\circ
%		(
%			\face[max=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%		&
		=
		-
		\map{\mtheta\circ\mtheta}[widetilde,spar,n]
		+
		\Sum[from={i=1},to={n-1}]{
			%(-1)^{n-i+1}
			(-1)^{i}
			\face[d=i,shpull]{{ \mtheta[tilde,n-1] }}
		}
		.
	%\end{equation}
	%\]
	\end{align*}
	Since~\(
		\dif[par]{\malpha}[widetilde,n]
		=
		(-1)^{(\dgcatdeg{\malpha}+1)(n+1)}
		\dif[par]{\malpha}[n]
	\),
	\eqref{res:morphisms_in_tot_differential}~becomes
	\begin{align*}
			\dif[par]{\malpha}[widetilde,n]
			&
			=
			(-1)^{n+1}
			%\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
%			-
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\face[max=n,shpull]{{ \dif[tilde,\algM] }}
			\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%			&
%			\qquad
%			{}
			+
			\map{\meta\circ\malpha}[widetilde,spar,n]
	\\
			&
			\qquad
			{}
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[widetilde,spar,n]
%	\\
%			&
%			\qquad
%			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	\\
			&=
%			(-1)^n
%			\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			(-1)^{n+1}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
			+
			\Sum[from={i=0},to={n-1}]{
				(-1)^{i}
				\face[min=i,shpull]{{
					\meta[tilde,n-i]
				}}
				\circ
				\face[max=(n-i),shpull]{{
					\malpha[tilde,i]
				}}
			}
	\\
			&\qquad
			{}
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\dif[tilde,\algM]
			\dif[ {\face[max=n,shpull]{\algM}} ]
			-
			\Sum[from={i=1},to=n]{
				(-1)^{\dgcatdeg{\malpha}(i+1)}
				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
				\circ
				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
			}
	\\
			&\qquad
			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	,\end{align*}


	Now for an object~\( \tup{\algM,\mtheta} \),
	we add to the collection~\( \tup{\mtheta[n]}[n\ge1] \)
	the element~\( \mtheta[0] = -\dif[\algM] \).
	We then
%	where~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\) is a map of degree~\( 1-n \).
%	and add to the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	%add to this
%	the
%	collection~
%	and write~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
	define the comodule
	operations~\( \ca[n] \colon \algM \to \dgcatC[tens=(n-1)]\tens\algM \)
	of degree~\( 2 - n \)
	by
	\[\begin{tikzcd}%[sep=scriptsize]
		\ca[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\mtheta[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
	\end{tikzcd}\]
	where the first map is the unit of adjunction.
	In particular, \( \ca[1] = -\dif[\algM] \).	
	Similarly, if
	\( \malpha \colon \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
	is a map of degree~\( \dgcatdeg{\malpha} \),
%	where
%	\(
%		\malpha[n]
%		\in
%		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n]{
%			{\face[max=n,shpull]{\algM}},
%			{\face[min=n,shpull]{\algM}}
%		}
%	\),
	we associate to it
	the map of \ainfty-comodules~\(
		\mf \colon \algM \to \algN
	\)
	of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \),
	where
	\(
		\mf[n]
		\colon
		\algM
		\to
		\dgcatC[tens=(n-1)]\tens[\dgcatA] \algN
	\)
	is the map of degree~\(
		\dgcatdeg{\malpha} + 1 - n
		=
		\dgcatdeg{\mf} + 1 - n
	\)
	given by
	\[\begin{tikzcd}%[sep=scriptsize]
		\mf[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\malpha[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algN } }}
		.
	\end{tikzcd}\]
	It is immediate that the composition map above
	agrees with the composition of maps of \ainfty-comodules.
%	Now the two lemmas show that the above two equations are exactly the
%	\ainfty-comodule equations.
	%Via the two lemmas,
	Via~\cref{res:add_comultiplication_map,res:base_change_face_maps},
	the other two equations above now become
	\begin{align*}
		\MoveEqLeft
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[\algM]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\ca[n+1]
		+
		\ca[n+1]
		%\dif[\algM]
		\ca[1]
	\\
		&
		=
		-
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			( \id[ {\dgcatC[tens=i]} ]\tens\ca[n-i+1] )
			\ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			(
				\id[tens=(i-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-i)]
			)
			\ca[n]
		}
	\\
	\shortintertext{and}
		\dif{\mf}[spar,n]
		&
		=
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[N]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\mf[n+1]
		+
		\Sum[from={i=0},to={n-1}]{
			(-1)^{i}
			\ca[n-i+1] \mf[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		(-1)^{\dgcatdeg{\malpha}}
		\mf[n+1]\ca[1]
		-
		\Sum[from={i=1},to={n}]{
			(-1)^{\dgcatdeg{\malpha}(i+1)}
			\mf[n-i+1] \ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={j=1},to={n-1}]{
			(-1)^{j-1}
			(
				\id[tens=(j-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-j)]
			)
			\ca[n]
		},
	\end{align*}
	which are exactly the \ainfty-comodule equations from earlier.	
%	For all objects~\( \tup{\algM,\mtheta} \),
%	we now extend the collection~\( \mtheta = \tup{\mtheta}[n\ge1] \)
%	by~\( \mtheta[0] = \dif[\algM] \).
%	Following the above convention with~\( \mtheta[tilde,n] \),
%	this allows us to write~\( \mtheta[tilde,0] = - \mtheta[0] = \dif[tilde,\algM] \).
%	Then the two above equations become
%	\[
%		0
%		=
%		\Sum[from={i=0},to={n}]{
%			(-1)^{i}
%			\face[min=i,shpull]{{ \mtheta[tilde,n-i] }}
%			\circ
%			\face[max=(n-i),shpull] {{ \mtheta[tilde,i] }}
%		}
%		+
%		\Sum[from={i=1},to={n-1}]{
%			(-1)^{i-1}
%			\face[d=i,shpull]{{
%				\mtheta[tilde,n-1]
%			}}
%		}
%	\]
%	and
%	\begin{align*}
%			\dif{\malpha}[widetilde,spar,n]
%			&=
%			\Sum[from={i=0},to={n}]{
%				(-1)^{i}
%				\face[min=i,shpull]{{
%					\meta[tilde,n-i]
%				}}
%				\circ
%				\face[max=(n-i),shpull]{{
%					\malpha[tilde,i]
%				}}
%			}
%	\\
%			&
%			{}
%			-
%			\Sum[from={i=0},to=n]{
%				(-1)^{\dgcatdeg{\malpha}(i+1)}
%				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
%				\circ
%				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
%			}
%			+
%			\Sum[from={j=1},to={n-1}]
%				(-1)^{j-1}
%				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
%	\end{align*}

	To verify that we get exactly \emph{homotopy-counital} \ainfty-cmodules,
	we notice that the
	equation~\eqref{eq:theta_n_equation}
	in the case~\( n = 2 \) yields that
	\[
		\dif[par]{\mtheta[2]}
		=
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		-
		\face[d=1,shpull]{\mtheta[1]}
		,
	\]
	so that we have a homotopy~\(
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		\simeq
		\face[d=1,shpull]{\mtheta[1]}
	\).
	Then the proof of \cref{res:cocycle_iff_degen=0},
	with equalities replaced by homotopies,
	shows that \( \mtheta[1] \)~being an isomorphism is equivalent to~\( \degen[d=0,shpull]{\mtheta[1]}\simeq\id \).
	Similarly, one adjusts the
	last part of the proof of \cref{res:descent=comodules}
	to obtain that~\(
		(\counit\tens\id[\algM])\ca[2]
		\simeq
		\id
	\),
	which means that \( \algM \)~is homotopy-counital.
\end{proof}


%	
%	We initially check that the maps~\( \ca[n] \colon \algM \to \algC[tens=(n-1)] \tens \algM \),
%%	so let us for~\( k\ge 1 \) check the equation
%%	\[
%%		\Sum {
%%			(-1)^{i+mj}
%%			(
%%				\id[tens=i] \tens \comult[m] \tens \id[tens=j]
%%			)
%%			\ca[n]
%%		}
%%		= 0
%%	\]
%%	for all~\( i,m,j,n \) such that
%%	\( i + m + j = k \)
%%	and~\( n = i + 1 + j \),
%%	and where we, in the case~\( j=0 \),
%	satisfy the equations for an \ainfty-comodule,
%	so let us for all~\( k\ge 1 \) check the equation
%	\[
%		\Sum {
%			(-1)^{(i-1)+m(n-i)}
%			(
%				\id[tens=(i-1)] \tens \comult[m] \tens \id[tens=(n-i)]
%			)
%			\ca[n]
%		}
%		= 0 ,
%	\]
%	where the sum runs over the positive
%	integers~\( i, m, n \) such
%	that~\( 0\le i\le n\)
%	and~\( n + m - 1 = k \)
%	and where we, in the
%	case~\( i=n \),
%	interpret \( \comult[m] \) as~\( \ca[m] \).
%	%In other words, the sum has
%	%By base change, we obtain
%	%In other words, the sum consists
%	We notice that the term~\( m(n-i) \) in the exponent
%	of the sign is always even. Indeed,
%	if~\( n-i > 0 \), then \( \comult[m] = \comult[m,upper=\algC] \)~is the \ainfty-operation
%	on~\( \algC \), and so \( \comult[m,upper=\algC] = 0 \)
%	unless~\( m = 2 \). Thus we are left with~\( (-1)^{i-1} \).
%	%Also, in order to rewrite this equation in terms
%	%of the maps~\( \mtheta[n] \), it is convenient to replace
%%	\( n , m \) by~\( n+1 , m+1 \),
%%	so we are left with the equation
%%	\[
%%%		\Sum[i={m+n-1 = k} ] {{
%%			\Sum[from={i=1},to={k-1}] {{
%%				(-1)^i
%%				\bigl(
%%					(
%%						\id[tens=(i-1)]
%%						\tens
%%						\comult[2,upper=\algC]
%%						\tens
%%						\id[tens=(n-i)]
%%					) \ca[(k-2)+1]
%%					-
%%					abe
%%				\bigr)
%%			}}
%%			=0
%%%		}}
%%	\]
%%	for all~\( k\ge 1 \).
%	Thus the equation may be reduced to
%	\begin{align*}
%		0
%			&=
%			\Sum[from={n=1},to={k}] {{
%				(-1)^{n-1}
%				(
%					\id[tens=(n-1)]
%					\tens
%					\ca[k+1-n]
%				)
%				\ca[n]
%			}}
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(k-i-1)]
%				)
%				\ca[k-1]
%			}}
%	\\
%			&=
%			\ca[k]\circ\ca[1]
%			- (-1)^{k} (\id[tens=(k-1)]\tens\ca[1]) \ca[k]
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				\bigl(
%					(
%						\id[tens=(i-1)]
%						\tens
%						\comult[2,upper=\algC]
%						\tens
%						\id[tens=(k-i-1)]
%					)
%					\ca[k-1]
%					-
%					(
%						\id[tens=i]
%						\tens
%						\ca[k-i]
%					)
%					\ca[i+1]
%				\bigr)
%			}}
%	\end{align*}
%%	Since the differential on~\( \algC \) is zero and \( \ca[1] = \dif[\algM] \), the first
%%	two terms are
%%	simply~\(
%%		-
%%		(-1)^{2-k}
%%		\dif[par] { \ca[k] }
%%	\).
%	Substituting \( n+1 \) for~\( k \), we obtain
%	that the equation we must verify is
%	\begin{align*}
%%		\dif[par] { \ca[n+1] }
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%		&=
%		\Sum[from={i=1},to={n-1}]
%			(-1)^{n-i}
%			\bigl(
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(n-i)]
%				)
%				\ca[n]
%	\\&
%		\qquad\qquad
%				{}-
%				(
%					\id[tens=i]
%					\tens
%					\ca[n-i+1]
%				)
%				\ca[i+1]
%			\bigr)
%		.
%	\end{align*}
%	This equation is very similar
%	%to the one in~\cref{res:homotopy_limit_dgcat},
%	to~\eqref{eq:theta_n_equation},
%	and we shall indeed derive it from that equation. Specifically, we claim that it is obtained
%	from~\eqref{eq:theta_n_equation} by composing
%	with \( (-1)^{n+2} = (-1)^{n} \) times the
%	unit~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \),
%	and we show this by comparing each term individually.
%	
%	We initially consider the
%	term~\(
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%	\).
%	We get by~\cref{res:base_change_face_maps}
%	that
%	this is exactly the unit~\(
%		\algM \to
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{ \algM }
%		}}
%	\)
%	composed with
%	\[
%		(-1)
%		\face[min=n,shpush]{\dif[\algM]}
%		\circ
%		(-1)^{n+1}
%		\mtheta[n]
%		-
%		(-1)^{1-n}
%		(-1)^{n+1}
%		\mtheta[n]
%		\circ
%		(-1)
%		\dif[\algM]
%		=
%		(-1)^{n}
%		\dif[par]{\mtheta[n]}
%		.
%	\]
%	This is exactly \( (-1)^n \)~times the left-hand side
%	term in~\eqref{eq:theta_n_equation}, as claimed.
%	
%	We next consider terms of the
%	form~\( ( \id[tens=i] \tens \ca[n-i+1] ) \ca[i+1] \).
%%	We proceed much as in the proof of \cref{res:equivariance=comodules}.
%%	Applying flat base change to the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%%			& \ssetX{i} \ar[d,"{\face[min=i]}"]
%%	\\
%%		\ssetX{j} \ar[r,"{\face[max=j]}"']
%%			& \ssetX{0}
%%	\end{tikzcd}\]
%%	we obtain
%%	\(
%%		\face[max=j,shpush] \face[min=i,shpull]
%%		\cong
%%		\face[min=i,shpull] \face[max=j,shpush]
%%	\)
%%	and~\(
%%		\face[max=j,shpull] \face[min=i,shpush]
%%		\cong
%%		\face[min=i,shpush] \face[max=j,shpull]
%%	\).\fxfatal{As stated, this diagram is WRONG!!}
%%	This allows us to
%%	rewrite the term~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \)
%%	as
%%	\begin{align*}\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=n,shpush] {{ \face[max=i,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[i]}"]
%%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algM } }}
%%				\ar[r]
%%					\& \face[max=i,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[max=j,shpush] {{
%%								\face[max=j,shpull] {{
%%									\algM
%%								}}
%%							}}
%%						}}
%%					}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		{} \ar[r,"{\mtheta[j]}"]
%%			\& \face[max=i,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[max=j,shpush] {{
%%						\face[min=j,shpull] {{
%%							\algM
%%						}}
%%					}}
%%				}}
%%			}}
%%			\ar[r,symbol={\cong}]
%%				\&[-1.5em] \face[max=i,shpush] {{
%%					 \face[max=j,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[min=j,shpull] {{
%%								\algM
%%							}}
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					\&[-1.5em] \face[max=i+j,shpush] {{	
%%						\face[min=(i+j),shpull] {{ \algM }}
%%					}}
%%	\invdot
%%	\end{tikzcd}\end{align*}
%%	the isomorphism being by base change.
%%	In other words, the composed
%%	map~\(
%%		( \id[tens=i]\tens\ca[j+1] )
%%		\ca[i+1]
%%	\)
%%	is the same as the map
%%	\begin{align*}
%%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=i+j,shpush] {{
%%				\face[max=(i+j),shpull] {{ \algM }}
%%			}}
%%			\ar[r,"{\face[max=j,shpull]{ \mtheta[i] }}"]
%%				\&\face[max=i+j,shpush] {{
%%					\face[max=j,shpull] {{
%%						\face[ min=i, shpull ] { \algM }
%%					}}
%%				}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\&{}= \face[max=i+j,shpush] {{
%%			\face[min=i,shpull] {{
%%				\face[ max=j, shpull ] { \algM }
%%			}}
%%		}}
%%		\ar[r,"{\face[min=i,shpull] { \mtheta[j] }}"]
%%			\&\face[max=i+j,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[ min=j, shpull ] { \algM }
%%				}}
%%			}}
%%			\ar[r,symbol={=}]
%%				\&[-1.5em] \face[max=i+j,shpush] {{
%%					\face[min=\smash{(i+j)},shpull] {{ \algM }}
%%				}}
%%				.
%%	\end{tikzcd}\end{align*}
%	By~\cref{res:base_change_face_maps},
%%	this map is the same as
%%	\( (-1)^{k+1} \) times the unit of adjunction~\(
%%		\algM
%%		\to
%%		\face[max=i+j,shpush] {{
%%			\face[max=(i+j),shpull] { \algM }
%%		}}
%%	\)
%%	composed with the
%%	term~\(
%%		\face[min=i,shpull] { \mtheta[j] }
%%		\circ
%%		\face[max=j,shpull] { \mtheta[i] }
%%	\)
%%	this is the same as the map
%%	\[\begin{tikzcd}%[sep=scriptsize]
%%		\algM
%%		\ar[r]
%%		&
%%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%		\ar[r,"{
%%			(-1)^{n-i+1}
%%			\face[min=i,shpull]{\mtheta[n-i]}
%%			\circ
%%			(-1)^{i+1}
%%			\face[max=(n-i),shpull]{\mtheta[i]}
%%		}"]
%%		&[7em]
%%		\face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%	\end{tikzcd}\]
%	this is the same as
%	the unit~\(
%		\algM
%		\to
%		\face[max=n,shpush]
%		\face[max=n,shpull]
%		\algM
%	\)
%	composed with
%	\[
%		(-1)^{n-i+1}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		(-1)^{i+1}
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		=
%		(-1)^{n}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		.
%	\]
%	This is \( (-1)^{n} \)~times one of the terms
%	on the right-hand side of~\eqref{eq:theta_n_equation}, as claimed.
%	
%	
%%	Similarly, we consider the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{n+1} \ar[r] \ar[d] & \ssetX{n} \ar[d]
%%	\\
%%		\ssetX{1} \ar[r] & \ssetX{0}
%%	\end{tikzcd}\]
%	Finally, we consider terms of the
%	form~\(
%		( \id[tens=(i-1)] \tens \comult[2] \tens \id[tens=(n-i)] ) \ca[n]
%		=
%		( \id[tens=(i-1)] \tens \comult[\algC] \tens \id[tens=(n-i)] ) \ca[n]
%	\) where~\( n-i> 0 \).
%	These are given by the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
%			\ar[r,"{(-1)^{n}\mtheta[n-1]}"]
%				\&[1.3em]
%				%\&
%				\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
%	\end{tikzcd}
%	\\[-.7em]
%	&
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{}
%				\ar[r]
%					\& \face[max=n-1,shpush] {{
%						\face[d=i,shpush] {{
%							\face[d=i,shpull] {{
%								\face[min=(n-1),shpull] { \algM }
%							}}
%						}}
%					}}
%					\ar[r,symbol={=}]
%						\&[-1.5em]
%						\face[min=n,shpush] {{
%							\face[max=n,shpull] {{ \algM }}
%						}} .
%	\end{tikzcd}
%	\end{align*}
%%	This map factors as
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r] \ar[d,dashed]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[n]}"]
%%			\ar[d,dashed]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%				\ar[d]
%%	\\
%%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%		\ar[r,dashed]
%%			& \face[max=n,shpush] {{
%%				\face[d=i,shpush] {{
%%					\face[d=i,shpull] {{
%%						\face[max=n,shpull] { \algM }
%%					}}
%%				}}
%%			}}
%%			\ar[r,"{\face[d=i,shpull]{\mtheta[n]}}"]
%%				& \face[max=n,shpush] {{
%%					\face[d=i,shpush] {{
%%						\face[d=i,shpull] {{
%%							\face[min=n,shpull] { \algM }
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}} .
%%	\end{tikzcd}\]
%	According to \cref{res:add_comultiplication_map}, this map
%	is the same as the
%	unit~\(
%		\algM
%		\to
%		\face[max=n+1,shpush] {{
%			\face[max=(n+1),shpull] { \algM }
%		}}
%	\)
%	composed with~\( (-1)^{n} \face[d=i,shpull] { \mtheta[n] } \).
%	This is again~\( (-1)^{n} \) times a term
%	from~\eqref{eq:theta_n_equation}, as claimed.
%	
%	With regards to th morphisms, suppose
%	that \( \malpha = \tup{\malpha[n]}[n\ge0] \)
%	is a
%	morphism~\( \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
%	of degree~\( \dgcatdeg{\malpha} \).
%	This consists of
%	maps~\(
%		\malpha[n]
%		\in
%		\Hom[d={\dgcatdeg{\malpha}-n}]{
%			{\face[max=n,shpull]{\algM}} ,
%			{\face[min=n,shpull]{\algN}}
%		}
%	\).
%	We use this to define a
%	map~\( \mf \colon \algM \to \algN \)
%	of \ainfty-comodules of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \).
%	For all~\( n\ge1 \), let~\( \mf[n] \colon \algM \to \algC[tens=(n-1)]\tens\algN \)
%	be the composition
%	\[\begin{tikzcd}
%		\algM
%		\ar[r]
%		&
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{\algM}
%		}}
%		\ar[r,"{
%			(-1)^{\dgcatdeg{\malpha}(n-1)}
%			\malpha[n-1]
%		}"]
%		&[4em]
%		\face[max=n,shpush]{{
%			\face[min=n,shpull]{\algN}
%		}}
%	\end{tikzcd}\]
%	
%	Proving that the morphisms inside our dg-category agree
%	with the morphisms
%	inside the dg-category~\( \catxcomod{\algC}[infty,hcu,formal] \)
%	amounts to showing that the equation~\eqref{res:morphisms_in_tot_differential}
%	agrees with the equation for a map of \ainfty-comodules
%	and that \eqref{res:morphisms_in_tot_composition}
%	agrees with the compositions.
%	This is similar acrobatics using the two lemmas above,
%	and we omit it. The homotopy counital condition is equivalent
%	to the condition that \( \mtheta[1] \)~is homotopy-invertible.
%\end{proof}

\endgroup

==> holim_dgcat/holim_dgcat_5010.tex <==
\begingroup

\chapter{Homotopy limits in dg-categories}

%\section{Framings in dg-categories}
%
%A framing on the category~\( \catdgcat \) is due to
%\textcite{holstein}: If \( \dgcatA \in \catdgcat \) and \( \ssetK\in\catsset \), then let
%\(
%	\dgcatA[powering=\ssetK]
%	=
%	\catloc { \ssetK, \dgcatA }
%	=
%	\catdgfun[infty,o] { \lurie{\ssetK} , \dgcatA }
%\).

%\begin{parabreak}[Tabuada's model structure on~\( \catdgcat \)]
	Given a dg-category~\( \dgcatA \), we denote by~\( \dgcatA[z0] \) the dg-category with the same objects as~\( \dgcatA \), but with hom complexes given by
	\(
		%\Hom[ \dgcatA[z0] ] { \vx, \vy } =
		%\cocy[nopar]{0} { \Hom[\dgcatA, * ] { \vx, \vy } }
		\dgcatA[z0,spar] { \vx , \vy } = \cocy{0} { \dgcatA { \vx , \vy } }
	\),
	the set of closed maps~\( \vx \to \vy \) in~\( \dgcatA \). We define~\( \dgcatA[h0] \) analogously.
	A map~\( \mf \in \dgcatA[d=0]{ \vx , \vy } \) in~\( \dgcatA \) is called a \textdef{homotopy equivalence} if its image in~\( \dgcatA[h0] \) is an isomorphism. As in homological algebra, this amounts the existence of a map \( \mg \in \dgcatA[d=0] { \vy , \vx } \) in the other direction along with correcting morphisms \( \mr[\vx] \in \dgcatA[d=-1] { \vx , \vx } \) and \( \mr[\vy] \in \dgcatA[d=-1] { \vy , \vy } \) such that
	\[
		\dif{ \mr[\vx] } = \mg \mf - \id[\vx]
		\qquad\text{and}\qquad
		\dif{ \mr[\vy] } = \mf \mg - \id[\vy].
	\]

	We recall from
	\textcite{tabuada,tabuada_dgcats_vs_simplicial_cats}
	the existence of a model structure on the \( 1 \)-category~\( \catdgcat \) with
	\begin{itemize}
		\item weak equivalences given by \textdef{quasi-equivalences}, i.e.
		functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
		\item the induced functor~\( \mF[parent=alg,h0] \colon \dgcatA[h0] \to \dgcatB[h0] \) is an equivalence of categories in the classical, non-enriched sense;
		\item for all~\( \vx, \vy \in \dgcatA \),
		\( \mF[\vx, \vy] \colon
		\dgcatA { \vx , \vy } \to \dgcatB { \mF { \vx } , \mF { \vy } } \)
		is a quasi-isomorphism of chain complexes;
		\end{enumerate}
		\item fibrations given by dg-functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
			\item the induced map
			\(
				\mF \colon
				\dgcatA[*] { \vx, \vy }
				\to
				\dgcatB[*] { \mF { \vx } , \mF { \vy } }
			\)
			is surjective for all objects~\( \vx, \vy \in \dgcatA \), and
			\item any map \( \mf \colon \mF { \vx } \to \vy \) in~\( \dgcatB \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatB } \) lifts as \( \mf = \mF { \mg } \) for some morphism \( \mg\colon \vx \to \vx[prime] \) in~\( \dgcatA \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatA } \).
		\end{enumerate}
	\end{itemize}
%	It is cofibrantly generated,
%	with
%	\begin{itemize}
%		\item the class~\( \setgencof \) consisting of the morphism \( \varnothing \into \ringk \)
%		\item the class~\( \setgentrivcof \)
%	\end{itemize}
	This model structure is combinatorial according to
	\textcite[Proposition~1.3.1.19]{ha}.
%\end{parabreak}

We shall use the tools developed in the preceding chapters to develop a notion of homotopy descent of quasi-coherent sheaves on affine schemes.
%We write \( \face[min=n] \) and~\( \face[max=n] \) for the two unique morphisms~\( \ordset{0} \into \ordset{n} \) in~\( \catdelta \) given by
%\( \face[min=n] { 0 } = 0 \) and~\( \face[max=n] { 0 } = n \).
%In other words, \( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
%and~\( \face[max=n] = \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
Much of the inspiration is from \textcite{explicit};
however, using the tools developed earlier
(specifically~\cref{ex:A_infty_fun_k_n_to_B}),
we are able to solve their Conjecture~1 and prove their
results in complete generality.



%\begin{theorem}
%	Suppose that \( \ssetX{*} \)~is a simplicial affine scheme with each~\( \ssetX{n} \) being regular and each \( \ssetX{n}\to \ssetX{m} \) flat surjective\fxfatal{This is supposed to be the same as faithfully flat, check this.}.
%	Then we have an equivalence of categories
%	\(
%		\invholim[\catdelta] { \catqcoh{\ssetX{n}} }
%		\cong
%		\catainftycomod { \catqcoh { \ssetX{0} } }
%	\).
%\end{theorem}

Recall from \cref{res:fat_tot} that
the homotopy limit of a \( \catdelta \)-diagram in~\( \catdgcat \) is given by
\[\textstyle
	\invholim[\catdelta] { \cosimpdgcatA{n} }
	=
	\invholim[\catdelta[plus]] { \cosimpdgcatA{n} }
	=
	\End[\ordset{n}\in\catdelta[plus]] { \fibrep[deltaplus] { \cosimpdgcatA{n} }{n} }
\]
where \( \fibrep[deltaplus] \colon \catdgcat\to\catdgcat[diag={\catdelta[plus,op]},inj,smash] \) is a fibrant replacement functor, taking a dg-category~\( \dgcatB \) to an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \).
We obtain such a functor from Holstein:

\begin{theorembreak}[{Theorem \parencite[section~3]{holstein}}]\label{res:holstein_resolution}
	If \( \dgcatB \)~is a dg-category, then
	\( \simpdgcatB{*} \in \catdgcat[diag={\catdelta[plus,op]}] \)
	given by
	\[
		\simpdgcatB{n}
%		= \catloc[infty] { \simp{n} , \dgcatA }
%		= \catdgfun[infty,o] { \simp[dg]{n} , \dgcatA }
		= \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \dgcatB }
	\]
	is an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \). Here,
	the~“\( \mathbf{\circ} \)”
%	means an object is an
%	\ainfty-functor~\( \mf \) such that
%	\(
%		\mf[1]
%		\colon
%		\ordset{n}[linearize=\ringk,arg={i,j}]
%		\to
%		\dgcatB { \mf { i } , \mf { j } }
%	\)
%	sends non-zero maps to isomorp
	means that the objects are \ainfty-functors~\( \mf \) such
	that~\( \co[nopar]{0} { \mf } \colon \ordset{n}[lin=\ringk]\to\dgcatB[h0] \)
	sends non-zero maps to isomorphisms.
	Equivalently, in the notation of~\cref{ex:A_infty_fun_k_n_to_B},
	\( \co[nopar]{0}{\mf[ij]} \)~is an isomorphism for all~\( i<j \).
\end{theorembreak}

%As a consequence, we deduce that

%\begin{corollary}
	In other words,
	if \( \cosimpdgcatA{*} \)~is a cosimplicial system of dg-categories,
	then its homotopy limit is given by
	\[\textstyle
		\invholim[\catdelta] { \cosimpdgcatA{n} }
		=
		\End[\ordset{n}\in\catdelta[plus]] {{
			\catainftyfun[o] { {\ordset{n}[linearize=\ringk]}  , \cosimpdgcatA{n} }
		}}
		.
	\]
%\end{corollary}
We wish to evaluate this expression more explicitly:

\begin{proposition}\label{res:homotopy_limit_dgcat}
	Suppose~\( \cosimpdgcatA{*} \) is a cosimplicial system of dg-categories. Then the homotopy limit
	\(
		\invholim[\catdelta] { \cosimpdgcatA{*} }
	\)
	is the dg-category with objects~\( \tup { \algM , \mtheta } \)
	where~\(
		\mtheta = \tup { {\mtheta[n]} }[n\ge 1]
	\)
	is a collection of morphisms~%
	\(
		\mtheta[n]
		\in
		\Hom[\cosimpdgcatA{n} , d=1-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algM } }
		}
	\),
	satisfying
	\begin{equation}\label{eq:theta_n_equation}
		\dif[par] { {\mtheta[n]} }
		=
		-
		\map{\mtheta\circ\mtheta}[spar,n]
		+
		\Sum[from={i=1},to={n-1}] {{
			(-1)^{n-i}
%			\bigl(
				\coface[d=i] {{ \mtheta[n-1] }}
%				-
%				\coface[min=i] {{ \mtheta[n-i] }}
%				\circ
%				\coface[max=n-i] {{ \mtheta[i] }}
%			\bigr)
		}}
	\end{equation}
	and with \( \mtheta[1] \)~invertible in~\( \co{0} { \cosimpdgcatA{1} } \).\fxfatal{Think about possible issues in the case~\( n = 1 \)}
	The composition~\( \mtheta\circ\mtheta \)
	is evaluated via~\eqref{res:morphisms_in_tot_composition}
	below with the conventions~\( \dgcatdeg{\mtheta} = 1 \)
	and~\( \mtheta[0] = 0 \).
	A morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	of degree~\( \dgcatdeg{\malpha} \)
	is a collection~\(
		\malpha = \tup { \malpha[n] }[n\ge0]
	\)
	of morphisms~\(
		\malpha[n]
		\in
		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algN } }
		}[smash]
	\).
	The composition of two morphisms is
	\begin{equation}\label{res:morphisms_in_tot_composition}
		\map{\mbeta\circ\malpha}[spar,n]
		=
		\Sum[from={i=0},to={n}] {
			(-1)^{\dgcatdeg{\malpha}(n-i)}
			\coface[min=i,nopar] { \mbeta[n-i] }
			\circ
			\coface[max=n-i,nopar] { \malpha[i] }
		}
	.\end{equation}
	The differential on a morphism is
	\begin{equation}\label{res:morphisms_in_tot_differential}
%	\begin{split}
			\dif[par]{\malpha}[n]
%			&
			=
			\dif[par]{\malpha[n]}
			+
			\map{\meta\circ\malpha}[spar,n]
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[spar,n]
			+
			(-1)^{\dgcatdeg{\malpha}}
			\Sum[from={j=1},to={n-1}]
%				\bigl(
					(-1)^{n-j}
					\coface[d=j,nopar] { \malpha[n-1] }
					.
%		\\
%					&{}
%					\qquad
%					+			
%					(-1)^{\dgcatdeg{\malpha}(n-j)}
%					\coface[min=j,nopar] { \meta[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \malpha[j] }
%		\\
%					&{}
%					\qquad
%					-
%					(-1)^{\dgcatdeg{\malpha}}(-1)^{n-j}
%					\coface[min=j,nopar] { \malpha[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \mtheta[j] }
%					
%				\bigr)	
%		.\end{split}
	\end{equation}
%	where the compositions are evaluated
%	via~\eqref{res:morphisms_in_tot_composition}
%	with the convention~\(
%		\dgcatdeg{\mtheta}
%		=
%		\dgcatdeg{\meta}
%		=
%		1
%	\).
\end{proposition}

This proves Conjecture~1 in \textcite{explicit}.

%To prove this, recall from \cdots\fxfatal{Insert reference} that this homotopy limit is given by
%For brevity, write \( \cosimpdgcatA{n} = \catqcoh { \ssetX { n } } \).


\begin{comment}
	Following \textcite{holstein}, let us spell out
	the resolution found in \cref{res:holstein_resolution}.
	The dg-category~\( \simpdgcatB{n} \) has objects
	dg-functors~\( \mF\colon \simp[dg]{n} \to \dgcatA \)
	such that \( \mF {{ \mf[i,i+1] }} \)~is invertible
	in~\( \dgcatA[h0] \)
	for all~\( i \).
%	A morphism~\( \malpha \) of degree~\( l \) between~\( \mF \colon\simp[dg]{n}\to\dgcatA \)
%	and~\( \mG \colon \simp[dg]{n} \to \dgcatA \)
%	consists of a
%	Hochschield cochain
	The morphism space
	between \( \mF \) and~\( \mG \)
	is
	\[
		\simpdgcatB{n}[*]{ \mF , \mG }
		=
%		\coch[hoch]{*} {
%			{\ordset{n}[linearize=\ringk]} ,
%			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
%		}
%		=
		\Hom[*,par=\big] {
			{\tensorcoalg[par=\big]{{\ordset{n}[linearize=\ringk,spar,shift=-1]}}},
			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
		}
		=
		\Prod[l\ge0] {{
			\Hom[*,par=\big] {
				{ \ordset{n}[ linearize=\ringk,
					reduce,return,
					tens=l,return,shift=-l
					]
				},
				{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
			}
		}}
		.
	\]
	The composition operation is\fxfatal{Add details about this.}.
	
	
	The differential on a
	map~\( \malpha \in \simpdgcatB{n}[d=m]{ \mF , \mG } \)
	is given by
	\begin{align*}
%		\dif[output=map] { \malpha } {{
%			\mf[i_{l-1},i_l]
%			\sotimes
%			\mf[i_{l-2},i_{l-1}]
%			\sotimes\cdots\sotimes
%			\mf[i_0,i_1]
%		}}
		\MoveEqLeft
		\dif[output=map] { \malpha } { i_0 , ... , i_l }
		=
		\dif[\dgcatA,output=map] { \malpha } { i_0 ,..., i_l }
		+ \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\mG { i_j , ... , i_l }
			\circ
			\malpha { i_0 , ... , i_j }
		}}
	\\
		& {} + (-1)^{m} \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\malpha { i_j , ... , i_l }
			\circ
			\mF { i_0 , ... , i_j }
		}}
	\end{align*}
\end{comment}

\begin{proof}[Proof of \cref{res:homotopy_limit_dgcat}]
	Using \citeauthor{holstein}'s theorem, we obtain the formula
	\begin{align*}
		\MoveEqLeft
		{\textstyle \invholim[\catdelta] { \cosimpdgcatA{n} } }
		=
		\End[\ordset{n}\in\catdelta[plus]] {
			\catainftyfun[o] {
				{\ordset{n}[linearize=\ringk]} ,
				\cosimpdgcatA{n}
			}
		}
	\\
			& = \Eq[par=\Big] {{
				\Prod[\ordset{n}\in\catdelta[plus]] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{n}
					}
				}
				\rightrightarrows
				\Prod[\ordset{n}\into\ordset{m}] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{m}
					}
				}
			}}.
	\end{align*}
	%A
	%functor~\( \mF \in \catdgfun[infty,o] { \simp[dg]{n} , \cosimpdgcatA{n} } \)
	%is determined by the
	%objects~\( \mF { 0 } , \mF { 1 } , \ldots , \mF { n } \in \cosimpdgcatA{n} \)
	%and a collection of morphisms~\(
	%	\mF { \mf[i_0 i_1 \cdots i_n] }
	%\)
	We note initially that the set of objects
	of~\( \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n} } \)
	is the subset of~\( \Hom[\catdgcat] { \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} , \cosimpdgcatA{n} } \)
	of functors satisfying this unital condition.
	Thus an object of this equalizer is a
	collection~\( \mF = \tup { {\mF[d=n]} }[\ordset{n}\in\catdelta[plus]] \)
	of dg-functors~\(
		\mF[d=n]
		\colon
		\Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}}
		\to
		\cosimpdgcatA{n}
	\)
	satisfying~\(
		\mvarphi[push] \circ \mF[d=n] = \mF[d=m] \circ \mvarphi[push]
	\)
	for all~\( \mvarphi\colon\ordset{n}\into\ordset{m} \)
	in~\( \catdelta[plus] \) (in an enriched sense, it consists of natural transformations between the \( \catdelta[plus] \)-diagrams~\( \Cob[plus]{}{\Bar[plus]{}{{\ordset{\smallbullet}[linearize=\ringk]}}}\to\cosimpdgcatA{*} \)).
	Now if~\( 0 \le i \le n \), we may consider
	the map \( \mvarphi \colon \ordset{0}\into\ordset{n} \) taking \( 0 \) to~\( i \). Then
	\(
		\mF[d=n] { i }
		= \mF[d=n] { \mvarphi[push] { 0 } }
		= \mvarphi[push] { {\mF[d=0] { 0 }} }.
	\)
	Thus all the functors~\( \mF[d=n] \) are determined on the object level by the one object~\( \algM := \mF[d=0] { 0 } \in \cosimpdgcatA{0} \).
	Similarly, on the morphism level, \( \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} \)~is freely generated by the morphisms~\( \mf[i_0 i_1 \cdots i_k] \colon i_0 \to i_k \)
	with~\( 0 \le i_0 < i_1 < \cdots < i_k \le n \). But if we
	consider the map~\( \mvarphi \colon \ordset{k} \into \ordset{n} \) given
	by~\( \mvarphi{j} = i_j \), we have
	\( \mf[i_0 i_1 \cdots i_k,smash] = \mvarphi[push] { \mf[01\cdots k] } \).
	In other words, \( \mF \)~is determined on the object level by what it does to the non-degenerate morphism~\( \mf[01\cdots k] \in \Cob[plus]{}{\Bar[plus]{}{{\ordset{k}[linearize=\ringk]}}} \).
	Furthermore, these non-degenerate morphisms may be chosen freely.
	%; this follows, for instance, from the projective cofibrancy of~\( \simp[dg]{n} \) over~\( \catdelta[plus] \).
	Summarizing, the objects of this equalizer consist of the data of an element~\( \algM \in \cosimpdgcatA{0} \) and for each~\( n \) a morphism%\fxfatal{To see that these generate freely, one sees that \( \Delta^n \) is a pushout of stuff each of which has these free generators, so these generators lift freely (after applying~\( \lurie \)).}
	\[
		\mtheta[n]
		:=
		\mF[d=n] { \mf[01\cdots n] }
		\colon
		\face[max=n,shpush]{ \algM }
		\longto
		\face[min=n,shpush]{ \algM }
		.
	\]
	The differential is as stated since this is the image of the differential on~\( \mf[01\cdots n] \).
	
	%where \( \face[min=n] \) and \( \face[max=n] \) are the unique
	%morphisms~\( \ordset{0} \into \ordset{n} \)
	%given by \( \face[min=n] { 0 } = 0 \) and \( \face[max=n] { 0 } = n \).
	%In other words,
	%\( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
	%and \( \face[max=n] =  \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
	%We shall denote such pairs by~\( \tup { \algM , {\mtheta[ibullet]} } \).
	
	%On the morphism level, we claim the equalizer in question is in fact the full subcategory
	%of~\(
	%\Prod{\catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n}}}
	%\)
	%consisting of these objects
	
	On the morphism level, suppose
	%\( \tup { \algM , {\mtheta[ibullet]} } \)
	%and~\( \tup { \algN , {\meta[ibullet]} } \)
	\( \mF[d=n] \) and~\( \mG[d=n] \)
	are objects of the equalizer.
	%A morphism
	%\(
	%	\tup { \algM , {\mtheta[ibullet]} }
	%	\to
	%	\tup { \algN , {\meta[ibullet]} }
	%\)
	%consists of the
	%morphisms~
	A morphism~\( \mF[*] \to \mG[*] \)
	of degree~\( d \)
	consists of a
	collection~\(
		\malpha[*] = \tup { {\malpha[d=n]} }[\ordset{n}\in\catdelta[plus]]
	\)
	of morphisms \( \malpha[d=n] \colon \mF[d=n] \to \mG[d=n] \)
	in~\( \catainftyfun[o]{ {\ordset{n}[linearize=\ringk]},\cosimpdgcatA{n} } \) that simultaneously lie in the equalizer.
	%The space of morphisms~\( \mF[d=n] \to \mG[d=n] \) is\fxfatal{Yes, if \( \catainftyfun[o] \)~is a full subcategory of~\( \catainftyfun \).}
%	\[
%		\catainftyfun[o]{
%			{\ordset{n}[linearize=\ringk]},
%			\cosimpdgcatA{n}
%		} { {\mF[d=n]} , {\mG[d=n]} }
%		=
%		\coch[hoch]{*} {
%			{ \ordset{n}[linearize=\ringk,reduce] } ,
%			{ \cosimpdgcatA{n}[ symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%		}
%	\]
%	and thus the morphism space of transformations~\( \mF[*]\to\mG[*] \) is
	From \cref{ex:A_infty_fun_k_n_to_B}, we therefore
	get that the space of non-identity transformations~\( \mF[*]\to\mG[*] \) is
	\begin{align*}
		\MoveEqLeft
		\End {
%			\coch[hoch,par=\big]{*} {
%				{ \ordset{n}[linearize=\ringk,reduce] } ,
%				{ \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%			}
			\Hom[*,par=\big] {
				\tensorcoalg{{
					\ordset{n}[linearize=\ringk,reduce,return,shift=-1],
					\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
						\cosimpdgcatA{n}
					}
				}}
			}
		}
%	\\
		=
		\End {
			\Hom[*,par=\big,
			%{\catcom{k}[diag=\ordset{n}\times\ordset{n}]}
			] {
				%\tensorcoalg{ {\ordset{n}[linearize=\ringk,reduce]} }
				\textstyle\dirsum[limits,l\ge0,return,operator] { {\ordset{n}[linearize=\ringk,reduce,return,tens=l]} }
				,
				{
%					\cosimpdgcatA{n}[
%						symbolputleft=\!\!,
%						leftrestrict=\mF[n],
%						rightrestrict=\mG[n]
%					]
					\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
						\cosimpdgcatA{n}
					}
				}
			}
		}
	%\\
	%	&=
	%	\End[ \ordset{n}\in\catdelta[plus] ] {
	%		\Hom[\catdgcat] { \simp[dg]{n} ,  }
	%	}
	\\
		&=
		\End {
			\Prod[l\ge0] {
				\Prod[0\le i_0<\cdots<i_l\le n] {
					\Hom[*,\ringk,par=\big%,\catcom{k}
					] {
						\ringk
						\mf[i_{n-1} i_n]
						%\sotimes
						%\mf[i_{n-2} i_{n-1} ]
						\sotimes
						\cdots
						\sotimes
						\mf[ i_0 i_1 ]
						,
						{\cosimpdgcatA{n}[arg={
							{\mF[d=n] { i_0 } } ,
							{\mG[d=n] { i_n } }
						}]}
					 }
				}
			}
		}
	\end{align*}
	(note that
	%\( \ordset{n}\to \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] \)
	\(
		\ordset{n}\mapsto
		\map{ \mF[d=n]\times\mG[d=n] }[spar,qpull] {
			\cosimpdgcatA{n}
		}
	\)~defines a semicosimplicial dg-quiver).
	%This means that \( \malpha \)~is determined freely\fxfatal{Add in details}
	%by what it does to 
	%As a cosimplicial quiver, \( \ordset{n}\mapsto \tensorcoalg { \ordset{n}[linearize=\ringk,reduce] } \) is freely generated
	Thus the transformation~\( \malpha[*] \) is freely determined
	by what it does to the
	non-degenerate elements~\( \mf[n-1,n] \sotimes \cdots \sotimes \mf[0,1] \),
	i.e.\ by the
	elements
	\[
		\malpha[d=n] {{ \mf[n-1,n] \sotimes \cdots \sotimes\mf[0,1] }}
		\in
		\cosimpdgcatA{n}[arg={
			{\mF[d=n] { i_0 } } ,
			{\mG[d=n] { i_n } }
		}]
		.
	\]
	Calling this element~\( \malpha[n] \),
	we obtain the desired description.
\end{proof}

\section{Homotopy descent of dg-schemes}

\newclassset\dgschemeX{\mathbf{X}}
\newclassset\dgschemeY{\mathbf{Y}}
\newclassset\dgschemeZ{\mathbf{Z}}
\newclassset\dgschemeU{\mathbf{U}}
\newsheaf\shM{\mathscr{M}}

By a \textdef{dg-scheme}\fxfatal{Riche and friends have all kinds of extra assumptions, including Noetherian and blah blah blah, but I do not see right now what we need it for.},
we shall mean a pair~\( \dgschemeX = \tup{\setX,\dgcatA[\dgschemeX]} \),
where \( \dgcatA[\dgschemeX] \)~is a sheaf of non-positively graded,
super-commutative \( \reg[\setX] \)-dg-algebras.
A \textdef{quasi-coherent dg-sheaf} over~\( \dgschemeX \)
is a sheaf of \( \dgcatA[\dgschemeX] \)-dg-modules~\( \shM[*] \)
on~\( \setX \)
such that each graded piece~\( \shM[d=i] \)
is a quasi-coherent sheaf of \( \reg[\setX] \)-modules.
The dg-category of such is denoted~\( \catdgqcoh{\dgschemeX} \).
It is called a \textdef{coherent dg-sheaf}
if its cohomology~\( \co{*}{ \shM } \)
is a locally finitely generated as a sheaf of
graded \( \co{*}{ \dgcatA[\dgschemeX] } \)-modules.
%The dg-category of such is denoted~\( \catqcoh{\dgschemeX} \),
%and its dg-derived category is denoted~\( \der[dg]{\catqcoh{\dgschemeX}} \).
%Its homotopy category~\( \co[nopar]{0}{\der[dg]{\catqcoh{\dgschemeX}}} \)
%recovers the classical derived category~\( \der{\catqcoh{\dgschemeX}} \).
The dg-derived categories of these
are denoted~\( \der[dg,smash,nopar]{ \catdgqcoh{\dgschemeX} } \)
and~\( \der[dg,smash,nopar]{ \catdgcoh{\dgschemeX} } \).
Their homotopy categories recover the classical derived categories,
\[
	\co{0}{{ \der[dg,nopar]{ \catdgqcoh{\dgschemeX} } }}
	=
	\der[nopar]{ \catqcoh{\setX} }
\qquad\text{and}\qquad
	\co{0}{{ \der[dg,nopar]{ \catdgcoh{\dgschemeX} } }}
	=
	\der[b,nopar]{ \catcoh{\setX} }
\]

Suppose now that \( \set{ \dgschemeU[i] \to \dgschemeY } \)~is an
affine fpqc covering of a dg-scheme~\( \dgschemeY \),
and write \( \dgschemeU[i_0\cdots i_n] = \dgschemeU[i_0]\cap\cdots\cap\dgschemeU[i_n] \).
Consider the \ancech groupoid~\(
	\dgschemeX[1]
	\rightrightarrows
	\dgschemeX[0]
\)
associated to this covering
%Consider the \textdef{\ancech nerve} with respect to this covering.
%This is the internal Kan complex in affine dg-schemes
%given by~\( \dgschemeX[0] = \Coprod{ \dgschemeU[i] } \),
%\( \dgschemeX[1] = \Coprod{ \dgschemeU[ij] } \), and more generally,
and the associated classifying space, the \ancech nerve, given by
\[\textstyle
	\dgschemeX[n]
	=
	\dgschemeX[1]
	\fibre[\dgschemeX[0]]
	\dgschemeX[1]
	\fibre[\dgschemeX[0]]
	\cdots
	\fibre[\dgschemeX[0]]
	\dgschemeX[1]
	=
	\Coprod{
		\dgschemeU[i_0 i_1 \cdots i_n]
	}
\]
(we note that we do not have to take derived intersections
as the maps involved are flat).
The simplicial structure on~\( \dgschemeX[ibullet] \)
is given by the usual formula.
Then \( \catdgqcoh{\dgschemeX[ibullet]} \)~becomes
a cosimplicial system of dg-categories
via pullbacks (which are already derived because of~fpqc).
Then descent theory in derived algebraic geometry tells
us that the natural map
\[\textstyle
%	\der[dg,nopar]{
		\catdgqcoh{\dgschemeY}
%	}
	\to
	\invholim[\catdelta]{
		%\der[dg,nopar]{
			\catdgqcoh{\dgschemeX[ibullet]}
		%}
	}
\]
is a quasi-equivalence of dg-categories, the homotopy limit being taken in dg-categories.


%\begin{theorem}\label{res:A_infty_comodules}
%	%Suppose that \( \ssetX{*} \)~is a simplicial affine scheme
%	%for which all face maps~\( \face[d=i]\colon\ssetX{n}\to\ssetX{n-1} \) are flat.
%	As in the introduction, suppose that \( \ssetX{1} \rightrightarrows \ssetX{0} \)~are a monoid in affine schemes
%	such that \( \face[d=0] \) and~\( \face[d=1] \) are flat,
%	and let~\( \ssetX{*} \) be its classifying space.
%	Let~\( \algC \) be the coalgebra~\( \algC = \reg { \ssetX{1} } \)
%	over the commutative ring~\( \algA = \reg { \ssetX { 0 } } \).
%	Then we have an equivalence of categories
%	\[\textstyle
%		\invholim[\catdelta] { \catcom { \catqcoh{\ssetX{n}} } }
%		\cong
%%		\catcomod[infty,hcu,formal] { \algC }
%		\catxcomod{ \algC }[infty,hcu,formal]
%	.\]
%	%where \( \algC \)~is the coalgebra \( \algC = \reg { \ssetX{1} } \), the underlying commutative ring
%	%is~\( \algA = \reg { \ssetX { 0 } } \).
%	%\fxfatal{For unity condition, we should add flatness somewhere.}\fxfatal{{\color{red}NEED HOMOTOPY COUNITAL CONDITION!}}
%	The \anrhs denotes the dg-category of \textdef{homotopy-counital}
%	%right
%	left
%	\ainfty-comodules over~\( \algC \) in the category~\( \catxmodx{\algA}{\algA} \), which, for us, means that the second coaction map~\( \ca[2]\colon\algM\to\algC\tens[\algA]\algM \)~is
%	homotopy-invertible. The “\categoryformat{formal}”
%	part means that we omit the condition that
%	the product~\(
%		\Prod[i\ge1]{ \ca[i] }
%		\colon
%		\algM
%		\to
%		\Prod[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\)
%	factors through the direct sum~\(
%		\dirsum[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\).
%	(We hope later to find sufficient conditions under which  we can remove
%	this “\categoryformat{formal}”.)
%\end{theorem}

\begin{theorem}\label{res:A_infty_comodules}
	Suppose that
	\( \dgschemeX[1] \rightrightarrows \dgschemeX[0] \)
	is a groupoid in dg-schemes with
	source and target maps~\( \face[d=0],\face[d=1] \)
	both~fpqc, and consider the associated classifying space~\( \dgschemeX[ibullet] \).
	Write~\( \cosimpdgcatA{n} = \dgcatA[\dgschemeX[n],smash] \)
	for the associated cosimplicial system of dg-algebras.
	Let~\( \dgcatA = \cosimpdgcatA{0} \)
	and~\( \dgcatC = \cosimpdgcatA{1} \),
	and note that \( \dgcatC \)~is a
	counital
	coalgebra\fxfatal{Is it cocomplete? Also, remember to assume it is \emph{affine}, or the \( \dgcatA \)'s will only be \emph{sheaves}.} in~\( \catxdgmodx{\dgcatA}{\dgcatA} \)
	via the map~\(
		\comult
		=
		\face[d=1,comor]
		\colon
		\dgcatC
		\to
		\dgcatC\tens[\dgcatA]\dgcatC
	\).
	Then we have an equivalence of dg-categories
	\[\textstyle
		\invholim[\catdelta]{
			%\der[dg,nopar]{
				\catdgqcoh{ \dgschemeX[ibullet] }
			%}
		}
		\cong
		\catxcomod{\dgcatC}[infty,hcu,formal]{\dgcatA}
		,
	\]
	where the \anrhs denotes the dg-category
	of formal, homotopy-counital \ainfty-comodules
	over~\( \dgcatC \)
	in~\( \catxdgmod{\dgcatA} \).
\end{theorem}

%\newmap\adjunit{u}[nopar]
%
%\begin{lemma}
%	Let the assumptions be as in the theorem.
%	For any~\( n\ge 0 \),
%	we shall write~\(
%		\adjunit[d=n]
%		\colon
%		\id[\cosimpdgcatA{0}]
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] }}
%	\)
%	for the unit of adjunction.
%	If~\( \algM \in \cosimpdgcatA{0} \),
%	we wirte~\( \adjunit[d=n,\algM] \) for the
%	map~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \).
%	
%	Let \( \algM , \algN , \algP \)~be objects of~\( \cosimpdgcatA{0} \),
%	and suppose we are given maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	\)
%	in~\( \cosimpdgcatA{j} \).
%	Then
%	\[
%%		\face[max=j,shpush] {{
%%			\face[min=j,shpull] {{ \adjunit[j] { \meta } }}
%%		}}[spar]
%		\adjunit
%		\circ
%		%\adjunit[i] { \mtheta }
%		\face[max=i,shpull] { \mtheta }
%		\circ
%		\adjunit[d=i,\algM]
%		=
%		\map {
%			\face[min=i,shpull] { \meta }
%			\circ
%			\face[max=j,shpull] { \mtheta }
%		}[spar]
%		\circ
%		\adjunit[i+j]
%	\]
%\end{lemma}

%We initially consider terms of the
%form~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \).
%As in the proof of \cref{res:equivariance=comodules},
%base change will be crucial.
%Applying flat base change to the pullback diagram
%\[\begin{tikzcd}
%	\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%		& \ssetX{i} \ar[d,"{\face[min=i]}"]
%\\
%	\ssetX{j} \ar[r,"{\face[max=j]}"']
%		& \ssetX{0}
%\end{tikzcd}\]
%we obtain
%\(
%	\face[max=j,shpush] \face[min=i,shpull]
%	\cong
%	\face[min=i,shpull] \face[max=j,shpush]
%\)
%and~\(
%	\face[max=j,shpull] \face[min=i,shpush]
%	\cong
%	\face[min=i,shpush] \face[max=j,shpull]
%\).
%This implies
%
%\begin{lemma}\label{res:base_change_face_maps}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given objects~\( \algM , \algN , \algP \in \cosimpdgcatA{0} \),
%	along with two maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(\smash{
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	}\)
%	in~\( \cosimpdgcatA{j} \), where~\( i , j \ge 0 \).
%	Then the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i,shpush] {{ \face[max=i,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algN } }}
%				\ar[r]
%					\& \face[max=i,shpush] {{
%						\face[min=i,shpull] {{
%							\face[max=j,shpush] {{
%								\face[max=j,shpull] {{
%									\algN
%								}}
%							}}
%						}}
%					}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{} \ar[r,"{\meta}"']
%			\& \face[max=i,shpush] {{
%				\face[min=i,shpull] {{
%					\face[max=j,shpush] {{
%						\face[min=j,shpull] {{
%							\algP
%						}}
%					}}
%				}}
%			}}
%			\ar[r,symbol={\cong}]
%				\&[-1.5em] \face[max=i,shpush] {{
%				 \face[max=j,shpush] {{
%						\face[min=i,shpull] {{
%							\face[min=j,shpull] {{
%								\algP
%							}}
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					\&[-1.5em] \face[max=i+j,shpush] {{	
%						\face[min=(i+j),shpull] {{ \algP }}
%					}}
%	\invdot
%	\end{tikzcd}\end{align*}
%	is the same as the composition
%	\begin{align*}
%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i+j,shpush] {{
%				\face[max=(i+j),shpull] {{ \algM }}
%			}}
%			\ar[r,"{\face[max=j,shpull]{ \mtheta }}"]
%				\&\face[max=i+j,shpush] {{
%					\face[max=j,shpull] {{
%						\face[ min=i, shpull ] { \algN }
%					}}
%				}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\&{}= \face[max=i+j,shpush] {{
%			\face[min=i,shpull] {{
%				\face[ max=j, shpull ] { \algN }
%			}}
%		}}
%		\ar[r,"{\face[min=i,shpull] { \meta }}"']
%			\&\face[max=i+j,shpush] {{
%				\face[min=i,shpull] {{
%					\face[ min=j, shpull ] { \algP }
%				}}
%			}}
%			\ar[r,symbol={=}]
%				\&[-1.5em] \face[max=i+j,shpush] {{
%					\face[min=\smash{(i+j)},shpull] {{ \algP }}
%				}}
%				.
%	\end{tikzcd}\end{align*}
%	In other words, the map is
%	the unit of adjunction~\(
%		\algM
%		\to
%		\face[max=i+j,shpush] {{
%			\face[max=(i+j),shpull] { \algM }
%		}}
%	\)
%	composed with the
%	map~\(\smash{
%		\face[min=i,shpull] { \meta }
%		\circ
%		\face[max=j,shpull] { \mtheta }
%	}\).
%\end{lemma}
%
%\begin{lemma}\label{res:add_comultiplication_map}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given
%	objects~\( \algM , \algN \in \cosimpdgcatA{0} \)
%	along with a
%	map~\(
%		\mtheta
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\).
%%	Then the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta}"]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%%				\ar[r]
%%					& \face[max=n,shpush] {{
%%						\face[d=i,shpush] {{
%%							\face[d=i,shpull] {{
%%								\face[min=n,shpull] { \algN }
%%							}}
%%						}}
%%					}}
%%					\ar[r,symbol={=}]
%%						&[-1.5em]
%%						\face[min=n+1,shpush] {{
%%							\face[max=\smash{(n+1)},shpull] {{ \algN }}
%%						}} .
%%	\end{tikzcd}\]
%%	is the same as the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%			\ar[r,"{ \face[d=i,shpull] { \mtheta } }"]
%%				& \face[max=n+1,shpush] {{
%%					\face[min=(n+1),shpull] { \algN }
%%				}}
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}}
%%					\invdot
%%	\end{tikzcd}\]
%	Let~\( 1 \le i < n \).
%	Then we have a commutative diagram
%	\[\begin{tikzcd}[sep=scriptsize]
%		\algM \ar[r] \ar[d,dashed]
%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%			\ar[d,dashed]
%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%				\ar[d]
%	\\
%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%		\ar[r,dashed]
%			& \face[max=n,shpush] {{
%				\face[d=i,shpush] {{
%					\face[d=i,shpull] {{
%						\face[max=n,shpull] { \algM }
%					}}
%				}}
%			}}
%			\ar[r,"{\face[d=i,shpull]{\mtheta}}"]
%				& \face[max=n,shpush] {{
%					\face[d=i,shpush] {{
%						\face[d=i,shpull] {{
%							\face[min=n,shpull] { \algN }
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					&[-1.5em]
%					\face[max=n+1,shpush] {{
%						\face[min=\smash{(n+1)},shpull] {{ \algN }}
%					}} .
%	\end{tikzcd}\]
%\end{lemma}

\begin{proof}[Proof of \cref{res:A_infty_comodules}]
	\Cref{res:homotopy_limit_dgcat} gives us the general form
	of the homotopy limits of~\( \cosimpdgcatA{*} \),
	so we use the same notation.
%	By adjunction, the resulting
%	morphism~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\),
%	where \( n\ge 1 \),
%	is equivalent to a
%	map
%	\(
%		\algM
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%		\xto{\mtheta[n]}
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%	\).
%	We add to this collection~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
%	Putting~\( \ca[n] = \mtheta[n-1] \) for all~\( n\ge 1 \),
	Thus an object of the homotopy limit
	is a pair~\( \tup{\algM,\mtheta} \),
	where
	\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)~is
	a collection of maps~\(
		\mtheta[n]
		\colon
		\face[max=n,shpull] { \algM }
		\to
		\face[min=n,shpull] { \algM }
	\) of degree~\( 1-n \),
	and a morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	is a collection~\(
		\malpha = \tup{\malpha[n]}[n\ge0]
	\)
	of maps~\(
		\malpha[n]
		\colon
		\face[max=n,shpull]{\algM}
		\to
		\face[min=n,shpull]{\algN}
	\)
	of degree~\( \dgcatdeg{\malpha} - n \).
%	For a morphism~\(
%		\malpha
%		\colon
%		\tup{\algM,\mtheta}
%		\to
%		\tup{\algN,\meta}
%	\)
%	in the homotopy limit,
	For such a morphism,
	we scale it to define a new morphism~\( \malpha[tilde] \) by
	\(
		\malpha[tilde,n]
		=
		(-1)^{\dgcatdeg{\malpha}(n+1)}
		\malpha[n]
	\).
%	For an object~\( \tup{\algM,\mtheta} \),
%	we extend the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	by \( \mtheta[0] = \dif[\algM] \), the differential on~\( \algM \).
	Regarding this~\( \mtheta \) as a degree~\( 1 \)
	morphism~\( \tup{\algM,\mtheta}\to\tup{\algM,\mtheta} \),
	we use the same notation as for morphisms and
	write~\(
		\mtheta[tilde,n]
		=
		(-1)^{n+1}
		\mtheta[n]
	\) for~\( n\ge 1 \).
%	We also write~\( \dif[tilde,\algM] = - \dif[\algM] \).
	We notice that \eqref{res:morphisms_in_tot_composition} becomes
	\[
		\map{\mbeta\circ\malpha}[spar,widetilde,n]
		=
		\Sum[from={i=0},to={n}]{
			(-1)^{\dgcatdeg{\mbeta}i}
			\face[min=i,shpull]{{ \mbeta[tilde,n-i] }}
			\circ
			\face[max=(n-i),shpull]{{ \malpha[tilde,i] }}
		}.
	\]
	Thus
	\eqref{eq:theta_n_equation}~becomes
	%\[%\begin{equation}\label{eq:infinity_comod_theta_equation}
	\begin{align*}
		%\dif[par]{{\mtheta[tilde,n]}}
%		\MoveEqLeft
%		(-1)^{n}
%		(
%			\face[min=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		(-1)^{n+1}
		\dif[ {\face[min=n,shpull]{\algM}} ]
		\circ
		\mtheta[tilde,n]
%		-
%		(-1)^{1-n}
%	\\
%		&
%		{}
		-
		\mtheta[tilde,n]
		\circ
%		(
%			\face[max=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%		&
		=
		-
		\map{\mtheta\circ\mtheta}[widetilde,spar,n]
		+
		\Sum[from={i=1},to={n-1}]{
			%(-1)^{n-i+1}
			(-1)^{i}
			\face[d=i,shpull]{{ \mtheta[tilde,n-1] }}
		}
		.
	%\end{equation}
	%\]
	\end{align*}
	Since~\(
		\dif[par]{\malpha}[widetilde,n]
		=
		(-1)^{(\dgcatdeg{\malpha}+1)(n+1)}
		\dif[par]{\malpha}[n]
	\),
	\eqref{res:morphisms_in_tot_differential}~becomes
	\begin{align*}
			\dif[par]{\malpha}[widetilde,n]
			&
			=
			(-1)^{n+1}
			%\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
%			-
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\face[max=n,shpull]{{ \dif[tilde,\algM] }}
			\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%			&
%			\qquad
%			{}
			+
			\map{\meta\circ\malpha}[widetilde,spar,n]
	\\
			&
			\qquad
			{}
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[widetilde,spar,n]
%	\\
%			&
%			\qquad
%			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	\\
			&=
%			(-1)^n
%			\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			(-1)^{n+1}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
			+
			\Sum[from={i=0},to={n-1}]{
				(-1)^{i}
				\face[min=i,shpull]{{
					\meta[tilde,n-i]
				}}
				\circ
				\face[max=(n-i),shpull]{{
					\malpha[tilde,i]
				}}
			}
	\\
			&\qquad
			{}
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\dif[tilde,\algM]
			\dif[ {\face[max=n,shpull]{\algM}} ]
			-
			\Sum[from={i=1},to=n]{
				(-1)^{\dgcatdeg{\malpha}(i+1)}
				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
				\circ
				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
			}
	\\
			&\qquad
			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	,\end{align*}


	Now for an object~\( \tup{\algM,\mtheta} \),
	we add to the collection~\( \tup{\mtheta[n]}[n\ge1] \)
	the element~\( \mtheta[0] = -\dif[\algM] \).
	We then
%	where~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\) is a map of degree~\( 1-n \).
%	and add to the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	%add to this
%	the
%	collection~
%	and write~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
	define the comodule
	operations~\( \ca[n] \colon \algM \to \dgcatC[tens=(n-1)]\tens\algM \)
	of degree~\( 2 - n \)
	by
	\[\begin{tikzcd}%[sep=scriptsize]
		\ca[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\mtheta[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
	\end{tikzcd}\]
	where the first map is the unit of adjunction.
	In particular, \( \ca[1] = -\dif[\algM] \).	
	Similarly, if
	\( \malpha \colon \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
	is a map of degree~\( \dgcatdeg{\malpha} \),
%	where
%	\(
%		\malpha[n]
%		\in
%		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n]{
%			{\face[max=n,shpull]{\algM}},
%			{\face[min=n,shpull]{\algM}}
%		}
%	\),
	we associate to it
	the map of \ainfty-comodules~\(
		\mf \colon \algM \to \algN
	\)
	of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \),
	where
	\(
		\mf[n]
		\colon
		\algM
		\to
		\dgcatC[tens=(n-1)]\tens[\dgcatA] \algN
	\)
	is the map of degree~\(
		\dgcatdeg{\malpha} + 1 - n
		=
		\dgcatdeg{\mf} + 1 - n
	\)
	given by
	\[\begin{tikzcd}%[sep=scriptsize]
		\mf[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\malpha[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algN } }}
		.
	\end{tikzcd}\]
	It is immediate that the composition map above
	agrees with the composition of maps of \ainfty-comodules.
%	Now the two lemmas show that the above two equations are exactly the
%	\ainfty-comodule equations.
	%Via the two lemmas,
	Via~\cref{res:add_comultiplication_map,res:base_change_face_maps},
	the other two equations above now become
	\begin{align*}
		\MoveEqLeft
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[\algM]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\ca[n+1]
		+
		\ca[n+1]
		%\dif[\algM]
		\ca[1]
	\\
		&
		=
		-
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			( \id[ {\dgcatC[tens=i]} ]\tens\ca[n-i+1] )
			\ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			(
				\id[tens=(i-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-i)]
			)
			\ca[n]
		}
	\\
	\shortintertext{and}
		\dif{\mf}[spar,n]
		&
		=
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[N]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\mf[n+1]
		+
		\Sum[from={i=0},to={n-1}]{
			(-1)^{i}
			\ca[n-i+1] \mf[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		(-1)^{\dgcatdeg{\malpha}}
		\mf[n+1]\ca[1]
		-
		\Sum[from={i=1},to={n}]{
			(-1)^{\dgcatdeg{\malpha}(i+1)}
			\mf[n-i+1] \ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={j=1},to={n-1}]{
			(-1)^{j-1}
			(
				\id[tens=(j-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-j)]
			)
			\ca[n]
		},
	\end{align*}
	which are exactly the \ainfty-comodule equations from earlier.	
%	For all objects~\( \tup{\algM,\mtheta} \),
%	we now extend the collection~\( \mtheta = \tup{\mtheta}[n\ge1] \)
%	by~\( \mtheta[0] = \dif[\algM] \).
%	Following the above convention with~\( \mtheta[tilde,n] \),
%	this allows us to write~\( \mtheta[tilde,0] = - \mtheta[0] = \dif[tilde,\algM] \).
%	Then the two above equations become
%	\[
%		0
%		=
%		\Sum[from={i=0},to={n}]{
%			(-1)^{i}
%			\face[min=i,shpull]{{ \mtheta[tilde,n-i] }}
%			\circ
%			\face[max=(n-i),shpull] {{ \mtheta[tilde,i] }}
%		}
%		+
%		\Sum[from={i=1},to={n-1}]{
%			(-1)^{i-1}
%			\face[d=i,shpull]{{
%				\mtheta[tilde,n-1]
%			}}
%		}
%	\]
%	and
%	\begin{align*}
%			\dif{\malpha}[widetilde,spar,n]
%			&=
%			\Sum[from={i=0},to={n}]{
%				(-1)^{i}
%				\face[min=i,shpull]{{
%					\meta[tilde,n-i]
%				}}
%				\circ
%				\face[max=(n-i),shpull]{{
%					\malpha[tilde,i]
%				}}
%			}
%	\\
%			&
%			{}
%			-
%			\Sum[from={i=0},to=n]{
%				(-1)^{\dgcatdeg{\malpha}(i+1)}
%				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
%				\circ
%				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
%			}
%			+
%			\Sum[from={j=1},to={n-1}]
%				(-1)^{j-1}
%				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
%	\end{align*}

	To verify that we get exactly \emph{homotopy-counital} \ainfty-cmodules,
	we notice that the
	equation~\eqref{eq:theta_n_equation}
	in the case~\( n = 2 \) yields that
	\[
		\dif[par]{\mtheta[2]}
		=
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		-
		\face[d=1,shpull]{\mtheta[1]}
		,
	\]
	so that we have a homotopy~\(
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		\simeq
		\face[d=1,shpull]{\mtheta[1]}
	\).
	Then the proof of \cref{res:cocycle_iff_degen=0},
	with equalities replaced by homotopies,
	shows that \( \mtheta[1] \)~being an isomorphism is equivalent to~\( \degen[d=0,shpull]{\mtheta[1]}\simeq\id \).
	Similarly, one adjusts the
	last part of the proof of \cref{res:descent=comodules}
	to obtain that~\(
		(\counit\tens\id[\algM])\ca[2]
		\simeq
		\id
	\),
	which means that \( \algM \)~is homotopy-counital.
\end{proof}


%	
%	We initially check that the maps~\( \ca[n] \colon \algM \to \algC[tens=(n-1)] \tens \algM \),
%%	so let us for~\( k\ge 1 \) check the equation
%%	\[
%%		\Sum {
%%			(-1)^{i+mj}
%%			(
%%				\id[tens=i] \tens \comult[m] \tens \id[tens=j]
%%			)
%%			\ca[n]
%%		}
%%		= 0
%%	\]
%%	for all~\( i,m,j,n \) such that
%%	\( i + m + j = k \)
%%	and~\( n = i + 1 + j \),
%%	and where we, in the case~\( j=0 \),
%	satisfy the equations for an \ainfty-comodule,
%	so let us for all~\( k\ge 1 \) check the equation
%	\[
%		\Sum {
%			(-1)^{(i-1)+m(n-i)}
%			(
%				\id[tens=(i-1)] \tens \comult[m] \tens \id[tens=(n-i)]
%			)
%			\ca[n]
%		}
%		= 0 ,
%	\]
%	where the sum runs over the positive
%	integers~\( i, m, n \) such
%	that~\( 0\le i\le n\)
%	and~\( n + m - 1 = k \)
%	and where we, in the
%	case~\( i=n \),
%	interpret \( \comult[m] \) as~\( \ca[m] \).
%	%In other words, the sum has
%	%By base change, we obtain
%	%In other words, the sum consists
%	We notice that the term~\( m(n-i) \) in the exponent
%	of the sign is always even. Indeed,
%	if~\( n-i > 0 \), then \( \comult[m] = \comult[m,upper=\algC] \)~is the \ainfty-operation
%	on~\( \algC \), and so \( \comult[m,upper=\algC] = 0 \)
%	unless~\( m = 2 \). Thus we are left with~\( (-1)^{i-1} \).
%	%Also, in order to rewrite this equation in terms
%	%of the maps~\( \mtheta[n] \), it is convenient to replace
%%	\( n , m \) by~\( n+1 , m+1 \),
%%	so we are left with the equation
%%	\[
%%%		\Sum[i={m+n-1 = k} ] {{
%%			\Sum[from={i=1},to={k-1}] {{
%%				(-1)^i
%%				\bigl(
%%					(
%%						\id[tens=(i-1)]
%%						\tens
%%						\comult[2,upper=\algC]
%%						\tens
%%						\id[tens=(n-i)]
%%					) \ca[(k-2)+1]
%%					-
%%					abe
%%				\bigr)
%%			}}
%%			=0
%%%		}}
%%	\]
%%	for all~\( k\ge 1 \).
%	Thus the equation may be reduced to
%	\begin{align*}
%		0
%			&=
%			\Sum[from={n=1},to={k}] {{
%				(-1)^{n-1}
%				(
%					\id[tens=(n-1)]
%					\tens
%					\ca[k+1-n]
%				)
%				\ca[n]
%			}}
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(k-i-1)]
%				)
%				\ca[k-1]
%			}}
%	\\
%			&=
%			\ca[k]\circ\ca[1]
%			- (-1)^{k} (\id[tens=(k-1)]\tens\ca[1]) \ca[k]
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				\bigl(
%					(
%						\id[tens=(i-1)]
%						\tens
%						\comult[2,upper=\algC]
%						\tens
%						\id[tens=(k-i-1)]
%					)
%					\ca[k-1]
%					-
%					(
%						\id[tens=i]
%						\tens
%						\ca[k-i]
%					)
%					\ca[i+1]
%				\bigr)
%			}}
%	\end{align*}
%%	Since the differential on~\( \algC \) is zero and \( \ca[1] = \dif[\algM] \), the first
%%	two terms are
%%	simply~\(
%%		-
%%		(-1)^{2-k}
%%		\dif[par] { \ca[k] }
%%	\).
%	Substituting \( n+1 \) for~\( k \), we obtain
%	that the equation we must verify is
%	\begin{align*}
%%		\dif[par] { \ca[n+1] }
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%		&=
%		\Sum[from={i=1},to={n-1}]
%			(-1)^{n-i}
%			\bigl(
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(n-i)]
%				)
%				\ca[n]
%	\\&
%		\qquad\qquad
%				{}-
%				(
%					\id[tens=i]
%					\tens
%					\ca[n-i+1]
%				)
%				\ca[i+1]
%			\bigr)
%		.
%	\end{align*}
%	This equation is very similar
%	%to the one in~\cref{res:homotopy_limit_dgcat},
%	to~\eqref{eq:theta_n_equation},
%	and we shall indeed derive it from that equation. Specifically, we claim that it is obtained
%	from~\eqref{eq:theta_n_equation} by composing
%	with \( (-1)^{n+2} = (-1)^{n} \) times the
%	unit~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \),
%	and we show this by comparing each term individually.
%	
%	We initially consider the
%	term~\(
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%	\).
%	We get by~\cref{res:base_change_face_maps}
%	that
%	this is exactly the unit~\(
%		\algM \to
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{ \algM }
%		}}
%	\)
%	composed with
%	\[
%		(-1)
%		\face[min=n,shpush]{\dif[\algM]}
%		\circ
%		(-1)^{n+1}
%		\mtheta[n]
%		-
%		(-1)^{1-n}
%		(-1)^{n+1}
%		\mtheta[n]
%		\circ
%		(-1)
%		\dif[\algM]
%		=
%		(-1)^{n}
%		\dif[par]{\mtheta[n]}
%		.
%	\]
%	This is exactly \( (-1)^n \)~times the left-hand side
%	term in~\eqref{eq:theta_n_equation}, as claimed.
%	
%	We next consider terms of the
%	form~\( ( \id[tens=i] \tens \ca[n-i+1] ) \ca[i+1] \).
%%	We proceed much as in the proof of \cref{res:equivariance=comodules}.
%%	Applying flat base change to the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%%			& \ssetX{i} \ar[d,"{\face[min=i]}"]
%%	\\
%%		\ssetX{j} \ar[r,"{\face[max=j]}"']
%%			& \ssetX{0}
%%	\end{tikzcd}\]
%%	we obtain
%%	\(
%%		\face[max=j,shpush] \face[min=i,shpull]
%%		\cong
%%		\face[min=i,shpull] \face[max=j,shpush]
%%	\)
%%	and~\(
%%		\face[max=j,shpull] \face[min=i,shpush]
%%		\cong
%%		\face[min=i,shpush] \face[max=j,shpull]
%%	\).\fxfatal{As stated, this diagram is WRONG!!}
%%	This allows us to
%%	rewrite the term~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \)
%%	as
%%	\begin{align*}\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=n,shpush] {{ \face[max=i,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[i]}"]
%%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algM } }}
%%				\ar[r]
%%					\& \face[max=i,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[max=j,shpush] {{
%%								\face[max=j,shpull] {{
%%									\algM
%%								}}
%%							}}
%%						}}
%%					}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		{} \ar[r,"{\mtheta[j]}"]
%%			\& \face[max=i,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[max=j,shpush] {{
%%						\face[min=j,shpull] {{
%%							\algM
%%						}}
%%					}}
%%				}}
%%			}}
%%			\ar[r,symbol={\cong}]
%%				\&[-1.5em] \face[max=i,shpush] {{
%%					 \face[max=j,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[min=j,shpull] {{
%%								\algM
%%							}}
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					\&[-1.5em] \face[max=i+j,shpush] {{	
%%						\face[min=(i+j),shpull] {{ \algM }}
%%					}}
%%	\invdot
%%	\end{tikzcd}\end{align*}
%%	the isomorphism being by base change.
%%	In other words, the composed
%%	map~\(
%%		( \id[tens=i]\tens\ca[j+1] )
%%		\ca[i+1]
%%	\)
%%	is the same as the map
%%	\begin{align*}
%%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=i+j,shpush] {{
%%				\face[max=(i+j),shpull] {{ \algM }}
%%			}}
%%			\ar[r,"{\face[max=j,shpull]{ \mtheta[i] }}"]
%%				\&\face[max=i+j,shpush] {{
%%					\face[max=j,shpull] {{
%%						\face[ min=i, shpull ] { \algM }
%%					}}
%%				}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\&{}= \face[max=i+j,shpush] {{
%%			\face[min=i,shpull] {{
%%				\face[ max=j, shpull ] { \algM }
%%			}}
%%		}}
%%		\ar[r,"{\face[min=i,shpull] { \mtheta[j] }}"]
%%			\&\face[max=i+j,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[ min=j, shpull ] { \algM }
%%				}}
%%			}}
%%			\ar[r,symbol={=}]
%%				\&[-1.5em] \face[max=i+j,shpush] {{
%%					\face[min=\smash{(i+j)},shpull] {{ \algM }}
%%				}}
%%				.
%%	\end{tikzcd}\end{align*}
%	By~\cref{res:base_change_face_maps},
%%	this map is the same as
%%	\( (-1)^{k+1} \) times the unit of adjunction~\(
%%		\algM
%%		\to
%%		\face[max=i+j,shpush] {{
%%			\face[max=(i+j),shpull] { \algM }
%%		}}
%%	\)
%%	composed with the
%%	term~\(
%%		\face[min=i,shpull] { \mtheta[j] }
%%		\circ
%%		\face[max=j,shpull] { \mtheta[i] }
%%	\)
%%	this is the same as the map
%%	\[\begin{tikzcd}%[sep=scriptsize]
%%		\algM
%%		\ar[r]
%%		&
%%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%		\ar[r,"{
%%			(-1)^{n-i+1}
%%			\face[min=i,shpull]{\mtheta[n-i]}
%%			\circ
%%			(-1)^{i+1}
%%			\face[max=(n-i),shpull]{\mtheta[i]}
%%		}"]
%%		&[7em]
%%		\face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%	\end{tikzcd}\]
%	this is the same as
%	the unit~\(
%		\algM
%		\to
%		\face[max=n,shpush]
%		\face[max=n,shpull]
%		\algM
%	\)
%	composed with
%	\[
%		(-1)^{n-i+1}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		(-1)^{i+1}
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		=
%		(-1)^{n}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		.
%	\]
%	This is \( (-1)^{n} \)~times one of the terms
%	on the right-hand side of~\eqref{eq:theta_n_equation}, as claimed.
%	
%	
%%	Similarly, we consider the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{n+1} \ar[r] \ar[d] & \ssetX{n} \ar[d]
%%	\\
%%		\ssetX{1} \ar[r] & \ssetX{0}
%%	\end{tikzcd}\]
%	Finally, we consider terms of the
%	form~\(
%		( \id[tens=(i-1)] \tens \comult[2] \tens \id[tens=(n-i)] ) \ca[n]
%		=
%		( \id[tens=(i-1)] \tens \comult[\algC] \tens \id[tens=(n-i)] ) \ca[n]
%	\) where~\( n-i> 0 \).
%	These are given by the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
%			\ar[r,"{(-1)^{n}\mtheta[n-1]}"]
%				\&[1.3em]
%				%\&
%				\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
%	\end{tikzcd}
%	\\[-.7em]
%	&
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{}
%				\ar[r]
%					\& \face[max=n-1,shpush] {{
%						\face[d=i,shpush] {{
%							\face[d=i,shpull] {{
%								\face[min=(n-1),shpull] { \algM }
%							}}
%						}}
%					}}
%					\ar[r,symbol={=}]
%						\&[-1.5em]
%						\face[min=n,shpush] {{
%							\face[max=n,shpull] {{ \algM }}
%						}} .
%	\end{tikzcd}
%	\end{align*}
%%	This map factors as
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r] \ar[d,dashed]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[n]}"]
%%			\ar[d,dashed]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%				\ar[d]
%%	\\
%%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%		\ar[r,dashed]
%%			& \face[max=n,shpush] {{
%%				\face[d=i,shpush] {{
%%					\face[d=i,shpull] {{
%%						\face[max=n,shpull] { \algM }
%%					}}
%%				}}
%%			}}
%%			\ar[r,"{\face[d=i,shpull]{\mtheta[n]}}"]
%%				& \face[max=n,shpush] {{
%%					\face[d=i,shpush] {{
%%						\face[d=i,shpull] {{
%%							\face[min=n,shpull] { \algM }
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}} .
%%	\end{tikzcd}\]
%	According to \cref{res:add_comultiplication_map}, this map
%	is the same as the
%	unit~\(
%		\algM
%		\to
%		\face[max=n+1,shpush] {{
%			\face[max=(n+1),shpull] { \algM }
%		}}
%	\)
%	composed with~\( (-1)^{n} \face[d=i,shpull] { \mtheta[n] } \).
%	This is again~\( (-1)^{n} \) times a term
%	from~\eqref{eq:theta_n_equation}, as claimed.
%	
%	With regards to th morphisms, suppose
%	that \( \malpha = \tup{\malpha[n]}[n\ge0] \)
%	is a
%	morphism~\( \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
%	of degree~\( \dgcatdeg{\malpha} \).
%	This consists of
%	maps~\(
%		\malpha[n]
%		\in
%		\Hom[d={\dgcatdeg{\malpha}-n}]{
%			{\face[max=n,shpull]{\algM}} ,
%			{\face[min=n,shpull]{\algN}}
%		}
%	\).
%	We use this to define a
%	map~\( \mf \colon \algM \to \algN \)
%	of \ainfty-comodules of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \).
%	For all~\( n\ge1 \), let~\( \mf[n] \colon \algM \to \algC[tens=(n-1)]\tens\algN \)
%	be the composition
%	\[\begin{tikzcd}
%		\algM
%		\ar[r]
%		&
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{\algM}
%		}}
%		\ar[r,"{
%			(-1)^{\dgcatdeg{\malpha}(n-1)}
%			\malpha[n-1]
%		}"]
%		&[4em]
%		\face[max=n,shpush]{{
%			\face[min=n,shpull]{\algN}
%		}}
%	\end{tikzcd}\]
%	
%	Proving that the morphisms inside our dg-category agree
%	with the morphisms
%	inside the dg-category~\( \catxcomod{\algC}[infty,hcu,formal] \)
%	amounts to showing that the equation~\eqref{res:morphisms_in_tot_differential}
%	agrees with the equation for a map of \ainfty-comodules
%	and that \eqref{res:morphisms_in_tot_composition}
%	agrees with the compositions.
%	This is similar acrobatics using the two lemmas above,
%	and we omit it. The homotopy counital condition is equivalent
%	to the condition that \( \mtheta[1] \)~is homotopy-invertible.
%\end{proof}

\endgroup

==> holim_dgcat/holim_dgcat_5011.tex <==
\begingroup

\chapter{Homotopy limits in dg-categories}

%\section{Framings in dg-categories}
%
%A framing on the category~\( \catdgcat \) is due to
%\textcite{holstein}: If \( \dgcatA \in \catdgcat \) and \( \ssetK\in\catsset \), then let
%\(
%	\dgcatA[powering=\ssetK]
%	=
%	\catloc { \ssetK, \dgcatA }
%	=
%	\catdgfun[infty,o] { \lurie{\ssetK} , \dgcatA }
%\).

%\begin{parabreak}[Tabuada's model structure on~\( \catdgcat \)]
	Given a dg-category~\( \dgcatA \), we denote by~\( \dgcatA[z0] \) the dg-category with the same objects as~\( \dgcatA \), but with hom complexes given by
	\(
		%\Hom[ \dgcatA[z0] ] { \vx, \vy } =
		%\cocy[nopar]{0} { \Hom[\dgcatA, * ] { \vx, \vy } }
		\dgcatA[z0,spar] { \vx , \vy } = \cocy{0} { \dgcatA { \vx , \vy } }
	\),
	the set of closed maps~\( \vx \to \vy \) in~\( \dgcatA \). We define~\( \dgcatA[h0] \) analogously.
	A map~\( \mf \in \dgcatA[d=0]{ \vx , \vy } \) in~\( \dgcatA \) is called a \textdef{homotopy equivalence} if its image in~\( \dgcatA[h0] \) is an isomorphism. As in homological algebra, this amounts the existence of a map \( \mg \in \dgcatA[d=0] { \vy , \vx } \) in the other direction along with correcting morphisms \( \mr[\vx] \in \dgcatA[d=-1] { \vx , \vx } \) and \( \mr[\vy] \in \dgcatA[d=-1] { \vy , \vy } \) such that
	\[
		\dif{ \mr[\vx] } = \mg \mf - \id[\vx]
		\qquad\text{and}\qquad
		\dif{ \mr[\vy] } = \mf \mg - \id[\vy].
	\]

	We recall from
	\textcite{tabuada,tabuada_dgcats_vs_simplicial_cats}
	the existence of a model structure on the \( 1 \)-category~\( \catdgcat \) with
	\begin{itemize}
		\item weak equivalences given by \textdef{quasi-equivalences}, i.e.
		functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
		\item the induced functor~\( \mF[parent=alg,h0] \colon \dgcatA[h0] \to \dgcatB[h0] \) is an equivalence of categories in the classical, non-enriched sense;
		\item for all~\( \vx, \vy \in \dgcatA \),
		\( \mF[\vx, \vy] \colon
		\dgcatA { \vx , \vy } \to \dgcatB { \mF { \vx } , \mF { \vy } } \)
		is a quasi-isomorphism of chain complexes;
		\end{enumerate}
		\item fibrations given by dg-functors~\( \mF \colon \dgcatA \to \dgcatB \) such that
		\begin{enumerate}[(i)]
			\item the induced map
			\(
				\mF \colon
				\dgcatA[*] { \vx, \vy }
				\to
				\dgcatB[*] { \mF { \vx } , \mF { \vy } }
			\)
			is surjective for all objects~\( \vx, \vy \in \dgcatA \), and
			\item any map \( \mf \colon \mF { \vx } \to \vy \) in~\( \dgcatB \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatB } \) lifts as \( \mf = \mF { \mg } \) for some morphism \( \mg\colon \vx \to \vx[prime] \) in~\( \dgcatA \)
			that becomes an isomorphism in~\( \Hdgcat { \dgcatA } \).
		\end{enumerate}
	\end{itemize}
%	It is cofibrantly generated,
%	with
%	\begin{itemize}
%		\item the class~\( \setgencof \) consisting of the morphism \( \varnothing \into \ringk \)
%		\item the class~\( \setgentrivcof \)
%	\end{itemize}
	This model structure is combinatorial according to
	\textcite[Proposition~1.3.1.19]{ha}.
%\end{parabreak}

We shall use the tools developed in the preceding chapters to develop a notion of homotopy descent of quasi-coherent sheaves on affine schemes.
%We write \( \face[min=n] \) and~\( \face[max=n] \) for the two unique morphisms~\( \ordset{0} \into \ordset{n} \) in~\( \catdelta \) given by
%\( \face[min=n] { 0 } = 0 \) and~\( \face[max=n] { 0 } = n \).
%In other words, \( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
%and~\( \face[max=n] = \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
Much of the inspiration is from \textcite{explicit};
however, using the tools developed earlier
(specifically~\cref{ex:A_infty_fun_k_n_to_B}),
we are able to solve their Conjecture~1 and prove their
results in complete generality.



%\begin{theorem}
%	Suppose that \( \ssetX{*} \)~is a simplicial affine scheme with each~\( \ssetX{n} \) being regular and each \( \ssetX{n}\to \ssetX{m} \) flat surjective\fxfatal{This is supposed to be the same as faithfully flat, check this.}.
%	Then we have an equivalence of categories
%	\(
%		\invholim[\catdelta] { \catqcoh{\ssetX{n}} }
%		\cong
%		\catainftycomod { \catqcoh { \ssetX{0} } }
%	\).
%\end{theorem}

Recall from \cref{res:fat_tot} that
the homotopy limit of a \( \catdelta \)-diagram in~\( \catdgcat \) is given by
\[\textstyle
	\invholim[\catdelta] { \cosimpdgcatA{n} }
	=
	\invholim[\catdelta[plus]] { \cosimpdgcatA{n} }
	=
	\End[\ordset{n}\in\catdelta[plus]] { \fibrep[deltaplus] { \cosimpdgcatA{n} }{n} }
\]
where \( \fibrep[deltaplus] \colon \catdgcat\to\catdgcat[diag={\catdelta[plus,op]},inj,smash] \) is a fibrant replacement functor, taking a dg-category~\( \dgcatB \) to an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \).
We obtain such a functor from Holstein:

\begin{theorembreak}[{Theorem \parencite[section~3]{holstein}}]\label{res:holstein_resolution}
	If \( \dgcatB \)~is a dg-category, then
	\( \simpdgcatB{*} \in \catdgcat[diag={\catdelta[plus,op]}] \)
	given by
	\[
		\simpdgcatB{n}
%		= \catloc[infty] { \simp{n} , \dgcatA }
%		= \catdgfun[infty,o] { \simp[dg]{n} , \dgcatA }
		= \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \dgcatB }
	\]
	is an injectively fibrant replacement of the constant \( \catdelta[plus] \)-diagram at~\( \dgcatB \). Here,
	the~“\( \mathbf{\circ} \)”
%	means an object is an
%	\ainfty-functor~\( \mf \) such that
%	\(
%		\mf[1]
%		\colon
%		\ordset{n}[linearize=\ringk,arg={i,j}]
%		\to
%		\dgcatB { \mf { i } , \mf { j } }
%	\)
%	sends non-zero maps to isomorp
	means that the objects are \ainfty-functors~\( \mf \) such
	that~\( \co[nopar]{0} { \mf } \colon \ordset{n}[lin=\ringk]\to\dgcatB[h0] \)
	sends non-zero maps to isomorphisms.
	Equivalently, in the notation of~\cref{ex:A_infty_fun_k_n_to_B},
	\( \co[nopar]{0}{\mf[ij]} \)~is an isomorphism for all~\( i<j \).
\end{theorembreak}

%As a consequence, we deduce that

%\begin{corollary}
	In other words,
	if \( \cosimpdgcatA{*} \)~is a cosimplicial system of dg-categories,
	then its homotopy limit is given by
	\[\textstyle
		\invholim[\catdelta] { \cosimpdgcatA{n} }
		=
		\End[\ordset{n}\in\catdelta[plus]] {{
			\catainftyfun[o] { {\ordset{n}[linearize=\ringk]}  , \cosimpdgcatA{n} }
		}}
		.
	\]
%\end{corollary}
We wish to evaluate this expression more explicitly:

\begin{proposition}\label{res:homotopy_limit_dgcat}
	Suppose~\( \cosimpdgcatA{*} \) is a cosimplicial system of dg-categories. Then the homotopy limit
	\(
		\invholim[\catdelta] { \cosimpdgcatA{*} }
	\)
	is the dg-category with objects~\( \tup { \algM , \mtheta } \)
	where~\(
		\mtheta = \tup { {\mtheta[n]} }[n\ge 1]
	\)
	is a collection of morphisms~%
	\(
		\mtheta[n]
		\in
		\Hom[\cosimpdgcatA{n} , d=1-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algM } }
		}
	\),
	satisfying
	\begin{equation}\label{eq:theta_n_equation}
		\dif[par] { {\mtheta[n]} }
		=
		-
		\map{\mtheta\circ\mtheta}[spar,n]
		+
		\Sum[from={i=1},to={n-1}] {{
			(-1)^{n-i}
%			\bigl(
				\coface[d=i] {{ \mtheta[n-1] }}
%				-
%				\coface[min=i] {{ \mtheta[n-i] }}
%				\circ
%				\coface[max=n-i] {{ \mtheta[i] }}
%			\bigr)
		}}
	\end{equation}
	and with \( \mtheta[1] \)~invertible in~\( \co{0} { \cosimpdgcatA{1} } \).\fxfatal{Think about possible issues in the case~\( n = 1 \)}
	The composition~\( \mtheta\circ\mtheta \)
	is evaluated via~\eqref{res:morphisms_in_tot_composition}
	below with the conventions~\( \dgcatdeg{\mtheta} = 1 \)
	and~\( \mtheta[0] = 0 \).
	A morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	of degree~\( \dgcatdeg{\malpha} \)
	is a collection~\(
		\malpha = \tup { \malpha[n] }[n\ge0]
	\)
	of morphisms~\(
		\malpha[n]
		\in
		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n] {
			{ \coface[max=n,nopar] { \algM } } ,
			{ \coface[min=n,nopar] { \algN } }
		}[smash]
	\).
	The composition of two morphisms is
	\begin{equation}\label{res:morphisms_in_tot_composition}
		\map{\mbeta\circ\malpha}[spar,n]
		=
		\Sum[from={i=0},to={n}] {
			(-1)^{\dgcatdeg{\malpha}(n-i)}
			\coface[min=i,nopar] { \mbeta[n-i] }
			\circ
			\coface[max=n-i,nopar] { \malpha[i] }
		}
	.\end{equation}
	The differential on a morphism is
	\begin{equation}\label{res:morphisms_in_tot_differential}
%	\begin{split}
			\dif[par]{\malpha}[n]
%			&
			=
			\dif[par]{\malpha[n]}
			+
			\map{\meta\circ\malpha}[spar,n]
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[spar,n]
			+
			(-1)^{\dgcatdeg{\malpha}}
			\Sum[from={j=1},to={n-1}]
%				\bigl(
					(-1)^{n-j}
					\coface[d=j,nopar] { \malpha[n-1] }
					.
%		\\
%					&{}
%					\qquad
%					+			
%					(-1)^{\dgcatdeg{\malpha}(n-j)}
%					\coface[min=j,nopar] { \meta[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \malpha[j] }
%		\\
%					&{}
%					\qquad
%					-
%					(-1)^{\dgcatdeg{\malpha}}(-1)^{n-j}
%					\coface[min=j,nopar] { \malpha[n-j] }
%					\circ
%					\coface[max=n-j,nopar] { \mtheta[j] }
%					
%				\bigr)	
%		.\end{split}
	\end{equation}
%	where the compositions are evaluated
%	via~\eqref{res:morphisms_in_tot_composition}
%	with the convention~\(
%		\dgcatdeg{\mtheta}
%		=
%		\dgcatdeg{\meta}
%		=
%		1
%	\).
\end{proposition}

This proves Conjecture~1 in \textcite{explicit}.

%To prove this, recall from \cdots\fxfatal{Insert reference} that this homotopy limit is given by
%For brevity, write \( \cosimpdgcatA{n} = \catqcoh { \ssetX { n } } \).


\begin{comment}
	Following \textcite{holstein}, let us spell out
	the resolution found in \cref{res:holstein_resolution}.
	The dg-category~\( \simpdgcatB{n} \) has objects
	dg-functors~\( \mF\colon \simp[dg]{n} \to \dgcatA \)
	such that \( \mF {{ \mf[i,i+1] }} \)~is invertible
	in~\( \dgcatA[h0] \)
	for all~\( i \).
%	A morphism~\( \malpha \) of degree~\( l \) between~\( \mF \colon\simp[dg]{n}\to\dgcatA \)
%	and~\( \mG \colon \simp[dg]{n} \to \dgcatA \)
%	consists of a
%	Hochschield cochain
	The morphism space
	between \( \mF \) and~\( \mG \)
	is
	\[
		\simpdgcatB{n}[*]{ \mF , \mG }
		=
%		\coch[hoch]{*} {
%			{\ordset{n}[linearize=\ringk]} ,
%			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
%		}
%		=
		\Hom[*,par=\big] {
			{\tensorcoalg[par=\big]{{\ordset{n}[linearize=\ringk,spar,shift=-1]}}},
			{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
		}
		=
		\Prod[l\ge0] {{
			\Hom[*,par=\big] {
				{ \ordset{n}[ linearize=\ringk,
					reduce,return,
					tens=l,return,shift=-l
					]
				},
				{\dgcatA[leftrestrict=\mF,rightrestrict=\mG]}
			}
		}}
		.
	\]
	The composition operation is\fxfatal{Add details about this.}.
	
	
	The differential on a
	map~\( \malpha \in \simpdgcatB{n}[d=m]{ \mF , \mG } \)
	is given by
	\begin{align*}
%		\dif[output=map] { \malpha } {{
%			\mf[i_{l-1},i_l]
%			\sotimes
%			\mf[i_{l-2},i_{l-1}]
%			\sotimes\cdots\sotimes
%			\mf[i_0,i_1]
%		}}
		\MoveEqLeft
		\dif[output=map] { \malpha } { i_0 , ... , i_l }
		=
		\dif[\dgcatA,output=map] { \malpha } { i_0 ,..., i_l }
		+ \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\mG { i_j , ... , i_l }
			\circ
			\malpha { i_0 , ... , i_j }
		}}
	\\
		& {} + (-1)^{m} \Sum[from={j=1},to={l-1}] {{
			(-1)^{j}
			\malpha { i_j , ... , i_l }
			\circ
			\mF { i_0 , ... , i_j }
		}}
	\end{align*}
\end{comment}

\begin{proof}[Proof of \cref{res:homotopy_limit_dgcat}]
	Using \citeauthor{holstein}'s theorem, we obtain the formula
	\begin{align*}
		\MoveEqLeft
		{\textstyle \invholim[\catdelta] { \cosimpdgcatA{n} } }
		=
		\End[\ordset{n}\in\catdelta[plus]] {
			\catainftyfun[o] {
				{\ordset{n}[linearize=\ringk]} ,
				\cosimpdgcatA{n}
			}
		}
	\\
			& = \Eq[par=\Big] {{
				\Prod[\ordset{n}\in\catdelta[plus]] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{n}
					}
				}
				\rightrightarrows
				\Prod[\ordset{n}\into\ordset{m}] {
					\catainftyfun[o] {
						{\ordset{n}[linearize=\ringk]} ,
						\cosimpdgcatA{m}
					}
				}
			}}.
	\end{align*}
	%A
	%functor~\( \mF \in \catdgfun[infty,o] { \simp[dg]{n} , \cosimpdgcatA{n} } \)
	%is determined by the
	%objects~\( \mF { 0 } , \mF { 1 } , \ldots , \mF { n } \in \cosimpdgcatA{n} \)
	%and a collection of morphisms~\(
	%	\mF { \mf[i_0 i_1 \cdots i_n] }
	%\)
	We note initially that the set of objects
	of~\( \catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n} } \)
	is the subset of~\( \Hom[\catdgcat] { \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} , \cosimpdgcatA{n} } \)
	of functors satisfying this unital condition.
	Thus an object of this equalizer is a
	collection~\( \mF = \tup { {\mF[d=n]} }[\ordset{n}\in\catdelta[plus]] \)
	of dg-functors~\(
		\mF[d=n]
		\colon
		\Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}}
		\to
		\cosimpdgcatA{n}
	\)
	satisfying~\(
		\mvarphi[push] \circ \mF[d=n] = \mF[d=m] \circ \mvarphi[push]
	\)
	for all~\( \mvarphi\colon\ordset{n}\into\ordset{m} \)
	in~\( \catdelta[plus] \) (in an enriched sense, it consists of natural transformations between the \( \catdelta[plus] \)-diagrams~\( \Cob[plus]{}{\Bar[plus]{}{{\ordset{\smallbullet}[linearize=\ringk]}}}\to\cosimpdgcatA{*} \)).
	Now if~\( 0 \le i \le n \), we may consider
	the map \( \mvarphi \colon \ordset{0}\into\ordset{n} \) taking \( 0 \) to~\( i \). Then
	\(
		\mF[d=n] { i }
		= \mF[d=n] { \mvarphi[push] { 0 } }
		= \mvarphi[push] { {\mF[d=0] { 0 }} }.
	\)
	Thus all the functors~\( \mF[d=n] \) are determined on the object level by the one object~\( \algM := \mF[d=0] { 0 } \in \cosimpdgcatA{0} \).
	Similarly, on the morphism level, \( \Cob[plus]{}{\Bar[plus]{}{{\ordset{n}[linearize=\ringk]}}} \)~is freely generated by the morphisms~\( \mf[i_0 i_1 \cdots i_k] \colon i_0 \to i_k \)
	with~\( 0 \le i_0 < i_1 < \cdots < i_k \le n \). But if we
	consider the map~\( \mvarphi \colon \ordset{k} \into \ordset{n} \) given
	by~\( \mvarphi{j} = i_j \), we have
	\( \mf[i_0 i_1 \cdots i_k,smash] = \mvarphi[push] { \mf[01\cdots k] } \).
	In other words, \( \mF \)~is determined on the object level by what it does to the non-degenerate morphism~\( \mf[01\cdots k] \in \Cob[plus]{}{\Bar[plus]{}{{\ordset{k}[linearize=\ringk]}}} \).
	Furthermore, these non-degenerate morphisms may be chosen freely.
	%; this follows, for instance, from the projective cofibrancy of~\( \simp[dg]{n} \) over~\( \catdelta[plus] \).
	Summarizing, the objects of this equalizer consist of the data of an element~\( \algM \in \cosimpdgcatA{0} \) and for each~\( n \) a morphism%\fxfatal{To see that these generate freely, one sees that \( \Delta^n \) is a pushout of stuff each of which has these free generators, so these generators lift freely (after applying~\( \lurie \)).}
	\[
		\mtheta[n]
		:=
		\mF[d=n] { \mf[01\cdots n] }
		\colon
		\face[max=n,shpush]{ \algM }
		\longto
		\face[min=n,shpush]{ \algM }
		.
	\]
	The differential is as stated since this is the image of the differential on~\( \mf[01\cdots n] \).
	
	%where \( \face[min=n] \) and \( \face[max=n] \) are the unique
	%morphisms~\( \ordset{0} \into \ordset{n} \)
	%given by \( \face[min=n] { 0 } = 0 \) and \( \face[max=n] { 0 } = n \).
	%In other words,
	%\( \face[min=n] = \face[d=0] \face[d=0] \cdots \face[d=0] \)
	%and \( \face[max=n] =  \face[d=n] \face[d=n-1] \cdots \face[d=1] \).
	%We shall denote such pairs by~\( \tup { \algM , {\mtheta[ibullet]} } \).
	
	%On the morphism level, we claim the equalizer in question is in fact the full subcategory
	%of~\(
	%\Prod{\catainftyfun[o] { {\ordset{n}[linearize=\ringk]} , \cosimpdgcatA{n}}}
	%\)
	%consisting of these objects
	
	On the morphism level, suppose
	%\( \tup { \algM , {\mtheta[ibullet]} } \)
	%and~\( \tup { \algN , {\meta[ibullet]} } \)
	\( \mF[d=n] \) and~\( \mG[d=n] \)
	are objects of the equalizer.
	%A morphism
	%\(
	%	\tup { \algM , {\mtheta[ibullet]} }
	%	\to
	%	\tup { \algN , {\meta[ibullet]} }
	%\)
	%consists of the
	%morphisms~
	A morphism~\( \mF[*] \to \mG[*] \)
	of degree~\( d \)
	consists of a
	collection~\(
		\malpha[*] = \tup { {\malpha[d=n]} }[\ordset{n}\in\catdelta[plus]]
	\)
	of morphisms \( \malpha[d=n] \colon \mF[d=n] \to \mG[d=n] \)
	in~\( \catainftyfun[o]{ {\ordset{n}[linearize=\ringk]},\cosimpdgcatA{n} } \) that simultaneously lie in the equalizer.
	%The space of morphisms~\( \mF[d=n] \to \mG[d=n] \) is\fxfatal{Yes, if \( \catainftyfun[o] \)~is a full subcategory of~\( \catainftyfun \).}
%	\[
%		\catainftyfun[o]{
%			{\ordset{n}[linearize=\ringk]},
%			\cosimpdgcatA{n}
%		} { {\mF[d=n]} , {\mG[d=n]} }
%		=
%		\coch[hoch]{*} {
%			{ \ordset{n}[linearize=\ringk,reduce] } ,
%			{ \cosimpdgcatA{n}[ symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%		}
%	\]
%	and thus the morphism space of transformations~\( \mF[*]\to\mG[*] \) is
	From \cref{ex:A_infty_fun_k_n_to_B}, we therefore
	get that the space of non-identity transformations~\( \mF[*]\to\mG[*] \) is
	\begin{align*}
		\MoveEqLeft
		\End {
%			\coch[hoch,par=\big]{*} {
%				{ \ordset{n}[linearize=\ringk,reduce] } ,
%				{ \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] }
%			}
			\Hom[*,par=\big] {
				\tensorcoalg{{
					\ordset{n}[linearize=\ringk,reduce,return,shift=-1]
				}},
				\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
					\cosimpdgcatA{n}
				}
			}
		}
%	\\
		=
		\End {
			\Hom[*,par=\big,
			%{\catcom{k}[diag=\ordset{n}\times\ordset{n}]}
			] {
				%\tensorcoalg{ {\ordset{n}[linearize=\ringk,reduce]} }
				\textstyle\dirsum[limits,l\ge0,return,operator] { {\ordset{n}[linearize=\ringk,reduce,return,tens=l,shift=-l]} }
				,
				{
%					\cosimpdgcatA{n}[
%						symbolputleft=\!\!,
%						leftrestrict=\mF[n],
%						rightrestrict=\mG[n]
%					]
					\map{\mF[d=n]\times\mG[d=n]}[spar,qpull] {
						\cosimpdgcatA{n}
					}
				}
			}
		}
	%\\
	%	&=
	%	\End[ \ordset{n}\in\catdelta[plus] ] {
	%		\Hom[\catdgcat] { \simp[dg]{n} ,  }
	%	}
	\\
		&=
		\End {
			\Prod[l\ge0] {
				\Prod[0\le i_0<\cdots<i_l\le n] {
					\Hom[*,\ringk,par=\big%,\catcom{k}
					] {
						\ringk
						\mf[i_{l-1} i_l]
						%\sotimes
						%\mf[i_{n-2} i_{n-1} ]
						\sotimes
						\cdots
						\sotimes
						\mf[ i_0 i_1 ]
						,
						{\cosimpdgcatA{n}[arg={
							{\mF[d=n] { i_0 } } ,
							{\mG[d=n] { i_l } }
						}]}
					 }
				}
			}
		}
	\end{align*}
	(note that
	%\( \ordset{n}\to \cosimpdgcatA{n}[symbolputleft=\!\!,leftrestrict=\mF[n],rightrestrict=\mG[n]] \)
	\(
		\ordset{n}\mapsto
		\map{ \mF[d=n]\times\mG[d=n] }[spar,qpull] {
			\cosimpdgcatA{n}
		}
	\)~defines a semicosimplicial dg-quiver).
	%This means that \( \malpha \)~is determined freely\fxfatal{Add in details}
	%by what it does to 
	%As a cosimplicial quiver, \( \ordset{n}\mapsto \tensorcoalg { \ordset{n}[linearize=\ringk,reduce] } \) is freely generated
	Thus the transformation~\( \malpha[*] \) is freely determined
	by what it does to the
	non-degenerate elements~\( \mf[n-1,n] \sotimes \cdots \sotimes \mf[0,1] \),
	i.e.\ by the
	elements
	\[
		\malpha[d=n] {{ \mf[n-1,n] \sotimes \cdots \sotimes\mf[0,1] }}
		\in
		\cosimpdgcatA{n}[arg={
			{\mF[d=n] { i_0 } } ,
			{\mG[d=n] { i_n } }
		}]
		.
	\]
	Calling this element~\( \malpha[n] \),
	we obtain the desired description.
\end{proof}

\section{Homotopy descent of dg-schemes}

\newclassset\dgschemeX{\mathbf{X}}
\newclassset\dgschemeY{\mathbf{Y}}
\newclassset\dgschemeZ{\mathbf{Z}}
\newclassset\dgschemeU{\mathbf{U}}
\newsheaf\shM{\mathscr{M}}
\newcategory\catdgaff{dgAff}

If \( \ringk \)~is a field, the category of \textdef{affine dg-schemes}
over~\( \ringk \)
is the opposite category~\( \catdgaff = \catdgalg[le0,com,spar,op] \)
to the category of non-positively graded, supercommutative dg-algebras
over~\( \ringk \).
If \( \dgschemeX \)~is a dg-scheme,
the associated dg-algebra is denoted~\( \dgcatA[\dgschemeX] \).
The category of \textdef{quasi-coherent dg-sheaves}
over~\( \tup{ \dgschemeX , \dgcatA[\dgschemeX] } \)
is the category~\( \catxdgmod{\dgcatA[\dgschemeX]} \)
of \( \dgcatA[\dgschemeX] \)-dg-modules.

%By a \textdef{dg-scheme}\fxfatal{Riche and friends have all kinds of extra assumptions, including Noetherian and blah blah blah, but I do not see right now what we need it for.},
%we shall mean a pair~\( \dgschemeX = \tup{\setX,\dgcatA[\dgschemeX]} \),
%where \( \dgcatA[\dgschemeX] \)~is a sheaf of non-positively graded,
%super-commutative \( \reg[\setX] \)-dg-algebras.
%A \textdef{quasi-coherent dg-sheaf} over~\( \dgschemeX \)
%is a sheaf of \( \dgcatA[\dgschemeX] \)-dg-modules~\( \shM[*] \)
%on~\( \setX \)
%such that each graded piece~\( \shM[d=i] \)
%is a quasi-coherent sheaf of \( \reg[\setX] \)-modules.
%The dg-category of such is denoted~\( \catdgqcoh{\dgschemeX} \).
%It is called a \textdef{coherent dg-sheaf}
%if its cohomology~\( \co{*}{ \shM } \)
%is a locally finitely generated as a sheaf of
%graded \( \co{*}{ \dgcatA[\dgschemeX] } \)-modules.
%%The dg-category of such is denoted~\( \catqcoh{\dgschemeX} \),
%%and its dg-derived category is denoted~\( \der[dg]{\catqcoh{\dgschemeX}} \).
%%Its homotopy category~\( \co[nopar]{0}{\der[dg]{\catqcoh{\dgschemeX}}} \)
%%recovers the classical derived category~\( \der{\catqcoh{\dgschemeX}} \).
%The dg-derived categories of these
%are denoted~\( \der[dg,smash,nopar]{ \catdgqcoh{\dgschemeX} } \)
%and~\( \der[dg,smash,nopar]{ \catdgcoh{\dgschemeX} } \).
%Their homotopy categories recover the classical derived categories,
%\[
%	\co{0}{{ \der[dg,nopar]{ \catdgqcoh{\dgschemeX} } }}
%	=
%	\der[nopar]{ \catqcoh{\setX} }
%\qquad\text{and}\qquad
%	\co{0}{{ \der[dg,nopar]{ \catdgcoh{\dgschemeX} } }}
%	=
%	\der[b,nopar]{ \catcoh{\setX} }
%\]
%
%Suppose now that \( \set{ \dgschemeU[i] \to \dgschemeY } \)~is an
%affine fpqc covering of a dg-scheme~\( \dgschemeY \),
%and write \( \dgschemeU[i_0\cdots i_n] = \dgschemeU[i_0]\cap\cdots\cap\dgschemeU[i_n] \).
%Consider the \ancech groupoid~\(
%	\dgschemeX[1]
%	\rightrightarrows
%	\dgschemeX[0]
%\)
%associated to this covering
%%Consider the \textdef{\ancech nerve} with respect to this covering.
%%This is the internal Kan complex in affine dg-schemes
%%given by~\( \dgschemeX[0] = \Coprod{ \dgschemeU[i] } \),
%%\( \dgschemeX[1] = \Coprod{ \dgschemeU[ij] } \), and more generally,
%and the associated classifying space, the \ancech nerve, given by
%\[\textstyle
%	\dgschemeX[n]
%	=
%	\dgschemeX[1]
%	\fibre[\dgschemeX[0]]
%	\dgschemeX[1]
%	\fibre[\dgschemeX[0]]
%	\cdots
%	\fibre[\dgschemeX[0]]
%	\dgschemeX[1]
%	=
%	\Coprod{
%		\dgschemeU[i_0 i_1 \cdots i_n]
%	}
%\]
%(we note that we do not have to take derived intersections
%as the maps involved are flat).
%The simplicial structure on~\( \dgschemeX[ibullet] \)
%is given by the usual formula.
%Then \( \catdgqcoh{\dgschemeX[ibullet]} \)~becomes
%a cosimplicial system of dg-categories
%via pullbacks (which are already derived because of~fpqc).
%Then descent theory in derived algebraic geometry tells
%us that the natural map
%\[\textstyle
%%	\der[dg,nopar]{
%		\catdgqcoh{\dgschemeY}
%%	}
%	\to
%	\invholim[\catdelta]{
%		%\der[dg,nopar]{
%			\catdgqcoh{\dgschemeX[ibullet]}
%		%}
%	}
%\]
%is a quasi-equivalence of dg-categories, the homotopy limit being taken in dg-categories.


%\begin{theorem}\label{res:A_infty_comodules}
%	%Suppose that \( \ssetX{*} \)~is a simplicial affine scheme
%	%for which all face maps~\( \face[d=i]\colon\ssetX{n}\to\ssetX{n-1} \) are flat.
%	As in the introduction, suppose that \( \ssetX{1} \rightrightarrows \ssetX{0} \)~are a monoid in affine schemes
%	such that \( \face[d=0] \) and~\( \face[d=1] \) are flat,
%	and let~\( \ssetX{*} \) be its classifying space.
%	Let~\( \algC \) be the coalgebra~\( \algC = \reg { \ssetX{1} } \)
%	over the commutative ring~\( \algA = \reg { \ssetX { 0 } } \).
%	Then we have an equivalence of categories
%	\[\textstyle
%		\invholim[\catdelta] { \catcom { \catqcoh{\ssetX{n}} } }
%		\cong
%%		\catcomod[infty,hcu,formal] { \algC }
%		\catxcomod{ \algC }[infty,hcu,formal]
%	.\]
%	%where \( \algC \)~is the coalgebra \( \algC = \reg { \ssetX{1} } \), the underlying commutative ring
%	%is~\( \algA = \reg { \ssetX { 0 } } \).
%	%\fxfatal{For unity condition, we should add flatness somewhere.}\fxfatal{{\color{red}NEED HOMOTOPY COUNITAL CONDITION!}}
%	The \anrhs denotes the dg-category of \textdef{homotopy-counital}
%	%right
%	left
%	\ainfty-comodules over~\( \algC \) in the category~\( \catxmodx{\algA}{\algA} \), which, for us, means that the second coaction map~\( \ca[2]\colon\algM\to\algC\tens[\algA]\algM \)~is
%	homotopy-invertible. The “\categoryformat{formal}”
%	part means that we omit the condition that
%	the product~\(
%		\Prod[i\ge1]{ \ca[i] }
%		\colon
%		\algM
%		\to
%		\Prod[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\)
%	factors through the direct sum~\(
%		\dirsum[i\ge1] {
%			\algC[tens={(i-1)}]
%			\tens[\algA]
%			\algM
%		}
%	\).
%	(We hope later to find sufficient conditions under which  we can remove
%	this “\categoryformat{formal}”.)
%\end{theorem}

\begin{theorem}\label{res:A_infty_comodules}
	Suppose that
	\( \dgschemeX[1] \rightrightarrows \dgschemeX[0] \)
	is a groupoid in affine dg-schemes,
%	with
%	source and target maps~\( \face[d=0],\face[d=1] \)
%	both~flat,
	and consider the associated classifying space~\( \dgschemeX[ibullet] \) given by
	\[\textstyle
		\dgschemeX[n]
		=
		\dgschemeX[1]
		\fibre[\dgschemeX[0]]
		\dgschemeX[1]
		\fibre[\dgschemeX[0]]
		\cdots
		\fibre[\dgschemeX[0]]
		\dgschemeX[1]
		.
	\]
	Write~\( \cosimpdgcatA{n} = \dgcatA[\dgschemeX[n],smash] \)
	for the associated cosimplicial system of dg-algebras.
	Let~\( \dgcatA = \cosimpdgcatA{0} \)
	and~\( \dgcatC = \cosimpdgcatA{1} \),
	and note that \( \dgcatC \)~is a
	counital
	coalgebra\fxfatal{Is it cocomplete? Also, remember to assume it is \emph{affine}, or the \( \dgcatA \)'s will only be \emph{sheaves}.} in~\( \catxdgmodx{\dgcatA}{\dgcatA} \)
	via the map~\(
		\comult
		=
		\face[d=1,comor]
		\colon
		\dgcatC
		\to
		\dgcatC\tens[\dgcatA]\dgcatC
	\).
	Then we have an equivalence of dg-categories
	\[\textstyle
		\invholim[\catdelta]{
			%\der[dg,nopar]{
				\catdgqcoh{ \dgschemeX[ibullet] }
			%}
		}
		\cong
		\catxcomod{\dgcatC}[infty,hcu,formal]{\dgcatA}
		,
	\]
	where the \anrhs denotes the dg-category
	of formal, homotopy-counital \ainfty-comodules
	over~\( \dgcatC \)
	in~\( \catxdgmod{\dgcatA} \).
\end{theorem}

%\newmap\adjunit{u}[nopar]
%
%\begin{lemma}
%	Let the assumptions be as in the theorem.
%	For any~\( n\ge 0 \),
%	we shall write~\(
%		\adjunit[d=n]
%		\colon
%		\id[\cosimpdgcatA{0}]
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] }}
%	\)
%	for the unit of adjunction.
%	If~\( \algM \in \cosimpdgcatA{0} \),
%	we wirte~\( \adjunit[d=n,\algM] \) for the
%	map~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \).
%	
%	Let \( \algM , \algN , \algP \)~be objects of~\( \cosimpdgcatA{0} \),
%	and suppose we are given maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	\)
%	in~\( \cosimpdgcatA{j} \).
%	Then
%	\[
%%		\face[max=j,shpush] {{
%%			\face[min=j,shpull] {{ \adjunit[j] { \meta } }}
%%		}}[spar]
%		\adjunit
%		\circ
%		%\adjunit[i] { \mtheta }
%		\face[max=i,shpull] { \mtheta }
%		\circ
%		\adjunit[d=i,\algM]
%		=
%		\map {
%			\face[min=i,shpull] { \meta }
%			\circ
%			\face[max=j,shpull] { \mtheta }
%		}[spar]
%		\circ
%		\adjunit[i+j]
%	\]
%\end{lemma}

%We initially consider terms of the
%form~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \).
%As in the proof of \cref{res:equivariance=comodules},
%base change will be crucial.
%Applying flat base change to the pullback diagram
%\[\begin{tikzcd}
%	\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%		& \ssetX{i} \ar[d,"{\face[min=i]}"]
%\\
%	\ssetX{j} \ar[r,"{\face[max=j]}"']
%		& \ssetX{0}
%\end{tikzcd}\]
%we obtain
%\(
%	\face[max=j,shpush] \face[min=i,shpull]
%	\cong
%	\face[min=i,shpull] \face[max=j,shpush]
%\)
%and~\(
%	\face[max=j,shpull] \face[min=i,shpush]
%	\cong
%	\face[min=i,shpush] \face[max=j,shpull]
%\).
%This implies
%
%\begin{lemma}\label{res:base_change_face_maps}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given objects~\( \algM , \algN , \algP \in \cosimpdgcatA{0} \),
%	along with two maps~\(
%		\mtheta
%		\colon
%		\face[max=i,shpull] { \algM }
%		\to
%		\face[min=i,shpull] { \algN }
%	\)
%	in~\( \cosimpdgcatA{i} \)
%	and~\(\smash{
%		\meta
%		\colon
%		\face[max=j,shpull] { \algN }
%		\to
%		\face[min=j,shpull] { \algP }
%	}\)
%	in~\( \cosimpdgcatA{j} \), where~\( i , j \ge 0 \).
%	Then the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i,shpush] {{ \face[max=i,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algN } }}
%				\ar[r]
%					\& \face[max=i,shpush] {{
%						\face[min=i,shpull] {{
%							\face[max=j,shpush] {{
%								\face[max=j,shpull] {{
%									\algN
%								}}
%							}}
%						}}
%					}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{} \ar[r,"{\meta}"']
%			\& \face[max=i,shpush] {{
%				\face[min=i,shpull] {{
%					\face[max=j,shpush] {{
%						\face[min=j,shpull] {{
%							\algP
%						}}
%					}}
%				}}
%			}}
%			\ar[r,symbol={\cong}]
%				\&[-1.5em] \face[max=i,shpush] {{
%				 \face[max=j,shpush] {{
%						\face[min=i,shpull] {{
%							\face[min=j,shpull] {{
%								\algP
%							}}
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					\&[-1.5em] \face[max=i+j,shpush] {{	
%						\face[min=(i+j),shpull] {{ \algP }}
%					}}
%	\invdot
%	\end{tikzcd}\end{align*}
%	is the same as the composition
%	\begin{align*}
%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=i+j,shpush] {{
%				\face[max=(i+j),shpull] {{ \algM }}
%			}}
%			\ar[r,"{\face[max=j,shpull]{ \mtheta }}"]
%				\&\face[max=i+j,shpush] {{
%					\face[max=j,shpull] {{
%						\face[ min=i, shpull ] { \algN }
%					}}
%				}}
%	\end{tikzcd}
%	\\[-.7em]
%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\&{}= \face[max=i+j,shpush] {{
%			\face[min=i,shpull] {{
%				\face[ max=j, shpull ] { \algN }
%			}}
%		}}
%		\ar[r,"{\face[min=i,shpull] { \meta }}"']
%			\&\face[max=i+j,shpush] {{
%				\face[min=i,shpull] {{
%					\face[ min=j, shpull ] { \algP }
%				}}
%			}}
%			\ar[r,symbol={=}]
%				\&[-1.5em] \face[max=i+j,shpush] {{
%					\face[min=\smash{(i+j)},shpull] {{ \algP }}
%				}}
%				.
%	\end{tikzcd}\end{align*}
%	In other words, the map is
%	the unit of adjunction~\(
%		\algM
%		\to
%		\face[max=i+j,shpush] {{
%			\face[max=(i+j),shpull] { \algM }
%		}}
%	\)
%	composed with the
%	map~\(\smash{
%		\face[min=i,shpull] { \meta }
%		\circ
%		\face[max=j,shpull] { \mtheta }
%	}\).
%\end{lemma}
%
%\begin{lemma}\label{res:add_comultiplication_map}
%	Let the assumptions be as in~\cref{res:A_infty_comodules}.
%	Suppose that we are given
%	objects~\( \algM , \algN \in \cosimpdgcatA{0} \)
%	along with a
%	map~\(
%		\mtheta
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\).
%%	Then the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta}"]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%%				\ar[r]
%%					& \face[max=n,shpush] {{
%%						\face[d=i,shpush] {{
%%							\face[d=i,shpull] {{
%%								\face[min=n,shpull] { \algN }
%%							}}
%%						}}
%%					}}
%%					\ar[r,symbol={=}]
%%						&[-1.5em]
%%						\face[min=n+1,shpush] {{
%%							\face[max=\smash{(n+1)},shpull] {{ \algN }}
%%						}} .
%%	\end{tikzcd}\]
%%	is the same as the composition
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r]
%%			& \face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%			\ar[r,"{ \face[d=i,shpull] { \mtheta } }"]
%%				& \face[max=n+1,shpush] {{
%%					\face[min=(n+1),shpull] { \algN }
%%				}}
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}}
%%					\invdot
%%	\end{tikzcd}\]
%	Let~\( 1 \le i < n \).
%	Then we have a commutative diagram
%	\[\begin{tikzcd}[sep=scriptsize]
%		\algM \ar[r] \ar[d,dashed]
%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%			\ar[r,"{\mtheta}"]
%			\ar[d,dashed]
%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algN } }}
%				\ar[d]
%	\\
%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%		\ar[r,dashed]
%			& \face[max=n,shpush] {{
%				\face[d=i,shpush] {{
%					\face[d=i,shpull] {{
%						\face[max=n,shpull] { \algM }
%					}}
%				}}
%			}}
%			\ar[r,"{\face[d=i,shpull]{\mtheta}}"]
%				& \face[max=n,shpush] {{
%					\face[d=i,shpush] {{
%						\face[d=i,shpull] {{
%							\face[min=n,shpull] { \algN }
%						}}
%					}}
%				}}
%				\ar[r,symbol={=}]
%					&[-1.5em]
%					\face[max=n+1,shpush] {{
%						\face[min=\smash{(n+1)},shpull] {{ \algN }}
%					}} .
%	\end{tikzcd}\]
%\end{lemma}

\begin{proof}[Proof of \cref{res:A_infty_comodules}]
	\Cref{res:homotopy_limit_dgcat} gives us the general form
	of the homotopy limits of~\( \cosimpdgcatA{*} \),
	so we use the same notation.
%	By adjunction, the resulting
%	morphism~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\),
%	where \( n\ge 1 \),
%	is equivalent to a
%	map
%	\(
%		\algM
%		\to
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%		\xto{\mtheta[n]}
%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%	\).
%	We add to this collection~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
%	Putting~\( \ca[n] = \mtheta[n-1] \) for all~\( n\ge 1 \),
	Thus an object of the homotopy limit
	is a pair~\( \tup{\algM,\mtheta} \),
	where
	\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)~is
	a collection of maps~\(
		\mtheta[n]
		\colon
		\face[max=n,shpull] { \algM }
		\to
		\face[min=n,shpull] { \algM }
	\) of degree~\( 1-n \),
	and a morphism~\(
		\malpha
		\colon
		\tup{\algM,\mtheta}
		\to
		\tup{\algN,\meta}
	\)
	is a collection~\(
		\malpha = \tup{\malpha[n]}[n\ge0]
	\)
	of maps~\(
		\malpha[n]
		\colon
		\face[max=n,shpull]{\algM}
		\to
		\face[min=n,shpull]{\algN}
	\)
	of degree~\( \dgcatdeg{\malpha} - n \).
%	For a morphism~\(
%		\malpha
%		\colon
%		\tup{\algM,\mtheta}
%		\to
%		\tup{\algN,\meta}
%	\)
%	in the homotopy limit,
	For such a morphism,
	we scale it to define a new morphism~\( \malpha[tilde] \) by
	\(
		\malpha[tilde,n]
		=
		(-1)^{\dgcatdeg{\malpha}(n+1)}
		\malpha[n]
	\).
%	For an object~\( \tup{\algM,\mtheta} \),
%	we extend the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	by \( \mtheta[0] = \dif[\algM] \), the differential on~\( \algM \).
	Regarding this~\( \mtheta \) as a degree~\( 1 \)
	morphism~\( \tup{\algM,\mtheta}\to\tup{\algM,\mtheta} \),
	we use the same notation as for morphisms and
	write~\(
		\mtheta[tilde,n]
		=
		(-1)^{n+1}
		\mtheta[n]
	\) for~\( n\ge 1 \).
%	We also write~\( \dif[tilde,\algM] = - \dif[\algM] \).
	We notice that \eqref{res:morphisms_in_tot_composition} becomes
	\[
		\map{\mbeta\circ\malpha}[spar,widetilde,n]
		=
		\Sum[from={i=0},to={n}]{
			(-1)^{\dgcatdeg{\mbeta}i}
			\face[min=i,shpull]{{ \mbeta[tilde,n-i] }}
			\circ
			\face[max=(n-i),shpull]{{ \malpha[tilde,i] }}
		}.
	\]
	Thus
	\eqref{eq:theta_n_equation}~becomes
	%\[%\begin{equation}\label{eq:infinity_comod_theta_equation}
	\begin{align*}
		%\dif[par]{{\mtheta[tilde,n]}}
%		\MoveEqLeft
%		(-1)^{n}
%		(
%			\face[min=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		(-1)^{n+1}
		\dif[ {\face[min=n,shpull]{\algM}} ]
		\circ
		\mtheta[tilde,n]
%		-
%		(-1)^{1-n}
%	\\
%		&
%		{}
		-
		\mtheta[tilde,n]
		\circ
%		(
%			\face[max=n,shpull]{{
%				%\mtheta[tilde,0]
%				\dif[tilde,\algM]
%			}}
%			-
%			\dif[i={\dgcatC[tens=n-1]}]
%			\tens
%			\id[\algM]
%		)
		\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%		&
		=
		-
		\map{\mtheta\circ\mtheta}[widetilde,spar,n]
		+
		\Sum[from={i=1},to={n-1}]{
			%(-1)^{n-i+1}
			(-1)^{i}
			\face[d=i,shpull]{{ \mtheta[tilde,n-1] }}
		}
		.
	%\end{equation}
	%\]
	\end{align*}
	Since~\(
		\dif[par]{\malpha}[widetilde,n]
		=
		(-1)^{(\dgcatdeg{\malpha}+1)(n+1)}
		\dif[par]{\malpha}[n]
	\),
	\eqref{res:morphisms_in_tot_differential}~becomes
	\begin{align*}
			\dif[par]{\malpha}[widetilde,n]
			&
			=
			(-1)^{n+1}
			%\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
%			-
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\face[max=n,shpull]{{ \dif[tilde,\algM] }}
			\dif[ {\face[max=n,shpull]{\algM}} ]
%	\\
%			&
%			\qquad
%			{}
			+
			\map{\meta\circ\malpha}[widetilde,spar,n]
	\\
			&
			\qquad
			{}
			-
			(-1)^{\dgcatdeg{\malpha}}
			\map{\malpha\circ\mtheta}[widetilde,spar,n]
%	\\
%			&
%			\qquad
%			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	\\
			&=
%			(-1)^n
%			\face[min=n,shpull]{{ \dif[tilde,\algN] }}
			(-1)^{n+1}
			\dif[ {\face[min=n,shpull]{\algN}} ]
			\circ
			\malpha[tilde,n]
			+
			\Sum[from={i=0},to={n-1}]{
				(-1)^{i}
				\face[min=i,shpull]{{
					\meta[tilde,n-i]
				}}
				\circ
				\face[max=(n-i),shpull]{{
					\malpha[tilde,i]
				}}
			}
	\\
			&\qquad
			{}
			+
			(-1)^{\dgcatdeg{\malpha}}
			\malpha[tilde,n]
			\circ
			%\dif[tilde,\algM]
			\dif[ {\face[max=n,shpull]{\algM}} ]
			-
			\Sum[from={i=1},to=n]{
				(-1)^{\dgcatdeg{\malpha}(i+1)}
				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
				\circ
				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
			}
	\\
			&\qquad
			{}
			+
			\Sum[from={j=1},to={n-1}]
				(-1)^{j-1}
				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
	,\end{align*}


	Now for an object~\( \tup{\algM,\mtheta} \),
	we add to the collection~\( \tup{\mtheta[n]}[n\ge1] \)
	the element~\( \mtheta[0] = -\dif[\algM] \).
	We then
%	where~\(
%		\mtheta[n]
%		\colon
%		\face[max=n,shpull] { \algM }
%		\to
%		\face[min=n,shpull] { \algM }
%	\) is a map of degree~\( 1-n \).
%	and add to the collection~\( \mtheta = \tup{\mtheta[n]}[n\ge1] \)
%	%add to this
%	the
%	collection~
%	and write~\( \mtheta[0] = \dif[\algM] \),
%	the differential on~\( \algM \).
	define the comodule
	operations~\( \ca[n] \colon \algM \to \dgcatC[tens=(n-1)]\tens\algM \)
	of degree~\( 2 - n \)
	by
	\[\begin{tikzcd}%[sep=scriptsize]
		\ca[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\mtheta[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
	\end{tikzcd}\]
	where the first map is the unit of adjunction.
	In particular, \( \ca[1] = -\dif[\algM] \).	
	Similarly, if
	\( \malpha \colon \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
	is a map of degree~\( \dgcatdeg{\malpha} \),
%	where
%	\(
%		\malpha[n]
%		\in
%		\Hom[\cosimpdgcatA{n},d=\dgcatdeg{\malpha}-n]{
%			{\face[max=n,shpull]{\algM}},
%			{\face[min=n,shpull]{\algM}}
%		}
%	\),
	we associate to it
	the map of \ainfty-comodules~\(
		\mf \colon \algM \to \algN
	\)
	of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \),
	where
	\(
		\mf[n]
		\colon
		\algM
		\to
		\dgcatC[tens=(n-1)]\tens[\dgcatA] \algN
	\)
	is the map of degree~\(
		\dgcatdeg{\malpha} + 1 - n
		=
		\dgcatdeg{\mf} + 1 - n
	\)
	given by
	\[\begin{tikzcd}%[sep=scriptsize]
		\mf[n]
		\colon
		\algM
		\ar[r]
		&
		\face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
		\ar[r,"{\malpha[tilde,n-1]}"]
		&%[3em]
		\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algN } }}
		.
	\end{tikzcd}\]
	It is immediate that the composition map above
	agrees with the composition of maps of \ainfty-comodules.
%	Now the two lemmas show that the above two equations are exactly the
%	\ainfty-comodule equations.
	%Via the two lemmas,
	Via~\cref{res:add_comultiplication_map,res:base_change_face_maps},
	the other two equations above now become
	\begin{align*}
		\MoveEqLeft
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[\algM]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\ca[n+1]
		+
		\ca[n+1]
		%\dif[\algM]
		\ca[1]
	\\
		&
		=
		-
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			( \id[ {\dgcatC[tens=i]} ]\tens\ca[n-i+1] )
			\ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={i=1},to={n-1}]{
			(-1)^{i}
			(
				\id[tens=(i-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-i)]
			)
			\ca[n]
		}
	\\
	\shortintertext{and}
		\dif{\mf}[spar,n]
		&
		=
		(-1)^{n+1}
		(
			\dif[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\id[N]
			-
			\id[\dgcatC\tens\cdots\tens\dgcatC]
			\tens
			\ca[1]
		)
		\mf[n+1]
		+
		\Sum[from={i=0},to={n-1}]{
			(-1)^{i}
			\ca[n-i+1] \mf[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		(-1)^{\dgcatdeg{\malpha}}
		\mf[n+1]\ca[1]
		-
		\Sum[from={i=1},to={n}]{
			(-1)^{\dgcatdeg{\malpha}(i+1)}
			\mf[n-i+1] \ca[i+1]
		}
	\\
		&
		\qquad
		{}
		+
		\Sum[from={j=1},to={n-1}]{
			(-1)^{j-1}
			(
				\id[tens=(j-1)]
				\tens
				\comult[\dgcatC]
				\tens
				\id[tens=(n-j)]
			)
			\ca[n]
		},
	\end{align*}
	which are exactly the \ainfty-comodule equations from earlier.	
%	For all objects~\( \tup{\algM,\mtheta} \),
%	we now extend the collection~\( \mtheta = \tup{\mtheta}[n\ge1] \)
%	by~\( \mtheta[0] = \dif[\algM] \).
%	Following the above convention with~\( \mtheta[tilde,n] \),
%	this allows us to write~\( \mtheta[tilde,0] = - \mtheta[0] = \dif[tilde,\algM] \).
%	Then the two above equations become
%	\[
%		0
%		=
%		\Sum[from={i=0},to={n}]{
%			(-1)^{i}
%			\face[min=i,shpull]{{ \mtheta[tilde,n-i] }}
%			\circ
%			\face[max=(n-i),shpull] {{ \mtheta[tilde,i] }}
%		}
%		+
%		\Sum[from={i=1},to={n-1}]{
%			(-1)^{i-1}
%			\face[d=i,shpull]{{
%				\mtheta[tilde,n-1]
%			}}
%		}
%	\]
%	and
%	\begin{align*}
%			\dif{\malpha}[widetilde,spar,n]
%			&=
%			\Sum[from={i=0},to={n}]{
%				(-1)^{i}
%				\face[min=i,shpull]{{
%					\meta[tilde,n-i]
%				}}
%				\circ
%				\face[max=(n-i),shpull]{{
%					\malpha[tilde,i]
%				}}
%			}
%	\\
%			&
%			{}
%			-
%			\Sum[from={i=0},to=n]{
%				(-1)^{\dgcatdeg{\malpha}(i+1)}
%				\face[min=i,shpull]{{ \malpha[tilde,n-i] }}
%				\circ
%				\face[max=(n-i),shpull]{{ \mtheta[tilde,i] }}
%			}
%			+
%			\Sum[from={j=1},to={n-1}]
%				(-1)^{j-1}
%				\face[d=j,shpull] {{ \malpha[tilde,n-1] }}
%	\end{align*}

	To verify that we get exactly \emph{homotopy-counital} \ainfty-cmodules,
	we notice that the
	equation~\eqref{eq:theta_n_equation}
	in the case~\( n = 2 \) yields that
	\[
		\dif[par]{\mtheta[2]}
		=
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		-
		\face[d=1,shpull]{\mtheta[1]}
		,
	\]
	so that we have a homotopy~\(
		\face[d=0,shpull]{\mtheta[1]}
		\circ
		\face[d=2,shpull]{\mtheta[1]}
		\simeq
		\face[d=1,shpull]{\mtheta[1]}
	\).
	Then the proof of \cref{res:cocycle_iff_degen=0},
	with equalities replaced by homotopies,
	shows that \( \mtheta[1] \)~being an isomorphism is equivalent to~\( \degen[d=0,shpull]{\mtheta[1]}\simeq\id \).
	Similarly, one adjusts the
	last part of the proof of \cref{res:descent=comodules}
	to obtain that~\(
		(\counit\tens\id[\algM])\ca[2]
		\simeq
		\id
	\),
	which means that \( \algM \)~is homotopy-counital.
\end{proof}


%	
%	We initially check that the maps~\( \ca[n] \colon \algM \to \algC[tens=(n-1)] \tens \algM \),
%%	so let us for~\( k\ge 1 \) check the equation
%%	\[
%%		\Sum {
%%			(-1)^{i+mj}
%%			(
%%				\id[tens=i] \tens \comult[m] \tens \id[tens=j]
%%			)
%%			\ca[n]
%%		}
%%		= 0
%%	\]
%%	for all~\( i,m,j,n \) such that
%%	\( i + m + j = k \)
%%	and~\( n = i + 1 + j \),
%%	and where we, in the case~\( j=0 \),
%	satisfy the equations for an \ainfty-comodule,
%	so let us for all~\( k\ge 1 \) check the equation
%	\[
%		\Sum {
%			(-1)^{(i-1)+m(n-i)}
%			(
%				\id[tens=(i-1)] \tens \comult[m] \tens \id[tens=(n-i)]
%			)
%			\ca[n]
%		}
%		= 0 ,
%	\]
%	where the sum runs over the positive
%	integers~\( i, m, n \) such
%	that~\( 0\le i\le n\)
%	and~\( n + m - 1 = k \)
%	and where we, in the
%	case~\( i=n \),
%	interpret \( \comult[m] \) as~\( \ca[m] \).
%	%In other words, the sum has
%	%By base change, we obtain
%	%In other words, the sum consists
%	We notice that the term~\( m(n-i) \) in the exponent
%	of the sign is always even. Indeed,
%	if~\( n-i > 0 \), then \( \comult[m] = \comult[m,upper=\algC] \)~is the \ainfty-operation
%	on~\( \algC \), and so \( \comult[m,upper=\algC] = 0 \)
%	unless~\( m = 2 \). Thus we are left with~\( (-1)^{i-1} \).
%	%Also, in order to rewrite this equation in terms
%	%of the maps~\( \mtheta[n] \), it is convenient to replace
%%	\( n , m \) by~\( n+1 , m+1 \),
%%	so we are left with the equation
%%	\[
%%%		\Sum[i={m+n-1 = k} ] {{
%%			\Sum[from={i=1},to={k-1}] {{
%%				(-1)^i
%%				\bigl(
%%					(
%%						\id[tens=(i-1)]
%%						\tens
%%						\comult[2,upper=\algC]
%%						\tens
%%						\id[tens=(n-i)]
%%					) \ca[(k-2)+1]
%%					-
%%					abe
%%				\bigr)
%%			}}
%%			=0
%%%		}}
%%	\]
%%	for all~\( k\ge 1 \).
%	Thus the equation may be reduced to
%	\begin{align*}
%		0
%			&=
%			\Sum[from={n=1},to={k}] {{
%				(-1)^{n-1}
%				(
%					\id[tens=(n-1)]
%					\tens
%					\ca[k+1-n]
%				)
%				\ca[n]
%			}}
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(k-i-1)]
%				)
%				\ca[k-1]
%			}}
%	\\
%			&=
%			\ca[k]\circ\ca[1]
%			- (-1)^{k} (\id[tens=(k-1)]\tens\ca[1]) \ca[k]
%	\\
%			&\qquad{}+
%			\Sum[from={i=1},to={k-2}] {{
%				(-1)^{i-1}
%				\bigl(
%					(
%						\id[tens=(i-1)]
%						\tens
%						\comult[2,upper=\algC]
%						\tens
%						\id[tens=(k-i-1)]
%					)
%					\ca[k-1]
%					-
%					(
%						\id[tens=i]
%						\tens
%						\ca[k-i]
%					)
%					\ca[i+1]
%				\bigr)
%			}}
%	\end{align*}
%%	Since the differential on~\( \algC \) is zero and \( \ca[1] = \dif[\algM] \), the first
%%	two terms are
%%	simply~\(
%%		-
%%		(-1)^{2-k}
%%		\dif[par] { \ca[k] }
%%	\).
%	Substituting \( n+1 \) for~\( k \), we obtain
%	that the equation we must verify is
%	\begin{align*}
%%		\dif[par] { \ca[n+1] }
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%		&=
%		\Sum[from={i=1},to={n-1}]
%			(-1)^{n-i}
%			\bigl(
%				(
%					\id[tens=(i-1)]
%					\tens
%					\comult[2,upper=\algC]
%					\tens
%					\id[tens=(n-i)]
%				)
%				\ca[n]
%	\\&
%		\qquad\qquad
%				{}-
%				(
%					\id[tens=i]
%					\tens
%					\ca[n-i+1]
%				)
%				\ca[i+1]
%			\bigr)
%		.
%	\end{align*}
%	This equation is very similar
%	%to the one in~\cref{res:homotopy_limit_dgcat},
%	to~\eqref{eq:theta_n_equation},
%	and we shall indeed derive it from that equation. Specifically, we claim that it is obtained
%	from~\eqref{eq:theta_n_equation} by composing
%	with \( (-1)^{n+2} = (-1)^{n} \) times the
%	unit~\( \algM \to \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }} \),
%	and we show this by comparing each term individually.
%	
%	We initially consider the
%	term~\(
%		\map{\id[tens=n]\tens\ca[1]}[spar] \ca[n+1]
%		-
%		(-1)^{1-n}
%		\ca[n+1]\ca[1]
%	\).
%	We get by~\cref{res:base_change_face_maps}
%	that
%	this is exactly the unit~\(
%		\algM \to
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{ \algM }
%		}}
%	\)
%	composed with
%	\[
%		(-1)
%		\face[min=n,shpush]{\dif[\algM]}
%		\circ
%		(-1)^{n+1}
%		\mtheta[n]
%		-
%		(-1)^{1-n}
%		(-1)^{n+1}
%		\mtheta[n]
%		\circ
%		(-1)
%		\dif[\algM]
%		=
%		(-1)^{n}
%		\dif[par]{\mtheta[n]}
%		.
%	\]
%	This is exactly \( (-1)^n \)~times the left-hand side
%	term in~\eqref{eq:theta_n_equation}, as claimed.
%	
%	We next consider terms of the
%	form~\( ( \id[tens=i] \tens \ca[n-i+1] ) \ca[i+1] \).
%%	We proceed much as in the proof of \cref{res:equivariance=comodules}.
%%	Applying flat base change to the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{i+j} \ar[r,"{\face[max=j]}"] \ar[d,"{\face[min=i]}"']
%%			& \ssetX{i} \ar[d,"{\face[min=i]}"]
%%	\\
%%		\ssetX{j} \ar[r,"{\face[max=j]}"']
%%			& \ssetX{0}
%%	\end{tikzcd}\]
%%	we obtain
%%	\(
%%		\face[max=j,shpush] \face[min=i,shpull]
%%		\cong
%%		\face[min=i,shpull] \face[max=j,shpush]
%%	\)
%%	and~\(
%%		\face[max=j,shpull] \face[min=i,shpush]
%%		\cong
%%		\face[min=i,shpush] \face[max=j,shpull]
%%	\).\fxfatal{As stated, this diagram is WRONG!!}
%%	This allows us to
%%	rewrite the term~\( ( \id[tens=i] \tens \ca[j+1] ) \ca[i+1] \)
%%	as
%%	\begin{align*}\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=n,shpush] {{ \face[max=i,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[i]}"]
%%				\& \face[max=i,shpush] {{ \face[min=i,shpull] { \algM } }}
%%				\ar[r]
%%					\& \face[max=i,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[max=j,shpush] {{
%%								\face[max=j,shpull] {{
%%									\algM
%%								}}
%%							}}
%%						}}
%%					}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		{} \ar[r,"{\mtheta[j]}"]
%%			\& \face[max=i,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[max=j,shpush] {{
%%						\face[min=j,shpull] {{
%%							\algM
%%						}}
%%					}}
%%				}}
%%			}}
%%			\ar[r,symbol={\cong}]
%%				\&[-1.5em] \face[max=i,shpush] {{
%%					 \face[max=j,shpush] {{
%%						\face[min=i,shpull] {{
%%							\face[min=j,shpull] {{
%%								\algM
%%							}}
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					\&[-1.5em] \face[max=i+j,shpush] {{	
%%						\face[min=(i+j),shpull] {{ \algM }}
%%					}}
%%	\invdot
%%	\end{tikzcd}\end{align*}
%%	the isomorphism being by base change.
%%	In other words, the composed
%%	map~\(
%%		( \id[tens=i]\tens\ca[j+1] )
%%		\ca[i+1]
%%	\)
%%	is the same as the map
%%	\begin{align*}
%%	\MoveEqLeft\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\algM \ar[r]
%%			\& \face[max=i+j,shpush] {{
%%				\face[max=(i+j),shpull] {{ \algM }}
%%			}}
%%			\ar[r,"{\face[max=j,shpull]{ \mtheta[i] }}"]
%%				\&\face[max=i+j,shpush] {{
%%					\face[max=j,shpull] {{
%%						\face[ min=i, shpull ] { \algM }
%%					}}
%%				}}
%%	\end{tikzcd}
%%	\\
%%	&\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%%		\&{}= \face[max=i+j,shpush] {{
%%			\face[min=i,shpull] {{
%%				\face[ max=j, shpull ] { \algM }
%%			}}
%%		}}
%%		\ar[r,"{\face[min=i,shpull] { \mtheta[j] }}"]
%%			\&\face[max=i+j,shpush] {{
%%				\face[min=i,shpull] {{
%%					\face[ min=j, shpull ] { \algM }
%%				}}
%%			}}
%%			\ar[r,symbol={=}]
%%				\&[-1.5em] \face[max=i+j,shpush] {{
%%					\face[min=\smash{(i+j)},shpull] {{ \algM }}
%%				}}
%%				.
%%	\end{tikzcd}\end{align*}
%	By~\cref{res:base_change_face_maps},
%%	this map is the same as
%%	\( (-1)^{k+1} \) times the unit of adjunction~\(
%%		\algM
%%		\to
%%		\face[max=i+j,shpush] {{
%%			\face[max=(i+j),shpull] { \algM }
%%		}}
%%	\)
%%	composed with the
%%	term~\(
%%		\face[min=i,shpull] { \mtheta[j] }
%%		\circ
%%		\face[max=j,shpull] { \mtheta[i] }
%%	\)
%%	this is the same as the map
%%	\[\begin{tikzcd}%[sep=scriptsize]
%%		\algM
%%		\ar[r]
%%		&
%%		\face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%		\ar[r,"{
%%			(-1)^{n-i+1}
%%			\face[min=i,shpull]{\mtheta[n-i]}
%%			\circ
%%			(-1)^{i+1}
%%			\face[max=(n-i),shpull]{\mtheta[i]}
%%		}"]
%%		&[7em]
%%		\face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%	\end{tikzcd}\]
%	this is the same as
%	the unit~\(
%		\algM
%		\to
%		\face[max=n,shpush]
%		\face[max=n,shpull]
%		\algM
%	\)
%	composed with
%	\[
%		(-1)^{n-i+1}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		(-1)^{i+1}
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		=
%		(-1)^{n}
%		\face[min=i,shpull]{\mtheta[n-i]}
%		\circ
%		\face[max=(n-i),shpull]{\mtheta[i]}
%		.
%	\]
%	This is \( (-1)^{n} \)~times one of the terms
%	on the right-hand side of~\eqref{eq:theta_n_equation}, as claimed.
%	
%	
%%	Similarly, we consider the pullback diagram
%%	\[\begin{tikzcd}
%%		\ssetX{n+1} \ar[r] \ar[d] & \ssetX{n} \ar[d]
%%	\\
%%		\ssetX{1} \ar[r] & \ssetX{0}
%%	\end{tikzcd}\]
%	Finally, we consider terms of the
%	form~\(
%		( \id[tens=(i-1)] \tens \comult[2] \tens \id[tens=(n-i)] ) \ca[n]
%		=
%		( \id[tens=(i-1)] \tens \comult[\algC] \tens \id[tens=(n-i)] ) \ca[n]
%	\) where~\( n-i> 0 \).
%	These are given by the composition
%	\begin{align*}
%	\MoveEqLeft
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		\algM \ar[r]
%			\& \face[max=n-1,shpush] {{ \face[max=(n-1),shpull] { \algM } }}
%			\ar[r,"{(-1)^{n}\mtheta[n-1]}"]
%				\&[1.3em]
%				%\&
%				\face[max=n-1,shpush] {{ \face[min=(n-1),shpull] { \algM } }}
%	\end{tikzcd}
%	\\[-.7em]
%	&
%	\begin{tikzcd}[sep=scriptsize,ampersand replacement=\&]
%		{}
%				\ar[r]
%					\& \face[max=n-1,shpush] {{
%						\face[d=i,shpush] {{
%							\face[d=i,shpull] {{
%								\face[min=(n-1),shpull] { \algM }
%							}}
%						}}
%					}}
%					\ar[r,symbol={=}]
%						\&[-1.5em]
%						\face[min=n,shpush] {{
%							\face[max=n,shpull] {{ \algM }}
%						}} .
%	\end{tikzcd}
%	\end{align*}
%%	This map factors as
%%	\[\begin{tikzcd}[sep=scriptsize]
%%		\algM \ar[r] \ar[d,dashed]
%%			& \face[max=n,shpush] {{ \face[max=n,shpull] { \algM } }}
%%			\ar[r,"{\mtheta[n]}"]
%%			\ar[d,dashed]
%%				& \face[max=n,shpush] {{ \face[min=n,shpull] { \algM } }}
%%				\ar[d]
%%	\\
%%		\face[max=n+1,shpush] {{ \face[max=(n+1),shpull] { \algM } }}
%%		\ar[r,dashed]
%%			& \face[max=n,shpush] {{
%%				\face[d=i,shpush] {{
%%					\face[d=i,shpull] {{
%%						\face[max=n,shpull] { \algM }
%%					}}
%%				}}
%%			}}
%%			\ar[r,"{\face[d=i,shpull]{\mtheta[n]}}"]
%%				& \face[max=n,shpush] {{
%%					\face[d=i,shpush] {{
%%						\face[d=i,shpull] {{
%%							\face[min=n,shpull] { \algM }
%%						}}
%%					}}
%%				}}
%%				\ar[r,symbol={=}]
%%					&[-1.5em]
%%					\face[max=n+1,shpush] {{
%%						\face[min=\smash{(n+1)},shpull] {{ \algM }}
%%					}} .
%%	\end{tikzcd}\]
%	According to \cref{res:add_comultiplication_map}, this map
%	is the same as the
%	unit~\(
%		\algM
%		\to
%		\face[max=n+1,shpush] {{
%			\face[max=(n+1),shpull] { \algM }
%		}}
%	\)
%	composed with~\( (-1)^{n} \face[d=i,shpull] { \mtheta[n] } \).
%	This is again~\( (-1)^{n} \) times a term
%	from~\eqref{eq:theta_n_equation}, as claimed.
%	
%	With regards to th morphisms, suppose
%	that \( \malpha = \tup{\malpha[n]}[n\ge0] \)
%	is a
%	morphism~\( \tup{\algM,\mtheta} \to \tup{\algN,\meta} \)
%	of degree~\( \dgcatdeg{\malpha} \).
%	This consists of
%	maps~\(
%		\malpha[n]
%		\in
%		\Hom[d={\dgcatdeg{\malpha}-n}]{
%			{\face[max=n,shpull]{\algM}} ,
%			{\face[min=n,shpull]{\algN}}
%		}
%	\).
%	We use this to define a
%	map~\( \mf \colon \algM \to \algN \)
%	of \ainfty-comodules of degree~\( \dgcatdeg{\mf} = \dgcatdeg{\malpha} \).
%	For all~\( n\ge1 \), let~\( \mf[n] \colon \algM \to \algC[tens=(n-1)]\tens\algN \)
%	be the composition
%	\[\begin{tikzcd}
%		\algM
%		\ar[r]
%		&
%		\face[max=n,shpush]{{
%			\face[max=n,shpull]{\algM}
%		}}
%		\ar[r,"{
%			(-1)^{\dgcatdeg{\malpha}(n-1)}
%			\malpha[n-1]
%		}"]
%		&[4em]
%		\face[max=n,shpush]{{
%			\face[min=n,shpull]{\algN}
%		}}
%	\end{tikzcd}\]
%	
%	Proving that the morphisms inside our dg-category agree
%	with the morphisms
%	inside the dg-category~\( \catxcomod{\algC}[infty,hcu,formal] \)
%	amounts to showing that the equation~\eqref{res:morphisms_in_tot_differential}
%	agrees with the equation for a map of \ainfty-comodules
%	and that \eqref{res:morphisms_in_tot_composition}
%	agrees with the compositions.
%	This is similar acrobatics using the two lemmas above,
%	and we omit it. The homotopy counital condition is equivalent
%	to the condition that \( \mtheta[1] \)~is homotopy-invertible.
%\end{proof}

\endgroup

==> intro/intro_1.tex <==
\chapter{Introduction}

This is a preparatory paper covering homotopical details
needed to define the derived category of \( \dgcatH \)-equivariant
\( \dgcatA \)-dg-modules in the case where \( \dgcatA \)~is a dg-algebra and \( \dgcatH \)~is a dg-Hopf-algebra acting on~\( \dgcatA \).
The example of interest is when \( \setX \)~is a regular, affine scheme and \( \algG \) an algebraic group acting on~\( \setX \),
and where \( \dgcatA = \difforms{\setX} \) and~\( \dgcatH = \difforms{\algG} \), both equipped with the \emph{zero} differential (\emph{not} the de Rham differential).

Compare this with the situation where \( \algA = \reg{\setX} \)~is an ordinary algebra and \( \algH = \reg{\algG} \)~is an ordinary Hopf algebra given by the functions on some algebraic group.
One way to define \( \algH \)-equivariant \( algH \)-modules
is to consider the cosimplicial system of algebras
\( \algA[d=n] = \algH[tens={n}] \tens \algA = \reg{{\algG[to=n]\times\setX}} \) and the corresponding system of Abelian
categories~\( \catxmod{\algA[d=n]} \). Then we may define the
category of \( \algH \)-equivariant \( \algA \)-modules by
the \emph{homotopy limit}
\[\textstyle
	\catxmod{\algA}[spar,equivar=\algH]
	=
	\invholim[\catdelta]{ \catxmod{ (\algH[tens=n]\tens\algA) } }
\]
with respect to the model structure on categories
described in~\textcite{rezk}.
